Bidirectional Type Checking for Relational Properties

Relational type systems have been designed for several applications including information flow, differential privacy, and cost analysis. In order to achieve the best results, these systems often use relational refinements and relational effects to maximally exploit the similarity in the structure of the two programs being compared. Relational type systems are appealing for relational properties because they deliver simpler and more precise verification than what could be derived from typing the two programs separately. However, relational type systems do not yet achieve the practical appeal of their non-relational counterpart, in part because of the lack of a general foundations for implementing them. In this paper, we take a step in this direction by developing bidirectional relational type checking for systems with relational refinements and effects. Our approach achieves the benefits of bidirectional type checking, in a relational setting. In particular, it significantly reduces the need for typing annotations through the combination of type checking and type inference. In order to highlight the foundational nature of our approach, we develop bidirectional versions of several relational type systems which incrementally combine many different components needed for expressive relational analysis.

==> RSTLC/relinf_figures.tex <==

\begin{figure}
  \centering
\[
\begin{array}{llll}
 \label{fig:syntax}
  \mbox{Unary types} 
  & \grt & ::= & \tbool ~|~\tint ~|~ \grt_1 \to \grt_2\\
  \mbox{Relational types} 
  &  \tau & ::= & \trbool ~|~ \trint ~|~  \tau_1 \to \tau_2 ~|~
      \tch{\grt_1}{\grt_2} \\
  \mbox{Expressions} & e & ::= & x  ~|~ n ~|~ \etrue ~|~ \efalse ~|~ \eif e
                                 \ethen e_1 \eelse e_2 ~|~ \efix
                                 f(x). e    ~|~ e_1 \eapp e_2 \\
  \mbox{Value} & v& := & n ~|~\etrue ~|~ \efalse ~|~ \efix f(x). e  
\end{array}
\] 
 \caption{Syntax of values and expressions in Rel Inf} 
  
\end{figure}

\begin{figure}
  \centering
\[
\begin{array}{llll}
 \label{fig:syntax}
   \mbox{Unary types} 
  & \grt & ::= & \tbool ~|~\tint ~|~ \grt_1 \to \grt_2\\
  \mbox{Relational types} 
  &  \tau & ::= & \trbool ~|~ \trint ~|~  \tau_1 \to \tau_2 ~|~
       \tch{\grt_1}{\grt_2}  \\
  \mbox{Expressions} & e & ::= & x  ~|~ n ~|~\etrue ~|~ \efalse ~|~ \eif e
                                 \ethen e_1 \eelse e_2 ~|~ \efix f(x). e
                                 ~|~ e_1 \eapp e_2 ~|~ \eswitch e  \\
  \mbox{Value} & v& := &n~|~ \etrue ~|~ \efalse ~|~ \efix f(x). e  
\end{array}
\] 
 \caption{Syntax of values and expressions in Rel Inf-CORE} 
  
\end{figure}

\begin{figure}
  \centering
\[
\begin{array}{llll}
 \label{fig:syntax}
  \mbox{Unary types} 
  & \grt & ::= & \tbool ~|~\tint ~|~ \grt_1 \to \grt_2\\
  \mbox{Relational types} 
  &  \tau & ::= & \trbool ~|~ \trint ~|~  \tau_1 \to \tau_2  ~|~
       \tch{\grt_1}{\grt_2} \\
  \mbox{Expressions} & e & ::= &\dots  ~|~ \eswitch e
                                 ~|~ (e:\tau)~|~ (e:\grt)\\
  \mbox{Value} & v& := &n ~|~ \etrue ~|~ \efalse ~|~ \efix f(x). e 
\end{array}
\] 
 \caption{Syntax of values and expressions in BiRelInf} 
\end{figure}

\begin{figure}
  \centering
  \begin{mathpar}
    \inferrule{\Omega(x) = \grt }{\Omega \jtype{}{}{x}{\grt}}~\textbf{var}
    \and
   \inferrule
    { \kw{b}  \in \{\etrue, \efalse \}}  
    { \Omega \jtype{}{}{\kw{b}}{\tbool}}~\textbf{bool}
   \and
    \inferrule{ }
  {
    \Omega \jtype{}{}{\econst}{\tint}
  }~\textbf{const}
    \and
    \inferrule{
    {\ifextra
    \awfty{\grt_1 \to \grt_2}
    \fi} \\
     x: \grt_1, f : \grt_1 \to
    \grt_2, \Omega  \jtype{}{}{e}{\grt_2}}
  {
    \Omega
    \jtype{}{}{ \efix f(x).e}{\grt_1 \to
    \grt_2}
}~\textbf{fix}
    \and
    \inferrule{
  \Omega \jtype{}{}{e_1}{\grt_1\to \grt_2} \\
  \Omega \jtype{}{}{e_2}{\grt_1}}
{
  \Omega \jtype{}{}{ e_1 \eapp e_2}{
  \grt_2}}~\textbf{app}
    \and
   \inferrule{\Omega \jtype{}{}{e}{\tbool} \\
      \Omega \jtype{}{}{e_1}{\tau} \\
      \Omega \jtype{}{}{e_2}{\tau}
    }
    {\Omega \jtype{}{}{\eif e \ethen e_1 \eelse e_2}{\tau}}~\textbf{if}
    \and
    \inferrule{
    \Omega \jtype{}{}{e}{\grt} \\
    \jasubtype{\grt}{\grt'} \\
}{
  \Omega \jtype{}{}{e}{\grt'}
}~{\pmb{\sqsubseteq}\wexec}
  \end{mathpar}
  \caption{ Rel Inf unary typing rules}
  \label{fig:rel-Inf-u-typing-rules}
\end{figure}


\begin{figure}
  \centering 
  \begin{mathpar}
    \inferrule
    {\Gamma(x) = \tau } 
    { \Gamma \jstype{x}{x}{\tau}}~\textbf{r-var}
    \and
    \inferrule
    { \kw{b}  \in \{\etrue, \efalse \}}  
    { \Gamma \jstype{\kw{b}}{\kw{b}}{\trbool}}~\textbf{r-bool}
    \and
    \inferrule
    {  |\Gamma|_1 \jtype{}{}{e_1}{\grt_1}   \\ |\Gamma|_2 \jtype{}{}{e_2}{\grt_2}  }  
    { \Gamma \jstype{e_1}{e_2}{  \tch{\grt_1}{\grt_2} }}~\textbf{r-switch}
    \and
    \inferrule{\Gamma \jstype{e}{e'}{\trbool} \\
      \Gamma \jstype{ e_1}{e_1'}{\tau} \\
      \Gamma \jstype{ e_2}{e_2'}{\tau}
    }
    {\Gamma \jstype{\eif e \ethen e_1 \eelse e_2}{\eif e' \ethen e_1' \eelse e_2'}{\tau}}~\textbf{r-if}
    \and
     \inferrule{
       \Delta; \Phi_a;  x: \tau_1, f : \tau_1 \to \tau_2, \Gamma   \jstype{e_1}{e_2}{\tau_2}
     }
     {\ctx \jstype{ \efix f(x).e_1}{\efix f(x).e_2}{
                \tau_1 \to \tau_2}}~\textbf{r-fix}
    \and
    \inferrule{\Gamma \jstype{e_1}{e_1'}{\tau_1}
      \to \tau_2 \\
      \Gamma \jstype{ e_2}{e_2'}{\tau_1}}
    {\Gamma \jstype{e_1 \eapp e_2}{e_1' \eapp
        e_2'}{\tau_2}}~\textbf{r-app}
   \and
   \inferrule{
    \Gamma \jstype{e_1}{e_2}{\tau}\\
     \jsubtype{\tau}{\tau'}~~ 
  }
  {\Gamma \jstype{e_1}{e_2}{\tau'}
  }~{\textbf{r-}\pmb{\sqsubseteq}}
  \end{mathpar}
 \caption{Rel Inf relational typing rules}
\label{fig:rel-inf-r-typing}
\end{figure}

\begin{figure}
  \centering 
  \begin{mathpar}
\inferrule{
 \jasubtype{\grt_1'}{\grt_1} \\
 \jasubtype{\grt_2}{\grt_2'} \\
}
{
 \jasubtype{\grt_1 \to \grt_2}{\grt_1' \to \grt_2'}
}~\textbf{$\to \wexec$}
\and
   \inferrule
{
}
{ \jasubtype{\grt}{\grt}
}\textbf{u-refl}
\and
\inferrule{
 \jasubtype{\grt_1}{\grt_2} \\
 \jasubtype{\grt_2}{\grt_3}
}
{
 \jasubtype{\grt_1}{\grt_3}
}\textbf{u-tran}
   \end{mathpar}
   \caption{unary subtyping rules for Rel Inf}
   \label{fig:rel-inf-u-subtyping}
 \end{figure}


\begin{figure}
  \centering 
  \begin{mathpar}
   \inferrule
{
\strut
}
{
 \jsubtype{\tch{\grt_1 \to \grt_2}{ \grt_1' \to \grt_2'  }  }{ \tch{\grt_1}{\grt_1'}
    \to \tch{\grt_2}{\grt_2'}  }
}~\textbf{$\to \wexec \wdiff$}
    \and
   \inferrule
{
  \jasubtype{\grt_1}{\grt_1'} \\
  \jasubtype{\grt_2}{\grt_2'} 
}
{
 \jsubtype{\tch{\grt_1}{\grt_2}}{\tch{\grt_1'}{
\grt_2'}}
}~\textbf{U}
    \and
    \inferrule{ }
{
 \jsubtype{\tau}{\tch{\trm{\tau}{1}}{\trm{\tau}{2}  }}
}~\textbf{W}
    \and
     \inferrule{
       \jsubtype{\tau_1'}{\tau_1} \\
       \jsubtype{\tau_2}{\tau_2'}
     }
     {
       \jsubtype{\tau_1 \to \tau_2}{\tau_1' \to \tau_2'}
     }~\textbf{$\to$}
     \and
     \inferrule
     {
     }
     {  \jsubtype{\tau}{\tau}
     }\textbf{refl}
     \and
     \inferrule{
       \jsubtype{\tau_1}{\tau_2} \\
       \jsubtype{\tau_2}{\tau_3}
     }
     {
       \jsubtype{\tau_1}{\tau_3}
     }\textbf{trans}
   \end{mathpar}
   \caption{relational subtyping rules for Rel Inf}
   \label{fig:rel-inf-r-subtyping}
 \end{figure}

\begin{figure*}
\[
\begin{array}{rcl}
   { | . |}_{i \in \{ 1,2 \}}  &  \quad  :  &  \textsf{Binary type}  \rightarrow \textsf{Unary type} \\
    {| \trint |}_{i} & \quad  = & \tint \\
    { |\trbool|}_{i}  & \quad = & \tbool \\
    {|\tau_1 \to \tau_2|}_{i} & \quad = & {|\tau_1|}_{i} \to
                                          {|\tau_2|}_{i} \\
  {|\tch{\grt_1}{\grt_2}|}_{i}  & \quad  = & \grt_i \\  
     { | \Gamma, x : \tau |   }_{i}  & \quad  = & { | \Gamma  | }_{i} , x : { | \tau  |  }_{i}  \\
       { | \emptyset |   }_{i}  & \quad  = &\emptyset \\
\end{array}
\]
 \caption{RelInf refinement removal operation}
  \label{fig:r-type-eq-rules}
\end{figure*}


\begin{figure*}
  \begin{mathpar}
\inferrule{
}
{
 \jeqtype{\trbool}{\trbool}}~\textbf{eq-boolr}
\and
\inferrule{
}
{
 \jeqtype{\trint}{\trint}}~\textbf{eq-intr}
\and
 \inferrule{
\jeqtype{\tau_1}{\tau_1'} \\
\jeqtype{\tau_2}{\tau_2'}
}
{
 \jeqtype{\tau_1 \to \tau_2}{\tau_1' \to \tau_2'}
}~\textbf{eq-fun}
 \and
\inferrule{
\jasubtype{\grt_1}{\grt_1'} \\
\jasubtype{\grt_1'}{\grt_1} \\
\jasubtype{\grt_2}{\grt_2'} \\
\jasubtype{\grt_2'}{\grt_2} 
}
{
 \jeqtype{\tch{\grt_1}{\grt_2} }{\tch{\grt_1'}{\grt_2'}}
}~\textbf{eq-U}
\end{mathpar}
  \caption{RelInf relational type equivalence rules}
  \label{fig:r-type-eq-rules}
\end{figure*}

\begin{figure}
  \centering 
  \begin{mathpar}
   \relinfcoreufix
  \and
   \relinfcoreuvar
\and
   \relinfcoreuconst
\and
  \relinfcoreusub
  \end{mathpar}
  % Definitions at typing-rules-min-defs.tex
  \caption{Rel Inf Core unary typing rules}
  \label{fig:rel-Inf-core-typing-rules}
\end{figure}

\begin{figure}
  \centering 
  \begin{mathpar}
 \inferrule{
    \trm{\Gamma}{1} \jtypeM{}{}{e_1}{\grt_1}~~\\
    \trm{\Gamma}{2} \jtypeM{}{}{e_2}{\grt_2}~~
    } {\Gamma \jstypet{\eswitch e_1}{\eswitch
        e_2}{\tch{\grt_1}{\grt_2}}}~\textbf{c-switch}
\and
   \relinfcorerfix
  \and
   \relinfcorervar
\and
   \relinfcorerconst
\and
  \relinfcorersub
  \end{mathpar}
  % Definitions at typing-rules-min-defs.tex
  \caption{Rel Inf Core relational typing rules}
  \label{fig:rel-Inf-core-typing-rules}
\end{figure}




\begin{figure}
  \centering 
  \begin{mathpar}
  \relinfembedrvar
 \and
  \relinfembedrconst
  \and
\relinfembedrfix
\and
  \inferrule
  {
     \Gamma \jelabct{t}{e_1}{e_2}{\tau}~~ \\
    \jsubtype{\tau}{\tau'} ~~\\
    e' = \ecoerce{\tau}{\tau'} ~~
  }
  {
    \Gamma \jelabt{t'}{e_1}{e_2}{e' \eapp e_1^*}{e' \eapp e_2^*}{\tau'} \\
  }~\textbf{e-r-$\sqsubseteq$}
  \and
\inferrule{
    \trm{\Gamma}{1} \jelabun{}{}{e_1}{e_1^*}{\grt_1}~~\\
    \trm{\Gamma}{2} \jelabun{}{}{e_2}{e_2^*}{\grt_2}
    } {\Gamma \jelabt{t_1-k_2}{e_1}{e_2}{\eswitch e_1^*}{\eswitch e_2^*}{\tch{\grt_1}{\grt_2}}}~\textbf{e-switch}
\end{mathpar}
  % Definitions at appendix/elaboration-rules-defs.tex
  \caption{Rel Inf binary embedding rules}
  \label{fig:relinf-binary-elab-rules}
\end{figure} 

\begin{figure}
  \centering 
  \begin{mathpar}
 \relinfembeduvar
\and
\relinfembeduconst
\and
\relinfembedufix
\and
\relinfembedusub
\end{mathpar}
  % Definitions at appendix/elaboration-rules-defs.tex
  \caption{Rel Inf unary embedding rules}
  \label{fig:relinf-unary-elab-rules}
\end{figure} 


\begin{figure}
  \centering 
  \begin{mathpar}
  \relinfalguvar
\and
  \relinfalgubool
\and
  \relinfalgusub
\and
   \relinfalguanno
 \and
 \relinfalguif
 \and
  \relinfalgufix
\end{mathpar}
  \caption{Rel Inf unary alg rules}
  \label{fig:relinf-unary-alg-rules}
\end{figure} 

\begin{figure}
  \centering 
  \begin{mathpar}
    \inferrule
    {\Gamma(x) = \tau } 
    { \Gamma \infdiffT{x}{x}{\tau}{}{}{}}~\textbf{alg-r-var}
    \and
    \inferrule
    { \kw{b}  \in \{\etrue, \efalse \}}  
    { \Gamma \infdiffT{\kw{b}}{\kw{b}}{\trbool}{}{}{}}~\textbf{alg-r-bool}
    \and
    \inferrule
  {
     \trm{\Gamma}{1}  \infexect{e_1}{\grt_1}{}{}{}{}\\
     \trm{\Gamma}{2}  \infexect{e_2}{\grt_2}{}{}{}{}
  }
  {
    \Gamma  \infdiffT{\eswitch e_1}{\eswitch e_2}{\tch{\grt_1}{\grt_2}}{}{}{}}~\textbf{alg-r-switch$\uparrow$}
   \and
    \inferrule
  {
   \trm{\Gamma}{1}  \chexect{e_1}{\grt_1}{}{}{}\\
   \trm{\Gamma}{2}  \chexect{e_2}{\grt_2}{}{}{}
  }
  {
    \Gamma  \chdiffT{\eswitch e_1}{\eswitch e_2}{\tch{\grt_1}{\grt_2}}{}{}
   }~\textbf{alg-r-switch$\downarrow$}
    \and
    \inferrule{\Gamma \infdiffT{e}{e'}{\trbool}{}{}{} \\
      \Gamma \chdiffT{ e_1}{e_1'}{\tau}{}{} \\
      \Gamma \chdiffT{ e_2}{e_2'}{\tau}{}{}
    }
    {\Gamma \chdiffT{\eif e \ethen e_1 \eelse e_2}{\eif e' \ethen e_1'
        \eelse e_2'}{\tau}{}{} }~\textbf{alg-r-if}
    \and
    \inferrule{
       \Gamma, x: \tau_1, f: \tau_1 \to \tau_2  \chdiffT{e_1}{e_2}{\tau_2}{}{}
     }
     {\Gamma \chdiffT{ \efix f(x).e_1}{\efix f(x).e_2}{
                \tau_1 \to \tau_2}{}{}}~\textbf{alg-r-fix}
    \and
    \inferrule{
      \Gamma \infdiffT{e_1}{e_1'}{\tau_1
        \to \tau_2}{}{}{} \\
      \Gamma \chdiffT{ e_2}{e_2'}{\tau_1}{}{}}
    {\Gamma \infdiffT{e_1 \eapp e_2}{e_1' \eapp e_2'}{\tau_2}{}{}{}}~\textbf{alg-r-app}
    \and
    \inferrule{
      \Gamma \infdiffT{e}{e'}{\tau'}{}{}{}\\
      \jeqtype{\tau'}{\tau} \\
    }
    { 
      \Gamma \chdiffT{e}{e'}{\tau}{}{}
    }~\textbf{alg-$\uparrow\downarrow$}
    \and
    \inferrule
    {
      \Gamma \chdiffT{e}{e'}{\tau}{}{}    
    }
    {
      \Gamma  \infdiffT{(e:\tau)}{(e:\tau)}{\tau}{}{}{}
    } ~\textbf{alg-r-anno-$\uparrow$} 
  \end{mathpar}
 \caption{Algorithmic typing rules for Rel Inf}
\label{fig:rel-inf-alg-typing}
\end{figure}

\begin{figure}
  \centering 
  \begin{mathpar}
    \inferrule{
}
{
 \jeqtype{\trbool}{\trbool}}~\textbf{alg-boolr}
\and
\inferrule{
}
{
 \jeqtype{\trint}{\trint}}~\textbf{alg-intr}
\and
    \inferrule{
     \jasubtype{\grt}{\grt'} \\
     \jasubtype{\grt'}{\grt}
    }
    {
      \jeqtype{ \tcho{\grt} }{\tcho{\grt'}}
    }~\textbf{alg-u}
    \and
     \inferrule{
       \jeqtype{\tau_1'}{\tau_1} \\
       \jeqtype{\tau_2}{\tau_2'}
     }
     {
       \jeqtype{\tau_1 \to \tau_2}{\tau_1' \to \tau_2'}
     }~\textbf{alg-$\to$}
   \end{mathpar}
   \caption{Algorithmic subtyping rules for Relational Inf}
   \label{fig:rel-Inf-alg-subtyping}
 \end{figure}


==> RSTLC/relinf_lemmas.tex <==
\subsection{RefInf proof}
% \begin{lem}[Reflexivity of Unary Algorithmic Subtyping] \label{lem:relInf-alg-unary-subtyping-refl}
%    $\jsubtype{\grt}{\grt}$.
% \end{lem}

% \begin{proof}
%   By induction on the unary type. \\
% \begin{mainitem}
% \caseL{\tbool}
      
% \caseL{\tint}
% \caseL{A_1 \to A_2}
% \end{mainitem}
% \end{proof}


\begin{lem} [Reflexivity of Algorithmic Binary Type Equivalence] \label{lem:relInf-refl-ty-eq}
  $\jeqtype{\tau}{\tau}$.
 \end{lem}
 \begin{proof}
   By induction on the binary type.
\begin{mainitem}
\caseL{$\trbool$}
It is proved by algorithmic binary type equivalence rule \textbf{alg-boolr}.
%%%%%%%%
\caseL{$\tau_1 \to \tau_2$ }
By IH on $\tau_1$,$\jeqtype{\tau_1}{\tau_1}$.\\
By IH on $\tau_2$, $\jeqtype{\tau_2}{\tau_2}$\\
By the above statements and rule \textbf{alg-$\to$}, we conclude\\
$\jeqtype{\tau_1 \to \tau_2}{\tau_1 \to \tau_2} $.
%%%%%%%%%%
\caseL{ $\tch{\grt_1}{\grt_2}$ }
TS: $\jeqtype{\tch{\grt_1}{\grt_2}}{ \tch{\grt_1}{\grt_2} }$.\\
By unary subtyping rule \textbf{u-refl}, $\jasubtype{\grt_1}{\grt_1} $
and $\jasubtype{\grt_2}{\grt_2} $.\\
By the above statements and rule \textbf{alg-u}, we conclude \\
 $\jeqtype{\tch{\grt_1}{\grt_2}}{ \tch{\grt_1}{\grt_2} }$.
\end{mainitem}
 \end{proof}



% \begin{lem}[Transitivity of Unary Algorithmic Subtyping] \label{lem:alg-unary-subtyping-trans}
%   If $ \jsubtype{\grt_1}{\grt_2}$ and $\jsubtype{\grt_2}{\grt_3}$, then $ \jsubtype{\grt_1}{\grt_3}$.
% \end{lem}

% \begin{proof}
%   By simultaneous induction on the first two subtyping derivation.
% \end{proof}

\begin{lem} [Existence of coercions for relational subtyping] \label{lem:relinf-elab}
  If $ \jsubtype{\tau}{\tau'}$ then there exists
  $\ecoerce{\tau}{\tau'}\!\!\in \mbox{Core}$ s.t.\ $
  \cdot
  \jtypediffMt{0}{\ecoerce{\tau}{\tau'}}{\ecoerce{\tau}{\tau'}}{\tau
    \to \tau'}$.
\end{lem}

\begin{proof}
 Proof is by induction on the subtyping derivation.  We denote the
  witness $e$ of type $\tau \to \tau'$ as $\ecoerce{\tau}{\tau'}$ for clarity.
\begin{mainitem}
    \caseL{\relinfsubto[(\star)][(\diam)]} 
    By IH on $(\star)$, $\exists \ecoerce{\tau_1'}{\tau_1}.~~ \cdot \jtypediffMt{0}{\ecoerce{\tau_1'}{\tau_1}}{\ecoerce{\tau_1'}{\tau_1}}{\tau_1' \to \tau_1}$\\
    By IH on $(\diam)$, $\exists \ecoerce{\tau_2}{\tau_2'}.~~\cdot \jtypediffMt{0}{\ecoerce{\tau_2}{\tau_2'}}{\ecoerce{\tau_2}{\tau_2'}}{\tau_2 \to \tau_2'}$\\
    
    Then, using these two statements,we can
    construct the following derivation where
    $e= \efix f(x). \efix f(y). \ecoerce{\tau_2}{\tau_2'} \eapp (x \eapp
    (\ecoerce{\tau_1'}{\tau_1} \eapp y))$
    
    $ \cdot \jtypediffMt{0}{e}{e}{(\tau_1 \to \tau_2)
      \to \tau_1' \to \tau_2'}$\\
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\caseL{\inferrule
{ }
{
 \cdot \jsubtype{\tau}{\tch{\trm{\tau}{1}}{\trm{\tau}{2}}}
}~\textbf{W}}
    Then, we can immediately construct the derivation using the rule \textbf{c-switch}.
    \begin{mathpar}
      \inferrule{ } { \cdot \jtypediffMt{0}{\efix f(x).
           \eswitch x}{\efix f(x).
           \eswitch x}{\tau \to
          \tch{\trm{\tau}{1}}{\trm{\tau}{2}}}
      } 
  \end{mathpar}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    % \caseL{\relrefsubrefl}
    % Then, we can immediately construct the derivation 
    % \begin{mathpar}
    %   \inferrule{ } { \Delta; \Phi; \cdot \jmintypesame{0}{\elam x. x}{\tau \tarrd{0} \tau}}
    % \end{mathpar}

    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \caseL{\relinfsubtrans[(\star)][(\diam)]}
    By IH on $(\star)$, $\exists \ecoerce{\tau_1}{\tau_2}.~~ \sorted{i}, \cdot \jtypediffMt{0}{\ecoerce{\tau_1}{\tau_2}}{\ecoerce{\tau_1}{\tau_2}}{\tau_1 \to \tau_2}$\\
    By IH on $(\diam)$, $\exists \ecoerce{\tau_2}{\tau_3}.~~ \sorted{i}, \cdot \jtypediffMt{0}{\ecoerce{\tau_2}{\tau_3}}{\ecoerce{\tau_2}{\tau_3}}{\tau_2 \to \tau_3}$\\

    Then, using $(\star)$ and $(\diam)$, we can construct the
    derivation simply by function composition
    \begin{mathpar}
      \inferrule{ } { \cdot \jmintypesamet{0}{\efix f(x). \ecoerce{\tau_2}{\tau_3} \eapp (\ecoerce{\tau_1}{\tau_2} \eapp x)}{\tau_1 \to \tau_3}
      } 
    \end{mathpar}

 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
    \caseL{\relinfsubstarrW}
    Then, we can immediately construct the following derivation where $e= {\efix f(x). \efix f(y). \eswitch (x \eapp y)}$ using the \textbf{c-switch} and \textbf{c-app} rules. \\
    $\cdot \jmintypesamet{0}{e}{(\tch{\grt_1 \to \grt_2}{\grt_1' \to
        {\grt_2'}}) \to \tch{\grt_1}{\grt_1'} \to
      \tch{\grt_2}{\grt_2'}}$\\

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\caseL{\relinfsubU}
 Then, we can immediately construct the following derivation where $e=
 {\efix f(x). \eswitch x}$ using the \textbf{c-switch} and
 \textbf{c-u-$\sqsubseteq$} rules.\\
 $\cdot \jmintypesamet{0}{e}{(\tch{\grt_1}{\grt_2}) \to \tch{\grt_1'}{\grt_2'} 
      }$.\\

\end{mainitem}
\end{proof}

\begin{thm} [Types are preserved by embedding]\label{thm:relinf-embedding-soundness}
\mbox{} \begin{enumerate}
  \item If $\Omega \jelabun{}{}{e}{e^*}{\grt}$, then
    $\Omega \jtypeM{}{}{e^*}{\grt}$ and $\Omega \jtype{}{}{e}{\grt}$.
  \item If
    $ \Gamma \jelabt{t}{e_1}{e_2}{e_1^*}{e_2^*}{\tau}$,
    then $ \Gamma \jstypet{e_1^*}{e_2^*}{\tau}$ and
    $ \Gamma \jstype{e_1}{e_2}{\tau}$.
\end{enumerate}
\end{thm}
%
\begin{proof}
By simultaneous induction on the given derivations.

 \textbf{Proof of
  \Cref{thm:relinf-embedding-soundness}.1:} \\
  \begin{mainitem}
   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
   \caseL{\relinfembedufix}
   By \Cref{thm:relinf-embedding-soundness}.1 on the premise, we get $  x: \grt_1, f : \grt_1 \to
    \grt_2, \Omega  \jtypeM{}{}{e}{\grt_2}$.
   Then, by unary core rule \textbf{c-fix},we conclude: $\relinfcoreufix$.
  \end{mainitem}



\textbf{Proof of \Cref{thm:relinf-embedding-soundness}.2:} \\
\begin{mainitem} 
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
  \caseL{$\relinfembedswitch[(\star)][(\diam)]$}
  By \Cref{thm:relinf-embedding-soundness}.1 on $(\star)$, we get $\Delta; \Phi; \Omega \jtypeM{}{}{e_1^*}{\grt_1}~~(\star\star)$. \\
  By \Cref{thm:relinf-embedding-soundness}.1 on $(\diam)$, we get $\Delta; \Phi; \Omega \jtypeM{}{}{e_2^*}{\grt_2}~~(\diam\diam)$. \\
  Then, we conclude as follows: $\relinfcoreswitch$ .
\end{mainitem}
\end{proof}

\begin{thm} [Completeness of embedding] \label{thm:relinf-embed-completeness}
  \mbox{}
  \begin{enumerate}
  \item If $ \Omega \jtype{}{}{e}{\grt}$, then there
    exists an $ e^*$ such that $\Omega
    \jelabun{}{}{e}{e^*}{\grt}$.
    \item If $ \Gamma  \jstype{e_1}{e_2}{\tau}$,
      then there exist $ e_1^*, e_2^*$ such that $ \Gamma
      \jelabt{t}{e_1}{e_2}{e_1^*}{e_2^*}{\tau}$.
  \end{enumerate}
\end{thm}
\begin{proof}
By simultaneous induction on the given typing derivations.

\begin{spacing}{1.3}
  \hspace{-1cm} \textbf{Proof of \Cref{thm:relinf-embed-completeness}.1:} \\
\begin{mainitem} 
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
    \caseL{\inferrule{
    \Omega \jtype{k}{t}{e}{\grt}~~(\star) \\
    \jasubtype{\grt}{\grt'}~~(\diam) \\
}{
  \Omega \jtype{}{}{e}{\grt'}
}~\textbf{$\sqsubseteq$ } } 
    By \Cref{thm:relinf-embed-completeness}.1 on $(\star)$, we get $\exists\, e^*$ such that $ \Omega \jelabun{}{}{e}{e^*}{\grt} ~~(\star\star)$. \\
    By \textbf{e-u-$\sqsubseteq$} rule using $(\star\star)$, $(\diam)$, we conclude as follows\\ $\relinfembedusub$

  \end{mainitem}

\end{spacing}
  
\begin{spacing}{1.3}
  \hspace{-1cm} \textbf{Proof of \Cref{thm:relinf-embed-completeness}.2:} \\

  \begin{mainitem}
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \caseL{  \inferrule
    {  |\Gamma|_1 \jtype{}{}{e_1}{\grt_1}~~(\star)   \\ |\Gamma|_2 \jtype{}{}{e_2}{\grt_2}~~(\diam)  }  
    { \Gamma \jstype{e_1}{e_2}{  \tch{\grt_1}{\grt_2} }}~\textbf{r-switch}}
    By \Cref{thm:relinf-core-completeness}.1 on $(\star)$, we get $\exists\, e_1^*$ such that $ |\Gamma|_1 \jelabcu{}{}{e_1}{\grt_1} ~~(\star\star)$. \\
    By \Cref{thm:relinf-core-completeness}.1 on $(\diam)$, we get $\exists\, e_2^*$ such that $  |\Gamma|_2 \jelabcu{}{}{e_2}{\grt_2} ~~(\diam\diam)$. \\
    By \textbf{e-switch} embedding rule using $(\star\star)$ and $(\diam\diam)$, we can conclude as follows:\\
    $\relinfembedswitch[(\star\star)][(\diam\diam)]$. \\
  
    \end{mainitem}
  \end{spacing}
\end{proof}

\begin{thm}[Soundness of algorithmic typechecking]\label{thm:relinf-typing-soundness}
\mbox{}
  \begin{enumerate}
  \item Assume that $\Omega \chexect{e}{\grt}{}{}{\Phi}$, then,
    $ \Omega
    \jtypeM{}{}{\erty{e}}{\grt}$.

  \item Assume that $\Omega \infexect{e}{\grt}{}{}{}{\Phi} $,then,
    $\Omega
    \jtypeM{}{}{\erty{e}}{\grt}$.
    % and $\Delta; \psi_a; \Phi_a \awfty{\grt} $

\item Assume that $\Gamma \vdash{e}\rdiff{e'}~{\downarrow}~\tau  $,then,
  $\Gamma
  \jtypediffMt{\suba{t}}{\erty{e}}{\erty{e'}}{\tau}$.

\item Assume that $\Gamma \vdash{e}\rdiff{e'}~{\uparrow}~\tau$ ,then,
  $\Gamma
  \jtypediffMt{\subta{t}}{\erty{e}}{\erty{e'}}{\tau}$.
\end{enumerate}  
\end{thm}
%
\begin{proof}
By simultaneous induction on the given algorithmic typing derivations.
\begin{spacing}{1.3}
  \hspace{-1cm} \textbf{Proof of
    \Cref{thm:relinf-typing-soundness}.1:} \\
\begin{mainitem}
   \caseL{ \relinfalgufix}
   By IH1 on the premise, we get $\Omega, x:\grt_1,f:\grt_1 \to \grt_2
   \jtypeM{}{}{\erty{e_1}}{\grt_2}~~(\star)$.\\
  By the unary core rule \textbf{c-u-fix} and $(\star)$, 
  We conclude $ \Omega
    \jtypeM{}{}{\efix f(x).\erty{e_1}}{\grt_1 \to \grt_2} $.
\end{mainitem}
\end{spacing}

\begin{spacing}{1.3}
  \hspace{-1cm} \textbf{Proof of
    \Cref{thm:relinf-typing-soundness}.2:} \\
\begin{mainitem}
   \caseL{ \relinfalguanno}
   By IH1 on the premise, we get $\Omega,
   \jtypeM{}{}{\erty{e}}{\grt}~~(\star)$.\\
  Because $ \erty{(e:\grt)} = \erty{e}$,
  We conclude $ \Omega
    \jtypeM{}{}{\erty{(e:\grt)}}{\grt } $.
\end{mainitem}
\end{spacing}

\begin{spacing}{1.3}
  \hspace{-1cm} \textbf{Proof of
    \Cref{thm:relinf-typing-soundness}.3:} \\
\begin{mainitem}
   \caseL{ \relinfalgrswitchch}
   By IH1 on the first premise, we get $|\Gamma|_1
   \jtypeM{}{}{\erty{e_1}}{\grt_1}~~(\star)$.\\
 By IH1 on the second premise, we get $|\Gamma|_2
   \jtypeM{}{}{\erty{e_2}}{\grt_2}~~(\diam)$.\\
  By relational core rule \textbf{c-switch} and $(\star)$ and $(\diam)$,
  We conclude $\Gamma
  \jtypediffMt{\suba{t}}{\eswitch \erty{e_1}}{\eswitch e_1\erty{e_2}}{\tch{\grt_1}{\grt_2}}$.
\end{mainitem}
\end{spacing}

\begin{spacing}{1.3}
  \hspace{-1cm} \textbf{Proof of
    \Cref{thm:relinf-typing-soundness}.4:} \\
\begin{mainitem}
  \caseL{ \relinfalgrswitchinf}
   By IH2 on the first premise, we get $|\Gamma|_1
   \jtypeM{}{}{\erty{e_1}}{\grt_1}~~(\star)$.\\
 By IH2 on the second premise, we get $|\Gamma|_2
   \jtypeM{}{}{\erty{e_2}}{\grt_2}~~(\diam)$.\\
  By relational core rule \textbf{c-switch} and $(\star)$ and $(\diam)$,
  We conclude $\Gamma
  \jtypediffMt{\suba{t}}{\eswitch \erty{e_1}}{\eswitch e_1\erty{e_2}}{\tch{\grt_1}{\grt_2}}$.
\end{mainitem}
\end{spacing}

\end{proof}

\begin{thm}[Completeness of algorithmic typechecking]\label{thm:relinf-typing-completeness}
\mbox{}
  \begin{enumerate}
  \item Assume that $\Omega \jtypeM{}{}{e}{\grt}$.
    Then, there exists $ e'$ such that $\Omega
    \chexect{e'}{\grt}{k}{t}{\Phi}$ and
    $\erty{e'} = e$.
  \item Assume that $\Gamma
    \jtypediffMt{t}{e_1}{e_2}{\tau}$.  Then, there exist $e_1',e_2'$
    such that $ \Gamma \vdash{e_1'}\rdiff{e_2'}~{\downarrow}~\tau
    $ and $\erty{e_1'} = e_1$ and $\erty{e_2'} = e_2$.
  \end{enumerate}  
\end{thm}
%
\begin{proof}
By simultaneous induction on the given Core typing derivations.
\begin{spacing}{1.3}
  \hspace{-1cm} \textbf{Proof of
    \Cref{thm:relinf-typing-completeness}.1:} \\
\begin{mainitem}
  \caseL{ \relinfcoreuvar}
We can conclude as follows
    \begin{mathpar}
    \inferrule{
      \relinfalguvar \\
      \jsubtype{\grt}{\grt}
    }
    {
      \Omega \chexect{x}{\grt}{0}{0}{\ctrue}
    }~\textbf{alg-u-$\uparrow\downarrow$}
\end{mathpar}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \caseL{\relinfcoreufix}
  By IH1 on the premise, we get exists $e''$ s.t $\Omega
    \chexect{e''}{\grt_2}{k}{t}{\Phi}~~(\star)$ .\\
  By algorithmic unary rule \textbf{alg-u-fix} and $(\star)$, we
  conclude where $e'=\efix f(x).e''$ and $\erty{e''} = e''$ \\
$\Omega
    \chexect{e'}{\grt_1 \to \grt_2}{k}{t}{\Phi}$. and $\erty{e'} =
    \efix f(x). \erty{e''}$.
  
\end{mainitem}
\end{spacing}


\begin{spacing}{1.3}
  \hspace{-1cm} \textbf{Proof of
    \Cref{thm:relinf-typing-completeness}.2:} \\
\begin{mainitem}
\caseL{$\relinfcorerapp$}
By IH on the first premise, $\exists \e_1,\e_1'$ such that 
\begin{enumih}
\item $\Gamma \chdiffrelinf{\e_1}{\e_1'}{\tau_1 \to \tau_2}{t_1}{\Phi_1}$
\item $\erty{\e_1} = e_1$ and $\erty{\e_1'} = e_1'$
\end{enumih}

By IH on the second premise, $\exists \e_2,\e_2'$ such that 
\begin{enumih}[resume]
\item $ \Gamma \chdiffrelinf{\e_2}{\e_2'}{\tau_1}{t_2}{\Phi_2}$
\item $\erty{\e_2} = e_2$ and $\erty{\e_2'} = e_2'$
\end{enumih}

Then, we can conclude as follows
\begin{enumconc}
\item 
  \begin{mathpar}
    \inferrule
    {\inferrule
      {
        {\inferrule
          {
            \Gamma \chdiffrelinf{\e_1}{\e_1'}{\tau_1 \to \tau_2}{t_1}{\Phi_1}
          }
          { \Gamma \infdiffrelinf{(\e_1:{\tau_1 \to \tau_2})}{\e_1':{\tau_1 \to \tau_2})}{\tau_1 \to \tau_2}{\cdot}{t_1}{\Phi_1} }~\textbf{alg-r-anno-$\uparrow$} 
        } \\
        \Gamma \chdifft{\e_2}{\e_2'}{\tau_1}{t_2'}{\Phi_2}
      }
      {
        \Gamma \infdiffrelinf{E_1}{E_2}{\tau_2}{t_2'}{t_1+t+t_2'}{\cand{\Phi_1}{\Phi_2}}
    }~\textbf{c-r-app}}
  {
    \Gamma \chdiffrelinf{E_1}{E_2}{\tau_2}{t_1+t+t_2}{\cand{\Phi_1}{\Phi_2}}
  }~\textbf{alg-r-$\uparrow\downarrow$} 
\end{mathpar} \\
where $E_1= (\e_1:\tau_1 \to \tau_2) \eapp \e_2$ and $E_2= (\e_1':\tau_1 \to \tau_2) \eapp \e_2'$.
\item By using b) and e) .
\item Using c) and f),  $\erty{ (\e_1:\tau_1 \to \tau_2)  \eapp \e_2} = e_1 \eapp e_2$ and $\erty{ (\e_1':\tau_1 \to \tau_2)  \eapp \e_2'} = e_1' \eapp e_2'$.
\end{enumconc}


\end{mainitem}
\end{spacing}

\end{proof}


==> RSTLC/relinfref_figures.tex <==

\begin{figure}
  \centering
\[
\begin{array}{llll}
 \label{fig:syntax}
  \mbox{Unary types} 
  & \grt & ::= & \tbool ~|~\tint ~|~ \grt_1 \to \grt_2 ~|~ \ulist{n}{\grt}
                 ~|~ \tsforall{i} \grt ~|~ \texists{i} \grt ~|~ \tcprod{C}{\grt}
                  ~|~ \tcimpl{C}{\grt}\\
  \mbox{Relational types} 
  &  \tau & ::= & \trbool ~|~ \trint ~|~  \tau_1 \to \tau_2 ~|~
      \tch{\grt_1}{\grt_2} ~|~ \tlist{n}{\alpha}{\tau} ~|~ \tsforall{i} \tau ~|~\\
                &&&  \texists{i} \tau~|~ \tbox{\tau} ~|~ \tcprod{C}{\tau}
                  ~|~ \tcimpl{C}{\tau} \\
  \mbox{Expressions} & e & ::= & x  ~|~ n ~|~ \etrue ~|~ \efalse ~|~ \eif e
                                 \ethen e_1 \eelse e_2 ~|~ \efix
                                 f(x). e    ~|~ e_1 \eapp e_2 ~|~\enil ~|~ \econs(e_1,e_2) ~|~  \\   &  & & \ecase e \eof \enil \rightarrow e_1 ~|~ h ::tl \rightarrow e_2  ~|~  \eLam. e ~|~ e \eApp ~|~ \\  & & & 
\epack e ~|~ \eunpack e_1 \eas x \ein e_2 ~|~ \elet x = e_1 \ein e_2  ~|~  \\ & & & 
\clet e_1 \eas x \ein e_2  ~|~ \ecelim e \\
  \mbox{Value} & v& := & \econst ~|~\etrue ~|~ \efalse ~|~ \efix f(x). e
                         ~|~ \enil ~|~ \econs(v_1,v_2) ~|~ \eLam e ~|~
                         \epack v 
\end{array}
\] 
 \caption{Syntax of values and expressions in RelInfRef} 
  
\end{figure}

\begin{figure}
  \centering
\[
\begin{array}{llll}
 \label{fig:syntax}
   \mbox{Unary types} 
  & \grt & ::= & \tbool ~|~\tint ~|~ \grt_1 \to \grt_2 ~|~ \ulist{n}{\grt}
                 ~|~ \tsforall{i} \grt ~|~ \texists{i} \grt ~|~ \tcprod{C}{\grt}
                  ~|~ \tcimpl{C}{\grt}\\
  \mbox{Relational types} 
  &  \tau & ::= & \trbool ~|~ \trint ~|~  \tau_1 \to \tau_2 ~|~
      \tch{\grt_1}{\grt_2} ~|~ \tlist{n}{\alpha}{\tau} ~|~ \tsforall{i} \tau ~|~\\
                &&&  \texists{i} \tau~|~ \tbox{\tau} ~|~ \tcprod{C}{\tau}
                  ~|~ \tcimpl{C}{\tau} \\
  \mbox{Expressions} & e & ::= & x  ~|~ \etrue ~|~ \efalse ~|~ \eif e
                                 \ethen e_1 \eelse e_2 ~|~ \efix f(x). e
                                 ~|~ e_1 \eapp e_2 ~|~  
  \eswitch e ~|~ \enoch e \\  &&&~|~ \esplit(e_1,e_2) \ewith C ~|~ \econtra e ~|~\eder e  ~|~ \eLam i. e ~|~ e [I] ~|~ \epack e \ewith I ~|~ \\
                   &&& \eunpack e_1 \eas (x,i) \ein e_2 
                       ~|~ \econsNC(e_1,e_2) ~|~ \econsC(e_1,e_2) ~|~
                       \efixNC f(x). e\\ &&& ~|~ \elet x = e_1 \ein e_2~|~ 
                       \left(\begin{minipage}[c]{15em}
                           $\ecase e \eof \enil \, \rightarrow e_1$ \\
                           $|~h\,::_{NC} tl\, \rightarrow e_2
                           ~|~h::_{C} tl~ \rightarrow e_3$
       \end{minipage}\right)  \\
  \mbox{Value} & v& := &\econst ~|~ \efix f(x).e ~|~  \efixNC f(x).e ~|~ 
                            ~|~ \enil \\
  &&& ~|~ \econsNC(v_1,v_2) ~|~ \econsC(v_1,v_2) ~|~ \eLam i. e ~|~ \epack v \ewith I
\end{array}
\] 
 \caption{Syntax of values and expressions in RelInfRef-CORE} 
  
\end{figure}

\begin{figure}
  \centering
\[
\begin{array}{llll}
 \label{fig:syntax}
  \mbox{Unary types} 
  & \grt & ::= & \tbool ~|~\tint ~|~ \grt_1 \to \grt_2 ~|~ \ulist{n}{\grt}
                 ~|~ \tsforall{i} \grt ~|~ \texists{i} \grt ~|~ \tcprod{C}{\grt}
                  ~|~ \tcimpl{C}{\grt}\\
  \mbox{Relational types} 
  &  \tau & ::= & \trbool ~|~ \trint ~|~  \tau_1 \to \tau_2 ~|~
      \tch{\grt_1}{\grt_2} ~|~ \tlist{n}{\alpha}{\tau} ~|~ \tsforall{i} \tau ~|~\\
                &&&  \texists{i} \tau~|~ \tbox{\tau} ~|~ \tcprod{C}{\tau}
                  ~|~ \tcimpl{C}{\tau} \\
  \mbox{Expressions} & e & ::= & x  ~|~ \etrue ~|~ \efalse ~|~ \eif e
                                 \ethen e_1 \eelse e_2 ~|~ \efix f(x). e
                                 ~|~ e_1 \eapp e_2 ~|~  
  \eswitch e ~|~ \enoch e \\  &&&~|~ \esplit(e_1,e_2) \ewith C ~|~ \econtra e ~|~\eder e  ~|~ \eLam i. e ~|~ e [I] ~|~ \epack e \ewith I ~|~ \\
                   &&& \eunpack e_1 \eas (x,i) \ein e_2 
                       ~|~ \econsNC(e_1,e_2) ~|~ \econsC(e_1,e_2) ~|~ \efixNC f(x). e\\
  &&& ~|~ (e:\tau) ~|~ (e:\grt) ~|~ \elet x = e_1 \ein e_2~|~
                       \left(\begin{minipage}[c]{15em}
                           $\ecase e \eof \enil \, \rightarrow e_1$ \\
                           $|~h\,::_{NC} tl\, \rightarrow e_2
                           ~|~h::_{C} tl~ \rightarrow e_3$
       \end{minipage}\right)  \\
  \mbox{Value} & v& := &\econst ~|~ \efix f(x).e ~|~  \efixNC f(x).e ~|~ 
                            ~|~ \enil \\
  &&& ~|~ \econsNC(v_1,v_2) ~|~ \econsC(v_1,v_2) ~|~ \eLam i. e ~|~ \epack v \ewith I
\end{array}
\] 
 \caption{Syntax of values and expressions in BiRelInfRef} 
\end{figure}


\begin{figure}
  \centering 
  \begin{mathpar}
    \inferrule
    {\Gamma(x) = \tau } 
    { \ctx \jstype{x}{x}{\tau}}~\textbf{r-var}
    \and
    \inferrule
    { \kw{b}  \in \{\etrue, \efalse \}}  
    { \ctx \jstype{\kw{b}}{\kw{b}}{\trbool}}~\textbf{r-bool}
    \and
    \inferrule{\ctx \jstype{e}{e'}{\trbool} \\
      \ctx \jstype{ e_1}{e_1'}{\tau} \\
      \ctx \jstype{ e_2}{e_2'}{\tau}
    }
    {\ctx \jstype{\eif e \ethen e_1 \eelse e_2}{\eif e' \ethen e_1' \eelse e_2'}{\tau}}~\textbf{r-if}
    \and
    \inferrule{
       \Delta; \Phi_a;  x: \tau_1, f : \tau_1 \to \tau_2, \Gamma   \jstype{e_1}{e_2}{\tau_2}
     }
     {\ctx \jstype{ \efix f(x).e_1}{\efix f(x).e_2}{
                \tau_1 \to \tau_2}}~\textbf{r-fix}
    \and
    \inferrule{\ctx \jstype{e_1}{e_1'}{\tau_1}
      \to \tau_2 \\
      \ctx \jstype{ e_2}{e_2'}{\tau_1}}
    {\ctx \jstype{e_1 \eapp e_2}{e_1' \eapp
        e_2'}{\tau_2}}~\textbf{r-app}
    \and
   \inferrule
{
\Delta; \Phi_a; \Gamma \jstype{e}{e}{\tau}~~\\\\
\forall x \in dom(\Gamma).~~
\Delta; \Phi_a  \jsubtype{\Gamma(x)}{\tbox{\Gamma(x)}} ~~
}
{
\Delta; \Phi_a; \Gamma,\Gamma' \jstype{e}{e}{\tbox{\tau}}
} ~\textbf{r-nochange}
\and
\inferrule{
    \ctx \jstype{e_1}{e_2}{\tau}~~\\
    \Delta; \Phi_a \jsubtype{\tau}{\tau'}~~ 
  }
  {\ctx \jstype{e_1}{e_2}{\tau'}
  }~{\textbf{r-}\pmb{\sqsubseteq}}
\and
    \inferrule
  {
    {\ifextra \Delta; \Phi_a \wfty{\tau_1 \to \tau_2}
      \fi} \\
    \Delta; \Phi_a;  x: \tau_1, f : \tbox{(\tau_1 \to \tau_2)}, \Gamma \jstype{e}{e}{\tau_2}~~\\
    \forall x \in dom(\Gamma).~~
    \Delta; \Phi_a  \jsubtype{\Gamma(x)}{\tbox{\Gamma(x)}}
  }
  {\ctx \jstype{ \efix f(x).e}{\efix f(x).e}{
              \tbox{(\tau_1 \to \tau_2)}}}~\textbf{r-fixNC}
\and
\inferrule{
    i::S, \ctx \jstype{e}{e'}{\tau}~~ \\\\
    i \not \in \fiv{\Phi_a; \Gamma}
  }
  { \ctx \jstype{\eLam e}{\eLam e'}{\tsforall{i} \tau }}~\textbf{r-iLam}
\and
 \inferrule{
    \ctx \jstype{e}{e'}{\tsforall{i} \tau } ~~\\\\
    \Delta \vdash I : S ~~
  }
  {\ctx \jstype{e \eApp}{e' \eApp}{\tau\{ I/
      i\}}}~\textbf{r-iApp}
\and
 \inferrule
{
  \ctx  \jstype{e}{e'}{\tau\{I/i\}}~~\\
  \Delta \sty{I}{\sort}~~
}
{
  \ctx  \jstype{\epack e}{\epack e'}{\texists{i} \tau}
} ~\textbf{r-pack}
\and
\inferrule
{
  \ctx \jstype{e_1}{e_1'}{\texists{i} \tau_1} ~~\\
  \sorted{i}, \Delta; \Phi_a; x: \tau_1, \Gamma \jstype{e_2}{e_2'}{\tau_2} ~~\\
  i \not\in FV(\Phi_a;\Gamma, \tau_2, t_2) \\
}
{
  \ctx  \jstype{\eunpack e_1 \eas x \ein  e_2}{\eunpack e_1' \eas x \ein  e_2'}{\tau_2}
}~\textbf{r-unpack1} 
\and
\inferrule
{
  \Delta; \Phi_a \wedge C; \Gamma \jstype{e}{e'}{\tau}
}
{
  \ctx  \jstype{e}{e'}{\tcimpl{C}{\tau}}
} ~\textbf{r-c-impII}
\and
\inferrule
{
  \ctx \jstype{e_1}{e_1 '}{\tcimpl{C}{\tau}}\\
  \Delta; \Phi_a \vDash C
}
{
  \ctx  \jstype{\ecelim e }{\ecelim e' }{\tau}
} ~\textbf{r-c-implE}
\and
\and
    \inferrule
    {  |\Gamma|_1 \jtype{}{}{e_1}{\grt_1}   \\ |\Gamma|_2 \jtype{}{}{e_2}{\grt_2}  }  
    { \Gamma \jstype{e_1}{e_2}{  \tch{\grt_1}{\grt_2}
      }}~\textbf{r-switch}
\and
\inferrule
{
  \ctx \jstype{e_1}{e_1 '}{{\tau_1}}\\
  \Delta; \Phi_a ; x :\tau_1, \Gamma   \jstype{ e_2}{e_2'}{\tau_2}
}
{
  \ctx  \jstype{\elet x = e_1 \ein e_2}{\elet x = e_1' \ein e_2'}{\tau_2}
} ~\textbf{r-let}
  \end{mathpar}
 \caption{RelInfRef typing rules1}
\label{fig:rel-inf-ref-typing1}
\end{figure}

\begin{figure}
\centering 
  \begin{mathpar}
\inferrule
  {
    {\ifextra
      \Delta; \Phi_a \wfty{\tau}
      \fi}
  }
  { \ctx
    \jstype{\enil}{\enil}{\tlist{0}{\alpha}{\tau}}}~\textbf{r-nil}
\and
\inferrule
  { \ctx \jstype{e_1}{e_1'}{\tau} \\
    \ctx \jstype{e_2}{e_2'}{\tlist{n}{\alpha}{\tau}}
  }
  { \ctx \jstype{ \econs(e_1,e_2) }{ \econs(e_1',e_2')}{\tlist{n+1}{\alpha+1}{\tau}}}~\textbf{r-cons1}
\and
 \inferrule
  { \ctx \jstype{e_1}{e_1'}{\tbox{\tau}} \\
    \ctx \jstype{e_2}{e_2'}{\tlist{n}{\alpha}{\tau}}}
  { \ctx \jstype{ \econs(e_1,e_2) }{
      \econs(e_1',e_2')}{\tlist{n+1}{\alpha}{\tau}}}~\textbf{r-cons2}
\and
\inferrule
  {\ctx \jstype{e}{e'}{\tlist{n}{\alpha}{\tau}} \\
   \Delta; \Phi_a \wedge n = 0  ;\Gamma \jstype{e_1}{e_1'}{\tau'} \\
   i, \Delta; \Phi_a \wedge n = i+1;  h: \tbox{\tau},
   tl : \tlist{i}{\alpha}{\tau}, \Gamma \jstype{e_2}{e_2'}{\tau'} ~~
\\
   i, \beta, \Delta; \Phi_a \wedge n = i+1 \wedge \alpha = \beta +1 ;
   h: \tau, tl : \tlist{i}{\beta}{\tau}, \Gamma \jstype{e_2}{e_2'}{\tau'} ~~
   }
  {\ctx \jstype{ \ecase e \eof \enil \rightarrow e_1 ~|~ h::tl \rightarrow
    e_2}{\ecase e' \eof \enil \rightarrow e_1' ~|~ h::tl \rightarrow
    e_2'}{\tau'}}~\textbf{r-caseL}
\and 
\inferrule
{
\Delta; \Phi_a \sat C \\
  \Delta; \Phi_a \wedge C; \Gamma \jstype{e}{e'}{\tau}
}
{
  \ctx  \jstype{e}{e'}{\tcprod{C}{\tau}}
} ~\textbf{r-c-andI}
\and
\inferrule
{
  \ctx \jstype{e_1}{e_1 '}{\tcprod{C}{\tau_1}}\\
  \Delta; \Phi_a \wedge C; x :\tau_1, \Gamma   \jstype{ e_2}{e_2'}{\tau_2}
}
{
  \ctx  \jstype{\clet e_1 \eas x \ein e_2}{\clet e_1' \eas x \ein e_2'}{\tau_2}
} ~\textbf{r-c-andE}
\and
\inferrule
  {
    \Delta; \Phi_a \wedge C; \Gamma  \jstype{e_1}{e_2}{\tau}\\
    \Delta; \Phi_a \wedge \neg C; \Gamma  \jstype{e_1}{e_2}{\tau}\\
    \Delta \wfcs{C}
  }
  {
    \ctx  \jstype{e_1}{e_2}{\tau} } ~\textbf{r-split}
\and
\inferrule
{
\Delta; \Phi_a \sat \bot \\
  \Delta; \Phi_a \wfty{\Gamma}
}
{
  \ctx \jstype{e_1}{e_2}{\tau}
} ~\textbf{r-contra}
\end{mathpar}
 \caption{RelInfRef typing rules 2}
\label{fig:rel-ref-typing2}
\end{figure}



\begin{figure}
  \centering 
  \begin{mathpar}
    \stint
%
\and
%
\stintU
%
\and
   \inferrule
     {
     }
     { \Delta; \Phi_a \jsubtype{\trbool}{\square \trbool}
     }\textbf{bool-$\square$}
    \and
     \inferrule{
       \Delta; \Phi_a\jsubtype{\tau_1'}{\tau_1} \\
      \Delta; \Phi_a \jsubtype{\tau_2}{\tau_2'}
     }
     {
       \Delta; \Phi_a\jsubtype{\tau_1 \to \tau_2}{\tau_1' \to \tau_2'}
     }~\textbf{$\to$}
     \and
     \inferrule
     {
     }
     { \Delta; \Phi_a \jsubtype{\tau}{\tau}
     }\textbf{refl}
     \and
     \inferrule{
     }
     {
       \Delta; \Phi_a \jsubtype{\square (\tau_1 \to \tau_2)}{ \square \tau_1 \to
         \square \tau_2}
     }\textbf{$\square$diff}
\and
 \inferrule{
     \sorted{i},\Delta; \Phi_a\jsubtype{ \tau }{  \tau' }  \\
      i \not \in \fiv{\Phi_a}
     }
     {
       \Delta; \Phi_a\jsubtype{\tsforall{i} \tau }{ \tsforall{i} \tau' }
     }\textbf{$\forall$diff}
\and
 \inferrule{   }
     {
       \Delta; \Phi_a\jsubtype{\square \tsforall{i} \tau }{
         \tsforall{i} \square \tau }
     }\textbf{$\forall \square$}
\and
 \inferrule{   }
     {
       \Delta; \Phi_a\jsubtype{\tch{\tsforall{i} \grt}{\tsforall{i}
           \grt' } }{    
         \tsforall{i}  \tch{\grt}{\grt'}  }
     }\textbf{$\forall $ U}
\and
  \stlist
%
\and
%
\stlistzero
%
\and
%
\stlistbox
%
\and
%
\stbox
%
\and
%
\stboxD
%
\and
%
\stboxB
\and
  \inferrule{ }
{
 \jsubtype{\tau}{\tch{\trm{\tau}{1}}{\trm{\tau}{2}  }}
}~\textbf{W}
%
\and
%
\inferrule
{
  \jasubtype{\grt_1}{\grt_1'} \\
  \jasubtype{\grt_2}{\grt_2'} 
}
{
 \jsubtype{\tch{\grt_1}{\grt_2}}{\tch{\grt_1'}{
\grt_2'}}
}~\textbf{U}
%
\and
%
\stexists
%
\and
%
\stexistsbox
%
\and
%
\stcprod
%
\and
%
\stcprodbox
%
\and
%
\stcimpl
%
\and
%
\stcimplbox
%
\and
\sttrans

   \end{mathpar}
   \caption{Relational subtyping rules for RelInfRef}
   \label{fig:rel-rel-subtyping}
 \end{figure}


\begin{figure}
  \centering 
  \begin{mathpar}
\inferrule{
 \Delta; \Phi_a \jasubtype{\grt_1'}{\grt_1} \\
 \Delta; \Phi_a \jasubtype{\grt_2}{\grt_2'} \\
}
{
 \Delta; \Phi_a \jasubtype{\grt_1 \to \grt_2}{\grt_1' \to \grt_2'}
}~\textbf{u-$\to \wexec$}
\and
\inferrule{
 \sorted{i},\Delta; \Phi_a \jasubtype{\grt}{\grt'} \\
i \not\in FV(\Phi_a)
}
{
 \Delta; \Phi_a \jasubtype{\tsforall{i} \grt}{ \tsforall{i} \grt'}
}\textbf{u-$\forall \wexec$}
\and
\stuexists
%
\and
%
\stucprod
%
\and
%
\stucimpl
%
\and
%
\sturefl 
%
\and
%
\stutrans
%
\and
%
\stulist
   \end{mathpar}
   \caption{Unary subtyping rules for RelInfRef}
   \label{fig:rel-inf-ref-u-subtyping}
 \end{figure}


\begin{figure*}
  \fbox{$\Delta; \Phi_a \jeqtype{\tau_1}{\tau_2}$}~~~checks whether $\tau_1$ is equivalent to $\tau_2$

\raggedright
\begin{mathpar}
\inferrule{ }
{ \Delta; \Phi_a \jeqtype{\trbool}{\trbool} } ~\textbf{eq-bool}
\and
\etint
%
\and
%
\inferrule{
  {\Delta; \Phi_a \jeqtype{ \tau_1 }{\tau_1' } } \and {\Delta; \Phi_a
    \jeqtype{ \tau_2 }{\tau_2' } }
 }
{ \Delta; \Phi_a \jeqtype{ \tau_1 \to \tau_2 }{ \tau_1' \to \tau_2'  } } ~\textbf{eq-$\forall$}
%
%
\and
%
\etlist
%
\and
%
\inferrule{
  i,\Delta; \Phi_a \jeqtype{ \tau }{\tau' }
 }
{ \Delta; \Phi_a \jeqtype{\tsforall{i} \tau }{ \tsforall{i} \tau' } } ~\textbf{eq-$\forall$}
%
\and
%
\etexists
%
\and
%
\etboxB
%
\and
%
\etunrel
%
\and
%
\etcimpl
%
\and
%
\etcprod
\end{mathpar} 
%\nocaptionrule
\caption{RelInfRef binary type equivalence rules}
\label{fig:binary-eq-rules}  
\end{figure*}


\begin{figure*}
  \centering
  \begin{mathpar}
\relrefinfmtyconst
\and
\relrefinfmtyvar
\and
\relrefinfmtyfix
\and
\relrefinfmtyapp
\and
\relrefinfmtyiLam
\and
\relrefinfmtyiApp
\and
\relrefinfmtypack
\and
\relrefinfmtyunpack
\and
\relrefinfmtynil
\and
\relrefinfmtycons
\and
\relrefinfmtylet
\and
\relrefinfmtycaseL
\and
\relrefinfmtycandIntro
\and
\relrefinfmtycandElim
\and
\relrefinfmtycimplIntro
\and
\relrefinfmtycimplElim
\and
\relrefinfmtysubsum
 \end{mathpar}
  % Definitions at typing-rules-min-defs.tex
  \caption{RelInfRef Core unary typing rules}
  \label{fig:relrelcore-typing-rules}
\end{figure*}


\begin{figure*}
  \centering
  \begin{mathpar}
    \inferrule{\Gamma(x) = \tau}{\ctx
      \jstypet{x}{x}{\tau}}~\textbf{c-r-var}
     \and
     \inferrule{
       {\ifextra
       \Delta; \Phi_a \wfty{\tau_1 \to \tau_2}
       \fi} \\
       \Delta; \Phi_a;  x: \tau_1, f : \tau_1 \to \tau_2, \Gamma  \jstypet{e_1}{e_2}{\tau_2}}
            {\ctx \jstypet{ \efix f(x).e_1}{\efix f(x).e_2}{
              \tau_1 \to \tau_2}}~\textbf{c-r-fix}
   \and
\inferrule
  {
    {\ifextra \Delta; \Phi_a \wfty{\tau_1 \to \tau_2}
      \fi} \\
    \Delta; \Phi_a;  x: \tau_1, f : \tbox{(\tau_1 \to \tau_2)}, \tbox{\Gamma} \jstypet{e}{e}{\tau_2}
  }
  {\nctx \jstypet{\efixNC f(x).e}{\efixNC f(x).e}{
              \tbox{(\tau_1 \to \tau_2)}}}~\textbf{c-r-fixNC}
  \and
     \inferrule
  { \ctx \jstypet{e_1}{e_1'}{\tau} \\
    \ctx \jstypet{e_2}{e_2'}{\tlist{n}{\alpha}{\tau}}
  }
  { \ctx \jstypet{ \econsC(e_1,e_2) }{ \econsC(e_1',e_2')}{\tlist{n+1}{\alpha+1}{\tau}}}~\textbf{c-r-cons1}
    \and
   \inferrule
  { \ctx \jstypet{e_1}{e_1'}{\tbox{\tau}} \\
    \ctx \jstypet{e_2}{e_2'}{\tlist{n}{\alpha}{\tau}}}
  { \ctx \jstypet{ \econsNC(e_1,e_2) }{ \econsNC(e_1',e_2')}{\tlist{n+1}{\alpha}{\tau}}}~\textbf{c-r-cons2}
    \and
    \inferrule
  {\ctx \jstypet{e}{e'}{\tlist{n}{\alpha}{\tau}}\\
   \Delta; \Phi_a \wedge n = 0  ;\Gamma \jstypet{e_1}{e_1'}{\tau'}\\
   i, \Delta; \Phi_a \wedge n = i+1;  h: \tbox{\tau},
   tl : \tlist{i}{\alpha}{\tau}, \Gamma \jstypet{e_2}{e_2'}{\tau'}
\\
   i, \beta, \Delta; \Phi_a \wedge n = i+1 \wedge \alpha = \beta +1 ;
   h': \tau, tl : \tlist{i}{\beta}{\tau}, \Gamma \jstypet{e_3}{e_3'}{\tau'}
   }
  {\ctx \jstypet{
      \begin{minipage}[c]{10em}
        ~ $\ecase e \eof \enil \, \rightarrow e_1$ \\
         $~~~~~~~~|~h\,::_{N} tl\, \rightarrow e_2$ \\
         $~~~~~~~~|~h'::_{C} tl' \rightarrow e_3$
      \end{minipage}
}{
      \begin{minipage}[c]{10em}
         ~ $\ecase e \eof \enil \, \rightarrow e_1'$ \\
         $~~~~~~~~|~h\,::_{N} tl\, \rightarrow e_2'$ \\
         $~~~~~~~~|~h'::_{C} tl' \rightarrow e_3'$
      \end{minipage}
}{\tau'}}~\textbf{c-r-caseL}
    \and
    \inferrule
{
\Delta; \Phi_a; \Gamma  \jstypet{e_1}{e_2}{\tbox{\tau}}
}
{
\Delta; \Phi_a; \Gamma  \jstypet{\eder e_1}{\eder e_2}{\tau}
} ~\textbf{c-der}
    \and 
    \inferrule
{
\Delta; \Phi_a; \tbox{\Gamma} \jstypet{e}{e}{\tau}
}
{
\Delta; \Phi_a; \tbox{\Gamma}, \Gamma' \jstypet{\enoch e}{\enoch e}{\tbox{\tau}}
} ~\textbf{c-nochange}
    \and
    \inferrule{
     \ctx \jstypet{e}{e'}{\tau}\\
     \Delta; \Phi_a \jeqtype{\tau}{\tau'} 
  }
  {\ctx \jstype{e}{e'}{\tau'} }
  ~{\textbf{c-r}-\pmb{\sqsubseteq}}
    \and
    \inferrule
  {
    \Delta; \Phi_a \wedge C; \Gamma \jstypet{e_1}{e_2}{\tau}\\
    \Delta; \Phi_a \wedge \neg C; \Gamma \jstypet{e_1'}{e_2'}{\tau}\\
  }
  {
    \ctx \jstypet{\esplit (e_1,e_1') \ewith C}{\esplit
      (e_2,e_2') \ewith C}{\tau} } ~\textbf{c-r-split}
   \and
   \inferrule
{
\Delta; \Phi_a \sat \bot \\
  \Delta; \Phi_a \wfty{\Gamma}
}
{
  \ctx \jstypet{\econtra  e_1}{\econtra  e_2}{\tau}
} ~\textbf{c-r-contra}
\and
\inferrule{
    \ctx \jstypet{e}{e'}{\tsforall{i} \tau}\\
    \Delta \vdash I : S
  }
  {\ctx \jstypet{e[I]}{e' [I]}{\tau\{ I/ i\}}}~\textbf{c-r-iApp}
\and
\inferrule{
    i::S, \ctx \jstypet{e}{e'}{\tau} \\
    i \not \in \fiv{\Phi_a; \Gamma}
  }
  { \ctx \jstypet{\eLam i. e}{\eLam i. e'}{\tsforall{i}
      \tau}}~\textbf{c-r-iLam}
\end{mathpar}
  % Definitions at typing-rules-min-defs.tex
  \caption{RelInfRef Core typing rules}
  \label{fig:relrelcore-typing-rules}
\end{figure*}

\begin{figure*}
  \centering
  \begin{mathpar}
\relrefcorecimplI
\and
\relrefcorecimplE
\and
\relrefcorecprodI
\and
\relrefcorecprodE
\and
\relrefcoreapp
\and
\relrefcorelet
\and
\inferrule
{
  \ctx  \jstypet{e}{e'}{\tau\{I/i\}}\\
  \Delta \sty{I}{\sort}
}
{
  \ctx  \jstypet{\epack e \ewith I}{\epack e' \ewith I}{\texists{i} \tau}
} ~\textbf{c-r-pack}
\and
\inferrule
{
  \ctx \jstypet{e_1}{e_1'}{\texists{i} \tau_1}\\
  \sorted{i}, \Delta; \Phi_a; x: \tau_1, \Gamma \jstypet{e_2}{e_2'}{\tau_2}\\
  i \not\in FV(\Phi_a;\Gamma, \tau_2, t_2) \\
}
{
  \ctx  \jstypet{\eunpack e_1 \eas (x, i) \ein  e_2}{\eunpack e_1' \eas (x, i) \ein  e_2'}{\tau_2}
}~\textbf{c-r-unpack1}
  \and
  \inferrule{
    \trm{\Gamma}{1} \jtypeM{}{}{e_1}{\grt_1}~~\\
    \trm{\Gamma}{2} \jtypeM{}{}{e_2}{\grt_2}~~
    } {\Gamma \jstypet{\eswitch e_1}{\eswitch e_2}{\tch{\grt_1}{\grt_2}}}~\textbf{c-switch}
\end{mathpar}
  % Definitions at typing-rules-min-defs.tex
  \caption{RelInfRef Core typing rules 2}
  \label{fig:relref-core-typing-rules-2}
\end{figure*}


\begin{figure*}
  \centering
  \begin{mathpar}
\relrefinfelfix
    \and
  \relrefinfelvar
       \and
\relrefinfelapp
\and
\relrefinfelnil
\and
\relrefinfelcons
\and
\relrefinfelcaseL
\and
\relrefinfeliLam
\and
\relrefinfeliApp
\and
\relrefinfelpack
\and
\relrefinfelunpack
\and
\relrefinfellet
\and
\relrefinfelcandIntro
\and
\relrefinfelcandElim
\and
\relrefinfelcimplIntro
\and
\relrefinfelcimplElim

\end{mathpar}
  \caption{RelInfRef embedding uanry typing rules 1}
  \label{fig:relrel-embedding-typing-rules-1}
\end{figure*}

\begin{figure*}
  \centering
  \begin{mathpar}
  \inferrule{\Gamma(x) = \tau}{\ctx \jelabsamet{0}{x}{x}{\tau}}~\textbf{e-r-var}
    \and
\relrefembedfix
    \and
     \relrefembedfixnc
       \and
\relrefembedcimplI
\and
\relrefembedcimplE
\and
\relrefembedcprodI
\and
\relrefembedcprodE

\end{mathpar}
  \caption{RelInfRef embedding typing rules 1}
  \label{fig:relrel-embedding-typing-rules-1}
\end{figure*}


\begin{figure*}
\begin{mathpar}
    \inferrule
  { \ctx \jelabct{t_1}{e_1}{e_1'}{\tau} \\
    \ctx \jelabct{t_2}{e_2}{e_2'}{\tlist{n}{\alpha}{\tau}}
  }
  { \ctx \jelabt{t_1+t_2}{ \econs(e_1,e_2) }{\econs(e_1',e_2')}{
      \econsC(e_1^*,e_2^*)}{
      \econsC(e_1'^*,e_2'^*)}{\tlist{n+1}{\alpha+1}{\tau}}}~\textbf{e-r-cons1}
  \and
    \inferrule
  { \ctx \jelabct{t_1}{e_1}{e_1'}{\tbox{\tau}} \\
    \ctx \jelabct{t_2}{e_2}{e_2'}{\tlist{n}{\alpha}{\tau}}}
  { \ctx \jelabt{t_1+t_2}{ \econs(e_1,e_2) }{\econs(e_1',e_2')}{
      \econsNC(e_1',e_2')}{
      \econsNC(e_1^*,e_2^*)}{\tlist{n+1}{\alpha}{\tau}}}~\textbf{e-r-cons2}
  \and
    \inferrule
  {
    \Delta; \Phi_a; \Gamma \jelabt{t}{e}{e}{e^*}{e^*}{\tau}~~ \\
    \forall x_i \in dom(\Gamma), ~~e_i = \ecoerce{\Gamma(x_i)}{\tbox{\Gamma(x_i)}}~~
  }
  {
    \Delta; \Phi_a; \Gamma, \Gamma' \jelabt{0}{e}{e}{\elet \overline{ y_i = e_i \eapp x_i} \ein \enoch e^* [\overline{y_i/x_i}]}{\elet \overline{ y_i = e_i \eapp x_i} \ein \enoch e^* [\overline{y_i/x_i}]}{\tbox{\tau}}
  } ~\textbf{e-nochange}
    \and
    \inferrule
  {\ctx \jelabct{t}{e}{e'}{\tlist{n}{\alpha}{\tau}}\\
   \Delta; \Phi_a \wedge n = 0  ;\Gamma \jelabct{t'}{e_1}{e_1'}{\tau'}\\
   i, \Delta; \Phi_a \wedge n = i+1;  h: \tbox{\tau},
   tl : \tlist{i}{\alpha}{\tau}, \Gamma \jelabct{t'}{e_2}{e_2'}{\tau'}
\\
   i, \beta, \Delta; \Phi_a \wedge n = i+1 \wedge \alpha = \beta +1 ;
   h: \tau, tl : \tlist{i}{\beta}{\tau}, \Gamma \jelabt{t'}{e_2}{e_2'}{e_2^{**}}{e_2'^{**}}{\tau'}
   }
   {\ctx \jelabt{t+t'}
     { \hspace{-1em}
       \begin{minipage}[c]{9em}
         ~ $\ecase e \eof \enil \rightarrow e_1$ \\
         $~~~~~~~~~~|~h\,:: tl \rightarrow e_2$
       \end{minipage}
     }
     {\hspace{0em}
       \begin{minipage}[c]{9em}
         ~ $\ecase e \eof \enil \rightarrow e_1'$ \\
         $~~~~~~~~~~|~h\,:: tl \rightarrow e_2'$
       \end{minipage}
     }
     {\hspace{-1em}
       \begin{minipage}[c]{10em}
         ~ $\ecase e^* \eof \enil \, \rightarrow e_1^*$ \\
         $~~~~~~~~|~h\,::_{NC} tl\, \rightarrow e_2^*$ \\
         $~~~~~~~~|~h::_{C} tl~~~ \rightarrow e_2^{**}$
       \end{minipage}\hspace{-0.5em}
     }{\hspace{0em}
       \begin{minipage}[c]{10em}
         ~ $\ecase e'^* \eof \enil \, \rightarrow e_1'^*$ \\
         $~~~~~~~~|~h\,::_{NC} tl\, \rightarrow e_2'^*$ \\
         $~~~~~~~~|~h::_{C} tl~~~ \rightarrow e_2'^{**}$
       \end{minipage}
     }{\tau'}}~\textbf{e-r-caseL}

    \and
    \inferrule{
    i::S, \ctx \jelabct{t}{e}{e'}{\tau} \\
    i \not \in \fiv{\Phi_a; \Gamma}
  }
  { \ctx \jelabt{0}{\eLam. e}{\eLam. e'}{\eLam i. e^*}{\eLam i. e'^*}{\tsforall{i} \tau}}~\textbf{e-r-iLam}
    \and
    \inferrule{
    \ctx \jelabct{t}{e}{e'}{\tsforall{i} \tau}\\
    \Delta \vdash I : S
  }
  {\ctx \jelabt{t+t'[I/i]}{e []}{e' []}{e^* [I]}{e'^* [I]}{\tau\{ I/ i\}}}~\textbf{e-r-iApp}
    \and
    \inferrule
  {
    \Delta; \Phi_a; \Gamma \jelabct{t}{e_1}{e_2}{\tau}~~ \\
    \Delta; \Phi_a \jsubtype{\tau}{\tau'} ~~\\
    e' = \ecoerce{\tau}{\tau'} ~~
  }
  {
    \Delta; \Phi_a; \Gamma \jelabt{t'}{e_1}{e_2}{e' \eapp e_1^*}{e' \eapp e_2^*}{\tau'} \\
  }~\textbf{e-r-$\sqsubseteq$}
    \and
    \inferrule
{
  \ctx  \jelabct{t}{e}{e'}{\tau\{I/i\}}\\
  \Delta \sty{I}{\sort}
}
{
  \ctx  \jelabt{t}{\epack e}{\epack e'}{\epack e^* \ewith I}{\epack e'^* \ewith I}{\texists{i} \tau}
} ~\textbf{e-r-pack}
    \and
   \inferrule
{
  \ctx \jelabct{t_1}{e_1}{e_1'}{\texists{i} \tau_1}\\
  \sorted{i}, \Delta; \Phi_a; x: \tau_1, \Gamma \jelabct{t_2}{e_2}{e_2'}{\tau_2}\\
  i \not\in FV(\Phi_a;\Gamma, \tau_2, t_2) \\
  e_1^{**} = \eunpack e_1^* \eas (x, i) \ein  e_2^* \\
  e_2^{**} = \eunpack e_1'^* \eas (x, i) \ein  e_2'^*
}
{
  \ctx  \jelabt{t_1+t_2}{\eunpack e_1 \eas x \ein  e_2}{\eunpack e_1' \eas x \ein  e_2'}{e_1^{**}}{e_2^{**}}{\tau_2}
}~\textbf{e-r-unpack}
   \and
   \inferrule
  {
    \Delta; C \wedge \Phi_a; \Gamma \jelabct{t}{e_1}{e_2}{\tau} \\
    \Delta; \neg C \wedge \Phi_a; \Gamma \jelabt{t}{e_1}{e_2}{e_1^{**}}{e_2^{**}}{\tau} \\
    \Delta \wfcs{C}
  }
  {
    \Delta; \Phi_a; \Gamma \jelabt{t}{e_1}{e_2}{\esplit (e_1^*, e_1^{**}) \ewith C}{\esplit (e_2^*, e_2^{**}) \ewith C}{\tau} \\
  }~\textbf{e-r-split} 
  \and
   \inferrule
  {
    \Delta; \Phi_a \sat \bot\\
    \Delta; \Phi_a \wfty{\Gamma}
  }
  {
    \ctx \jelabt{t}{e_1}{e_2}{\econtra e_1}{\econtra e_2}{\tau} \\
  }~\textbf{e-r-contra}
\and
\inferrule{
    \trm{\Gamma}{1} \jelabun{k_1}{t_1}{e_1}{e_1^*}{\grt_1}~~\\
    \trm{\Gamma}{2} \jelabun{k_2}{t_2}{e_2}{e_2^*}{\grt_2}
    } {\Gamma \jelabt{t_1-k_2}{e_1}{e_2}{\eswitch e_1^*}{\eswitch e_2^*}{\tch{\grt_1}{\grt_2}}}~\textbf{e-switch}
  \end{mathpar}
  % Definitions at appendix/elaboration-rules-defs.tex
  \caption{RelInfRef embedding rules}
  \label{fig:elab-rules}
\end{figure*} 


\begin{figure*}
\begin{mathpar}
%\astuint
%
\and
%\astuunit
%\and
%
\inferrule{
\Delta; \psi_a; \Phi_a \jalgasubtype{\grt_1'}{\grt_1}{\Phi_1} \\
\Delta; \psi_a; \Phi_a \jalgasubtype{\grt_2}{\grt_2'}{\Phi_2}
}
{
\Delta; \psi_a; \Phi_a  \jalgasubtype{\grt_1 \to \grt_2}{\grt_1' \to \grt_2'}{\cand{\Phi_1}{\Phi_2}}
}~\textbf{alg-u-fun}

%
\and
%\astuprod
%\and
%\astusum
%\and
%
\astulist
%
\and
%
\inferrule
{
i, \Delta; \psi_a; \Phi_a \jalgasubtype{\grt}{\grt'}{\Phi_1} \\
}
{
\Delta; \psi_a; \Phi_a  \jalgasubtype{\tsforall{i} \grt}{\tsforall{i} \grt'}{\cforall{i}{\sort}{\cand{\Phi_1}{\Phi_2}}}
}\textbf{alg-u-$\forall$}

%
\and
%
\astuexists
%
\and
%
\astucimpl
%
\and
%
\astucprod
\end{mathpar} 
\caption{RelInfRef Algortihmic unary subtyping rules}
\label{fig:un-subtyping-rules}  
\end{figure*} 

\begin{figure*}
\begin{mathpar}
\astint
%
\and
%
% \astintbox
% %
\and
%\astunit
%\and
%
% \astunitbox
% %
\and
%
\inferrule{
\Delta; \psi_a; \Phi_a \jalgeqtype{\tau_1}{\tau_1'}{\Phi_1} \\
\Delta; \psi_a; \Phi_a \jalgeqtype{\tau_2}{\tau_2'}{\Phi_2}
}
{
\Delta; \psi_a; \Phi_a  \jalgeqtype{\tau_1 \to \tau_2}{\tau_1' \to \tau_2'}{\cand{\Phi_1}{\Phi_2}}
}~\textbf{alg-r-fun}
%
\and
%\astprod
%\and
%\astsum
%\and
%
\astlist
%
\and
%
% \astlistzero
% %
% \and
%
\inferrule
{
i, \Delta; \psi_a; \Phi_a \jalgeqtype{\tau}{\tau'}{\Phi} \\
}
{
\Delta; \psi_a; \Phi_a  \jalgeqtype{\tsforall{i} \tau}{\tsforall{i} \tau'}{\cforall{i}{\sort}{\Phi}}
}\textbf{$\forall$}
%
\and
%
\astexists
%
\and
%
% \astunrel
% %
% \and
%
% \astboxL
% %
% \and
% %
\astboxB
%
\and
% \astboxBR
% %
% \and
% %
% \astboxpushl
% %
% \and
% %
% \astboxpushr
% %
% \and
% %
%
% \astfunbox
% %
% \and
% %
% \astlistboxl
% %
% \and
% %
% \astlistboxr
% %
% \and
% %
% \astprodboxl
% %
% \and
% %
% \astprodboxr
% %
% \and
%
% \astsumboxl
% %
% \and
% %
% \astsumboxr
% %
% \and
%
% \astforallboxl
% %
% \and
% %
% \astforallboxr
% %
% \and
% %
% \astexistsboxl
% %
% \and
% %
% \astexistsboxr
% %
% \and
% %
\astunrel
%
\and
%
\astcimpl
%
\and
%
\astcprod
\end{mathpar}
  % Definitions at appendix/elaboration-rules-defs.tex
  \caption{RelInfRef alg eq binary rules}
  \label{fig:elab-rules}
\end{figure*} 


\begin{figure*}
\begin{mathpar}
\rrfinfvar
\and
\rrfchfix
\and
\rrfinfapp
\and
\rrfchiLam
\and
\rrfinfiApp
\and
\rrfchpack
\and
\rrfchunpack
\and
\rrfchcons
\and
\rrfchnil
\and
\rrfchcaseL
\and
\rrfchlet
\and
\rrfinfanno
\and
\rrfchupdown

\end{mathpar}
  \caption{RelInfRef alg unary rules  1}
  \label{fig:rrf-alg-u-rules-1}
\end{figure*} 

\begin{figure*}
\begin{mathpar}
\rrfchcandIntro
\and
\rrfchcimplIntro
\and
\rrfinfcimplElim
\and
\rrfchcandElim
\and
\rrfchsplit
\and
\rrfchcontra
\end{mathpar}
  \caption{RelInfRef alg unary rules  2}
  \label{fig:rrf-alg-u-rules-2}
\end{figure*} 

\begin{figure*}
\begin{mathpar}
  \inferrule
  {
    \Delta; {\psi_a}; \Phi_a; \tbox{\Gamma}  \chdifft{e}{e}{\tau}{t'}{\Phi}
  }
  {
    \Delta; \psi_a; \Phi_a; \Gamma', \tbox{\Gamma} \chdifft{\enoch e}{\enoch e}{\tbox{\tau}}{t}{\Phi}
  } ~\textbf{alg-r-nochange-$\downarrow$}
  \and
  \inferrule
{
  \bctx \infdifft{e_1}{e_2}{\tbox{\tau}}{\psi}{t}{\Phi}
}
{
  \bctx \infdifft{\eder e_1}{\eder e_2}{\tau}{\psi}{t}{\Phi}
}~\textbf{alg-r-der-$\uparrow$}
  \and
  % \chRder
  % \and
  \inferrule
{
\Gamma(x) = \tau
}
{
\bctx \infdifft{x}{x}{\tau}{\emptypsi}{0}{\ctrue}
} ~\textbf{alg-r-var-$\uparrow$}
  \and
  \inferrule
{
 \Delta; {\psi_a};  \Phi_a; f : \tau_1 \to \tau_2, x:\tau_1, \Gamma \chdifft{e}{e'}{\tau_2}{t'}{\Phi}
}
{
\bctx \chdifft{\efix f(x).e}{\efix f(x).e'}{\tau_1 \to \tau_2}{t}{\Phi}
} ~\textbf{alg-r-fix-$\downarrow$}
  \and
   \inferrule
{
    % \forall x_i \in \fvars{\efixNC f(x).e}.~ \exists \tau_i. ~\Gamma(x_i) = \tbox{\tau_i}\\
    \Delta; {\psi_a};  \Phi_a; f : \tbox{(\tau_1 \to \tau_2)}, x:\tau_1, \tbox{\Gamma} \chdifft{e}{e'}{\tau_2}{t'}{\Phi}
}
{
\Delta; \psi_a; \Phi_a; \Gamma', \tbox{\Gamma} \chdifft{\efixNC f(x).e}{\efixNC f(x).e}{\tbox{(\tau_1 \to \tau_2)}}{t}{\Phi}
} ~\textbf{alg-r-fix-$\downarrow\square$}
\and
  \inferrule
{
\bctx  \infdifft{e_1}{e_1'}{\tau_1 \to \tau_2}{\psi}{t_1}{\Phi_1} \\
\Delta; { \psi_a}; \Phi_a; \Gamma \chdifft{e_2}{e_2'}{\tau_1}{t_2}{\Phi_2}
}
{
\bctx  \infdifft{e_1 \eapp e_2}{e_1' \eapp e_2'}{\tau_2}{\psi}{t_1+t_2+t_e}{\cand{\Phi_1}{\Phi_2}}
}~\textbf{alg-r-app-$\uparrow$}
  \and
\inferrule
{
\Delta, \psi_a; \Phi \wfty{\tau}
}
{
\bctx  \chdifft{\enil}{\enil}{\tlist{n}{\alpha}{\tau}}{t}{\ceq{n}{0}}
}~\textbf{alg-r-nil-$\downarrow$}
  \and
   \inferrule
{
\freshSize{i,\beta} \\
\Delta; {\psi_a}; \Phi_a; \Gamma  \chdifft{e_1}{e_1'}{\tau}{t_1}{\Phi_1} \\
\Delta; {i,\beta,\psi_a}; \Phi_a; \Gamma
\chdifft{e_2}{e_2'}{\tlist{i}{\beta}{\tau}}{t_2}{\Phi_2}\\
\Phi_2' = \cand{\ceq{n}{(i+1)}}{\cexists{\beta}{\ssize}{\cand{\Phi_2}{\ceq{\alpha}{\beta+1}}}}
}
{
  \bctx \chdifft{\econsC(e_1,e_2)}{\econsC(e_1',e_2')}{\tlist{n}{\alpha}{\tau}}{t}{\cand{\Phi_1}{\cexists{i}{\ssize}{\Phi_2'}}}
}~\textbf{alg-r-consC-$\downarrow$}
  \and
  \inferrule
{
\freshSize{i} \\
\Delta; {\psi_a}; \Phi_a; \Gamma  \chdifft{e_1}{e_1'}{\tbox{\tau}}{t_1}{\Phi_1} \\
\Delta; {i,\psi_a}; \Phi_a; \Gamma
\chdifft{e_2}{e_2'}{\tlist{i}{\alpha}{\tau}}{t_2}{\Phi_2}\\
\Phi_2' = \cand{\Phi_2}{\ceq{n}{(i+1)}}
}
{
\bctx \chdifft{\econsNC(e_1,e_2)}{\econsNC(e_1',e_2')}{\tlist{n}{\alpha}{\tau}}{t}{\cand{\Phi_1}{\cexists{i}{\ssize}{\Phi_2'}}}
}~\textbf{alg-r-consNC-$\downarrow$}
  \and
  \inferrule
{
\bctx \infdifft{e}{e'}{\tlist{n}{\alpha}{\tau}}{\psi}{t_1}{\Phi_e}\\
\Delta; {  \psi_a}; \cand{\ceqz{n}}{\Phi_a}; \Gamma  \chdifft{e_1}{e_1'}{\tau'}{t_2}{\Phi_1} \\
\sized{i},\Delta; { \psi_a};  \cand{\ceq{n}{i+1}}{\Phi_a}; h :\tbox{\tau}, tl:\tlist{i}{\alpha}{\tau}, \Gamma \chdifft{e_2}{e_2'}{\tau'}{t_2}{\Phi_2}\\
\sized{i}, \sized{\beta},\Delta; { \psi_a};  \cand{\cand{\ceq{n}{i+1}}{\ceq{\alpha}{\beta + 1}}}{\Phi_a}; h :\tau, tl:\tlist{i}{\beta}{\tau}, \Gamma \chdifft{e_3}{e_3'}{\tau'}{t_2}{\Phi_3}\\
\Phi_{body} = {\cand{(\cimpl{\ceqz{n}}{\Phi_1})}{(\cforall{i}{\ssize}{\cimpl{(\ceq{n}{i+1})}{(\cand{\Phi_2}{\cforall{\beta}{\ssize}{\cimpl{(\ceq{\alpha}{\beta+1})}{\Phi_3}}})}})}}
}
{
\bctx \chdifft{\hspace{0em}
       \begin{minipage}[c]{10em}
         ~$\ecase e \eof \enil \, \rightarrow e_1$ \\
         $~~~~~~|~h\,::_{NC} tl\, \rightarrow e_2$ \\
         $~~~~~~|~h::_{C} tl~~~ \rightarrow e_3$
       \end{minipage}\hspace{0em}
     }{\hspace{0em}
       \begin{minipage}[c]{10em}
         ~ $\ecase e' \eof \enil \, \rightarrow e_1'$ \\
         $~~~~~~~~|~h\,::_{NC} tl\, \rightarrow e_2'$ \\
         $~~~~~~~~|~h::_{C} tl~~~ \rightarrow e_3'$
       \end{minipage}
     }{\tau'}{t}{\cand{\Phi_e}{\Phi_{body}}}
}~\textbf{alg-r-caseL-$\downarrow$}

  % \and
  % \chRsplit
\end{mathpar}

% \nocaptionrule
% Definitions at alg-typing-rules-defs.tex
\caption{RelInfRef  algorithmic typing rules (Part 1).}
\label{fig:selected-alg-typing-rules} 
\end{figure*} 


\begin{figure*}
  \begin{mathpar}
    \inferrule
  {
    \sorted{i}, \bctx \chdifft{e}{e'}{\tau}{t_e}{\Phi}
  }
  {
    \bctx  \chdifft{\eLam i. e}{\eLam i. e'}{\tsforall{i}
        \tau}{t}{(\cforall{i}{\sort}{\Phi})}
  } ~\textbf{alg-r-iLam-$\downarrow$}
    \and
    \inferrule
{
  \bctx  \infdifft{e}{e'}{\tsforall{i} \tau'}{\psi}{t}{\Phi} \\
  \Delta \sty{I}{S}
}
{
  \bctx \infdifft{e \, [I]}{e' \, [I]}{\tau'\{I/i\}}{\psi}{t+t_e[I/i]}{\Phi}
} ~\textbf{alg-r-iApp-$\uparrow$}
    \and
    \inferrule
  {
    \Delta; {\psi_a}; \Phi_a; \Gamma  \chdifft{e}{e'}{\tau\{I/i\}}{t}{\Phi}\\
    \Delta  \sty{I}{\sort}
}
{
  \bctx  \chdifft{\epack e \ewith I}{\epack e' \ewith I}{\texists{i} \tau}{t}{\Phi}
} ~\textbf{alg-r-pack-$\downarrow$}
    \and
    \inferrule
{
  \bctx \infdifft{e_1}{e_1'}{\texists{i} {\tau_1}}{\psi}{t_1}{\Phi_1} \\
  \sorted{i}, \Delta; { \psi_a}; \Phi_a; x: \tau_1, \Gamma
  \chdifft{e_2}{e_2'}{\tau_2}{t_2}{\Phi_2} \\
i \not\in FV(\Phi_a;\Gamma, \tau_2) \\
\Phi = {(\cand{\Phi_1}{\cforall{i}{\sort}{\Phi_2}})}
}
{
  \bctx  \chdifft{\eunpack e_1 \eas (x, i) \ein e_2}{\eunpack e_1' \eas (x, i) \ein e_2'}{\tau_2}{t}{\Phi}
}~\textbf{alg-r-unpack-$\downarrow$}
    \and
    \inferrule
{
  \Delta; \psi_a; \Phi \wedge C;  \Gamma \chdifft{e_1}{e_1}{\tau}{t}{\Phi}
}
{
  \bctx \chdifft{e_1}{e_2}{\tcprod{C}{\tau}}{t}{\cand{C}{(\cimpl{C}{\Phi})}}
} ~\textbf{alg-r-c-andI$\downarrow$}
    \and
    \inferrule
{
  \bctx \infdifft{e_1}{e_1'}{\tcprod{C}{\tau_1}}{\psi}{t_1}{\Phi_1} \\
  \Delta;   \psi_a; \Phi \wedge C;   x :\tau_1,  \Gamma  \chdifft{e_2}{e_2'}{\tau_2}{t_2}{\Phi_2} \\
  \Phi_2' = {\cimpl{C}{\Phi_2}}
}
{
  \bctx  \chdifft{\clet e_1 \eas x \ein e_2}{\clet e_1' \eas x \ein e_2'}{\tau_2}{t}{\cand{\Phi_1}{\Phi_2'}}
} ~\textbf{alg-r-c-andE$\downarrow$}
    \and
    \inferrule{
  \bctx \infdifft{e}{e'}{\tau'}{\psi}{t'}{\Phi_1}\\
  \Delta; { \psi_a}; \Phi_a \jalgeqtype{\tau'}{\tau}{\Phi_2} \\
}
{
  \bctx \chdifft{e}{e'}{\tau}{t}{{\cand{\Phi_1}{\Phi_2}}}
} ~\textbf{alg-r-$\uparrow\downarrow$}
    \and
    \inferrule
{
  \bctx \chdifft{e}{e'}{\tau}{t}{\Phi}\\
  \Delta; \Phi_a \wfty{\tau} \\
  \fivars{\tau} \in \Delta
}
{
  \bctx  \infdifft{(e:\tau)}{(e':\tau)}{\tau}{\cdot}{t}{\Phi}
} ~\textbf{alg-r-anno-$\uparrow$}
    \and
    \inferrule{
  \Delta; \psi_a; C \wedge \Phi_a; \Gamma \chdifft{e_1}{e_1'}{\tau}{t}{\Phi_1}\\\\
  \Delta; \psi_a; \neg C \wedge \Phi_a; \Gamma \chdifft{e_2}{e_2'}{\tau}{t}{\Phi_2}\\
  \Delta  \wfcs{C}
}
{
  \bctx \chdifft{\esplit (e_1, e_2) \ewith C}{\esplit (e_1', e_2') \ewith C}{\tau}{t}{\cand{\cimpl{C}{\Phi_1}}{\cimpl{\neg C}{\Phi_2}}}
} ~\textbf{alg-r-split$\downarrow$}
   \and
  \inferrule{
  \Delta; \psi_a; \Phi_a \sat \bot
}
{
  \bctx \chdifft{\econtra e}{\econtra e'}{\tau}{t}{\ctrue}
} ~\textbf{alg-r-contra$\downarrow$}
\and
  \inferrule
  {
    \Delta; \psi_a; \Phi; \trm{\Gamma}{1}  \infexecT{e_1}{\grt_1}{\psi_1}{}{}{\Phi_1}\\
    \Delta; \psi_a; \Phi; \trm{\Gamma}{2}  \infexecT{e_2}{\grt_2}{\psi_2}{}{}{\Phi_2}
  }
  {
    \bctx  \infdifft{\eswitch e_1}{\eswitch e_2}{\tch{\grt_1}{\grt_2}}{\psi_1,\psi_2}{}{\cand{\Phi_1}{\Phi_2
  }}}~\textbf{alg-r-switch$\uparrow$}
\and
\inferrule
  {
    \Delta; \psi_a; \Phi; \trm{\Gamma}{1}  \chexecT{e_1}{\grt_1}{}{}{\Phi_1}\\
    \Delta; \psi_a; \Phi; \trm{\Gamma}{2}
    \chexecT{e_2}{\grt_2}{}{}{\Phi_2} \\
    %\jalgasubtype{A}{B}{c}
  }
  {
    \bctx  \chdifft{\eswitch e_1}{\eswitch e_2}{\tch{\grt_1}{\grt_2}}{t}{(\cand{\Phi_1}{\Phi_2})}
   }~\textbf{alg-r-switch$\downarrow$}
  \end{mathpar}
\caption{RelInfRef algorithmic typing rules (Part 2).}
\label{fig:selected-alg-typing-rules2} 
\end{figure*} 


==> RSTLC/relinfref_lemmas.tex <==

\subsection{RefInfRef proof}
\begin{lem} [Substitution of RelInfRef unary Core] \label{lem:rrf-unary-substitution}
Assume that 
\begin{enumerate}
\item $\Delta;\Psi_a;\Omega \jtypeMt{0}{0}{e_1}{\grt}~~(1)$.
\item $\Delta;\Psi_a;\Omega,x:\grt \jtypeMt{0}{0}{e_1'}{\grt'}~~(2)$.
\end{enumerate}
then $\Delta;\Psi_a;\Omega \jtypeMt{0}{0}{e_1'[e_1/x]}{\grt'} $.
\end{lem}
\begin{proof}
By induction on the typing derivation of the second assumption (2).\\
\caseL{  \relrefinfmtyvar}
   \textbf{Subcase: } $z=x$.\\
 TS: $ \Delta;\Psi_a;\Omega \jtypeMt{}{}{z[e_1/x]}{\grt'} $.   \\
   Because $x=z$,$z[e_1/x]=e_1$, STS: $ \ctx
   \jtypeMt{}{}{e_1}{\grt'} $.\\
   From $(\Omega,x:\grt)(z) = \grt'$ and $x=z$, we know $\grt=\grt'$.\\
   By the above statements, STS: $ \Delta;\Psi_a;\Omega
   \jtypeMt{}{}{e_1}{\grt} $, which is proved by the assumption.\\
   \textbf{Subcase:}  $z \not = x$.\\
   we know: $\Omega(z) = \grt' ~~(\star)$.\\
   TS: $ \Delta;\Psi_a;\Omega \jtypeMt{}{}{z[e_1/x]}{\grt'} $. \\
   Because $x\not =z$, $z[e_1/x]=z$, STS: $ \Delta;\Psi_a;\Omega
   \jtypeMt{}{}{z}{\grt'} $.\\
   By the core rule \textbf{c-r-vars} and $(\star)$, we construct the
   derivation :\\
  $ \inferrule{\Omega(z) = \grt'}{\Delta;\Psi_a;\Omega
      \jtypeMt{}{}{z}{\grt'}}~\textbf{c-r-var} $

%%%%%%%%%%%%%%%%%%%%%%%%%%
\caseL{\relrefinfmtyfix }
$e_1'=\efix f(z).e_1$, $\grt'=\grt_1 \to \grt_2$.\\
 TS:  $ \Delta; \Phi_a; \Omega \jtypeMt{}{}{\efix f(z). (e_1''[e_1/x])}{\grt'} $. \\
By IH on (1) and (3), $ \Delta;\Psi_a;\Omega
 \jtypeMt{}{}{e_1''[e_1/x]}{\grt_2}~~(4) $.\\
By core rule \textbf{c-fix} and (4), we can derive :\\
$ \Delta; \Phi_a; \Omega \jtypeMt{}{}{\efix f(z). (e_1''[e_1/x])}{\grt'} $.
\end{proof}


\begin{lem} [Substitution of RelInfRef Core] \label{lem:rrf-substitution}
Assume that 
\begin{enumerate}
\item $\Delta;\Psi_a;\Gamma \jtypediffMt{t}{e_1}{e_2}{\tau}~~(1)$.
\item $\Delta;\Psi_a;\Gamma,x:\tau \jtypediffMt{t}{e_1'}{e_2'}{\tau'}~~(2)$.
\end{enumerate}
then $\Delta;\Psi_a;\Gamma \jtypediffMt{t}{e_1'[e_1/x]}{e_2'[e_2/x]}{\tau'} $.
\end{lem}

\begin{proof}
By induction on the typing derivation of the second assumption (2).\\
\begin{mainitem}
\caseL{  \inferrule{(\Gamma,x:\tau)(z) = \tau'}{\ctx,x:\tau
      \jstypet{z}{z}{\tau'}}~\textbf{c-r-var}}
   \textbf{Subcase: } $z=x$.\\
    TS: $ \ctx \jstypet{z[e_1/x]}{z[e_2/x]}{\tau'} $.  \\
   Because $x=z$,$z[e_1/x]=e_1$, $z[e_2/x]=e_1$, STS: $ \ctx
   \jstypet{e_1}{e_2}{\tau'} $.\\
   From $(\Gamma,x:\tau)(z) = \tau'$ and $x=z$, we know $\tau=tau'$.\\
   By the above statements, STS: $ \ctx
   \jstypet{e_1}{e_2}{\tau} $, which is proved by the assumption.\\
   \textbf{Subcase:}  $z \not = x$.\\
   we know: $\Gamma(z) = \tau' ~~(\star)$.\\
   TS: $ \ctx \jstypet{z[e_1/x]}{z[e_2/x]}{\tau'} $. \\
   Because $x\not =z$, $z[e_1/x]=z$, $z[e_2/x]=z$, STS: $ \ctx
   \jstypet{z}{z}{\tau'} $.\\
   By the core rule \textbf{c-r-vars} and $(\star)$, we construct the
   derivation :\\
  $ \inferrule{\Gamma(z) = \tau'}{\ctx
      \jstypet{z}{z}{\tau'}}~\textbf{c-r-var} $
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\caseL{\inferrule
{
\Delta; \Phi_a; \Gamma,x:\tau  \jstypet{e_1''}{e_2''}{\tbox{\tau'}}~~(3)
}
{
\Delta; \Phi_a; \Gamma,x:\tau  \jstypet{\eder e_1''}{\eder e_2''}{\tau'}
} ~\textbf{c-der}}
  $e_1'=\eder e_1''$, $e_2'=\eder e_2''$.\\
  TS:  $ \Delta; \Phi_a; \Gamma \jstypet{\eder (e_1''[e_1/x])}{\eder
    (e_2''[e_2/x])}{\tau'} $. \\
 By IH on (1) and (3), $ \Delta;\Psi_a;\Gamma
 \jtypediffMt{t}{e_1''[e_1/x]}{e_2''[e_2/x]}{\square \tau'}~~(4) $.\\
By core rule \textbf{c-der} and (4), we can derive \\
$\inferrule
{
\Delta; \Phi_a; \Gamma,x:\tau  \jstypet{e_1''[e_1/x]}{e_2''[e_2/x]}{\tbox{\tau'}}~~(4)
}
{
\Delta; \Phi_a; \Gamma,x:\tau \jstypet{\eder (e_1''[e_1/x])}{\eder
    (e_2''[e_2/x])}{\tau'}
} ~\textbf{c-der} $.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\caseL{  \inferrule{
       \Delta; \Phi_a;  z: \tau_1, f : \tau_1 \to \tau_2, \Gamma,x:\tau
       \jstypet{e_1''}{e_2''}{\tau_2}~~(3) }
            {\ctx,x:\tau \jstypet{ \efix f(z).e_1''}{\efix f(z).e_2''}{
              \tau_1 \to \tau_2}}~\textbf{c-r-fix}  
}
 $e_1'=\efix f(z).e_1$, $e_2'=\efix f(z).e_2'',\tau'=\tau_1 \to \tau_2$.\\
 TS:  $ \Delta; \Phi_a; \Gamma \jstypet{\efix f(z). (e_1''[e_1/x])}{\efix f(z).
    (e_2''[e_2/x])}{\tau'} $. \\
By IH on (1) and (3), $ \Delta;\Psi_a;\Gamma
 \jtypediffMt{t}{e_1''[e_1/x]}{e_2''[e_2/x]}{ \tau_2}~~(4) $.\\
By core rule \textbf{c-r-fix} and (4), we can derive :\\
$ \Delta; \Phi_a; \Gamma \jstypet{\efix f(z). (e_1''[e_1/x])}{\efix f(z).
    (e_2''[e_2/x])}{\tau'} $.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\caseL{ \inferrule
  {
    \Delta; \Phi_a;  z: \tau_1, f : \tbox{(\tau_1 \to \tau_2)}, \tbox{\Gamma},x:\tau \jstypet{e}{e}{\tau_2}~~(3)
  }
  {\nctx,\Gamma',x:\tau \jstypet{\efixNC f(z).e}{\efixNC f(z).e}{
              \tbox{(\tau_1 \to \tau_2)}}}~\textbf{c-r-fixNC}  }
 $e_1'=\efix f(z).e$, $e_2'=\efix f(z).e,\tau'=\tbox{(\tau_1 \to \tau_2)}$.\\
 TS:  $ \nctx,\Gamma' \jstypet{\efix f(z). (e[e_1/x])}{\efix f(z).
    (e[e_2/x])}{\tau'} $. \\
By IH on (1) and (3), $  \Delta; \Phi_a;  z: \tau_1, f : \tbox{(\tau_1 \to \tau_2)}, \tbox{\Gamma}
 \jtypediffMt{t}{e_1''[e_1/x]}{e_2''[e_2/x]}{ \tau_2}~~(4) $.\\
By core rule \textbf{c-r-fixNC} and (4), we can derive :\\
$ \nctx,\Gamma' \jstypet{\efix f(z). (e[e_1/x])}{\efix f(z).
    (e[e_2/x])}{\tau'} $. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\caseL{ \inferrule
  { \ctx,x:\tau \jstypet{e_3}{e_3'}{\tau''}~~(3) \\
    \ctx,x:\tau \jstypet{e_4}{e_4'}{\tlist{n}{\alpha}{\tau''}}~~(4)
  }
  { \ctx,x:\tau \jstypet{ \econsC(e_3,e_4) }{
      \econsC(e_3',e_4')}{\tlist{n+1}{\alpha+1}{\tau''}}}~\textbf{c-r-cons1}
}
$e_1'=\econsC(e_3,e_4) $,
$e_2'=\econsC(e_3',e_4'),\tau'=\tlist{n+1}{\alpha+1}{\tau''}$.\\

TS: $ \ctx \jstypet{\econsC(e_3[e_1/x],e_4[e_1/x]) }{
  \econsC(e_3'[e_2/x],e_4'[e_2/x]) }{\tau'}   $.\\
By IH on (1) and (3),$\ctx
\jstypet{e_3[e_1/x]}{e_3'[e_2/x]}{\tau''}~~(5)$.\\
By IH on (1) and (4),$\ctx
\jstypet{e_4[e_1/x]}{e_4'[e_2/x]}{\tau''}~~(6)$.\\
By core rule \textbf{c-r-fixNC} and (5),(6), we can derive :\\
$ \ctx \jstypet{\econsC(e_3[e_1/x],e_4[e_1/x]) }{
  \econsC(e_3'[e_2/x],e_4'[e_2/x]) }{\tau'}   $.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\caseL{ \inferrule
{
\Delta; \Phi_a; \tbox{\Gamma},x:\tau \jstypet{e}{e}{\tau''}~~(3)
}
{
\Delta; \Phi_a; \tbox{\Gamma}, \Gamma',x:\tau \jstypet{\enoch e}{\enoch e}{\tbox{\tau''}}
} ~\textbf{c-nochange} }
$e_1'=\enoch e $,
$e_2'=\enoch e,\tau'=\tbox{\tau''}$.\\
TS: $ \ctx \jstypet{\enoch e[e_1/x] }{
  \enoch e[e_2/x]) }{\tau'}   $.\\
By IH on (1) and (3),$\ctx
\jstypet{e[e_1/x]}{e[e_2/x]}{\tau''}~~(4)$.\\
By core rule \textbf{c-nochange} and (4), we can derive :\\
$ \ctx \jstypet{\enoch e[e_1/x] }{
  \enoch e[e_2/x]) }{\tau'}  $
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\caseL{\inferrule{
    \Delta; \Phi_a; \trm{\Gamma}{1} \jtypeMt{k_1}{t_1}{e_1''}{\grt_1}~~(3)\\
    \Delta; \Phi_a; \trm{\Gamma}{2} \jtypeMt{k_2}{t_2}{e_2''}{\grt_2}~~(4)
    } {\ctx \jtypediffMt{t_1-k_2}{\eswitch e_1''}{\eswitch e_2''}{\tch{\grt_1}{\grt_2}}}~\textbf{c-switch}}
$e_1'=\eswitch e_1'' $,
$e_2'=\eswitch e_2'',\tau'=\tch{\grt_1}{\grt_2}$.\\
TS: $ \ctx \jstypet{e_1' }{e_2' }{\tau'}   $.\\
By \Cref{lem:rrf-unary-substitution} on (1) and (3),$\Delta; \Phi_a; \trm{\Gamma}{1} 
\jtypeMt{}{}{e_1''[e_1/x]}{\grt_1}~~(5)$.\\
By \Cref{lem:rrf-unary-substitution} on (1) and (4),$\Delta; \Phi_a; \trm{\Gamma}{2} 
\jtypeMt{}{}{e_2''[e_2/x]}{\grt_2}~~(6)$.\\
By \textbf{c-switch} and (5),(6), we conclude that $ \ctx \jstypet{e_1' }{e_2' }{\tau'} $.
\end{mainitem} 
\end{proof}


\begin{lem}[Reflexivity of Unary Algorithmic Subtyping] \label{lem:rrf-alg-unary-subtyping-refl}
   $\Delta ; \Phi_a \jalgasubtype{\grt}{\grt}{\Phi}$ and $\Delta; \Phi_a \sat \Phi$.
\end{lem}

\begin{proof}
  By induction on the unary type.
\end{proof}

\begin{lem} [Reflexivity of Algorithmic Binary Type Equivalence] \label{lem:rrf-refl-ty-eq}
$\forall \Delta, \psi_a, \Phi_a$, there exists $\Phi$ s.t $\Delta; \psi_a; \Phi_a \jalgeqtype{\tau}{\tau}{\Phi}$ and $\Delta; \psi_a; \Phi_a \sat{\Phi}$.
 \end{lem}
 \begin{proof}
   By induction on the binary type.  Most cases are the same as \textbf{RelRef}'s corresponding
   proof.
  \begin{mainitem}
   \caseL{$\tch{\grt_1}{\grt_2} $}
    By algorithmic equivalence rule \textbf{U}.\\
  \begin{mathpar}
\inferrule
{
  \Delta; \psi_a; \Phi_a \jalgasubtype{\grt_1}{\grt_1}{\Phi_1}~~(\star)  \\
  \Delta; \psi_a; \Phi_a \jalgasubtype{\grt_1}{\grt_1}{\Phi_1}   \\
  \Delta; \psi_a; \Phi_a \jalgasubtype{\grt_2}{\grt_2}{\Phi_2}~~(\diam)  \\
  \Delta; \psi_a; \Phi_a \jalgasubtype{\grt_2}{\grt_2}{\Phi_2} 
}
{\Delta; \psi_a; \Phi_a \jalgeqtype{\tch{\grt_1}{\grt_2}}{\tch{\grt_1}{\grt_2}}{\cand{\cand{\Phi_1}{\Phi_1}}{\cand{\Phi_2}{\Phi_2}}}
}\textbf{U}
  \end{mathpar}  
  By \Cref{lem:rrf-alg-unary-subtyping-refl} on $(\star)$ and
  $(\diam)$, we conclude \\
 $\Delta; \psi_a; \Phi_a \jalgeqtype{\tch{\grt_1}{\grt_2}
 }{\tch{\grt_1}{\grt_2}}{\Phi_1 \land \Phi_1 \land \Phi_2 \land \Phi_2}$ and $\Delta; \psi_a; \Phi_a \sat{\Phi_1 \land \Phi_1 \land \Phi_2 \land \Phi_2}$.
\end{mainitem} 
 \end{proof}


\begin{lem}[Transitivity of Unary Algorithmic Subtyping] \label{lem:rrf-alg-unary-subtyping-trans}
  If $\Delta ; \Phi_a \jalgasubtype{\grt_1}{\grt_2}{\Phi_1}$ and $\Delta ; \Phi_a \jalgasubtype{\grt_2}{\grt_3}{\Phi_2}$ and $\Delta; \Phi_a \sat \cand{\Phi_1}{\Phi_2}$, then $\Delta ; \Phi_a \jalgasubtype{\grt_1}{\grt_3}{\Phi_3}$ for some $\Phi_3$ such that $\Delta; \Phi_a \sat \Phi_3$.
\end{lem}

\begin{proof}
  By induction on the first two algorithmic subtyping derivation.
  \begin{mainitem}
   \caseL{\inferrule{
\Delta; \psi_a; \Phi_a \jalgasubtype{\grt_1'}{\grt_1}{\Phi_1}~~(1) \\
\Delta; \psi_a; \Phi_a \jalgasubtype{\grt_2}{\grt_2'}{\Phi_2}~~(2)
}
{
\Delta; \psi_a; \Phi_a  \jalgasubtype{\grt_1 \to \grt_2}{\grt_1' \to \grt_2'}{\cand{\Phi_1}{\Phi_2}}
}~\textbf{alg-u-fun}, \inferrule{
\Delta; \psi_a; \Phi_a \jalgasubtype{\grt_1''}{\grt_1'}{\Phi_1'}~~(3) \\
\Delta; \psi_a; \Phi_a \jalgasubtype{\grt_2'}{\grt_2''}{\Phi_2}~~(4)
}
{
\Delta; \psi_a; \Phi_a  \jalgasubtype{\grt_1' \to \grt_2'}{\grt_1'' \to \grt_2''}{\cand{\Phi_1'}{\Phi_2'}}
}~\textbf{alg-u-fun}}
  By IH on (1) and (3), we get\\
 $\jalgasubtype{\grt_1''}{\grt_1}{\Phi_1 \land \Phi_1'} $ and $\Delta;
  \Phi_a \sat \Phi_1 \land \Phi_1'$.\\
 By IH on (2) and (4), we get\\
 $\jalgasubtype{\grt_2}{\grt_2''}{\Phi_2 \land \Phi_2'} $ and $\Delta;
  \Phi_a \sat \Phi_2 \land \Phi_2'$.\\
By rule \textbf{alg-u-fun} and above statements, we conclude \\
$\Delta; \psi_a; \Phi_a  \jalgasubtype{\grt_1 \to \grt_2}{\grt_1'' \to
  \grt_2''}{\cand{\Phi_1'}{\Phi_2'} \land \Phi_1 \land \Phi_2}$.
  \end{mainitem}
\end{proof}

\begin{thm}[Soundness of the Algorithmic Unary Subtyping]\label{thm:relrefinf-alg-unary-subtyping-soundness}
    Assume that 
    \begin{enumerate}
    \item $\Delta ; \psi_a; \Phi_a \jalgasubtype{\grt}{\grt'}{\Phi}$
    \item $\fivars{\Phi_a,\grt, \grt'} \subseteq \Delta, \psi_a$ 
    % \item $\Delta; \psi_a; \Phi_a \awfty{\grt} $
    % \item $\Delta; \psi_a; \Phi_a \awfty{\grt'} $
    \item $\Delta; \suba{\Phi_a} \sat \suba{\Phi}$ is
      provable s.t $\subsat{\Delta}{\theta_a}{\psi_a}$ is derivable.
    \end{enumerate}
    Then $\Delta ; \suba{\Phi_a} \jasubtype{\suba{\grt}}{\suba{\grt'}}$.
    
\end{thm} 
\begin{proof}
  By induction on the algorithmic unary subtyping derivation.
\begin{mainitem}
\caseL{\inferrule{
\Delta; \psi_a; \Phi_a \jalgasubtype{\grt_1'}{\grt_1}{\Phi_1}~~(1) \\
\Delta; \psi_a; \Phi_a \jalgasubtype{\grt_2}{\grt_2'}{\Phi_2}~~(2)
}
{
\Delta; \psi_a; \Phi_a  \jalgasubtype{\grt_1 \to \grt_2}{\grt_1' \to \grt_2'}{\cand{\Phi_1}{\Phi_2}}
}~\textbf{alg-u-fun}}
By IH on (1) and assumption 2,3, we get $ \Delta ; \suba{\Phi_a}
\jasubtype{\suba{\grt_1'}}{\suba{\grt_1}}   $.\\
By IH on (2) and assumption 2,3, we get $ \Delta ; \suba{\Phi_a}
\jasubtype{\suba{\grt_2}}{\suba{\grt_2'}}   $. \\
By subtyping rule \textbf{$\to \wexec$}, then we conclude\\
$\Delta ; \suba{\Phi_a} \jasubtype{\suba{\grt_1 \to
    \grt_2}}{\suba{\grt_1' \to \grt_2'}}$.
\end{mainitem}
\end{proof}

\begin{thm}[Completeness of the Unary Algorithmic Subtyping]\label{thm:rrf-alg-subtyping-completeness}
  Assume that $\Delta; \Phi_a \jasubtype{\grt}{\grt'}$. Then
  $\exists\, \Phi.$ such that
  $\Delta ; \Phi_a \jalgasubtype{\grt}{\grt'}{\Phi}$ and
  $\Delta; \Phi_a \sat \Phi$.
\end{thm} 

\begin{proof}
  By induction on the unary subtyping derivation.
\begin{mainitem}
\caseL{\inferrule{
 \Delta; \Phi_a \jasubtype{\grt_1'}{\grt_1}~~(1) \\
 \Delta; \Phi_a \jasubtype{\grt_2}{\grt_2'}~~(2) \\
}
{
 \Delta; \Phi_a \jasubtype{\grt_1 \to \grt_2}{\grt_1' \to \grt_2'}
}~\textbf{$\to \wexec$} }
        By IH on (1), there exists $\Phi_1$ s.t   $\Delta ; \Phi_a \jalgasubtype{\grt_1'}{\grt_1}{\Phi_1}$ and
  $\Delta; \Phi_a \sat \Phi_1$.\\
     By IH on (2), there exists $\Phi_2$ s.t   $\Delta ; \Phi_a \jalgasubtype{\grt_2}{\grt_2'}{\Phi_2}$ and
  $\Delta; \Phi_a \sat \Phi_2$.\\
  By \textbf{alg-u-fun} and the above statements, we conclude there
  eixsts $\Phi=\Phi_1 \land \Phi_2$, s.t  $\Delta ; \Phi_a
  \jalgasubtype{\grt_1 \to \grt_2}{\grt_1' \to \grt_2'}{\Phi}$ and
  $\Delta; \Phi_a \sat \Phi$.\\
\end{mainitem}
\end{proof}

\begin{thm}[Soundness of the Algorithmic Binary Type Equality]\label{thm:alg-ty-eq-soundness}
    Assume that
    \begin{enumerate}
    \item  $\Delta ; \psi_a; \Phi_a \jalgeqtype{\tau}{\tau'}{\Phi}$
    \item $\fivars{\Phi_a,\tau, \tau'} \subseteq \Delta, \psi_a$ 
    % \item $\Delta; \psi_a; \Phi_a \wfty{\tau} $
    % \item $\Delta; \psi_a; \Phi_a \wfty{\tau'} $
    \item $\Delta; \suba{\Phi_a} \sat \suba{\Phi}$ is
      provable s.t $\subsat{\Delta}{\theta_a}{\psi_a}$ is derivable.
    \end{enumerate}
    Then $\Delta ; \suba{\Phi_a}  \jeqtype{\suba{\tau}}{\suba{\tau'}}$.

\end{thm} 
\begin{proof}
  By induction on the algorithmic binary type equivalence
  derivation. Same as RelRef.
   \begin{mainitem}
  \caseL{\astunrel } 
  From assumption 3, $\Delta; \suba{\Phi_a} \sat \suba{(\Phi_1 \land \Phi_1' \land \Phi_2 \land \Phi_2')}$\\
  we know $\Delta; \suba{\Phi_a} \sat \suba{\Phi_1} ~~(a)$\\
  $\Delta; \suba{\Phi_a} \sat \suba{\Phi_1'} ~~(b)$\\
  $\Delta; \suba{\Phi_a} \sat \suba{\Phi_2} ~~(c)$\\
  $\Delta; \suba{\Phi_a} \sat \suba{\Phi_2'} ~~(d)$\\
  By IH on the first premise and (a), the second and (b), the third and (c) and the fourth and (d) and the rule \textbf{eq-U}, we can conclude that 
  $\Delta ; \suba{\Phi_a}  \jeqtype{\suba{U( \grt_1,\grt_2 )}}{\suba{U(\grt_1',\grt_2') }}$.
  \end{mainitem}
\end{proof}

\begin{thm}[Completeness of the Binary Algorithmic Type Equivalence]\label{thm:rrf-alg-ty-eq-completeness}
   Assume that $\Delta; \Phi_a \jeqtype{\tau}{\tau'}$. Then $\exists\, \Phi.$ such that  $\Delta ; \Phi_a \jalgeqtype{\tau}{\tau'}{\Phi}$ and $\Delta; \Phi_a \sat \Phi$.     
\end{thm} 

\begin{proof}
  By induction on the binary subtyping derivation. Same as RelRef.
  \begin{mainitem}
  \caseL{\etunrel } 
  By IH on the first premise, we know $\Delta ; \Phi_a \jalgasubtype{\grt_1}{\grt_1'}{\Phi_1}$ and $\Delta; \Phi_a \vDash \Phi_1$.\\
  Similarly by IH on the other premises respectively, we get\\
  $\Delta ; \Phi_a \jalgasubtype{\grt_1'}{\grt_1}{\Phi_1'}$ and $\Delta; \Phi_a \vDash \Phi_1'$\\
  $\Delta ; \Phi_a \jalgasubtype{\grt_2}{\grt_2'}{\Phi_2}$ and $\Delta; \Phi_a \vDash \Phi_2$ \\
  $\Delta ; \Phi_a \jalgasubtype{\grt_2'}{\grt_2}{\Phi_2'}$ and $\Delta; \Phi_a \vDash \Phi_2'$\\
  By the above statements and the relational algorithmic type equivalence rule \textbf{U}, we conclude where $\Phi= \Phi_1 \land \Phi_1' \land \Phi_2 \land \Phi_2'$:\\
   $\Delta ; \Phi_a \jalgeqtype{U(\grt_1,\grt_2)  }{U(\grt_1',\grt_2')  }{\Phi}$ and $\Delta; \Phi_a \vDash \Phi$
  \end{mainitem}
\end{proof}

\begin{lem} [Existence of coercions for relational subtyping] \label{lem:relrefinf-sub-elab}
  If $\Delta; \Phi_a \jsubtype{\tau}{\tau'}$ then there exists
  $\ecoerce{\tau}{\tau'}\!\!\in \mbox{Core}$ s.t.\ $\Delta; \Phi;
  \cdot
  \jtypediffMt{0}{\ecoerce{\tau}{\tau'}}{\ecoerce{\tau}{\tau'}}{\tau
    \to \tau'}$.
\end{lem}

\begin{proof}
  Proof is by induction on the subtyping derivation. We denote the
  witness $e$ of type $\tau \to \tau'$ as $\ecoerce{\tau}{\tau'}$ for clarity.

\begin{mainitem}
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \caseL{\stintU}
    Then, we can construct the derivation using the primitive function $\mbox{box}_{U} : \tbox{\tch{\tint}{\tint}} \to \trint$
    \begin{mathpar}
      \inferrule{ } { \Delta; \Phi; \cdot \jmintypesamet{0}{\efix f(x). \mbox{box}_{U} x}{\tbox{\tch{\tint}{\tint}} \to \trint}
      }
    \end{mathpar}

  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 5
    \caseL{\inferrule
{
}
{
\Delta; \Phi_a  \jsubtype{\tch{\tsforall{i} \grt
  }{\tsforall{i} {\grt'}}}{\tsforall{i}  {\tch{\grt}{\grt'}}}
}~\textbf{$\forall$U}}
    Then, we can immediately construct the following derivation where $e= {\efix f(x). \eLam i. \eswitch (x \, [i])}$ using the \textbf{c-switch} and \textbf{c-iApp} rules. \\
    $\Delta; \Phi; \cdot \jmintypesamet{0}{e}{(\tch{\tsforall{i} \grt}{\tsforall{i} \grt'}) \to {\tsforall{i} \tch{\grt}{\grt'}}}$\\


\end{mainitem}

\end{proof}


\begin{thm} [Types are preserved by embedding] \label{thm:relrefinf-min-soundness}
\mbox{} \begin{enumerate}
  \item If $\Delta; \Phi_a; \Omega \jelabun{}{}{e}{e^*}{\grt}$, then
    $\Delta; \Phi_a; \Omega \jtypeM{}{}{e^*}{\grt}$ and $\Delta; \Phi_a; \Omega \jtype{}{}{e}{\grt}$.
  \item If
    $\Delta; \Phi_a; \Gamma \jelabt{t}{e_1}{e_2}{e_1^*}{e_2^*}{\tau}$,
    then $\Delta; \Phi_a; \Gamma \jstypet{e_1^*}{e_2^*}{\tau}$ and
    $\Delta; \Phi_a; \Gamma \jstype{e_1}{e_2}{\tau}$.
\end{enumerate}
\end{thm}
%
\begin{proof}
By simultaneous induction on the given derivations.

\textbf{Proof of
  \Cref{thm:relrefinf-min-soundness}.1:} \\
  \begin{mainitem}
   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
   \caseL{\relrefinfelfix}
   By \Cref{thm:relinf-embedding-soundness}.1 on the premise, we get $  x: \grt_1, f : \grt_1 \to
    \grt_2, \Omega  \jtypeM{}{}{e}{\grt_2}$.
   Then, by unary core rule \textbf{c-fix},we conclude: $\relrefinfmtyfix$.
  \end{mainitem}

\begin{spacing}{1.3}
  \hspace{-1cm} \textbf{Proof of \Cref{thm:relrefinf-min-soundness}.2:} \\
\begin{mainitem} 
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
  \caseL{$\relrefinfelswitch[(\star)][(\diam)]$}
  By \Cref{thm:relrefinf-min-soundness}.1 on $(\star)$, we get $\Delta; \Phi; \Omega \jtypeMt{k_1}{t_1}{e_1^*}{\grt_1}~~(\star\star)$. \\
  By \Cref{thm:relrefinf-min-soundness}.1 on $(\diam)$, we get $\Delta; \Phi; \Omega \jtypeMt{k_2}{t_2}{e_2^*}{\grt_2}~~(\diam\diam)$. \\
  Then, we conclude as follows: $\relrefinfmtyswitch$ 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
  \caseL{$\relrefinfelrsubsum[(\star)][(\diam)]$}
  By \Cref{thm:relrefinf-min-soundness}.2 on $(\star)$,  $\Delta; \Phi; \Gamma \jtypediffMt{t}{e_1^*}{e_2^*}{\tau}~~(\star\star)$. \\
  By \Cref{lem:relrefinf-sub-elab} using $(\diam)$, we know that $\Delta; \Phi; \cdot \jtypediffMt{0}{e'}{e'}{\tau \to \tau'}~~(\diam\diam)$.\\
  By applying \textbf{c-r-app} rule 
  on $(\star\star)$ and $(\diam\diam)$, we get
  $\Delta; \Phi; \Gamma \jtypediffMt{t}{e' \eapp e_1^*}{e' \eapp e_2^*}{\tau'}~~(\spadesuit)$. \\
  By reflexivity of binary type equivalence, we know 
  $\Delta; \Phi_a \jeqtype{\tau'}{\tau'}~~(\spadesuit\spadesuit)$.\\
  Then, we conclude as
  follows:
  \begin{mathpar}
       \inferrule{ 
     \ctx \jtypediffMt{t}{e' \eapp e_1^*}{e' \eapp e_2^*}{\tau'}~~(\spadesuit)\\
     \Delta; \Phi_a \jeqtype{\tau'}{\tau'} ~~(\spadesuit\spadesuit)\\\\
  }
  {\ctx \jtypediffMt{t'}{e' \eapp e_1^*}{e' \eapp e_2^*}{\tau'} }
  ~{\textbf{c-r}-\pmb{\sqsubseteq}}
  \end{mathpar}

  \end{mainitem}

\end{spacing}

\end{proof}

\begin{thm} [Completeness of embedding] \label{thm:relrefinf-min-completeness}
  \mbox{}
  \begin{enumerate}
  \item If $\Delta; \Phi_a; \Omega \jtype{}{}{e}{\grt}$, then there
    exists an $ e^*$ such that $\Delta; \Phi; \Omega
    \jelabun{}{}{e}{e^*}{\grt}$.
    \item If $\Delta; \Phi_a; \Gamma  \jstype{e_1}{e_2}{\tau}$,
      then there exist $ e_1^*, e_2^*$ such that $\Delta; \Phi_a; \Gamma
      \jelabt{t}{e_1}{e_2}{e_1^*}{e_2^*}{\tau}$.
  \end{enumerate}
\end{thm}
\begin{proof}
By simultaneous induction on the given {\tname} derivations.
\begin{spacing}{1.3}
  \hspace{-1cm} \textbf{Proof of \Cref{thm:relrefinf-min-completeness}.1:} \\
\begin{mainitem} 
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
    \caseL{\inferrule{
    \Delta; \Phi_a;\Omega \jtype{k}{t}{e}{\grt}~~(\star) \\
    \Delta; \Phi_a;\jasubtype{\grt}{\grt'}~~(\diam) \\
}{
 \Delta; \Phi_a; \Omega \jtype{}{}{e}{\grt'}
}~\textbf{$\sqsubseteq$ } } 
    By \Cref{thm:relrefinf-min-completeness}.1 on $(\star)$, we get $\exists\, e^*$ such that $ \Delta; \Phi_a;\Omega \jelabun{}{}{e}{e^*}{\grt} ~~(\star\star)$. \\
    By \textbf{e-u-$\sqsubseteq$} rule using $(\star\star)$,
    $(\diam)$, we conclude as follows\\ $\relrefinfelsubsum$



  \end{mainitem}

\end{spacing}

  
\begin{spacing}{1.3}
  \hspace{-1cm} \textbf{Proof of \Cref{thm:relrefinf-min-completeness}.2:} \\

  \begin{mainitem}
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \caseL{  \inferrule
    { \Delta; \Phi; |\Gamma|_1 \jtype{}{}{e_1}{\grt_1}~~(\star)   \\ \Delta; \Phi;|\Gamma|_2 \jtype{}{}{e_2}{\grt_2}~~(\diam)  }  
    { \Delta; \Phi;\Gamma \jstype{e_1}{e_2}{  \tch{\grt_1}{\grt_2}
      }}~\textbf{r-switch} }

    By \Cref{thm:relrefinf-min-completeness}.1 on $(\star)$, we get $\exists\, e_1^*$ such that $\Delta; \Phi; \Omega \jelabcu{k_1}{t_1}{e_1}{\grt_1} ~~(\star\star)$. \\
    By \Cref{thm:relrefinf-min-completeness}.1 on $(\diam)$, we get $\exists\, e_2^*$ such that $\Delta; \Phi; \Omega \jelabcu{k_2}{t_2}{e_2}{\grt_2} ~~(\diam\diam)$. \\
    By \textbf{e-switch} embedding rule using $(\star\star)$ and $(\diam\diam)$, we can conclude as follows:\\
    $\relrefinfelswitch[(\star\star)][(\diam\diam)]$. \\

 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \caseL{\relreftync[(\star)][(\diam)]}
    By IH2 on $(\star)$, we get $\exists\, e^*$ such that $\Delta; \Phi_a; \Gamma \jelabt{t}{e}{e}{e^*}{e^*}{\tau} ~~(\dagg)$. \\
    By \lemref{lem:relref-elab} on $(\diam)$, we get $\exists e_i= \ecoerce{\Gamma(x_i)}{\tbox{(\Gamma(x_i)}}$ for all $x_i \in dom(\Gamma)~~(\dagg\dagg)$.\\
    By \textbf{e-nochange} embedding rule using $(\dagg)$ and $(\dagg\dagg )$, we can conclude as follows:\\
    $\relrefembednochange[(\dagg)][(\dagg\dagg)]$. 
    
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
   \caseL{\relreftycaseL[(\star)][(\diam)][(\dagg)][(\spadesuit)]}
    By IH2 on $(\star)$, we get $\exists\, e^*$  and $\exists\, e'^*$ s.t. $\Delta; \Phi_a; \Gamma \jelabt{t}{e}{e'}{e^*}{e'^*}{\tlist{n}{\alpha}{\tau}} ~~(\star\star)$. \\
   By IH2 on $(\diam)$, we get $\exists\, e_1^*$  and $\exists\, e_1'^*$ s.t. $\Delta; \ceqz{n} \wedge \Phi_a; \Gamma \jelabt{t}{e_1}{e_1'}{e_1^*}{e_1'^*}{\tau'} ~~(\diam\diam)$. \\
   By IH2 on $(\dagg)$, we get $\exists\, e_2^*$  and $\exists\, e_2'^*$ s.t. \\$\sorted{i}, \Delta; \ceq{n}{i+1} \wedge \Phi_a; h :\tbox{\tau}, tl : \tlist{i}{\alpha}{\tau}, \Gamma \jelabt{t}{e_2}{e_2'}{e_2^*}{e_2'^*}{\tau'} ~(\dagg\dagg)$. \\
   By IH2 on $(\spadesuit)$, we get $\exists\, e_2^{**}$  and $\exists\, e_2'^{**}$ s.t.\\ $\sorted{i}, \sorted{\beta}, \Delta; \ceq{n}{i+1} \wedge \ceq{\alpha}{\beta+1} \wedge \Phi_a; h :\tau, tl : \tlist{i}{\beta}{\tau}, \Gamma \jelabt{t}{e_2}{e_2'}{e_2^{**}}{e_2'^{**}}{\tau'} ~(\spadesuit\spadesuit)$. \\
    
    By \textbf{e-caseL} embedding rule using $(\star\star)$, $(\diam\diam)$, and $(\spadesuit\spadesuit)$, we can conclude as follows\\
    $\relrefembedcaseL$

     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

    \caseL{\relreftyfixnc[(\star)][(\diam)]}
    By IH2 on $(\star)$, we get $\exists\, e^*$ such that $\Delta; \Phi_a; x: \tau_1, f: \tbox{(\tau_1 \to \tau_2)}, \Gamma \jelabt{t}{e}{e}{e^*}{e^*}{\tau_2} ~~(\star\star)$. \\
    By \Cref{lem:relrefinf-sub-elab}  on $(\diam)$, we get $\exists e_i= \ecoerce{\Gamma(x_i)}{\tbox{(\Gamma(x_i)}}$ for all $x_i \in dom(\Gamma)~~(\diam\diam)$.\\
    
    By \textbf{e-fixNC} embedding rule using $(\star\star)$ and $(\diam\diam )$, we can conclude as follows:\\
    $\relrefembedfixnc$. 


    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
    \caseL{\relreftyilam[(\star)]}
    By IH2 on $(\star)$, we get $\exists\, e^*$ and $\exists\, e'^*$ such that $\sorted{i}, \Delta; \Phi_a; \Gamma \jelabt{t}{e}{e'}{e^*}{e'^*}{\tau} ~~(\star\star)$. \\
    By \textbf{e-iLam} embedding rule using $(\star\star)$ , we can conclude as follows:\\
    $\relrefembedilam$. 

    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
    \caseL{\relreftyiapp[(\star)][(\diam)]}
    By IH2 on $(\star)$, we get $\exists\, e^*$ such that $\Delta; \Phi_a; \Gamma \jelabt{t}{e}{e'}{e^*}{e'^*}{\tsforall{i} \tau} ~~(\star\star)$. \\
    By \textbf{e-iApp} embedding rule using $(\star\star)$ and $(\diam)$, we can conclude as follows:\\
    $\relrefembediapp$. 

    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
    \caseL{\relreftypack[(\star)][(\diam)]}
    By IH2 on $(\star)$, we get $\exists\, e^*$ and $\exists\, e'^*$ such that $\Delta; \Phi_a; \Gamma \jelabt{t}{e}{e'}{e^*}{e'^*}{\tau\{I/i\}} ~~(\star\star)$. \\
    By \textbf{e-pack} embedding rule using $(\star\star)$ and $(\diam)$ , we can conclude as follows:\\
    $\relrefembedpack$. 

    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
    \caseL{\relreftyunpack[(\star)][(\diam)]}
    By IH2 on $(\star)$, we get $\exists\, e_1^*$ and $\exists\, e_1'^*$ such that $\Delta; \Phi_a; \Gamma \jelabt{t}{e_1}{e_1'}{e_1^*}{e_1'^*}{\texists{i} \tau_1} ~~(\star\star)$. \\
    By IH2 on $(\diam)$, we get $\exists\, e_2^*$ and $\exists\, e_2'^*$ such that $\sorted{i}, \Delta; \Phi_a; x: \tau_1, \Gamma \jelabt{t}{e_2}{e_2'}{e_2^*}{e_2'^*}{\tau_2} ~~(\diam\diam)$. \\
    By \textbf{e-unpack} embedding rule using $(\star\star)$ and $(\diam\diam)$ , we can conclude as follows:\\
    $\relrefembedunpack$. 

   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
    \caseL{$\relreftysub[(\star)][(\diam)]$}  
    By IH2 on $(\star)$, we get $\exists\, e_1^*,e_2^*$ such that $\Delta; \Phi_a; \Gamma \jelabct{t}{e_1}{e_2}{\tau} ~~(\star\star)$. \\
    By \Cref{lem:relrefinf-sub-elab} on $(\diam)$, we can show that $\exists e' = \ecoerce{\tau}{\tau'}~~(\diam\diam)$.\\
    By \textbf{e-r-$\sqsubseteq$} rule using $(\star\star)$,
    $(\diam\diam)$ and $(\diam)$, we conclude as follows\\ 
   $\relrefembedsub$

  
    \end{mainitem}
\end{spacing}
\end{proof}

\begin{thm}[Soundness of algorithmic typechecking]\label{thm:relrefinf-alg-typing-soundness}
\mbox{}
  \begin{enumerate}
  \item Assume that $\uctx \chexect{e}{\grt}{}{}{\Phi} \rightarrow {\color{red}\Phi}$ and
    $\fivars{\Phi_a,\Omega,\grt} \subseteq dom(\Delta, \psi_a) $
    and $\theta_a$ is a valid substitution for $\psi_a$ s.t.
    $\Delta; \suba{\Phi_a} \sat \suba{\Phi}$ holds. Then,
    $\Delta; \suba{\Phi_a}; \suba{\Omega}
    \jtypeM{}{}{\erty{e}}{\suba{\grt}}$.

  \item Assume that $\uctx \infexect{e}{\grt}{}{}{}{\Phi} \Rightarrow \Phi$ and
    $\fivars{\Phi_a,\Omega} \subseteq dom(\Delta, \psi_a)$ and
    $ \theta_a$ is the valid substitutions for 
    $\psi_a$ such that $\Delta; \suba{\Phi_a} \sat \suba{\Phi}$
    holds. Then,
    $\Delta; \suba{\Phi_a}; \suba{\Omega}
    \jtypeM{}{}{\erty{e}}{\suba{\grt}}$.
    % and $\Delta; \psi_a; \Phi_a \awfty{\grt} $

\item Assume that $\bctx \chdifft{e}{e'}{\tau}{t}{\Phi}$ and
  $\fivars{\Phi_a,\Gamma,\tau} \subseteq dom(\Delta, \psi_a)$ and
  $\theta_a$ is a valid substitution for $\psi_a$ such that
  $\Delta; \suba{\Phi_a} \sat \suba{\Phi}$ holds. Then,
  $\Delta; \suba{\Phi_a}; \suba{\Gamma}
  \jtypediffMt{\suba{t}}{\erty{e}}{\erty{e'}}{\suba{\tau}}$.

\item Assume that $\bctx \infdifft{e}{e'}{\tau}{\psi}{t}{\Phi}$ and
  $\fivars{\Phi_a,\Gamma} \subseteq dom(\Delta, \psi_a) $ 
  and $ \theta_a$ is the valid substitution for  $\psi_a$
  such that $\Delta; \suba{\Phi_a} \sat \suba{\Phi}$ holds. Then,
  $\Delta; \suba{\Phi_a}; \suba{\Gamma}
  \jtypediffMt{\subta{t}}{\erty{e}}{\erty{e'}}{\suba{\tau}}$.
\end{enumerate}  
\end{thm}
%
\begin{proof}
By simultaneous induction on the given algorithmic typing derivations.

\begin{spacing}{1.3}
  \hspace{-1cm} \textbf{Proof of \Cref{thm:relrefinf-alg-typing-soundness}.1:} \\
  
  % Unless otherwise stated, assume that we can partition $\Delta$ as
  % $\Delta = \Delta_e, \Delta_u$ and $\forall \theta~\forall\theta_e.$
  % $\Delta_u \sat \sub{\Phi}{\theta~\theta_e}$ is provable where
  % $\subsat{\Delta_u}{\theta}{\psi}$ and
  % $\subsat{\cdot}{\theta_e}{\Delta_e}$ are derivable.
\begin{mainitem}
  \setlength{\itemsep}{10pt}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % \caseL{\chpair}
%   TS: $\Delta; \suba{\Phi_a}; \suba{\Omega}  \jtypeM{\suba{k}}{\suba{t}}{\la \erty{e_1}, \erty{e_2} \ra}{\suba{\grt_1} \ttimes \suba{\grt_2}}$. \\
% By the main assumptions, we have
% $\fivars{\Phi_a,\Omega,\grt,k, t} \subseteq dom(\Delta, \psi_a)~~(\star)$ \\
% $\Delta; \suba{\Phi_a} \sat \suba{(\cexists{k_1,t_1}{\scost}{\cand{\Phi_1}{\cexists{k_2,t_2}{\scost}{\cand{\Phi_2}{\cand{\ceq{(t_1+t_2)}{t}}{\ceq{(k_1+k_2)}{k}}}}}})}~~(\star\star)$ \\
% Using $(\star)$,  $(\star\star)$'s derivation must be in a form such that we have
% \begin{enumih}
% \item $\Delta \sty{K_1}{\scost}$ and  $\Delta \sty{T_1}{\scost}$ 
% \item $\Delta \sty{K_2}{\scost}$ and  $\Delta \sty{T_2}{\scost}$ 
% \item $\Delta; \suba{\Phi_a} \sat \subaex{\Phi_1}{k_1\mapsto K_1, t_1 \mapsto T_1}$
% \item $\Delta; \suba{\Phi_a} \sat \subaex{\Phi_2}{k_2 \mapsto K_2, t_2 \mapsto T_2}$
% \item $\Delta; \suba{\Phi_a} \sat {\cand{\ceq{(T_1+T_2)}{\suba{t}}}{\ceq{(K_1+K_2)}{\suba{k}}}}$
% \end{enumih}

% By \Cref{thm:alg-typing-soundness}.1 on the first premise using $(\star)$ and c), we can show that
% \begin{equation}
%   \label{eq:alg-usound-pair1}
%       \Delta; \suba{\Phi_a}; \suba{\Omega}  \jtypeM{K_1}{T_1}{\erty{e_1}}{\suba{\grt_1}}
% \end{equation}
% By \Cref{thm:alg-typing-soundness}.1 on the second premise using $(\star)$ and d), we can show that
% \begin{equation}
%   \label{eq:alg-usound-pair2}
%       \Delta; \suba{\Phi_a}; \suba{\Omega}  \jtypeM{K_2}{T_2}{\erty{e_2}}{\suba{\grt_2}}
% \end{equation}
% Combining \cref{eq:alg-usound-pair1,eq:alg-usound-pair2} with \textbf{c-prod} rule, we get \\
% $      \Delta; \suba{\Phi_a}; \suba{\Omega}  \jtypeM{K_1+ K_2}{T_1+T_2}{\la \erty{e_1}, \erty{e_2} \ra}{\suba{\grt_1} \ttimes \suba{\grt_2}}$. \\
% Then, by using e) with the  \textbf{c-}$\pmb{\sqsubseteq}\wexec$ rule
% , we can conclude that $\Delta; \suba{\Phi_a}; \suba{\Omega}  \jtypeM{\suba{k}}{\suba{t}}{\la \erty{e_1}, \erty{e_2} \ra}{\suba{\grt_1} \ttimes \suba{\grt_2}}$. \\

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \caseL{\rrfchupdown}
  TS: $\Delta; \suba{\Phi_a}; \suba{\Omega}  \jtypeMt{\suba{k}}{\suba{t}}{\erty{e}}{\suba{\grt}}$. \\
By the main assumptions, we have
$\fivars{\Phi_a,\Omega,\grt} \subseteq dom(\Delta, \psi_a)~~(\star)$ and \\
$\Delta; \suba{\Phi_a} \sat \suba{{\cand{\Phi_1}{\Phi_2}}}~~(\star\star)$ \\
% By \Cref{invariant:alg-typechecking} using $(\star)$ and the first premise, we get $ \fivars{\grt',k', t',\Phi_1} \subseteq
% dom(\Delta, \psi; \psi_a)~(\diam)$.\\
Using $(\star)$ and $ (\diam)$,  $(\star\star)$'s derivation must be in a form such that we have
\begin{enumih}
\item $\subsat{\Delta}{\theta_a}{\psi_a}$
\item $\Delta; \suba{\Phi_a} \sat \suba{\Phi_1}$
\item $\Delta; \suba{\Phi_a} \sat \suba{\Phi_2}$
\end{enumih}
By IH2 on the first premise using $(\star)$, a) and b), we can show that
\begin{equation}
  \label{eq:alg-usound-updown1}
      \Delta; \suba{\Phi_a}; \suba{\Omega}  \jtypeMt{\subta{k'}}{\suba{t'}}{\erty{e}}{\suba{\grt'}}
\end{equation}
By \Cref{thm:relrefinf-alg-unary-subtyping-soundness} using the second premise and c), we obtain
\begin{equation}
  \label{eq:alg-usound-updown2}
      \Delta; \suba{\Phi_a} \jasubtype{\suba{\grt'}}{{\suba{\grt}}}
\end{equation}
Note that due to $(\star)$,  we can conclude by the  \textbf{c-}${\pmb{\sqsubseteq}\wexec}$ rule using \cref{eq:alg-usound-updown1,eq:alg-usound-updown2} that  $\Delta; \suba{\Phi_a}; \suba{\Omega}  \jtypeMt{\suba{k}}{\suba{t}}{\erty{e}}{\suba{\grt}}$.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \caseL{\rrfchfix}
  TS: $\Delta; \suba{\Phi_a}; \suba{\Omega}  \jtypeMt{\suba{k}}{\suba{t}}{\efix f(x). \erty{e}}{\suba{\grt_1} \to \suba{\grt_2}}$. \\
By the main assumptions, we have
$\fivars{\Phi_a,\Omega,\grt_1 \to \grt_2 } \subseteq dom(\Delta, \psi_a)~~(\star)$ and \\
$\Delta; \suba{\Phi_a} \sat \suba{\Phi}~~(\star\star)$ \\
Using $(\star)$, we can show that
\begin{enumih}
\item $\fivars{\Phi_a,\Omega,\grt_1, \grt_1 \to \grt_2} \subseteq dom(\Delta, \psi_a).$\\
\end{enumih}
We also can show that $(\star\star)$'s derivation must be in a form such that we have
\begin{enumih}[resume]
\item $\Delta; \suba{\Phi_a} \sat \suba{\Phi}$
\end{enumih}
By IH1 on the first premise using a) and b), we can show that
\begin{equation}
  \label{eq:alg-usound-fix}
      \Delta; \suba{\Phi_a}; x:\suba{\grt_1},f: {\suba{\grt_1} \to \suba{\grt_2}}, \suba{\Omega}  \jtypeMt{\suba{k'}}{\suba{t'}}{\erty{e}}{\suba{\grt_2}}
    \end{equation}
    By the \textbf{c-fix} rule using \cref{eq:alg-usound-fix}, we obtain \\
    $\Delta; \suba{\Phi_a}; \suba{\Omega}  \jtypeMt{0}{0}{\efix
      f(x). \erty{e}}{\suba{\grt_1} \to \suba{\grt_2}}$. \\


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \caseL{\rrfchiLam}
  TS: $\Delta; \suba{\Phi_a}; \suba{\Omega}  \jtypeMt{\suba{k}}{\suba{t}}{\eLam i. \erty{e}}{\tsforall{i} \suba{\grt}}$. \\
By the main assumptions, we have
$\fivars{\Phi_a,\Omega, \tsforall{i} \grt} \subseteq dom(\Delta, \psi_a)~~(\star)$ and \\
$\Delta; \suba{\Phi_a} \sat \suba{\cforall{i}{S}{\Phi}}~~(\star\star)$ \\
Using $(\star)$, we can show that
\begin{enumih}
\item $\fivars{\Phi_a,\Omega, \grt} \subseteq i, dom( \Delta, \psi_a).$
\end{enumih}
We can also show that $(\star\star)$'s derivation must be in a form such that we have
\begin{enumih}[resume]
\item $\sorted{i}, \Delta; \suba{\Phi_a} \sat \suba{\Phi}$
\end{enumih}
By IH1 on the premise using a) and b), we can show that
\begin{equation}
  \label{eq:alg-usound-iLam}
      \sorted{i}, \Delta; \suba{\Phi_a}; \suba{\Omega}  \jtypeMt{\suba{k_e}}{\suba{t_e}}{\erty{e}}{\suba{\grt}}
    \end{equation}
    By the \textbf{c-iLam} rule using \cref{eq:alg-usound-iLam}, we obtain 
    $\Delta; \suba{\Phi_a}; \suba{\Omega}  \jtypeMt{0}{0}{\eLam i. \erty{e}}{\tsforall{i} \suba{\grt}}$. \\
   

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \caseL{\rrfchpack}
  TS: $\Delta; \suba{\Phi_a}; \suba{\Omega}  \jtypeMt{\suba{k}}{\suba{t}}{\epack \erty{e} \ewith I }{\texists{i} \suba{\grt}}$. \\ 
By the main assumptions, we have
$\fivars{\Phi_a,\Omega, \texists{i} \grt} \subseteq dom(\Delta, \psi_a)~~(\star)$ and \\
$\Delta; \suba{\Phi_a} \sat \suba{\Phi}~~(\star\star)$ \\
Using $(\star)$ and the second premise, we can show that
\begin{enumih}
\item $\fivars{\Phi_a,\Omega, \grt\{I/i\}} \subseteq dom(\Delta, \psi_a).$
\end{enumih}
By IH1 on the premise using a) and $(\star\star)$, we can show that
\begin{equation}
  \label{eq:alg-usound-pack}
       \Delta; \suba{\Phi_a}; \suba{\Omega}  \jtypeMt{\suba{k}}{\suba{t}}{\erty{e}}{\suba{\grt}\{I/i\}}
    \end{equation}
    By the \textbf{c-pack} rule using \cref{eq:alg-usound-pack} and the second premise, we obtain \\
    $\Delta; \suba{\Phi_a}; \suba{\Omega}  \jtypeMt{\suba{k}}{\suba{t}}{\epack \erty{e} \ewith I}{\texists{i} \suba{\grt}}$. 



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \caseL{\rrfchunpack}
  TS: $\Delta; \suba{\Phi_a}; \suba{\Omega}  \jtypeMt{\suba{k}}{\suba{t}}{\eunpack \erty{e_1} \ewith (x,i) \ein \erty{e_2}}{\suba{\grt_2}}$. \\ 
By the main assumptions, we have
$\fivars{\Phi_a,\Omega, \grt_2} \subseteq dom(\Delta, \psi_a)~~(\star)$ and \\
$\Delta; \suba{\Phi_a} \sat \suba{\cand{\Phi_1}{\cforall{i}{\sort}{\Phi_2}}}~~(\star\star)$ \\
% By \Cref{invariant:alg-typechecking} using the first premise and $(\star)$, we get $ \fivars{\grt_1,k_1, t_1,\Phi_1} \subseteq dom(\Delta, \psi; \psi_a)~(\diam)$.\\
Using $(\star)$, $ (\diam)$ and the 3rd premise,  $(\star\star)$'s derivation must be in a form such that we have
\begin{enumih}
\item $\Delta; \suba{\Phi_a} \sat \suba{\Phi_1}$
\item $\sorted{i}, \Delta; \suba{\Phi_a} \sat \suba{\Phi_2}$
\end{enumih}
By IH2 on the first premise using $(\star)$, a) , we can show that
\begin{equation}
  \label{eq:alg-usound-unpack1}
      \Delta; \suba{\Phi_a}; \suba{\Omega}  \jtypeMt{\subta{k_1}}{\subta{t_1}}{\erty{e_1}}{\texists{i} \suba{\grt_1}}
\end{equation}
From $(\star)$, we can show that
\begin{enumih}[resume]
 \item $\fivars{\Phi_a, \grt_1, \Omega, \grt_2} \subseteq i,  dom(\Delta, \psi, \psi_a)$
\end{enumih}
By IH1 on the second premise using b), c), $(\star)$ , we obtain
\begin{equation}
  \label{eq:alg-usound-unpack2}
     \sorted{i}, \Delta; \suba{\Phi_a}; x: \subta{\grt_1}, \suba{\Omega} \jtypeMt{K_2}{T_2}{\erty{e_2}}{\suba{\grt_2}}
\end{equation}
Then by the \textbf{c-unpack} rule using \cref{eq:alg-usound-unpack1,eq:alg-usound-unpack2}, we can show that $\Delta; \suba{\Phi_a}; \suba{\Omega}  \jtypeMt{\subta{k_1} + K_1 +\kunpack}{\subta{t_1}+T_2+\kunpack}{\eunpack \erty{e_1} \ewith (x,i) \ein \erty{e_2}}{\suba{\grt_2}}$. \\


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \caseL{\rrfchsplit}
  TS: $\Delta; \suba{\Phi_a}; \suba{\Omega}  \jtypeMt{\suba{k}}{\suba{t}}{\esplit (\erty{e_1}, \erty{e_2}) \ewith C}{\suba{\grt}}$. \\ 
By the main assumptions, we have
$\fivars{\Phi_a,\Omega, \grt} \subseteq dom(\Delta, \psi_a)~~(\star)$ and \\
$\Delta; \suba{\Phi_a} \sat \suba{(\cand{\cimpl{C}{\Phi_1}}{\cimpl{\neg C}{\Phi_2}})}~~(\star\star)$ \\
Using $(\star)$ and the third premise, we can show that
\begin{enumih}
\item $\fivars{C\wedge \Phi_a,\Omega, \grt} \subseteq dom(\Delta, \psi_a).$
\item $\fivars{\neg C\wedge \Phi_a,\Omega, \grt} \subseteq dom(\Delta, \psi_a).$
\end{enumih}


Using $(\star\star)$ and the third premise, we can show that
\begin{enumih}[resume]
\item $\Delta; C \wedge \suba{\Phi_a} \sat \suba{\Phi_1}$
\item $\Delta; \neg C \wedge \suba{\Phi_a} \sat \suba{\Phi_2}$
\end{enumih}
By IH1 on the first premise using $(\star)$ and c), we can show that
\begin{equation}
  \label{eq:alg-usound-split1}
       \Delta; C \wedge \suba{\Phi_a}; \suba{\Omega}  \jtypeMt{\suba{k}}{\suba{t}}{\erty{e_1}}{\suba{\grt}\{\suba{I}/i\}}
    \end{equation}
By IH1 on the second premise using $(\star)$ and d), we can show that
\begin{equation}
  \label{eq:alg-usound-split2}
       \Delta; \neg C \wedge \suba{\Phi_a}; \suba{\Omega}  \jtypeMt{\suba{k}}{\suba{t}}{\erty{e_2}}{\suba{\grt}\{\suba{I}/i\}}
    \end{equation}
    By the \textbf{c-split} rule using \cref{eq:alg-usound-split1,eq:alg-usound-split2} and the third premise, we obtain \\ $\Delta; \suba{\Phi_a}; \suba{\Omega}  \jtypeMt{\suba{k}}{\suba{t}}{\esplit (\erty{e_1}, \erty{e_2}) \ewith C}{\suba{\grt}}$.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \caseL{\rrfchcimplIntro}
  TS: $\Delta; \suba{\Phi_a}; \suba{\Omega}  \jtypeMt{\suba{k}}{\suba{t}}{ \erty{e} }{\tcimpl{\suba{C}}{\suba{\grt}}}$. \\ 
By the main assumptions, we have
$\fivars{\Phi_a,\Omega, \tcimpl{C}{\grt}, k, t} \subseteq dom(\Delta, \psi_a)~~(\star)$ and \\
$\Delta; \suba{\Phi_a} \sat \suba{(\cimpl{C}{\Phi})}~~(\star\star)$ \\
Using $(\star)$, we can show that
\begin{enumih}
\item $\fivars{C \wedge \Phi_a,\Omega, \grt} \subseteq dom(\Delta, \psi_a).$
\end{enumih}
By IH1 on the premise using $(\star)$ and a), we can show that
\begin{equation}
  \label{eq:alg-usound-cimpl}
       \Delta; \suba{C} \wedge \suba{\Phi_a}; \suba{\Omega}  \jtypeMt{\suba{k}}{\suba{t}}{\erty{e}}{\suba{\grt}}
    \end{equation}
    By the \textbf{c-cimpI} rule using \cref{eq:alg-usound-cimpl}, we obtain  $\Delta; \suba{\Phi_a}; \suba{\Omega}  \jtypeMt{\suba{k}}{\suba{t}}{ \erty{e} }{\tcimpl{\suba{C}}{\suba{\grt}}}$.


\end{mainitem}
\end{spacing}




\begin{spacing}{1.3}
  \hspace{-1cm} \textbf{Proof of \Cref{thm:relrefinf-alg-typing-soundness}.2:} \\
\begin{mainitem} 
 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \caseL{\rrfinfanno}
  TS: $\Delta; \suba{\Phi_a}; \suba{\Omega}  \jtypeMt{\suba{k}}{\suba{t}}{\erty{\eanno{e}{\grt}{k}{t}}}{\suba{\grt}}$. \\  
Since by definition,  $\forall e. ~\erty{(e:{\_})} = \erty{e}$, STS: $\Delta; \suba{\Phi_a}; \suba{\Omega}  \jtypeMt{\suba{k}}{\suba{t}}{\erty{e}}{\suba{\grt}}$. \\  
By the main assumptions, we have
$\fivars{\Phi_a,\Omega} \subseteq dom(\Delta, \psi_a)~~(\star)$ and $\Delta; \suba{\Phi_a} \sat \suba{\Phi}~~(\star\star)$ \\
Using the third premise, we can show that
\begin{enumih}
\item $\fivars{\Phi_a,\Omega, \grt} \subseteq dom(\Delta, \psi_a).$
\end{enumih}
By IH1  on the first premise using $(\star\star)$ and a), we can conclude that\\
$ \Delta; \suba{\Phi_a}; \suba{\Omega}  \jtypeMt{\suba{k}}{\suba{t}}{\erty{e}}{\suba{\grt}}.$
 
 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \caseL{\rrfinfapp}
  TS: $\Delta; \suba{\Phi_a}; \suba{\Omega}  \jtypeMt{\subaex{(k_1+k_2+k_e+\kapp)}{\theta_2}}{\subaex{(t_1+t_2+t_e+\kapp)}{\theta_2}}{\erty{e_1} \eapp \erty{e_2}}{\suba{\grt_2}}$. \\
By the main assumptions, we have
$\fivars{\Phi_a,\Omega} \subseteq dom(\Delta, \psi_a)~~(\star)$ and \\
$\Delta; \suba{\Phi_a} \sat
\suba{(\cand{\Phi_1}{\Phi_2})}~~(\star\star)$ such that $\subsat{\Delta}{\theta_a}{\psi_a}$ are derivable. \\
From $(\star\star)$, we know\\
\begin{enumih}
\item $ \Delta; \suba{\Phi_a} \sat
\suba{\Phi_1} $
\item $ \Delta; \suba{\Phi_a} \sat
\suba{\Phi_2} $
\end{enumih}
By IH  on the first premise using $(\star)$ and (a), we obtain
\begin{equation}
 \Delta; \suba{\Phi_a}; \suba{\Omega}  \jtypeMt{\subta{k_1}}{\subta{t_1}}{\erty{e_1}}{\suba{\grt_1} \to \suba{\grt_2}}\label{eq:alg-bsound-app1}
\end{equation}
By IH2  on the third premise using $(\star)$ and (b), we obtain
\begin{equation}
  \Delta; \suba{\Phi_a}; \suba{\Omega}  \jtypeMt{K_2}{T_2}{\erty{e_2}}{\subta{\grt_1}}
  \label{eq:alg-bsound-app22}
\end{equation}
Then, by using \textbf{c-app} rule using \cref{eq:alg-bsound-app1,eq:alg-bsound-app22}, we can show that \\
$\Delta; \suba{\Phi_a}; \suba{\Omega}
\jtypeMt{\subta{k_1}+\subta{k_e}+K_2}{\subta{t_1}+\subta{t_e}+T_2}{\erty{e_1}
  \eapp \erty{e_2}}{\suba{\grt_2}  }$.\\


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \caseL{\rrfinfiApp}
  TS: $\Delta; \suba{\Phi_a}; \suba{\Omega}  \jtypeMt{\subta{(k+k_e[I/i])}}{\subta{(t+t_e[I/i])}}{\erty{e} \eapp [I]}{\subta{(\grt'\{I/i\})}}$. \\
By the main assumptions, we have
$\fivars{\Phi_a,\Omega} \subseteq dom(\Delta, \psi_a)~~(\star)$ and \\
$\Delta; \suba{\Phi_a} \sat \suba{\Phi_2}~~(\star\star)$ such that $\subsat{\Delta}{\theta_a}{\psi_a}$ are derivable. \\
By IH2  on the first premise using $(\star)$, we obtain
\begin{equation}
 \Delta; \suba{\Phi_a}; \suba{\Omega}  \jtypeMt{\subta{k}}{\subta{t}}{\erty{e}}{\tsforall{i} \suba{\grt'}}\label{eq:alg-bsound-iApp1}
\end{equation} 
Then, by \textbf{c-iApp} rule using \cref{eq:alg-bsound-iApp1} and the
second premise, we can conclude that\\  $\Delta; \suba{\Phi_a};
\suba{\Omega}
\jtypeMt{\subta{k}+\subta{k_e}[I/i]}{\subta{t}+\subta{t_e}[I/i]}{\erty{e}\eapp
  [I]}{\suba{\grt'}\{I/i\}}$.
\end{mainitem}
\end{spacing}

\begin{spacing}{1.3}
  \hspace{-1cm} \textbf{Proof of \Cref{thm:relrefinf-alg-typing-soundness}.3:} \\
\begin{mainitem} 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \caseL{\relrefalgtynochange}
  TS: $\Delta; \suba{\Phi_a}; \suba{\Gamma'}, \tbox{\suba{\Gamma}} \jtypedifft{\suba{t}}{\enoch |e|}{\enoch |e|}{\tbox{\suba{\tau}}}$.\\
  By the main assumptions, we have
  $\fivars{\Phi_a,\Gamma', \tbox{\Gamma}, \tau} \subseteq dom(\Delta, \psi_a)~~(\star)$ and \\
  $\Delta; \suba{\Phi_a} \sat \suba{\Phi}~~(\star\star)$ \\
  Using $(\star)$, we can show that
  \begin{enumih}
  \item $\fivars{\Phi_a,\tbox{\Gamma}, \tau} \subseteq  dom(\Delta, \psi_a).$
  \end{enumih}
  % Using $(\star)$,  $(\star\star)$'s derivation must be in a form such that we have
  % \begin{enumih} [resume]
  % \item $\Delta; \suba{\Phi_a} \sat \ceq{0}{\suba{t}}$
  % \item $\Delta \sty{T'}{\scost}$ for some $T'$
  % \item $\Delta; \suba{\Phi_a} \sat \subaex{\Phi}{t' \mapsto T'}$
  % \end{enumih}

By IH3 on the premise using a) and $(\star\star)$, we can show that
  \begin{equation}
    \label{eq:rrf-alg-bsound-noch}
    \Delta;\suba{\Phi_a}; \suba{\tbox{\Gamma}}  \jtypedifft{T'}{\erty{e}}{\erty{e}}{\suba{\tau}}
  \end{equation}
  By the \textbf{c-nochange} rule using
  \cref{eq:rrf-alg-bsound-noch}, we obtain  $\Delta; \suba{\Phi_a};
  \suba{\Gamma'}, \tbox{\suba{\Gamma}}  \jtypedifft{0}{\enoch \erty{e}
  }{\enoch \erty{e} }{\tbox{\suba{\tau}}}$.\\

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \caseL{\relrefalgtycaseL}
TS:\begin{mathpar}
\Delta; \suba{\Phi_a}; \suba{\Gamma} \jtypedifft{\suba{t}}{\hspace{-1em}
       \begin{minipage}[c]{10em}
         ~ $\ecase e \eof \enil \, \rightarrow \erty{e_1}$ \\
         $~~~~~~~~|~h\,::_{N} tl\, \rightarrow \erty{e_2}$ \\
         $~~~~~~~~|~h::_{C} tl \rightarrow \erty{e_3}$
       \end{minipage}\hspace{-1em}
     }{\hspace{-1em}
       \begin{minipage}[c]{10em}
         ~ $\ecase e' \eof \enil \, \rightarrow \erty{e_1'}$ \\
         $~~~~~~~~|~h\,::_{N} tl\, \rightarrow \erty{e_2'}$ \\
         $~~~~~~~~|~h::_{C} tl \rightarrow \erty{e_3'}$
       \end{minipage}
     }{\suba{\tau'}}
\end{mathpar}\\
  By the main assumptions, we have
  $\fivars{\Phi_a,\Gamma, \tau'} \subseteq dom(\Delta, \psi_a)~~(\star)$ and \\
  $\Delta; \suba{\Phi_a} \sat \suba{(\cand{\Phi_e}{\Phi_{body}})}~~(\star\star)$ \\
% By $(\star)$, we get $ \fivars{\tlist{n}{\alpha}{\tau}, t_1,\Phi_e} \subseteq dom(\Delta, \psi; \psi_a)~(\diam)$.\\
Using $(\star)$, $(\star\star)$'s derivation must be in a form such that we have
\begin{enumih}
\item $\Delta; \suba{\Phi_a} \sat \suba{\Phi_e}$
\item $\Delta; {\ceq{\suba{n}}{0}} \wedge \suba{\Phi_a} \sat \suba{\Phi_1}$
\item $\sorted{i}, \Delta; {\ceq{\suba{n}}{i+1}} \wedge \suba{\Phi_a} \sat \suba{\Phi_2}$
\item $\sorted{i},\sorted{\beta}, \Delta; {\ceq{\suba{n}}{i+1}} \wedge{\ceq{\suba{\alpha}}{\beta+1}} \wedge \suba{\Phi_a} \sat \suba{\Phi_3}$
\end{enumih}
By IH4 on the first premise using a) and $(\star)$, we can show that
  \begin{equation}
    \label{eq:rrf-bsound-caseL1}
    \Delta;\suba{\Phi_a}; \suba{\Gamma}  \jtypedifft{\subta{t_1}}{\erty{e}}{\erty{e'}}{\tlist{\suba{n}}{\suba{\alpha}}{\suba{\tau}}}
  \end{equation}

By IH3 on the second premise using b) and $(\star)$, we can show that
  \begin{equation}
    \label{eq:rrf-bsound-caseL2}
    \Delta; {\ceq{\suba{n}}{0}} \wedge \suba{\Phi_a}; \suba{\Gamma}  \jtypedifft{T_2}{\erty{e_1}}{\erty{e_1'}}{{\suba{\tau'}}}
  \end{equation}

By IH3 on the third premise using c) and $(\star)$, we can show that
  \begin{equation}
    \label{eq:rrf-bsound-caseL3}
    \sorted{i}, \Delta; {\ceq{\suba{n}}{i+1}} \wedge \suba{\Phi_a}; \suba{\Gamma}  \jtypedifft{T_2}{\erty{e_2}}{\erty{e_2'}}{{\suba{\tau'}}}
  \end{equation}

By IH3 on the fourth premise using d) and $(\star)$, we can show that
  \begin{equation}
    \label{eq:rrf-bsound-caseL4}
    \sorted{i}, \sorted{\beta}, \Delta; {\ceq{\suba{n}}{i+1}} \wedge{\ceq{\suba{\alpha}}{\beta+1}} \wedge \suba{\Phi_a}; \suba{\Gamma}  \jtypedifft{T_2}{\erty{e_3}}{\erty{e_3'}}{{\suba{\tau'}}}
  \end{equation}
  Then by \textbf{c-r-caseL} rule using
  \cref{eq:rrf-bsound-caseL1,eq:rrf-bsound-caseL2,eq:rrf-bsound-caseL3,eq:rrf-bsound-caseL4},
  we can show that 
 \begin{mathpar}
\Delta; \suba{\Phi_a}; \suba{\Gamma} \jtypedifft{\subta{t_1}+T_2}{\hspace{-1em}
       \begin{minipage}[c]{10em}
         ~ $\ecase e \eof \enil \, \rightarrow \erty{e_1}$ \\
         $~~~~~~~~|~h\,::_{N} tl\, \rightarrow \erty{e_2}$ \\
         $~~~~~~~~|~h::_{C} tl \rightarrow \erty{e_3}$
       \end{minipage}\hspace{-1em}
     }{\hspace{-1em}
       \begin{minipage}[c]{10em}
         ~ $\ecase e' \eof \enil \, \rightarrow \erty{e_1'}$ \\
         $~~~~~~~~|~h\,::_{N} tl\, \rightarrow \erty{e_2'}$ \\
         $~~~~~~~~|~h::_{C} tl \rightarrow \erty{e_3'}$
       \end{minipage}
     }{\suba{\tau'}}
\end{mathpar}\\

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \caseL{\relrefalgtyconsnc}
 TS: $\Delta; \suba{\Phi_a}; \suba{\Gamma} \jtypedifft{\suba{t}}{\econsNC(\erty{e_1},\erty{e_2})}{\econsNC(\erty{e_1'},\erty{e_2'})}{\tlist{\suba{n}}{\suba{\alpha}}{\suba{\tau}}}$.\\
 By the main assumptions, we have
  $\fivars{\Phi_a,\Gamma, \tlist{n}{\alpha}{\tau}} \subseteq dom(\Delta, \psi_a)~~(\star)$ and \\
 $\Delta; \suba{\Phi_a} \sat \suba{({\cand{\Phi_1}{\cexists{i}{\ssize}{\Phi_2'}}})}~~(\star\star)$ \\
Using $(\star)$,  $(\star\star)$'s derivation must be in a form such that we have
\begin{enumih}
\item $\Delta; \suba{\Phi_a} \sat \suba{\Phi_1}$
\item  $\Delta \sty{I}{\ssize}$ 
\item $\Delta; \suba{\Phi_a} \sat \subaex{\Phi_2}{ i \mapsto I}$
\item $\Delta; \suba{\Phi_a} \sat \ceq{(I+1)}{\suba{n}}$
\end{enumih}

By IH3 on the second premise using $(\star)$ and a), we can show that
\begin{equation}
  \label{eq:rrf-bsound-cons1}
      \Delta; \suba{\Phi_a}; \suba{\Gamma}  \jtypedifft{T_1}{\erty{e_1}}{\erty{e_1'}}{\tbox{\suba{\tau}}}
\end{equation}

By IH3 on the third premise using $(\star)$ and b), we can show that
\begin{equation}
  \label{eq:rrf-bsound-cons2}
      \Delta; \suba{\Phi_a}; \suba{\Gamma}  \jtypedifft{T_2}{\erty{e_2}}{\erty{e_2'}}{\tlist{I}{\suba{\alpha}}{\suba{\tau}}}
\end{equation}
By \textbf{c-r-cons2} typing rule using \cref{eq:rrf-bsound-cons1,eq:rrf-bsound-cons2}, we obtain
\\ $\Delta; \suba{\Phi_a}; \suba{\Gamma} \jtypedifft{T_1+T_2}{\econsNC(\erty{e_1},\erty{e_2})}{\econsNC(\erty{e_1'},\erty{e_2'})}{\tlist{I+1}{\suba{\alpha}}{\suba{\tau}}}$. \\
We conclude by applying \textbf{c-r-}${\pmb{\sqsubseteq}}$ rule to this using d) .

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\end{mainitem}
\end{spacing}



\begin{spacing}{1.3}
  \hspace{-1cm} \textbf{Proof of \Cref{thm:relrefinf-alg-typing-soundness}.4:} \\
\begin{mainitem} 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\caseL{\relrefalgtyanno}
  TS: $\Delta; \suba{\Phi_a}; \suba{\Gamma}  \jtypedifft{\suba{t}}{\erty{\eannobi{e}{\tau}{t}}}{\erty{\eannobi{e'}{\tau}{t}}}{\suba{\tau}}$. \\  
Since by definition,  $\forall e. ~\erty{\eannobi{e}{\_}{\_}} = \erty{e}$, STS: $\Delta; \suba{\Phi_a}; \suba{\Gamma}  \jtypedifft{\suba{t}}{\erty{e}}{\erty{e'}}{\suba{\tau}}$. \\  
By the main assumptions, we have
$\fivars{\Phi_a,\Gamma} \subseteq dom(\Delta, \psi_a)~~(\star)$ and $\Delta; \suba{\Phi_a} \sat \suba{\Phi}~~(\star\star)$ \\
Using the third premise, we can show that
\begin{enumih}
\item $\fivars{\Phi_a,\Gamma, \tau} \subseteq dom(\Delta, \psi_a).$
\end{enumih}
By IH4 on the first premise using $(\star\star)$ and a), we can conclude that\\
$ \Delta; \suba{\Phi_a}; \suba{\Gamma}
\jtypedifft{\suba{t}}{\erty{e}}{\erty{e'}}{\suba{\tau}}.$

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \caseL{\relrefalgtyder}
  TS: $\Delta; \suba{\Phi_a}; \suba{\Gamma}
  \jtypediffMt{\subta{t}}{\eder \erty{e}}{\eder \erty{e'}}{\subta{\tau}}$. \\
By the main assumptions, we have
$\fivars{\Phi_a,\Gamma} \subseteq dom(\Delta, \psi_a)~~(\star)$ and \\
$\Delta; \suba{\Phi_a} \sat \suba{\Phi}~~(\star\star)$ such that $\subsat{\Delta}{\theta_a}{\psi_a}$ are derivable. \\
By IH4  on the first premise using
$(\star)$ and $\star\star$, we obtain
\begin{equation}
 \Delta; \suba{\Phi_a}; \suba{\Gamma}  \jtypedifft{\suba{t}}{\erty{e}}{\erty{e'}}{\tbox{\suba{\tau}}}\label{eq:rrf-alg-bsound-der1}
\end{equation} 
Then, by \textbf{c-der} rule using \cref{eq:rrf-alg-bsound-der1}, we can
conclude that\\  $\Delta; \suba{\Phi_a}; \suba{\Gamma}
\jtypedifft{\subta{t}}{\eder \erty{e}}{\eder \erty{e'}}{\subta{\tau}}$.

\end{mainitem}
\end{spacing}


\end{proof}

\begin{thm}[Completeness of algorithmic typechecking]\label{thm:rrf-alg-typing-completeness}
\mbox{}
  \begin{enumerate}
  \item Assume that $\Delta; \Phi_a; \Omega \jtypeM{}{}{e}{\grt}$.
    Then, there exists $ e'$ such that $\Delta; \cdot; \Phi_a; \Omega
    \chexect{e'}{\grt}{k}{t}{\Phi}$ and $\Delta; \Phi_a \sat \Phi$ and
    $\erty{e'} = e$.
  \item Assume that $\Delta; \Phi_a; \Gamma
    \jtypediffMt{t}{e_1}{e_2}{\tau}$.  Then, there exist $e_1',e_2'$
    such that $\Delta; \cdot; \Phi_a; \Gamma
    \chdifft{e_1'}{e_2'}{\tau}{t}{\Phi}$ and $\Delta; \Phi_a \sat \Phi$
    and $\erty{e_1'} = e_1$ and $\erty{e_2'} = e_2$.
  \end{enumerate}  
\end{thm}
%
\begin{proof}
By simultaneous induction on the given Core typing derivations.


\begin{spacing}{1.3}
  \hspace{-1cm} \textbf{Proof of \Cref{thm:rrf-alg-typing-completeness}.1:} \\
\begin{mainitem} 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\caseL{\relrefinfmtyvar}
We can conclude as follows
  \begin{mathpar}
    \inferrule{
      \rrfinfvar[\cdot] \\
      \Delta ; \Phi_a \jalgasubtype{\grt}{\grt}{\Phi}
    }
    {
      \uctx \chexecT{x}{\grt}{}{}{\ctrue}
    }~\textbf{alg-r-$\uparrow\downarrow$}
  \end{mathpar}
  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\caseL{\relrefinfmtycons}
By IH1 on the first premise, $\exists e_1'$ such that 
\begin{enumih}
\item $\Delta; \cdot; \Phi_a; \Omega \chexecT{e_1'}{\grt}{k_1}{t_1}{\Phi_1}$
\item $\Delta; \Phi_a  \sat \Phi_1$
\item $\erty{e_1'} = e_1$
\end{enumih}


By IH1 on the second premise, $\exists e_2'$ such that 
\begin{enumih}[resume]
\item $\Delta; \cdot; \Phi_a; \Omega \chexecT{e_2'}{\ulist{n}{\grt}}{k_2}{t_2}{\Phi_2}$
\item $\Delta; \Phi_a  \sat \Phi_2$
\item $\erty{e_2'} = e_2$
\end{enumih}


Then, we can conclude as follows 
\begin{enumconc}
\item 
  \begin{mathpar}
     \inferrule
{
\freshSize{i} \\
\Delta; {\psi_a}; \Phi_a; \Omega  \chexecT{e_1'}{\grt}{k_1'}{t_1'}{\Phi_1'}\\
\Delta; {i,k_2',t_2',\psi_a}; \Phi_a; \Omega
\chexecT{e_2'}{\ulist{i}{\grt}}{k_2'}{t_2'}{\Phi_2'}\\
\Phi_2'' = (\cand{\Phi_2}{\cand{\ceq{n+1}{(i+1)}}})
}
{
\uctx \chexecT{\econsC(e_1',e_2')}{\ulist{n+1}{\grt}}{k_1+k_2}{t_1+t_2}{\cand{\Phi_1'}{\cexists{i}{\ssize}{\Phi_2''}}}
}~\textbf{alg-u-cons-$\downarrow$}
  \end{mathpar}
\item Using c) and f), $\erty{\econsC(e_1',e_2')} = \econsC(e_1,e_2)$.
\end{enumconc}
\end{mainitem}
\end{spacing}

\begin{spacing}{1.3}
  \hspace{-1cm} \textbf{Proof of \Cref{thm:rrf-alg-typing-completeness}.2:} \\
\begin{mainitem} 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\caseL{\relrefcoreder}

By IH2 on the premise, $\exists e_1',e_2'$ such that 
\begin{enumih}
\item $\Delta; \cdot; \Phi_a; \Gamma \chdiff{e_1'}{e_2'}{\tau}{t}{\Phi}$
\item $\Delta; \Phi_a  \sat \Phi$
\item $\erty{e_1'} = e_1$ and $\erty{e_2'} = e_2$
\end{enumih}
Then, we can conclude by using a), b) and c) as follows:\\
 $\chRdert[\cdot][']$ and 

 \begin{enumconc}
 \item \begin{mathpar}
     \inferrule { {\inferrule { \chRdert[\cdot]['] } {\Delta; \cdot;
           \Phi_a; \Gamma \infdifft{(\eder
               e_1':\tau)}{(\eder
             e_2':\tau)}{\tau}{\cdot}{t}{\Phi} }
         ~\textbf{alg-r-anno-$\uparrow$}
       } \\
       \Delta ; \Phi_a \jalgeqtype{\tau}{\tau}{\Phi'}~~\text{by~}\Cref{lem:relref-refl-ty-eq} } { \Delta;
       \cdot; \Phi_a; \Gamma \chdifft{ (\eder
           e_1':\tau)}{(\eder
           e_2':\tau)}{\tau}{t}{\cand{\Phi}{\Phi'}}
     } ~\textbf{alg-r-$\uparrow\downarrow$}
   \end{mathpar}
\item By c), $\erty{(\eder
           e_i':\tau)} = \eder{\erty{e_i'}}$.
\item By b) and \Cref{lem:rrf-refl-ty-eq}.
 \end{enumconc}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\caseL{$\relrefcoresub$}
By IH2 on the first premise, $\exists e_1',e_2'$ such that 
\begin{enumih}
\item $\Delta; \cdot; \Phi_a; \Gamma \chdifft{e_1'}{e_2'}{\tau}{t}{\Phi_1}$
\item $\Delta; \Phi_a  \sat \Phi_1$
\item $\erty{e_1'} = e$ and $\erty{e_2'} = e'$
\end{enumih}
By IH2 on the second premise, 
\begin{enumih}[resume]
\item $\Delta ; \Phi_a \jalgeqtype{\tau}{\tau'}{\Phi_2}$ 
\item  $\Delta; \Phi_a \sat \Phi_2$.
\end{enumih}
Then, we can conclude as follows
\begin{enumconc}
\item By using a) and d) 
  \begin{mathpar}
    \inferrule
    {
      {\inferrule
        {
          \Delta; \cdot; \Phi_a; \Gamma \chdifft{e_1'}{e_2'}{\tau}{t}{\Phi_1}
        }
        {\Delta; \cdot; \Phi_a; \Gamma  \infdifft{(e_1':\tau)}{(e_2':\tau)}{\tau}{\cdot}{t}{\Phi_1}
        } ~\textbf{alg-r-anno-$\uparrow$} 
      } \\
      \Delta ; \Phi_a \jalgeqtype{\tau}{\tau'}{\Phi_2} 
    }
    { \Delta; \cdot; \Phi_a; \Gamma \chdifft{ (e_1':\tau) }{(e_2':\tau)}{\tau'}{t'}{\cand{\Phi_1}{\Phi_2}}
       } ~\textbf{alg-r-$\uparrow\downarrow$}
  \end{mathpar}
\item By using b), e) ,we can show that $\Delta; \Phi_a \sat {\cand{\Phi_1}{\Phi_2}}$
\item By c), $\erty{(e_1':\tau)} = e_1'$ and $(e_2':\tau) = e_2'$
\end{enumconc}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\caseL{$\relrefcoreapp$}
By IH2 on the first premise, $\exists \e_1,\e_1'$ such that 
\begin{enumih}
\item $\Delta; \cdot; \Phi_a; \Gamma \chdifft{\e_1}{\e_1'}{\tau_1 \to \tau_2}{t_1}{\Phi_1}$
\item $\Delta; \Phi_a  \sat \Phi_1$
\item $\erty{\e_1} = e_1$ and $\erty{\e_1'} = e_1'$
\end{enumih}

By IH2 on the second premise, $\exists \e_2,\e_2'$ such that 
\begin{enumih}[resume]
\item $\Delta; \cdot; \Phi_a; \Gamma \chdifft{\e_2}{\e_2'}{\tau_1}{t_2}{\Phi_2}$
\item $\Delta; \Phi_a  \sat \Phi_2$
\item $\erty{\e_2} = e_2$ and $\erty{\e_2'} = e_2'$
\end{enumih}

Then, we can conclude as follows
\begin{enumconc}
\item 
  \begin{mathpar}
    \inferrule
    {\inferrule
      {
        {\inferrule
          {
            \Delta; \cdot; \Phi_a; \Gamma \chdifft{\e_1}{\e_1'}{\tau_1 \to \tau_2}{t_1}{\Phi_1}
          }
          {\Delta; \cdot; \Phi_a; \Gamma \infdifft{(\e_1:{\tau_1 \to \tau_2})}{\e_1':{\tau_1 \to \tau_2})}{\tau_1 \to \tau_2}{\cdot}{t_1}{\Phi_1} }~\textbf{alg-r-anno-$\uparrow$} 
        } \\
        \Delta;  \cdot; \Phi_a; \Gamma \chdifft{\e_2}{\e_2'}{\tau_1}{t_2'}{\Phi_2}
      }
      {
        \Delta; \cdot; \Phi_a; \Gamma \infdifft{E_1}{E_2}{\tau_2}{t_2'}{t_1+t+t_2'}{\cand{\Phi_1}{\Phi_2}}
    }~\textbf{c-r-app}}
  {
    \Delta; \cdot; \Phi_a; \Gamma \chdifft{E_1}{E_2}{\tau_2}{t_1+t+t_2}{\cand{\Phi_1}{\Phi_2}}
  }~\textbf{alg-r-$\uparrow\downarrow$} 
\end{mathpar} \\
where $E_1= (\e_1:\tau_1 \to \tau_2) \eapp \e_2$ and $E_2= (\e_1':\tau_1 \to \tau_2) \eapp \e_2'$.
\item By using b) and e) .
\item Using c) and f),  $\erty{ (\e_1:\tau_1 \to \tau_2)  \eapp \e_2} = e_1 \eapp e_2$ and $\erty{ (\e_1':\tau_1 \to \tau_2)  \eapp \e_2'} = e_1' \eapp e_2'$.
\end{enumconc}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\caseL{$\relrefcoreunpack$}
By IH2 on the first premise, $\exists \e_1,\e_1'$ such that 
\begin{enumih}
\item $\Delta; \cdot; \Phi_a; \Gamma \chdifft{\e_1}{\e_1'}{\texists{i}\tau_1}{t_1}{\Phi_1}$
\item $\Delta; \Phi_a  \sat \Phi_1$
\item $\erty{\e_1} = e_1$ and $\erty{\e_1'} = e_1'$
\end{enumih}

By IH2 on the second premise, $\exists \e_2,\e_2'$ such that 
\begin{enumih}[resume]
\item $\sorted{i}, \Delta; \cdot; \Phi_a; x: \tau_1, \Gamma \chdifft{\e_2}{\e_2'}{\tau_2}{t_2}{\Phi_2}$
\item $\sorted{i}, \Delta; \Phi_a  \sat \Phi_2$
\item $\erty{\e_2} = e_2$ and $\erty{\e_2'} = e_2'$
\end{enumih}

Then, we can conclude as follows
\begin{enumconc}
\item \begin{mathpar}
    \inferrule { {\inferrule{ \Delta; \cdot; \Phi_a; \Gamma
          \chdifft{\e_1}{\e_1'}{\texists{i}\tau_1}{t_1}{\Phi_1}~~(a) }
        { \Delta; \cdot; \Phi_a; \Gamma
          \infdifft{E_1}{E_1'}{\texists{i}\tau_1}{\cdot}{t_1}{\Phi_1}
        }~\textbf{alg-r-anno-$\uparrow$} } \\
      \sorted{i}, \Delta;  \Phi_a; x: \tau_1, \Gamma \chdifft{\e_2}{\e_2'}{\tau_2}{t_2'}{\Phi_2} \\
      \Phi'=
      {\cand{\Phi_1}{\Phi_2'}}
    } {\Delta; \cdot; \Phi_a; \Gamma \chdifft{\eunpack E_1 \eas (x, i)
        \ein \e_2}{\eunpack E_1' \eas (x, i) \ein
        \e_2'}{\tau_2}{t_1+t_2}{\Phi'}
    }~\textbf{alg-r-unpack-$\downarrow$}
  \end{mathpar}
  where $E_1= (\e_1:\texists{i}\tau_1)$ and
  $E_2= (\e_1':\texists{i}\tau_1)$
\item By using b) and e).
\item Using c) and f),  $\erty{\eunpack  (\e_1:\texists{i}\tau_1) \eas (x,i) \ein \e_2} = \eunpack e_1 \eas (x,i) \ein e_2$ and  $\erty{\eunpack  (\e_1':\texists{i}\tau_1) \eas (x,i) \ein \e_2'} = \eunpack e_1' \eas (x,i) \ein e_2'$.
\end{enumconc}

\end{mainitem}
\end{spacing}



\end{proof}


==> RSTLC/relref_figures.tex <==
\begin{figure}
  \centering
\[
\begin{array}{llll}
 \label{fig:syntax}
   \mbox{Types} 
  &  \tau & ::= & \trbool ~|~ \tubool ~|~  \tau_1 \to \tau_2  ~|~
                  \tlist{n}{\alpha}{\tau} ~|~ \tsforall{i} \tau ~|~
                  \texists{i} \tau~|~ \tbox{\tau} ~|~ \tcprod{C}{\tau}
                  ~|~ \tcimpl{C}{\tau}
  \\
  \mbox{Expressions} & e & ::= & x  ~|~ \etrue ~|~ \efalse ~|~ \eif e
                                 \ethen e_1 \eelse e_2 ~|~ \efix
                                 f(x). e ~|~ e_1 \eapp e_2 ~|~ \enil
                                 ~|~ \econs(e_1,e_2) \\ &&&~|~ (\ecase e \eof \enil \rightarrow e_1 
 |~ h ::tl \rightarrow e_2)
~|~ \eLam e ~|~e \eApp ~|~ \elet x = e_1 \ein e_2 \\ 
&&&~|~ \epack e ~|~  \eunpack e_1 \eas x \ein e_2 ~|~ \clet e_1 \eas x
    \ein e_2 ~|~ \ecelim e \\
  \mbox{Value} & v& := & \etrue ~|~ \efalse ~|~ \efix f(x). v ~|~
                         \enil ~|~ \econs(e_1,e_2)  ~|~ \eLam e ~|~ \epack v \\
  \mbox{Index terms} & I, n,\alpha & \bnfdef & i \bnfalt \szero
                                               \bnfalt  \splusone{I} \bnfalt
\splus{I_1}{I_2} \bnfalt \sminus{I_1}{I_2} \bnfalt
\sdiv{I_1}{I_2} \bnfalt \smult{I_1}{I_2} \bnfalt
\sceil{I} \bnfalt \sfloor{I} \bnfalt
\smin{I_1}{I_2} \bnfalt  \smax{I_1}{I_2}.
\end{array}
\] 
 \caption{Syntax of values and expressions,index terms in RelRef} 
  
\end{figure}

\begin{figure}
  \centering
\[
\begin{array}{llll}
 \label{fig:syntax}
   &  \tau & ::= & \trbool ~|~ \tubool ~|~  \tau_1 \to \tau_2  ~|~
                  \tlist{n}{\alpha}{\tau} ~|~ \tsforall{i} \tau ~|~
                  \texists{i} \tau~|~ \tbox{\tau} ~|~ \tcprod{C}{\tau}
  ~|~ \tcimpl{C}{\tau}\\
  \mbox{Expressions} & e & ::= & x  ~|~ \etrue ~|~ \efalse  ~|~ \eif e
                                 \ethen e_1 \eelse e_2 ~|~ \efix
                                 f(x). e ~|~ \efixNC f(x).e ~|~ e_1
                                 \eapp e_2 ~|~  \enoch e\\ 
    &&& ~|~ \esplit(e_1,e_2) \ewith C ~|~  \econtra e ~|~\eder e ~|~ \eLam i. e
                                 ~|~ e [I] ~|~ \epack e \ewith I \\
      &&& ~|~ \eunpack e_1 \eas (x,i) \ein e_2 
   ~|~ \clet e_1 \eas x \ein e_2 ~|~ \ecelim e ~|~ \elet x = e_1 \ein e_2 \\
  &&& ~|~ \econsNC(e_1,e_2) ~|~ \econsC(e_1,e_2) ~|~
                       \left(\begin{minipage}[c]{13em}
                           $\ecase e \eof \enil \, \rightarrow e_1$ \\
                           $|~h\,::_{NC} tl\, \rightarrow e_2
                           ~|~h::_{C} tl~ \rightarrow e_3$
            \end{minipage}\right)  \\
  \mbox{Value} & v& := & \etrue ~|~ \efalse ~|~ \efix f(x). v  ~|~
                         \efixNC f(x).e ~|~
                         \enil ~|~ \econs(e_1,e_2)  ~|~ \epack e 
                         \ewith I \\  
                        &&&~|~ \eLam i. e ~|~ \econsNC(v_1,v_2) ~|~ \econsC(v_1,v_2)   
\end{array}
\] 
 \caption{Syntax of values and expressions in RelRef CORE} 
  
\end{figure}

\begin{figure}
  \centering
\[
\begin{array}{llll}
 \label{fig:syntax}
    &  \tau & ::= & \trbool ~|~ \tubool ~|~  \tau_1 \to \tau_2  ~|~
                  \tlist{n}{\alpha}{\tau} ~|~ \tsforall{i} \tau ~|~
                  \texists{i} \tau~|~ \tbox{\tau} ~|~ \tcprod{C}{\tau}
  ~|~ \tcimpl{C}{\tau}\\
  \mbox{Expressions} & e & ::= & x  ~|~ \etrue ~|~ \efalse  ~|~ \eif e
                                 \ethen e_1 \eelse e_2 ~|~ \efix
                                 f(x). e ~|~ \efixNC f(x).e ~|~ e_1
                                 \eapp e_2 ~|~  \enoch e\\ 
    &&& ~|~ \esplit(e_1,e_2) \ewith C ~|~  \econtra e ~|~\eder e ~|~ \eLam i. e
                                 ~|~ e [I] ~|~ \epack e \ewith I \\
      &&& ~|~ \eunpack e_1 \eas (x,i) \ein e_2  ~|~ (e:\tau)
   ~|~ \clet e_1 \eas x \ein e_2 ~|~ \ecelim e ~|~ \elet x = e_1 \ein e_2 \\
  &&& ~|~ \econsNC(e_1,e_2) ~|~ \econsC(e_1,e_2) ~|~
                       \left(\begin{minipage}[c]{13em}
                           $\ecase e \eof \enil \, \rightarrow e_1$ \\
                           $|~h\,::_{NC} tl\, \rightarrow e_2
                           ~|~h::_{C} tl~ \rightarrow e_3$
            \end{minipage}\right)  \\
  \mbox{Value} & v& := & \etrue ~|~ \efalse ~|~ \efix f(x). v ~|~ \efixNC f(x).e~|~
                         \enil ~|~ \econs(e_1,e_2)  ~|~ \epack e 
                         \ewith I \\  
                        &&&~|~ \eLam i. e ~|~ \econsNC(v_1,v_2) ~|~ \econsC(v_1,v_2)   
\end{array}
\] 
 \caption{Syntax of values and expressions in BiRelRef} 
  
\end{figure}


%  typing rule for RelRef

\begin{figure}
  \centering 
  \begin{mathpar}
    \inferrule
    {\Gamma(x) = \tau } 
    { \ctx \jstype{x}{x}{\tau}}~\textbf{rr-var}
    \and
    \inferrule
    { \kw{b}  \in \{\etrue, \efalse \}}  
    { \ctx \jstype{\kw{b}}{\kw{b}}{\trbool}}~\textbf{rr-bool}
    \and
    \inferrule
    { \kw{b_1, b_2}  \in \{\etrue, \efalse \}}  
    { \ctx \jstype{\kw{b_1}}{\kw{b_2}}{\tubool}}~\textbf{rr-u-bool}
    \and
    \inferrule{\ctx \jstype{e}{e'}{\trbool} \\
      \ctx \jstype{ e_1}{e_1'}{\tau} \\
      \ctx \jstype{ e_2}{e_2'}{\tau}
    }
    {\ctx \jstype{\eif e \ethen e_1 \eelse e_2}{\eif e' \ethen e_1' \eelse e_2'}{\tau}}~\textbf{rr-if}
    \and
    \inferrule{
       \Delta; \Phi_a;  x: \tau_1, f : \tau_1 \to \tau_2, \Gamma   \jstype{e_1}{e_2}{\tau_2}
     }
     {\ctx \jstype{ \efix f(x).e_1}{\efix f(x).e_2}{
                \tau_1 \to \tau_2}}~\textbf{rr-fix}
    \and
    \inferrule{\ctx \jstype{e_1}{e_1'}{\tau_1}
      \to \tau_2 \\
      \ctx \jstype{ e_2}{e_2'}{\tau_1}}
    {\ctx \jstype{e_1 \eapp e_2}{e_1' \eapp
        e_2'}{\tau_2}}~\textbf{rr-app}
    \and
   \inferrule
{
\Delta; \Phi_a; \Gamma \jstype{e}{e}{\tau}~~\\\\
\forall x \in dom(\Gamma).~~
\Delta; \Phi_a  \jsubtype{\Gamma(x)}{\tbox{\Gamma(x)}} ~~
}
{
\Delta; \Phi_a; \Gamma,\Gamma' \jstype{e}{e}{\tbox{\tau}}
} ~\textbf{rr-nochange}
\and
\inferrule{
    \ctx \jstype{e_1}{e_2}{\tau}~~\\
    \Delta; \Phi_a \jsubtype{\tau}{\tau'}~~ 
  }
  {\ctx \jstype{e_1}{e_2}{\tau'}
  }~{\textbf{rr-}\pmb{\sqsubseteq}}
\and
    \inferrule
  {
    {\ifextra \Delta; \Phi_a \wfty{\tau_1 \to \tau_2}
      \fi} \\
    \Delta; \Phi_a;  x: \tau_1, f : \tbox{(\tau_1 \to \tau_2)}, \Gamma \jstype{e}{e}{\tau_2}~~\\
    \forall x \in dom(\Gamma).~~
    \Delta; \Phi_a  \jsubtype{\Gamma(x)}{\tbox{\Gamma(x)}}
  }
  {\ctx,\Gamma' \jstype{ \efix f(x).e}{\efix f(x).e}{
              \tbox{(\tau_1 \to \tau_2)}}}~\textbf{rr-fixNC}
\and
\inferrule{
    i::S, \ctx \jstype{e}{e'}{\tau}~~ \\\\
    i \not \in \fiv{\Phi_a; \Gamma}
  }
  { \ctx \jstype{\eLam e}{\eLam e'}{\tsforall{i} \tau }}~\textbf{rr-iLam}
\and
 \inferrule{
    \ctx \jstype{e}{e'}{\tsforall{i} \tau } ~~\\\\
    \Delta \sty{I}{\sort}
  }
  {\ctx \jstype{e \eApp}{e' \eApp}{\tau\{ I/
      i\}}}~\textbf{rr-iApp}
\and
 \inferrule
{
  \ctx  \jstype{e}{e'}{\tau\{I/i\}}~~\\
  \Delta \sty{I}{\sort}~~
}
{
  \ctx  \jstype{\epack e}{\epack e'}{\texists{i} \tau}
} ~\textbf{rr-pack}
\and
\inferrule
{
  \ctx \jstype{e_1}{e_1'}{\texists{i} \tau_1} ~~\\
  \sorted{i}, \Delta; \Phi_a; x: \tau_1, \Gamma \jstype{e_2}{e_2'}{\tau_2} ~~\\
  i \not\in FV(\Phi_a;\Gamma, \tau_2, t_2) \\
}
{
  \ctx  \jstype{\eunpack e_1 \eas x \ein  e_2}{\eunpack e_1' \eas x \ein  e_2'}{\tau_2}
}~\textbf{rr-unpack1} 
\and
\inferrule
{
  \Delta; \Phi_a \wedge C; \Gamma \jstype{e}{e'}{\tau}
}
{
  \ctx  \jstype{e}{e'}{\tcimpl{C}{\tau}}
} ~\textbf{rr-c-impII}
\and
\inferrule
{
  \ctx \jstype{e_1}{e_1 '}{\tcimpl{C}{\tau}}\\
  \Delta; \Phi_a \vDash C
}
{
  \ctx  \jstype{\ecelim e }{\ecelim e' }{\tau}
} ~\textbf{rr-c-implE}
  \end{mathpar}
 \caption{Relational Refinement typing rules1}
\label{fig:rel-ref-typing1}
\end{figure}

\begin{figure}
\centering 
  \begin{mathpar}
\inferrule
  {
    {\ifextra
      \Delta; \Phi_a \wfty{\tau}
      \fi}
  }
  { \ctx
    \jstype{\enil}{\enil}{\tlist{0}{\alpha}{\tau}}}~\textbf{rr-nil}
\and
\inferrule
  { \ctx \jstype{e_1}{e_1'}{\tau} \\
    \ctx \jstype{e_2}{e_2'}{\tlist{n}{\alpha}{\tau}}
  }
  { \ctx \jstype{ \econs(e_1,e_2) }{ \econs(e_1',e_2')}{\tlist{n+1}{\alpha+1}{\tau}}}~\textbf{rr-cons1}
\and
 \inferrule
  { \ctx \jstype{e_1}{e_1'}{\tbox{\tau}} \\
    \ctx \jstype{e_2}{e_2'}{\tlist{n}{\alpha}{\tau}}}
  { \ctx \jstype{ \econs(e_1,e_2) }{
      \econs(e_1',e_2')}{\tlist{n+1}{\alpha}{\tau}}}~\textbf{rr-cons2}
\and
\inferrule
  {\ctx \jstype{e}{e'}{\tlist{n}{\alpha}{\tau}} \\
   \Delta; \Phi_a \wedge n = 0  ;\Gamma \jstype{e_1}{e_1'}{\tau'} \\
   i, \Delta; \Phi_a \wedge n = i+1;  h: \tbox{\tau},
   tl : \tlist{i}{\alpha}{\tau}, \Gamma \jstype{e_2}{e_2'}{\tau'} ~~
\\
   i, \beta, \Delta; \Phi_a \wedge n = i+1 \wedge \alpha = \beta +1 ;
   h: \tau, tl : \tlist{i}{\beta}{\tau}, \Gamma \jstype{e_2}{e_2'}{\tau'} ~~
   }
  {\ctx \jstype{ \ecase e \eof \enil \rightarrow e_1 ~|~ h::tl \rightarrow
    e_2}{\ecase e' \eof \enil \rightarrow e_1' ~|~ h::tl \rightarrow
    e_2'}{\tau'}}~\textbf{rr-caseL}
\and 
\inferrule
{
\Delta; \Phi_a \sat C \\
  \Delta; \Phi_a \wedge C; \Gamma \jstype{e}{e'}{\tau}
}
{
  \ctx  \jstype{e}{e'}{\tcprod{C}{\tau}}
} ~\textbf{rr-c-andI}
\and
\inferrule
{
  \ctx \jstype{e_1}{e_1 '}{\tcprod{C}{\tau_1}}\\
  \Delta; \Phi_a \wedge C; x :\tau_1, \Gamma   \jstype{ e_2}{e_2'}{\tau_2}
}
{
  \ctx  \jstype{\clet e_1 \eas x \ein e_2}{\clet e_1' \eas x \ein e_2'}{\tau_2}
} ~\textbf{rr-c-andE}
\and
\inferrule
  {
    \Delta; \Phi_a \wedge C; \Gamma  \jstype{e_1}{e_2}{\tau}\\
    \Delta; \Phi_a \wedge \neg C; \Gamma  \jstype{e_1}{e_2}{\tau}\\
    \Delta \wfcs{C}
  }
  {
    \ctx  \jstype{e_1}{e_2}{\tau} } ~\textbf{rr-split}
\and
\inferrule
{
\Delta; \Phi_a \sat \bot \\
  \Delta; \Phi_a \wfty{\Gamma}
}
{
  \ctx \jstype{e_1}{e_2}{\tau}
} ~\textbf{rr-contra}
\end{mathpar}
 \caption{Relational Refinement typing rules (2)}
\label{fig:rel-ref-typing2}
\end{figure}



\begin{figure}
  \centering 
  \begin{mathpar}
    \inferrule{
    }
    {
      \jsubtype{\trbool}{\tubool}
    }~\textbf{bool}
    \and
     \inferrule{
       \jsubtype{\tau_1'}{\tau_1} \\
       \jsubtype{\tau_2}{\tau_2'}
     }
     {
       \jsubtype{\tau_1 \to \tau_2}{\tau_1' \to \tau_2'}
     }~\textbf{$\to$}
     \and
     \inferrule
     {
     }
     {  \jsubtype{\tau}{\tau}
     }\textbf{refl}
     \and
     \inferrule{
     }
     {
       \jsubtype{\square (\tau_1 \to \tau_2)}{ \square \tau_1 \to
         \square \tau_2}
     }\textbf{$\to\square$diff}
\and
  \stlist
%
\and
%
\stlistzero
%
\and
%
\stlistbox
%
\and
%
\stint
%
\and
%
\stbox
%
\and
%
\stboxD
%
\and
%
\stboxB
%
\and
%
\sttrans
%
\and
%
\relrefsubforallD
%
\and
%
\relrefsubforallboxD
%
\and
%
\stexists
%
\and
\stexistsbox
\and
\stcimpl
\and
\stcimplbox
\and
\stcprod
\and
\stcprodbox

   \end{mathpar}
   \caption{Subtyping rules for RelRef}
   \label{fig:rel-ref-subtyping}
 \end{figure}



\begin{figure*}
  \raggedright
  \fbox{$\Delta; \Phi_a \jeqtype{\tau_1}{\tau_2}$}~~~checks
  whether $\tau_1$ is equivalent to $\tau_2$.
  \begin{mathpar}
 \relrefeqfun
  % \and
  % \relrefeqlist
\and
  \etlist
  \and 
  \etboxB
  \and
  \etexists
  \and
\etcprod
 \and
\relrefeqcimpl
\and
\relrefeqforall

\end{mathpar}
  \caption{RelRef type equivalence rules}
  \label{fig:type-eq-rules}
\end{figure*}

\begin{figure*}
  \centering
  \begin{mathpar}
    \inferrule{\Gamma(x) = \tau}{\ctx
      \jstypet{x}{x}{\tau}}~\textbf{c-r-var}
     \and
     \inferrule{
       {\ifextra
       \Delta; \Phi_a \wfty{\tau_1 \to \tau_2}
       \fi} \\
       \Delta; \Phi_a;  x: \tau_1, f : \tau_1 \to \tau_2, \Gamma  \jstypet{e_1}{e_2}{\tau_2}}
            {\ctx \jstypet{ \efix f(x).e_1}{\efix f(x).e_2}{
              \tau_1 \to \tau_2}}~\textbf{c-r-fix}
   \and
\inferrule
  {
    {\ifextra \Delta; \Phi_a \wfty{\tau_1 \to \tau_2}
      \fi} \\
    \Delta; \Phi_a;  x: \tau_1, f : \tbox{(\tau_1 \to \tau_2)}, \tbox{\Gamma} \jstypet{e}{e}{\tau_2}
  }
  {\nctx,\Gamma' \jstypet{\efixNC f(x).e}{\efixNC f(x).e}{
              \tbox{(\tau_1 \to \tau_2)}}}~\textbf{c-r-fixNC}
  \and
     \inferrule
  { \ctx \jstypet{e_1}{e_1'}{\tau} \\
    \ctx \jstypet{e_2}{e_2'}{\tlist{n}{\alpha}{\tau}}
  }
  { \ctx \jstypet{ \econsC(e_1,e_2) }{ \econsC(e_1',e_2')}{\tlist{n+1}{\alpha+1}{\tau}}}~\textbf{c-r-cons1}
    \and
   \inferrule
  { \ctx \jstypet{e_1}{e_1'}{\tbox{\tau}} \\
    \ctx \jstypet{e_2}{e_2'}{\tlist{n}{\alpha}{\tau}}}
  { \ctx \jstypet{ \econsNC(e_1,e_2) }{ \econsNC(e_1',e_2')}{\tlist{n+1}{\alpha}{\tau}}}~\textbf{c-r-cons2}
    \and
    \inferrule
  {\ctx \jstypet{e}{e'}{\tlist{n}{\alpha}{\tau}}\\
   \Delta; \Phi_a \wedge n = 0  ;\Gamma \jstypet{e_1}{e_1'}{\tau'}\\
   i, \Delta; \Phi_a \wedge n = i+1;  h: \tbox{\tau},
   tl : \tlist{i}{\alpha}{\tau}, \Gamma \jstypet{e_2}{e_2'}{\tau'}
\\
   i, \beta, \Delta; \Phi_a \wedge n = i+1 \wedge \alpha = \beta +1 ;
   h': \tau, tl : \tlist{i}{\beta}{\tau}, \Gamma \jstypet{e_3}{e_3'}{\tau'}
   }
  {\ctx \jstypet{
      \begin{minipage}[c]{10em}
        ~ $\ecase e \eof \enil \, \rightarrow e_1$ \\
         $~~~~~~~~|~h\,::_{N} tl\, \rightarrow e_2$ \\
         $~~~~~~~~|~h'::_{C} tl' \rightarrow e_3$
      \end{minipage}
}{
      \begin{minipage}[c]{10em}
         ~ $\ecase e' \eof \enil \, \rightarrow e_1'$ \\
         $~~~~~~~~|~h\,::_{N} tl\, \rightarrow e_2'$ \\
         $~~~~~~~~|~h'::_{C} tl' \rightarrow e_3'$
      \end{minipage}
}{\tau'}}~\textbf{c-r-caseL}
    \and
    \inferrule
{
\Delta; \Phi_a; \Gamma  \jstypet{e_1}{e_2}{\tbox{\tau}}
}
{
\Delta; \Phi_a; \Gamma  \jstypet{\eder e_1}{\eder e_2}{\tau}
} ~\textbf{c-der}
    \and 
    \inferrule
{
\Delta; \Phi_a; \tbox{\Gamma} \jstypet{e}{e}{\tau}
}
{
\Delta; \Phi_a; \tbox{\Gamma}, \Gamma' \jstypet{\enoch e}{\enoch e}{\tbox{\tau}}
} ~\textbf{c-nochange}
    \and
    \inferrule{
     \ctx \jstypet{e}{e'}{\tau}\\
     \Delta; \Phi_a \jeqtype{\tau}{\tau'} 
  }
  {\ctx \jstypet{e}{e'}{\tau'} }
  ~{\textbf{c-r-$\equiv$}}
    \and
    \inferrule
  {
    \Delta; \Phi_a \wedge C; \Gamma \jstypet{e_1}{e_2}{\tau}\\
    \Delta; \Phi_a \wedge \neg C; \Gamma \jstypet{e_1'}{e_2'}{\tau}\\
  }
  {
    \ctx \jstypet{\esplit (e_1,e_1') \ewith C}{\esplit
      (e_2,e_2') \ewith C}{\tau} } ~\textbf{c-r-split}
   \and
   \inferrule
{
\Delta; \Phi_a \sat \bot \\
  \Delta; \Phi_a \wfty{\Gamma}
}
{
  \ctx \jstypet{\econtra  e_1}{\econtra  e_2}{\tau}
} ~\textbf{c-r-contra}
\and
\inferrule{
    \ctx \jstypet{e}{e'}{\tsforall{i} \tau}\\
    \Delta \vdash I : S
  }
  {\ctx \jstypet{e[I]}{e' [I]}{\tau\{ I/ i\}}}~\textbf{c-r-iApp}
\and
\inferrule{
    i::S, \ctx \jstypet{e}{e'}{\tau} \\
    i \not \in \fiv{\Phi_a; \Gamma}
  }
  { \ctx \jstypet{\eLam i. e}{\eLam i. e'}{\tsforall{i}
      \tau}}~\textbf{c-r-iLam}
  \end{mathpar}
  % Definitions at typing-rules-min-defs.tex
  \caption{RelRef Core typing rules 1}
  \label{fig:relref-core-typing-rules-1}
\end{figure*}

\begin{figure*}
  \centering
  \begin{mathpar}
\relrefcorecimplI
\and
\relrefcorecimplE
\and
\relrefcorecprodI
\and
\relrefcorecprodE
\and
\relrefcoreapp
\and
\relrefcorelet
\and
\inferrule
{
  \ctx  \jstypet{e}{e'}{\tau\{I/i\}}\\
  \Delta \sty{I}{\sort}
}
{
  \ctx  \jstypet{\epack e \ewith I}{\epack e' \ewith I}{\texists{i} \tau}
} ~\textbf{c-r-pack}
\and
\inferrule
{
  \ctx \jstypet{e_1}{e_1'}{\texists{i} \tau_1}\\
  \sorted{i}, \Delta; \Phi_a; x: \tau_1, \Gamma \jstypet{e_2}{e_2'}{\tau_2}\\
  i \not\in FV(\Phi_a;\Gamma, \tau_2, t_2) \\
}
{
  \ctx  \jstypet{\eunpack e_1 \eas (x, i) \ein  e_2}{\eunpack e_1' \eas (x, i) \ein  e_2'}{\tau_2}
}~\textbf{c-r-unpack1}
\end{mathpar}
  % Definitions at typing-rules-min-defs.tex
  \caption{RelRef Core typing rules 2}
  \label{fig:relref-core-typing-rules-2}
\end{figure*}

\begin{figure*}
  \centering
  \begin{mathpar}
  \inferrule{\Gamma(x) = \tau}{\ctx \jelabsamet{0}{x}{x}{\tau}}~\textbf{e-r-var}
    \and
\relrefembedfix
    \and
     \relrefembedfixnc
       \and
\relrefembedcimplI
\and
\relrefembedcimplE
\and
\relrefembedcprodI
\and
\relrefembedcprodE

\end{mathpar}
  \caption{RelRel embedding typing rules 1}
  \label{fig:relrel-embedding-typing-rules-1}
\end{figure*}

\begin{figure*}
\begin{mathpar}
    \relrefembedconsOne
  \and
    \relrefembedconsTwo
  \and
    \relrefembednochange
    \and
   \relrefembedcaseL
    \and
    \relrefembedilam
    \and
    \relrefembediapp
    \and
   \relrefembedsub
    \and
   \relrefembedpack
    \and
   \relrefembedunpack
   \and
   \relrefembedsplit
  \and
   \relrefembedcontra
  \end{mathpar}
  % Definitions at appendix/elaboration-rules-defs.tex
  \caption{RelRel embedding rules 2}
  \label{fig:elab-rules}
\end{figure*} 

\begin{figure}[t]
\begin{mathpar}
 \relrefalgeqfun
  \and
 \relrefalgeqforall
\and
  \relrefalgeqlista
% \and
% \relrefalgeqlistb
\and
\relrefalgeqexists
\and
\relrefalgeqcprod
\and
\relrefalgeqbox
\and
\relrefalgeqcimpl
% \astexistsboxl
% \and
% \astexistsboxr
% \and
% \astforallboxl
% \and
% \astforallboxr
\end{mathpar}
% \nocaptionrule

% Definitions at appendix/alg-type-eq-rules-defs.tex
\caption{ relref algorithmic type equivalence rules}
\label{fig:alg-type-eq-rules}  
\end{figure} 

\begin{figure*}
\begin{mathpar}
  \inferrule
  {
    \Delta; { \psi_a}; \Phi_a; \tbox{\Gamma}  \chdifft{e}{e}{\tau}{t'}{\Phi}
  }
  {
    \Delta; \psi_a; \Phi_a; \Gamma', \tbox{\Gamma} \chdifft{\enoch e}{\enoch e}{\tbox{\tau}}{t}{\Phi}
  } ~\textbf{alg-r-nochange-$\downarrow$}
  \and
  \inferrule
{
  \bctx \infdifft{e_1}{e_2}{\tbox{\tau}}{\psi}{t}{\Phi}
}
{
  \bctx \infdifft{\eder e_1}{\eder e_2}{\tau}{\psi}{t}{\Phi}
}~\textbf{alg-r-der-$\uparrow$}
  \and
  % \chRder
  % \and
  \inferrule
{
\Gamma(x) = \tau
}
{
\bctx \infdifft{x}{x}{\tau}{\emptypsi}{0}{\ctrue}
} ~\textbf{alg-r-var-$\uparrow$}
  \and
  \inferrule
{
 \Delta; {\psi_a};  \Phi_a; f : \tau_1 \to \tau_2, x:\tau_1, \Gamma \chdifft{e}{e'}{\tau_2}{t'}{\Phi}
}
{
\bctx \chdifft{\efix f(x).e}{\efix f(x).e'}{\tau_1 \to \tau_2}{t}{\Phi}
} ~\textbf{alg-r-fix-$\downarrow$}
  \and
   \inferrule
{
    % \forall x_i \in \fvars{\efixNC f(x).e}.~ \exists \tau_i. ~\Gamma(x_i) = \tbox{\tau_i}\\
    \Delta; {\psi_a};  \Phi_a; f : \tbox{(\tau_1 \to \tau_2)}, x:\tau_1, \tbox{\Gamma} \chdifft{e}{e'}{\tau_2}{t'}{\Phi}
}
{
\Delta; \psi_a; \Phi_a; \Gamma', \tbox{\Gamma} \chdifft{\efixNC f(x).e}{\efixNC f(x).e}{\tbox{(\tau_1 \to \tau_2)}}{t}{\Phi}
} ~\textbf{alg-r-fix-$\downarrow\square$}
\and
  \inferrule
{
\bctx  \infdifft{e_1}{e_1'}{\tau_1 \to \tau_2}{\psi}{t_1}{\Phi_1} \\
\Delta; {\psi_a}; \Phi_a; \Gamma \chdifft{e_2}{e_2'}{\tau_1}{t_2}{\Phi_2}
}
{
\bctx  \infdifft{e_1 \eapp e_2}{e_1' \eapp e_2'}{\tau_2}{\psi}{t_1+t_2+t_e}{\cand{\Phi_1}{\Phi_2}}
}~\textbf{alg-r-app-$\uparrow$}
  \and
\inferrule
{
\Delta, \psi_a; \Phi \wfty{\tau}
}
{
\bctx  \chdifft{\enil}{\enil}{\tlist{n}{\alpha}{\tau}}{t}{\ceq{n}{0}}
}~\textbf{alg-r-nil-$\downarrow$}
  \and
   \inferrule
{
\freshSize{i,\beta} \\
\Delta; {\psi_a}; \Phi_a; \Gamma  \chdifft{e_1}{e_1'}{\tau}{t_1}{\Phi_1} \\
\Delta; {i,\beta,\psi_a}; \Phi_a; \Gamma
\chdifft{e_2}{e_2'}{\tlist{i}{\beta}{\tau}}{t_2}{\Phi_2}\\
\Phi_2' = \cand{\ceq{n}{(i+1)}}{\cexists{\beta}{\ssize}{\cand{\Phi_2}{\ceq{\alpha}{\beta+1}}}}
}
{
  \bctx \chdifft{\econsC(e_1,e_2)}{\econsC(e_1',e_2')}{\tlist{n}{\alpha}{\tau}}{t}{\cand{\Phi_1}{\cexists{i}{\ssize}{\Phi_2'}}}
}~\textbf{alg-r-consC-$\downarrow$}
  \and
  \inferrule
{
\freshSize{i} \\
\Delta; {\psi_a}; \Phi_a; \Gamma  \chdifft{e_1}{e_1'}{\tbox{\tau}}{t_1}{\Phi_1} \\
\Delta; {i,\psi_a}; \Phi_a; \Gamma
\chdifft{e_2}{e_2'}{\tlist{i}{\alpha}{\tau}}{t_2}{\Phi_2}\\
\Phi_2' = \cand{\Phi_2}{\ceq{n}{(i+1)}}
}
{
\bctx \chdifft{\econsNC(e_1,e_2)}{\econsNC(e_1',e_2')}{\tlist{n}{\alpha}{\tau}}{t}{\cand{\Phi_1}{\cexists{i}{\ssize}{\Phi_2'}}}
}~\textbf{alg-r-consNC-$\downarrow$}
  \and
  \inferrule
{
\bctx \infdifft{e}{e'}{\tlist{n}{\alpha}{\tau}}{\psi}{t_1}{\Phi_e}\\
\Delta; {  \psi_a}; \cand{\ceqz{n}}{\Phi_a}; \Gamma  \chdifft{e_1}{e_1'}{\tau'}{t_2}{\Phi_1} \\
\sized{i},\Delta; {\psi_a};  \cand{\ceq{n}{i+1}}{\Phi_a}; h :\tbox{\tau}, tl:\tlist{i}{\alpha}{\tau}, \Gamma \chdifft{e_2}{e_2'}{\tau'}{t_2}{\Phi_2}\\
\sized{i}, \sized{\beta},\Delta; { \psi_a};  \cand{\cand{\ceq{n}{i+1}}{\ceq{\alpha}{\beta + 1}}}{\Phi_a}; h :\tau, tl:\tlist{i}{\beta}{\tau}, \Gamma \chdifft{e_3}{e_3'}{\tau'}{t_2}{\Phi_3}\\
\Phi_{body} = {\cand{(\cimpl{\ceqz{n}}{\Phi_1})}{(\cforall{i}{\ssize}{\cimpl{(\ceq{n}{i+1})}{(\cand{\Phi_2}{\cforall{\beta}{\ssize}{\cimpl{(\ceq{\alpha}{\beta+1})}{\Phi_3}}})}})}}
}
{
\bctx \chdifft{\hspace{0em}
       \begin{minipage}[c]{10em}
         ~$\ecase e \eof \enil \, \rightarrow e_1$ \\
         $~~~~~~|~h\,::_{NC} tl\, \rightarrow e_2$ \\
         $~~~~~~|~h::_{C} tl~~~ \rightarrow e_3$
       \end{minipage}\hspace{0em}
     }{\hspace{0em}
       \begin{minipage}[c]{10em}
         ~ $\ecase e' \eof \enil \, \rightarrow e_1'$ \\
         $~~~~~~~~|~h\,::_{NC} tl\, \rightarrow e_2'$ \\
         $~~~~~~~~|~h::_{C} tl~~~ \rightarrow e_3'$
       \end{minipage}
     }{\tau'}{t}{{(\cand{\Phi_e}{\Phi_{body}})}}
}~\textbf{alg-r-caseL-$\downarrow$}

  % \and
  % \chRsplit
\end{mathpar}

% \nocaptionrule
% Definitions at alg-typing-rules-defs.tex
\caption{Selected algorithmic typing rules (Part 1).}
\label{fig:selected-alg-typing-rules} 
\end{figure*} 


\begin{figure*}
  \begin{mathpar}
    \inferrule
  {
    \sorted{i}, \bctx \chdifft{e}{e'}{\tau}{t_e}{\Phi}
  }
  {
    \bctx  \chdifft{\eLam i. e}{\eLam i. e'}{\tsforall{i}
        \tau}{t}{(\cforall{i}{\sort}{\Phi})}
  } ~\textbf{alg-r-iLam-$\downarrow$}
    \and
    \inferrule
{
  \bctx  \infdifft{e}{e'}{\tsforall{i} \tau'}{\psi}{t}{\Phi} \\
  \Delta \sty{I}{S}
}
{
  \bctx \infdifft{e \, [I]}{e' \, [I]}{\tau'\{I/i\}}{\psi}{t+t_e[I/i]}{\Phi}
} ~\textbf{alg-r-iApp-$\uparrow$}
    \and
    \inferrule
  {
    \Delta; {\psi_a}; \Phi_a; \Gamma  \chdifft{e}{e'}{\tau\{I/i\}}{t}{\Phi}\\
    \Delta  \sty{I}{\sort}
}
{
  \bctx  \chdifft{\epack e \ewith I}{\epack e' \ewith I}{\texists{i} \tau}{t}{\Phi}
} ~\textbf{alg-r-pack-$\downarrow$}
    \and
    \inferrule
{
  \bctx \infdifft{e_1}{e_1'}{\texists{i} {\tau_1}}{\psi}{t_1}{\Phi_1} \\
  \sorted{i}, \Delta; { \psi_a}; \Phi_a; x: \tau_1, \Gamma
  \chdifft{e_2}{e_2'}{\tau_2}{t_2}{\Phi_2} \\
i \not\in FV(\Phi_a;\Gamma, \tau_2) \\
\Phi = {(\cand{\Phi_1}{\cforall{i}{\sort}{\Phi_2}})}
}
{
  \bctx  \chdifft{\eunpack e_1 \eas (x, i) \ein e_2}{\eunpack e_1' \eas (x, i) \ein e_2'}{\tau_2}{t}{\Phi}
}~\textbf{alg-r-unpack-$\downarrow$}
    \and
    \inferrule
{
  \Delta; \psi_a; \Phi \wedge C;  \Gamma \chdifft{e_1}{e_1}{\tau}{t}{\Phi}
}
{
  \bctx \chdifft{e_1}{e_2}{\tcprod{C}{\tau}}{t}{\cand{C}{(\cimpl{C}{\Phi})}}
} ~\textbf{alg-r-c-andI$\downarrow$}
    \and
    \inferrule
{
  \bctx \infdifft{e_1}{e_1'}{\tcprod{C}{\tau_1}}{\psi}{t_1}{\Phi_1} \\
  \Delta;   \psi_a; \Phi \wedge C;   x :\tau_1,  \Gamma  \chdifft{e_2}{e_2'}{\tau_2}{t_2}{\Phi_2} \\
  \Phi_2' = {\cimpl{C}{\Phi_2}}
}
{
  \bctx  \chdifft{\clet e_1 \eas x \ein e_2}{\clet e_1' \eas x \ein e_2'}{\tau_2}{t}{{(\cand{\Phi_1}{\Phi_2'})}}
} ~\textbf{alg-r-c-andE$\downarrow$}
   \and 
 \inferrule
{
  \Delta; \psi_a; \Phi \wedge C;  \Gamma \chdifft{e_1}{e_1}{\tau}{t}{\Phi}
}
{
  \bctx \chdifft{e_1}{e_2}{\tcimpl{C}{\tau}}{t}{(\cimpl{C}{\Phi})}
} ~\textbf{alg-r-c-implI$\downarrow$}
    \and
    \inferrule
{
  \bctx \infdifft{e}{e'}{\tcimpl{C}{\tau}}{\psi}{t_1}{\Phi} 
}
{
  \bctx  \infdifft{\ecelim e}{\ecelim e'}{\tau}{}{t}{{(\cand{C}{\Phi})}}
} ~\textbf{alg-r-c-implE$\downarrow$}
    \and
    \inferrule{
  \bctx \infdifft{e}{e'}{\tau'}{\psi}{t'}{\Phi_1}\\
  \Delta; { \psi_a}; \Phi_a \jalgeqtype{\tau'}{\tau}{\Phi_2} \\
}
{
  \bctx \chdifft{e}{e'}{\tau}{t}{{\cand{\Phi_1}{\Phi_2}}}
} ~\textbf{alg-r-$\uparrow\downarrow$}
    \and
    \inferrule
{
  \bctx \chdifft{e}{e'}{\tau}{t}{\Phi}\\
  \Delta; \Phi_a \wfty{\tau} \\
  \fivars{\tau} \in \Delta
}
{
  \bctx  \infdifft{(e:\tau)}{(e':\tau)}{\tau}{\cdot}{t}{\Phi}
} ~\textbf{alg-r-anno-$\uparrow$}
    \and
    \inferrule{
  \Delta; \psi_a; C \wedge \Phi_a; \Gamma \chdifft{e_1}{e_1'}{\tau}{t}{\Phi_1}\\\\
  \Delta; \psi_a; \neg C \wedge \Phi_a; \Gamma \chdifft{e_2}{e_2'}{\tau}{t}{\Phi_2}\\
  \Delta  \wfcs{C}
}
{
  \bctx \chdifft{\esplit (e_1, e_2) \ewith C}{\esplit (e_1', e_2') \ewith C}{\tau}{t}{\cand{\cimpl{C}{\Phi_1}}{\cimpl{\neg C}{\Phi_2}}}
} ~\textbf{alg-r-split$\downarrow$}
   \and
  \inferrule{
  \Delta; \psi_a; \Phi_a \sat \bot
}
{
  \bctx \chdifft{\econtra e}{\econtra e'}{\tau}{t}{\ctrue}
} ~\textbf{alg-r-contra$\downarrow$}
\and
 \inferrule{\Gamma \infdifft{e}{e'}{\trbool}{}{}{\Phi_1} \\
      \Gamma \chdifft{ e_1}{e_1'}{\tau}{}{\Phi_2} \\
      \Gamma \chdifft{ e_2}{e_2'}{\tau}{}{\Phi_3}
    }
    {\Gamma \chdifft{\eif e \ethen e_1 \eelse e_2}{\eif e' \ethen e_1'
        \eelse e_2'}{\tau}{}{\Phi_1 \land \Phi_2 \land \Phi_3}}~\textbf{alg-r-if}
  \end{mathpar}
\caption{Selected algorithmic typing rules (Part 2).}
\label{fig:selected-alg-typing-rules2} 
\end{figure*} 



==> RSTLC/relref_lemmas.tex <==
\subsection{RelRef proof}
\begin{lem} [Substitution of RelRef Core] \label{lem:relref-substitution}
Assume that 
\begin{enumerate}
\item $\Delta;\Psi_a;\Gamma \jstypet{e_1}{e_2}{\tau}~~(1)$.
\item $\Delta;\Psi_a;\Gamma,x:\tau \jstypet{e_1'}{e_2'}{\tau'}~~(2)$.
\end{enumerate}
then $\Delta;\Psi_a;\Gamma \jstypet{e_1'[e_1/x]}{e_2'[e_2/x]}{\tau'} $.
\end{lem}

\begin{proof}
By induction on the typing derivation of the second assumption (2).\\
\begin{mainitem}
\caseL{  \inferrule{(\Gamma,x:\tau)(z) = \tau'}{\ctx,x:\tau
      \jstypet{z}{z}{\tau'}}~\textbf{c-r-var}}
   \textbf{Subcase: } $z=x$.\\
    TS: $ \ctx \jstypet{z[e_1/x]}{z[e_2/x]}{\tau'} $.  \\
   Because $x=z$,$z[e_1/x]=e_1$, $z[e_2/x]=e_1$, STS: $ \ctx
   \jstypet{e_1}{e_2}{\tau'} $.\\
   From $(\Gamma,x:\tau)(z) = \tau'$ and $x=z$, we know $\tau=\tau'$.\\
   By the above statements, STS: $ \ctx
   \jstypet{e_1}{e_2}{\tau} $, which is proved by the assumption.\\
   \textbf{Subcase:}  $z \not = x$.\\
   we know: $\Gamma(z) = \tau' ~~(\star)$.\\
   TS: $ \ctx \jstypet{z[e_1/x]}{z[e_2/x]}{\tau'}$. \\
   Because $x\not =z$, $z[e_1/x]=z$, $z[e_2/x]=z$, STS: $ \ctx
   \jstypet{z}{z}{\tau'} $.\\
   By the core rule \textbf{c-r-vars} and $(\star)$, we construct the
   derivation :\\
  $ \inferrule{\Gamma(z) = \tau'}{\ctx
      \jstypet{z}{z}{\tau'}}~\textbf{c-r-var} $
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\caseL{\inferrule
{
\Delta; \Phi_a; \Gamma,x:\tau  \jstypet{e_1''}{e_2''}{\tbox{\tau'}}~~(3)
}
{
\Delta; \Phi_a; \Gamma,x:\tau  \jstypet{\eder e_1''}{\eder e_2''}{\tau'}
} ~\textbf{c-der}}
  $e_1'=\eder e_1''$, $e_2'=\eder e_2''$.\\
  TS:  $ \Delta; \Phi_a; \Gamma \jstypet{\eder (e_1''[e_1/x])}{\eder
    (e_2''[e_2/x])}{\tau'} $. \\
 By IH on (1) and (3), $ \Delta;\Psi_a;\Gamma
 \jtypediffMt{t}{e_1''[e_1/x]}{e_2''[e_2/x]}{\square \tau'}~~(4) $.\\
By core rule \textbf{c-der} and (4), we can derive \\
$\inferrule
{
\Delta; \Phi_a; \Gamma,x:\tau  \jstypet{e_1''[e_1/x]}{e_2''[e_2/x]}{\tbox{\tau'}}~~(4)
}
{
\Delta; \Phi_a; \Gamma,x:\tau \jstypet{\eder (e_1''[e_1/x])}{\eder
    (e_2''[e_2/x])}{\tau'}
} ~\textbf{c-der} $.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\caseL{  \inferrule{
       \Delta; \Phi_a;  z: \tau_1, f : \tau_1 \to \tau_2, \Gamma,x:\tau
       \jstypet{e_1''}{e_2''}{\tau_2}~~(3) }
            {\ctx,x:\tau \jstypet{ \efix f(z).e_1''}{\efix f(z).e_2''}{
              \tau_1 \to \tau_2}}~\textbf{c-r-fix}  
}
 $e_1'=\efix f(z).e_1''$, $e_2'=\efix f(z).e_2'',\tau'=\tau_1 \to \tau_2$.\\
 TS:  $ \Delta; \Phi_a; \Gamma \jstypet{\efix f(z). (e_1''[e_1/x])}{\efix f(z).
    (e_2''[e_2/x])}{\tau'} $. \\
By IH on (1) and (3), $ \Delta;\Psi_a;  z: \tau_1, f : \tau_1 \to \tau_2, \Gamma
 \jtypediffMt{t}{e_1''[e_1/x]}{e_2''[e_2/x]}{ \tau_2}~~(4) $.\\
By core rule \textbf{c-r-fix} and (4), we can derive :\\
$ \Delta; \Phi_a; \Gamma \jstypet{\efix f(z). (e_1''[e_1/x])}{\efix f(z).
    (e_2''[e_2/x])}{\tau'} $.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\caseL{ \inferrule
  {
    \Delta; \Phi_a;  z: \tau_1, f : \tbox{(\tau_1 \to \tau_2)}, \tbox{\Gamma},x:\tau \jstypet{e}{e}{\tau_2}~~(3)
  }
  {\nctx,\Gamma',x:\tau \jstypet{\efixNC f(z).e}{\efixNC f(z).e}{
              \tbox{(\tau_1 \to \tau_2)}}}~\textbf{c-r-fixNC}  }
 $e_1'=\efix f(z).e$, $e_2'=\efix f(z).e,\tau'=\tbox{(\tau_1 \to \tau_2)}$.\\
 TS:  $ \nctx,\Gamma' \jstypet{\efix f(z). (e[e_1/x])}{\efix f(z).
    (e[e_2/x])}{\tau'} $. \\
By IH on (1) and (3), $  \Delta; \Phi_a;  z: \tau_1, f : \tbox{(\tau_1 \to \tau_2)}, \tbox{\Gamma}
 \jtypediffMt{t}{e[e_1/x]}{e[e_2/x]}{ \tau_2}~~(4) $.\\
By core rule \textbf{c-r-fixNC} and (4), we can derive :\\
$ \nctx,\Gamma' \jstypet{\efix f(z). (e[e_1/x])}{\efix f(z).
    (e[e_2/x])}{\tau'} $. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\caseL{ \inferrule
  { \ctx,x:\tau \jstypet{e_3}{e_3'}{\tau''}~~(3) \\
    \ctx,x:\tau \jstypet{e_4}{e_4'}{\tlist{n}{\alpha}{\tau''}}~~(4)
  }
  { \ctx,x:\tau \jstypet{ \econsC(e_3,e_4) }{
      \econsC(e_3',e_4')}{\tlist{n+1}{\alpha+1}{\tau''}}}~\textbf{c-r-cons1}
}
$e_1'=\econsC(e_3,e_4) $,
$e_2'=\econsC(e_3',e_4'),\tau'=\tlist{n+1}{\alpha+1}{\tau''}$.\\

TS: $ \ctx \jstypet{\econsC(e_3[e_1/x],e_4[e_1/x]) }{
  \econsC(e_3'[e_2/x],e_4'[e_2/x]) }{\tau'}   $.\\
By IH on (1) and (3),$\ctx
\jstypet{e_3[e_1/x]}{e_3'[e_2/x]}{\tau''}~~(5)$.\\
By IH on (1) and (4),$\ctx
\jstypet{e_4[e_1/x]}{e_4'[e_2/x]}{\tlist{n}{\alpha}{\tau''}}~~(6)$.\\
By core rule \textbf{c-r-cons1} and (5),(6), we can derive :\\
$ \ctx \jstypet{\econsC(e_3[e_1/x],e_4[e_1/x]) }{
  \econsC(e_3'[e_2/x],e_4'[e_2/x]) }{\tau'}   $.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\caseL{ \inferrule
{
\Delta; \Phi_a; \tbox{\Gamma},x:\tau \jstypet{e}{e}{\tau''}~~(3)
}
{
\Delta; \Phi_a; \tbox{\Gamma}, \Gamma',x:\tau \jstypet{\enoch e}{\enoch e}{\tbox{\tau''}}
} ~\textbf{c-nochange} }
$e_1'=\enoch e $,
$e_2'=\enoch e,\tau'=\tbox{\tau''}$.\\
TS: $ \ctx \jstypet{\enoch e[e_1/x] }{
  \enoch e[e_2/x] }{\tau'}   $.\\
By IH on (1) and (3),$\ctx
\jstypet{e[e_1/x]}{e[e_2/x]}{\tau''}~~(4)$.\\
By core rule \textbf{c-nochange} and (4), we can derive :\\
$ \ctx \jstypet{\enoch e[e_1/x] }{
  \enoch e[e_2/x]) }{\tau'}   $
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\end{mainitem} 
\end{proof}

\begin{lem} [Reflexivity of Algorithmic Binary Type Equivalence] \label{lem:relref-refl-ty-eq}
  $\forall \Delta, \psi_a,\Phi_a,\tau.$ there exists $\Phi$ s.t $\Delta; \psi_a; \Phi_a \jalgeqtype{\tau}{\tau}{\Phi}$ and $\Delta; \psi_a; \Phi_a \sat{\Phi}$.
 \end{lem}
 \begin{proof}
   By induction on the binary type.\\
   \begin{mainitem}
   \caseL{ $\tsforall{i} \tau$ }
    Assume $\Delta, \psi_a,\Phi_a$.\\
    TS: $ \exists \Phi$ s.t $ \Delta; \psi_a; \Phi_a
    \jalgeqtype{\tsforall{i} \tau}{\tsforall{i} \tau}{\Phi} $ and
    $\Delta; \psi_a; \Phi_a \sat{\Phi}$\\
    By IH on $\tau$ where $\Delta'=i,\Delta$, $ \exists \Phi'$ s.t $ \Delta'; \psi_a; \Phi_a
    \jalgeqtype{\tau}{\tau}{\Phi'} $ and
    $\Delta'; \psi_a; \Phi_a \sat{\Phi'}$.\\
    By the above statement and algorithmic type eq rules
    \textbf{alg-r-forall}, we conclude the following statement where
    $\Phi=\tsforall{i} \Phi'$.\\
    $  \Delta; \psi_a; \Phi_a
    \jalgeqtype{\tsforall{i} \tau}{\tsforall{i} \tau}{\Phi} $  and
    $\Delta; \psi_a; \Phi_a \sat{\Phi}$\\
   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \caseL{$\tau_1 \to \tau_2$ }
    Assume $\Delta, \psi_a,\Phi_a$.\\
    TS: $ \exists \Phi$ s.t $ \Delta; \psi_a; \Phi_a
    \jalgeqtype{ \tau_1 \to \tau_2 }{\tau_1 \to \tau_2}{\Phi} $ and
    $\Delta; \psi_a; \Phi_a \sat{\Phi}$\\
     By IH on $\tau_1$, $ \exists \Phi_1$ s.t $ \Delta; \psi_a; \Phi_a
    \jalgeqtype{\tau_1}{\tau_1}{\Phi_1} $ and
    $\Delta; \psi_a; \Phi_a \sat{\Phi_1}$.\\
    By IH on $\tau_2$, $ \exists \Phi_2$ s.t $ \Delta; \psi_a; \Phi_a
    \jalgeqtype{\tau_2}{\tau_2}{\Phi_2} $ and
    $\Delta; \psi_a; \Phi_a \sat{\Phi_2}$.\\
     By the above statement and algorithmic type eq rules
    \textbf{alg-r-fun}, we conclude the following statement where
    $\Phi=\cand{\Phi_1}{\Phi_2}$.\\
     $  \Delta; \psi_a; \Phi_a
    \jalgeqtype{\tau_1 \to \tau_2}{\tau_1 \to \tau_2}{\Phi} $  and
    $\Delta; \psi_a; \Phi_a \sat{\Phi}$\\

  %%%%%%%%%%%
   \caseL{  $\tlist{n}{\alpha}{\tau}$ }
      Assume $\Delta, \psi_a,\Phi_a$.\\
    TS: $ \exists \Phi$ s.t $ \Delta; \psi_a; \Phi_a
    \jalgeqtype{ \tlist{n}{\alpha}{\tau} }{\tlist{n}{\alpha}{\tau}}{\Phi} $ and
    $\Delta; \psi_a; \Phi_a \sat{\Phi}$\\
      By IH on $\tau$, $ \exists \Phi_1$ s.t $ \Delta; \psi_a; \Phi_a
    \jalgeqtype{\tau}{\tau}{\Phi_1} $ and
    $\Delta; \psi_a; \Phi_a \sat{\Phi_1}$.\\
      By the above statement and algorithmic type eq rules
    \textbf{alg-r-list}, we conclude the following statement where
    $\Phi=\cand{\Phi_1}{n=n\land \alpha = \alpha}$.\\
     $  \Delta; \psi_a; \Phi_a
    \jalgeqtype{\tlist{n}{\alpha}{\tau} }{ \tlist{n}{\alpha}{\tau} }{\Phi} $  and
    $\Delta; \psi_a; \Phi_a \sat{\Phi}$\\
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
   \caseL{  $\texists{i} \tau$ }
    Assume $\Delta, \psi_a,\Phi_a$.\\
    TS: $ \exists \Phi$ s.t $ \Delta; \psi_a; \Phi_a
    \jalgeqtype{ \texists{i} \tau}{ \texists{i} \tau }{\Phi} $ and
    $\Delta; \psi_a; \Phi_a \sat{\Phi}$\\
      By IH on $\tau$, choose $i \not\in FV(\Phi_a)$, $ \exists \Phi_1$ s.t $ i,\Delta; \psi_a; \Phi_a
    \jalgeqtype{\tau}{\tau}{\Phi_1} $ and
    $i,\Delta; \psi_a; \Phi_a \sat{\Phi_1}$.\\
      By the above statement and algorithmic type eq rules
    \textbf{alg-r-$\exists$}, we conclude the following statement where
    $\Phi=\tsforall{i} \Phi_1$.\\
      $  \Delta; \psi_a; \Phi_a
    \jalgeqtype{  \texists{i} \tau }{ \texists{i} \tau  }{\Phi} $  and
    $\Delta; \psi_a; \Phi_a \sat{\Phi}$\\

   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
   \caseL{ $\tbox{\tau}$ }
     Assume $\Delta, \psi_a,\Phi_a$.\\
    TS: $ \exists \Phi$ s.t $ \Delta; \psi_a; \Phi_a
    \jalgeqtype{ \tbox{\tau}}{ \tbox{\tau} }{\Phi} $ and
    $\Delta; \psi_a; \Phi_a \sat{\Phi}$\\
      By IH on $\tau$,$ \exists \Phi_1$ s.t $ \Delta; \psi_a; \Phi_a
    \jalgeqtype{\tau}{\tau}{\Phi_1} $ and
    $\Delta; \psi_a; \Phi_a \sat{\Phi_1}$.\\
      By the above statement and algorithmic type eq rules
    \textbf{B-$\square$}, we conclude the following statement where
    $\Phi= \Phi_1$.\\
   $  \Delta; \psi_a; \Phi_a
    \jalgeqtype{ \tbox{\tau} }{ \tbox{\tau}  }{\Phi} $  and
    $\Delta; \psi_a; \Phi_a \sat{\Phi}$\\

    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \caseL{ $\tcprod{C}{\tau}$ }
     Assume $\Delta, \psi_a,\Phi_a$.\\
    TS: $ \exists \Phi$ s.t $ \Delta; \psi_a; \Phi_a
    \jalgeqtype{ \tcprod{C}{\tau} }{ \tcprod{C}{\tau} }{\Phi} $ and
    $\Delta; \psi_a; \Phi_a \sat{\Phi}$\\
      By IH on $\tau$,$ \exists \Phi_1$ s.t $ \Delta; \psi_a; \Phi_a
    \jalgeqtype{\tau}{\tau}{\Phi_1} $ and
    $\Delta; \psi_a; \Phi_a \sat{\Phi_1}$.\\
    By the above statement and algorithmic type eq rules
    \textbf{alg-r-cprod}, we conclude the following statement where
    $\Phi= \cand{C \leftrightarrow C}{\Phi}_1$.\\
    $  \Delta; \psi_a; \Phi_a
    \jalgeqtype{ \tcprod{C}{\tau} }{ \tcprod{C}{\tau}  }{\Phi} $  and
    $\Delta; \psi_a; \Phi_a \sat{\Phi}$\\
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \caseL{ $\tcimpl{C}{\tau}$ }
     Assume $\Delta, \psi_a,\Phi_a$.\\
    TS: $ \exists \Phi$ s.t $ \Delta; \psi_a; \Phi_a
    \jalgeqtype{ \tcimpl{C}{\tau} }{ \tcimpl{C}{\tau} }{\Phi} $ and
    $\Delta; \psi_a; \Phi_a \sat{\Phi}$\\
      By IH on $\tau$,$ \exists \Phi_1$ s.t $ \Delta; \psi_a; \Phi_a
    \jalgeqtype{\tau}{\tau}{\Phi_1} $ and
    $\Delta; \psi_a; \Phi_a \sat{\Phi_1}$.\\
    By the above statement and algorithmic type eq rules
    \textbf{alg-r-cimpl}, we conclude the following statement where
    $\Phi= \cand{C \leftrightarrow C}{\Phi}_1$.\\
     $  \Delta; \psi_a; \Phi_a
    \jalgeqtype{ \tcimpl{C}{\tau} }{ \tcimpl{C}{\tau}  }{\Phi} $  and
    $\Delta; \psi_a; \Phi_a \sat{\Phi}$\\
  \end{mainitem}
   
 \end{proof}

\begin{thm}[Soundness of the Algorithmic Binary Type Equality]\label{thm:relref-alg-ty-eq-soundness}
    Assume that
    \begin{enumerate}
    \item  $\Delta ; \psi_a; \Phi_a \jalgeqtype{\tau}{\tau'}{\Phi}$
    \item $\fivars{\Phi_a,\tau, \tau'} \subseteq \Delta, \psi_a$ 
    % \item $\Delta; \psi_a; \Phi_a \wfty{\tau} $
    % \item $\Delta; \psi_a; \Phi_a \wfty{\tau'} $
    \item $\Delta; \suba{\Phi_a} \sat \suba{\Phi}$ is
      provable and $\subsat{\Delta}{\theta_a}{\psi_a}$ is derivable.
    \end{enumerate}
    Then $\Delta ; \suba{\Phi_a}  \jeqtype{\suba{\tau}}{\suba{\tau'}}$.

\end{thm} 
\begin{proof}
  By induction on the algorithmic binary type equivalence
  derivation.\\
  \begin{mainitem}
  \caseL{ \relrefalgeqfun }
  Assume $\fivars{\Phi_a,\tau_1 \to \tau_2, \tau_1' \to \tau_2'} \subseteq \Delta, \psi_a$ and
  $\Delta; \suba{\Phi_a} \sat \suba{\Phi}$ is provable and
  $\subsat{\Delta}{\theta_a}{\psi_a}$ is derivable.\\
   TS: $\Delta ; \suba{\Phi_a}
   \jeqtype{\suba{(\tau_1 \to \tau_2)}}{\suba{(\tau_1' \to \tau_2')}}$.\\
   We know $\Phi= \Phi_1 \land \Phi_2$ s.t $\fivars{\Phi_a,\tau_1,
     \tau_1' } \subseteq \Delta, \psi_a$ and $\Delta; \suba{\Phi_a} \sat \suba{\Phi_1}$ is
      provable.\\
   Similaryly, $\fivars{\Phi_a,\tau_2,
     \tau_2' } \subseteq \Delta, \psi_a$ and $\Delta; \suba{\Phi_a} \sat \suba{\Phi_2}$ is
      provable.\\
   By IH on $ \Delta; \psi_a; \Phi_a
   \jalgeqtype{\tau_1}{\tau_1'}{\Phi_1}$ with the same substitution
   $\theta_a$ and the above statements, $\Delta ; \suba{\Phi_a}  \jeqtype{\suba{\tau_1}}{\suba{\tau_1'}}$.\\
   By IH on $ \Delta; \psi_a; \Phi_a
   \jalgeqtype{\tau_1}{\tau_1'}{\Phi_2}$  with the same substitution
   $\theta_a$ and the above statements , $\Delta ; \suba{\Phi_a} 
   \jeqtype{\suba{\tau_2}}{\suba{\tau_2'}}$.\\
   By the above statements and RelRef type equivalence rule
   \textbf{eq-fun}, we conclude that \\
    $$\Delta ; \suba{\Phi_a}
   \jeqtype{\suba{(\tau_1 \to \tau_2)}}{\suba{(\tau_1' \to \tau_2')}}$$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \caseL{\relrefalgeqlista}
  Assume $\fivars{\Phi_a, \tlist{n}{\alpha}{\tau}, \tlist{n'}{\alpha'}{\tau'}} \subseteq \Delta, \psi_a$ and
  $\Delta; \suba{\Phi_a} \sat \suba{\Phi'}$ is provable and
  $\subsat{\Delta}{\theta_a}{\psi_a}$ is derivable.\\
   TS: $\Delta ; \suba{\Phi_a}
   \jeqtype{\suba{(\tlist{n}{\alpha}{\tau})}}{\suba{(\tlist{n'}{\alpha'}{\tau'})}}$.\\
    We know $\Phi'= \Phi \land \ceq{n}{n'} \land \ceq{\alpha}{\alpha'}
    $ s.t\\
    From assumption $\fivars{\Phi_a, \tlist{n}{\alpha}{\tau},
      \tlist{n'}{\alpha'}{\tau'}} \subseteq \Delta, \psi_a$, we know $\fivars{\Phi_a,\tau,n,\alpha,
     \tau',n',\alpha' } \subseteq \Delta, \psi_a$. \\
    From assumption  $\Delta; \suba{\Phi_a} \sat \suba{\Phi'}$, we get $\Delta;
   \suba{\Phi_a} \sat \suba{\Phi}$ is provable and $\Delta;
   \suba{\Phi_a} \sat \suba{(\ceq{n}{n'})} $ and $\Delta;
   \suba{\Phi_a} \sat \suba{(\ceq{\alpha}{\alpha'})}$. \\
   By IH on the first premise $\Delta; \psi_a; \Phi_a
   \jalgeqtype{\tau}{\tau'}{\Phi}$  with the same substitution
   $\theta_a$ and the above statements, $\Delta ; \suba{\Phi_a} 
   \jeqtype{\suba{\tau}}{\suba{\tau'}}$.\\
   By the above statements and RelRef type equivalence rule
   \textbf{eq-list}, we conclude that \\
    $$\Delta ; \suba{\Phi_a}
   \jeqtype{\suba{ (\tlist{n}{\alpha}{\tau})
     }}{\suba{(\tlist{n'}{\alpha'}{\tau'})}}$$.\\

   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
   \caseL{ \relrefalgeqforall }
     Assume $\fivars{\Phi_a,\tsforall{i} \tau, \tsforall{i} \tau' } \subseteq \Delta, \psi_a$ and
  $\Delta; \suba{\Phi_a} \sat \suba{\Phi'}$ is provable and
  $\subsat{\Delta}{\theta_a}{\psi_a}$ is derivable.\\
   TS: $\Delta ; \suba{\Phi_a}
   \jeqtype{\suba{\tsforall{i} \tau }}{\suba{\tsforall{i} \tau' }}$.\\
   We know $\Phi'= \tsforall{i} \Phi$ s.t\\
    From assumption $\fivars{\Phi_a, \tsforall{i} \tau,
      \tsforall{i} \tau'  } \subseteq \Delta, \psi_a$, we know
    $\fivars{\Phi_a,\tau,\tau',i } \subseteq (i,\Delta), \psi_a$. \\
      From assumption  $\Delta; \suba{\Phi_a} \sat \suba{\tsforall{i} \Phi}$, we get $i,\Delta;
   \suba{\Phi_a} \sat \suba{\Phi}$ is provable.\\
  By IH on the first premise $i, \Delta; \psi_a; \Phi_a
  \jalgeqtype{\tau}{\tau'}{\Phi}$ with the above statements, $ i,\Delta ; \suba{\Phi_a}
   \jeqtype{\suba{\tau }}{\suba{\tau' }}$.\\
   By the above statements and RelRef type equivalence rule
   \textbf{eq-$\forall$}, we conclude that \\
    $$\Delta ; \suba{\Phi_a}
   \jeqtype{\suba{ \tsforall{i} \tau
     }}{\suba{ \tsforall{i} \tau' }}$$.\\

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \caseL{\relrefalgeqcprod }
     Assume $\fivars{\Phi_a,\tcprod{C}{\tau}, \tcprod{C'}{\tau'} } \subseteq \Delta, \psi_a$ and
  $\Delta; \suba{\Phi_a} \sat \suba{\Phi'}$ is provable and
  $\subsat{\Delta}{\theta_a}{\psi_a}$ is derivable.\\
   TS: $\Delta ; \suba{\Phi_a}
   \jeqtype{\suba{ (\tcprod{C}{\tau}) }}{\suba{(\tcprod{C'}{\tau'}) }}$.\\
   We know $\Phi'= C \leftrightarrow C' \land  \Phi$ s.t\\
    From assumption $\fivars{\Phi_a, \tcprod{C}{\tau}, \tcprod{C'}{\tau'}  } \subseteq \Delta, \psi_a$, we know
    $\fivars{\Phi_a,\tau,\tau',C,C' } \subseteq \Delta, \psi_a$. \\
      From assumption  $\Delta; \suba{\Phi_a} \sat \suba{ ( C \leftrightarrow C' \land \Phi)}$, we get $\Delta;
   \suba{\Phi_a} \sat \suba{\Phi}$ is provable and $\Delta;
   \suba{\Phi_a} \sat \suba{ C}$ and $\Delta; \suba{\Phi_a} \sat \suba{ C'}$.\\
   By IH on the first premise $ \Delta; \psi_a; \Phi_a
  \jalgeqtype{\tau}{\tau'}{\Phi}$ with the above statements, $ \Delta ; \suba{\Phi_a}
   \jeqtype{\suba{\tau }}{\suba{\tau' }}$.\\
   By the above statements and RelRef type equivalence rule
   \textbf{eq-c-prod}, we conclude that \\
    $$\Delta ; \suba{\Phi_a}
   \jeqtype{\suba{ (\tcprod{C}{\tau})
     }}{\suba{ (\tcprod{C'}{\tau'}) }}$$.\\
  \end{mainitem}

\end{proof}

\begin{thm}[Completeness of the Binary Algorithmic Type Equivalence]\label{thm:relref-alg-ty-eq-completeness}
   Assume that $\Delta; \Phi_a \jeqtype{\tau}{\tau'}$. Then $\exists\, \Phi.$ such that  $\Delta ; \Phi_a \jalgeqtype{\tau}{\tau'}{\Phi}$ and $\Delta; \Phi_a \sat \Phi$.  
\end{thm} 

\begin{proof}
  By induction on the binary equivalence typing derivation.\\
\begin{mainitem}
\caseL{ \relrefeqfun }
 By IH on the first premise $\Delta; \Phi_a
 \jeqtype{\tau_1}{\tau_1'}$, there exists $\Phi_1$ s.t $\Delta ; \Phi_a \jalgeqtype{\tau_1}{\tau_1'}{\Phi_1}$ and $\Delta; \Phi_a \sat \Phi_1$.  \\
By IH on the second premise $\Delta; \Phi_a
 \jeqtype{\tau_2}{\tau_2'}$, there exists $\Phi_2$ s.t $\Delta ;
 \Phi_a \jalgeqtype{\tau_2}{\tau_2'}{\Phi_2}$ and $\Delta; \Phi_a \sat
 \Phi_2$.  \\
 By the above statements and algorithmic type equivalence rules
 \textbf{alg-r-fun} with an empty $\Psi_a$, we conclude the following statement where
 $\Phi=\Phi_1 \land \Phi_2$.\\
$\Delta ; \Phi_a \jalgeqtype{\tau_1 \to \tau_2}{\tau_1 \to \tau_2}{\Phi}$ and $\Delta; \Phi_a \sat \Phi$.  

  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\caseL{ \relrefeqlist }
 By IH on the third premise $\Delta; \Phi_a
 \jeqtype{\tau}{\tau'}$, there exists $\Phi_1$ s.t $\Delta ; \Phi_a
 \jalgeqtype{\tau}{\tau'}{\Phi_1}$ and $\Delta; \Phi_a \sat \Phi_1$.
 \\
  By the above statements, the first and second premises and algorithmic type equivalence rules
 \textbf{alg-r-list} with an empty $\Psi_a$, we conclude the following statement where
 $\Phi=\Phi_1 \land \ceq{n}{n'} \land \ceq{\alpha}{\alpha'} $.\\
$\Delta ; \Phi_a \jalgeqtype{  \tlist{n}{\alpha}{\tau}
}{\tlist{n'}{\alpha'
}{\tau'}}{\Phi}$ and $\Delta; \Phi_a \sat \Phi$.  \\

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\caseL{\relrefeqbox}
  By IH on the premise $\Delta; \Phi_a
 \jeqtype{\tau}{\tau'}$, there exists $\Phi_1$ s.t $\Delta ; \Phi_a
 \jalgeqtype{\tau}{\tau'}{\Phi_1}$ and $\Delta; \Phi_a \sat \Phi_1$.
 \\
   By the above statements and algorithmic type equivalence rules
 \textbf{alg-r-$\square$} with an empty $\Psi_a$, we conclude the following statement where
 $\Phi=\Phi_1 $.\\
  $\Delta ; \Phi_a \jalgeqtype{  \tbox{\tau}
}{\tbox{\tau'}}{\Phi}$ and $\Delta; \Phi_a \sat \Phi$.  \\
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
  \caseL{\relrefeqforall}
   By IH on the premise $i,\Delta; \Phi_a
 \jeqtype{\tau}{\tau'}$, there exists $\Phi_1$ s.t $i,\Delta ; \Phi_a
 \jalgeqtype{\tau}{\tau'}{\Phi_1}$ and $i,\Delta; \Phi_a \sat \Phi_1$.
 \\
  By the above statements and algorithmic type equivalence rules
 \textbf{alg-r-forall} with an empty $\Psi_a$, we conclude the
 following statement where $\Phi=\tsforall{i} \Phi_1 $.\\
   $\Delta ; \Phi_a \jalgeqtype{  \tsforall{i} \tau
}{ \tsforall{i} \tau' }{\Phi}$ and $\Delta; \Phi_a \sat \Phi$.  \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\caseL{\relrefeqcprod}
 By IH on the third premise $\Delta; \Phi_a
 \jeqtype{\tau}{\tau'}$, there exists $\Phi_1$ s.t $i,\Delta ; \Phi_a
 \jalgeqtype{\tau}{\tau'}{\Phi_1}$ and $\Delta; \Phi_a \sat \Phi_1$.
 \\
  From the first two premises $\Delta; C' \wedge \Phi_a \sat C$ and $
  \Delta; C \wedge \Phi_a \sat C' $, we know that $ \Delta; \Phi_a
  \sat C \leftrightarrow C' $.\\
  By the above statements and the algorithmic type equivalence rules
 \textbf{alg-r-cprod} with an empty $\Psi_a$, we conclude the
 following statement where $\Phi=C \leftrightarrow C' \land \Phi_1 $.\\
 $\Delta ; \Phi_a \jalgeqtype{  \tcprod{C}{\tau} 
}{ \tcprod{C'}{\tau'} }{\Phi}$ and $\Delta; \Phi_a \sat \Phi$.  \\
\end{mainitem}
\end{proof}

\begin{lem} [Existence of coercions for relational subtyping] \label{lem:relref-elab}
  If $\Delta; \Phi_a \jsubtype{\tau}{\tau'}$ then there exists
  $e\!\!\in \mbox{RelRef Core}$ s.t.\ $\Delta; \Phi_a;
  \cdot
  \jstypet{e}{e}{\tau
    \to \tau'}$.
\end{lem}
\begin{proof}
 Proof is by induction on the subtyping derivation.  We denote the
  witness $e$ of type $\tau \to \tau'$ as $\ecoerce{\tau}{\tau'}$ for clarity.
\begin{mainitem}
    \caseL{\relrefsubto[(\star)][(\diam)]} 
    By IH on $(\star)$, $\exists \ecoerce{\tau_1'}{\tau_1}.~~\Delta; \Phi_a; \cdot \jstypet{\ecoerce{\tau_1'}{\tau_1}}{\ecoerce{\tau_1'}{\tau_1}}{\tau_1' \to \tau_1}$\\
    By IH on $(\diam)$, $\exists \ecoerce{\tau_2}{\tau_2'}.~~\Delta;
    \Phi_a; \cdot \jstypet{\ecoerce{\tau_2}{\tau_2'}}{\ecoerce{\tau_2}{\tau_2'}}{\tau_2 \to \tau_2'}$\\
    
    Then, using these two statements,we can
    construct the following derivation where
    $e= \efix f(x). \efix f(y). \ecoerce{\tau_2}{\tau_2'} \eapp (x \eapp
    (\ecoerce{\tau_1'}{\tau_1} \eapp y))$
    
    $\Delta; \Phi_a; \cdot \jstypet{e}{e}{(\tau_1 \to \tau_2)
      \to \tau_1' \to \tau_2'}$\\
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
   \caseL{\stint}
    Then, we can construct the derivation using the primitive function $\mbox{box}_{\tint} : \trint \to \tbox{\trint}$
    \begin{mathpar}
      \inferrule{ } { \Delta; \Phi_a; \cdot \jstypet{\efix f(x). \mbox{box}_{\tint} x}{\efix f(x). \mbox{box}_{\tint} x}{\trint \to \tbox{\trint}}
      }
    \end{mathpar}
     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \caseL{\stbox}
    Then, we can immediately construct the derivation using the rule \textbf{c-der}.
    \begin{mathpar}
      \inferrule{ } { \Delta; \Phi_a; \cdot \jstypet{\efix f(x). \eder
          x}{\efix f(x). \eder x }{\tbox{\tau} \to \tau}
      }
    \end{mathpar} 
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \caseL{\stboxD}
    Then, we can immediately construct the derivation using the rule \textbf{c-nochange}.
    \begin{mathpar}
      \inferrule{ } { \Delta; \Phi_a; \cdot \jstypet{\efix f(x). \enoch x}{\efix f(x). \enoch x}{\tbox{\tau} \to \tbox{\tbox{\tau}}}
      }
    \end{mathpar}
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \caseL{\stboxB[(\star)]}
    By IH on $(\star)$, $\exists \ecoerce{\tau_1}{\tau_2}.~~ \Delta; \Phi_a; \cdot \jstypet{\ecoerce{\tau_1}{\tau_2}}{\ecoerce{\tau_1}{\tau_2}}{\tau_1 \to \tau_2}$\\

    Then, using $(\star)$ and the rules  \textbf{c-der} and \textbf{c-nochange}, we can construct the derivation 
    \begin{mathpar}
      \inferrule{ } { \Delta; \Phi_a; \cdot  \jstypet{\efix f(x). \enoch ( \ecoerce{\tau_1}{\tau_2} \eapp (\eder x))}{\efix f(x). \enoch ( \ecoerce{\tau_1}{\tau_2} \eapp (\eder x))}{\tbox{\tau_1} \to \tbox{\tau_2}}
      } 
    \end{mathpar}
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \caseL{\strefl}
    Then, we can immediately construct the derivation 
    \begin{mathpar}
      \inferrule{ } { \Delta; \Phi_a; \cdot  \jstypet{\efix
          f(x). x}{\efix f(x).x}{\tau \to \tau}}
    \end{mathpar}
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \caseL{\sttrans[(\star)][(\diam)]}
    By IH on $(\star)$, $\exists \ecoerce{\tau_1}{\tau_2}.~~ \sorted{i}, \Delta; \Phi_a; \cdot \jstypet{\ecoerce{\tau_1}{\tau_2}}{\ecoerce{\tau_1}{\tau_2}}{\tau_1 \to \tau_2}$\\
    By IH on $(\diam)$, $\exists \ecoerce{\tau_2}{\tau_3}.~~ \sorted{i}, \Delta; \Phi_a; \cdot \jstypet{\ecoerce{\tau_2}{\tau_3}}{\ecoerce{\tau_2}{\tau_3}}{\tau_2 \to \tau_3}$\\

    Then, using $(\star)$ and $(\diam)$, we can construct the
    derivation simply by function composition
    \begin{mathpar}
      \inferrule{ } { \Delta; \Phi_a; \cdot \jstypet{\efix f(x). \ecoerce{\tau_2}{\tau_3} \eapp (\ecoerce{\tau_1}{\tau_2} \eapp x)}{\efix f(x). \ecoerce{\tau_2}{\tau_3} \eapp (\ecoerce{\tau_1}{\tau_2} \eapp x)}{\tau_1 \to \tau_3}
      } 
    \end{mathpar}
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
    \caseL{\starrboxD}
    Then, we can immediately construct the derivation  where $e= \efix f(x). \efix (y). \enoch (\eder x) \eapp (\eder y))$\\
    $\Delta; \Phi_a; \cdot \jstypet{e}{e}{\tbox{(\tau_1 \to \tau_2)} \to \tbox{\tau_1} \to \tbox{\tau_2}}$\\

 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
    \caseL{\relrefsubforallD[(\star)]}
    By IH on $(\star)$, $\exists \ecoerce{\tau}{\tau'}.~~ \sorted{i}, \Delta; \Phi_a; \cdot \jstypet{\ecoerce{\tau}{\tau'}}{\ecoerce{\tau}{\tau'}}{\tau \to \tau'}$\\
    
    Then, using this, and the \textbf{c-r-iLam} and \textbf{c-r-iApp} rules,
    we can construct the following derivation:\\
    
    $\Delta; \Phi_a; \cdot \jstypet{\efix f(x). \eLam
      i. \ecoerce{\tau}{\tau'}\eapp(x \eapp  [i])}{\efix f(x). \eLam
      i. \ecoerce{\tau}{\tau'}\eapp(x \eapp  [i])}{(\tsforall{i} \tau)
      \to \tsforall{i} \tau' }$\\
  
   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
    \caseL{\relrefsubforallboxD}
    Then, we can immediately construct the following derivation using the \textbf{c-der},  \textbf{c-nochange}, \textbf{c-r-iLam} and \textbf{c-r-iApp} rules.\\
    
    $\Delta; \Phi_a; \cdot \jstypet{\efix f(x). \eLam
      i. \enoch((\eder x)\, [i])}{\efix f(x). \eLam
      i. \enoch((\eder x)\, [i])}{\tbox{(\tsforall{i} \tau)} \to
      \tsforall{i} \tbox{\tau} }$\\

    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 5
    \caseL{\stlist[(\star)][(\diam)][(\dagg)]}
    By IH on $(\dagg)$, $\exists \ecoerce{\tau}{\tau'}.~~\Delta; \Phi_a; \cdot \jmintypesamet{0}{\ecoerce{\tau}{\tau'}}{\tau \to \tau'}$\\
    We first construct the more generic term for type:\\
    \begin{equation}
      \trunit \to \tforallN{n}  \tforallN{n'} \tforallN{\alpha} \tforallN{\alpha'} (\tcprod{(n=n' \wedge \alpha \leq \alpha')} \tlist{n}{\alpha}{\tau}) \to \tlist{n'}{\alpha'}{\tau'}
    \label{eq:sub-list}
  \end{equation}
  and then instantiate the term for \cref{eq:sub-list} later.\\
  It can be shown that such a derivation can be constructed for
  expression \\
    \begin{minipage}[t]{1.0\linewidth}
      $e'= \efix \mbox{fList}(\_). \eLam n. \eLam n'. \eLam \alpha. \eLam \alpha'. \efix f(x). \clet x \eas e \ein \\
      ~~~~~~\ecase e \eof \\
      ~~~~~~~~\enil \rightarrow \enil \\
      ~~~~~~|~h\,::_{N} tl\, \rightarrow \elet r = \mbox{fList} \eapp
      () \,[n-1]\,[n'-1] \, [\alpha]  \, [\alpha'] \eapp tl\\
      ~~~~~~ \ein \econsNC(\enoch (\ecoerce{\tau}{\tau'} \eapp \eder h), r) \\
      ~~~~~~|~h::_{C} tl\, \rightarrow \elet r = \mbox{fList} \eapp ()
      \, [n-1] \,[n'-1]\,[\alpha-1]  \, [\alpha'-1] \eapp tl \\
      ~~~~~~ \ein \econsC(\ecoerce{\tau}{\tau'} \eapp h, r)
      $ 
    \end{minipage}
    \\\\
    Then, we can instantiate \mbox{fList} using $(\star)$ and $(\diam)$ as follows where \\
    \begin{minipage}[t]{1.0\linewidth}
    $e''= \efix f(x).\mbox{fList} \eapp () \eapp [n] [n'] [\alpha] [\alpha'] \eapp x$
  \end{minipage}
\\
    
    $\Delta; \Phi_a; \cdot \jmintypesamet{0}{e''}{\tlist{n}{\alpha}{\tau} \to \tlist{n'}{\alpha'}{\tau'}}$\\

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
    \caseL{\stlistbox} 
    We first construct the more generic term for type
    \begin{equation}
    \trunit \to \tforallN{n} \tforallN{\alpha} \tlist{n}{\alpha}{\tbox{\tau}} \to
    \tbox{(\tlist{n}{\alpha}{\tau})}\label{eq:sub-list-box} 
  \end{equation}

    and then instantiate the term for \cref{eq:sub-list-box} later.
    It can be shown that such a derivation can be constructed for expression \\
    \begin{minipage}[t]{1.0\linewidth}
      $e'= \efix \mbox{fList}(\_). \eLam n. \eLam \alpha. \efix f(x). \\
      ~~~~~~\ecase e \eof \\
      ~~~~~~~~\enil \rightarrow \enoch (\enil)  \\
      ~~~~~~|~h\,::_{N} tl\, \rightarrow \elet r = \mbox{fList} \eapp () \,[n-1] \, [\alpha] \eapp tl \ein \\
      ~~~~~~~~~~~~~~~~~~~~~~~~~~~~\enoch (\econsNC(\eder h, \eder r)) \\
      ~~~~~~|~h::_{C} tl\, \rightarrow \elet r = \mbox{fList} \eapp () \, [n-1] \,[\alpha-1] \eapp tl \ein \\
      ~~~~~~~~~~~~~~~~~~~~~~~~~~~~\enoch(\econsC(\eder h, \eder r))
      $ 
    \end{minipage}
    \\\\
    Then, we can instantiate \mbox{fList} with a concrete $n$ and $\alpha$ as follows where \begin{minipage}[t]{1.0\linewidth}
    $e''= \efix f(x). \mbox{fList} \eapp () \eapp [n] [\alpha] \eapp x $
  \end{minipage}

    $\Delta; \Phi_a; \cdot \jmintypesame{0}{e''}{\tlist{n}{\alpha}{\tbox{\tau}} \to \tbox{(\tlist{n}{\alpha}{\tau})}}$\\
    
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
    \caseL{\stlistzero}
    We first construct the more generic term for type
    \begin{equation}
    \trunit \to \tforallN{n} \tforallN{\alpha} (\tcprod{\alpha=0}{\tlist{n}{\alpha}{\tau}}) \to \tlist{n}{\alpha}{\tbox{\tau}}\label{eq:sub-list-zero}   
  \end{equation}
    and then instantiate the term for \cref{eq:sub-list-zero} later.
    It can be shown that such a derivation can be constructed for expression\\
    \begin{minipage}[t]{1.0\linewidth}
      $e'= \efix \mbox{fList}(\_). \eLam n. \eLam \alpha. \efix f(x). \clet x \eas e \ein \\
      ~~~~~~\ecase e \eof  \\
      ~~~~~~~~\enil \rightarrow \enil \\
      ~~~~~~|~h\,::_{N} tl\, \rightarrow \elet r = \mbox{fList} \eapp () \,[n-1] [\alpha] \eapp tl \ein \econsNC(\enoch h, r) \\
      ~~~~~~|~h::_{C} tl\, \rightarrow \econtra $ 
    \end{minipage}
    \\\\
    Then, we can instantiate \mbox{fList} with a concrete $n$ and
    $\alpha$ (note the premise $\alpha=0$) as follows
    where \begin{minipage}[t]{1.0\linewidth}
      $e''= \efix f(x). \mbox{fList} \eapp () \eapp [n] [\alpha] \eapp x $
  \end{minipage}

    $\Delta; \Phi_a; \cdot \jmintypesamet{0}{e''}{\tlist{n}{0}{\tau} \to \tlist{n}{0}{\tbox{\tau}}}$\\
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
    \caseL{\stexists[(\star)]}
    By IH on $(\star)$, $\exists \ecoerce{\tau}{\tau'}.~~ \sorted{i}, \Delta; \Phi; \cdot \jmintypesamet{0}{\ecoerce{\tau}{\tau'}}{\tau \to \tau'}$\\
    
    Then, using this and the \textbf{c-r-pack} and \textbf{c-r-unpack} rules,
    we can construct the following derivation where $e= \efix f(x). \eunpack x \eas (y, i) \ein \epack (\ecoerce{\tau}{\tau'} \eapp y)  \ewith i$\\
    
    $\Delta; \Phi_a; \cdot \jmintypesamet{0}{e}{(\texists{i} \tau) \to \texists{i} \tau' }$\\
    
   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
    \caseL{\stexistsbox}
    Then, we can immediately construct the following derivation using the \textbf{c-der}, \textbf{c-nochange}, \textbf{c-r-pack} and \textbf{c-r-unpack} rules in in \Cref{fig:relcostcore-typing1,fig:relcostcore-typing4} where $e= \efix f(x). \eunpack x \eas  (y, i) \ein \enoch(\epack \eder y \ewith i)$. \\
    
    $\Delta; \Phi_a; \cdot \jmintypesamet{0}{e}{(\texists{i} \tbox{\tau}) \to \tbox{(\texists{i} \tau)} }$\\
   
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
    \caseL{\stcimpl[(\star)][(\diam)]}
    By IH on $(\diam)$, $\exists \ecoerce{\tau}{\tau'}.~~ \Delta; \Phi_a; \cdot \jmintypesamet{0}{\ecoerce{\tau}{\tau'}}{\tau \to \tau'}$\\
    
    Then, using this and the premise $(\star)$ along with the \textbf{c-r-c-implI} and \textbf{c-r-c-implE} rules,
    we can construct the following derivation where $e= \efix f(x). \ecoerce{\tau}{\tau'} \eapp (\ecelim x) $\\
    
    $\Delta; \Phi_a; \cdot \jmintypesamet{0}{e}{(\tcimpl{C}{\tau}) \to \tcimpl{C'}{\tau'}}$\\

   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
    \caseL{\stcimplbox}
    Then, we can immediately construct the following derivation using the \textbf{c-der}, \textbf{c-nochange} and \textbf{c-r-c-implE} rules where $e= \elam x. \enoch(\ecelim \eder x)$. \\
    
    $\Delta; \Phi_a; \cdot \jmintypesamet{0}{e}{\tbox{(\tcimpl{C} \tau)} \to  (\tcimpl{C} \tbox{\tau}) }$\\
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
   \caseL{\stcprod[(\star)][(\diam)]}
    By IH on $(\diam)$, $\exists \ecoerce{\tau}{\tau'}.~~ \Delta; \Phi; \cdot \jmintypesamet{0}{\ecoerce{\tau}{\tau'}}{\tau \to \tau'}$\\
     
    Then, using this and the premise $(\star)$ along with the \textbf{c-r-c-prodI} and \textbf{c-r-c-prodE} rules,
    we can construct the following derivation where $e= \efix f(x). \clet x \eas y \ein \ecoerce{\tau}{\tau'} \eapp y $\\
    
    $\Delta; \Phi_a; \cdot \jmintypesamet{0}{e}{(\tcprod{C}{\tau}) \to \tcprod{C'}{\tau'}}$\\

 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
    \caseL{\stcprodbox}
    Then, we can immediately construct the following derivation using
    the \textbf{c-der}, \textbf{c-nochange}, \textbf{c-r-c-prodI} and
    \textbf{c-r-c-prodE} rules where $e= \efix f(x). \clet x \eas y \ein \enoch(\eder y)$. \\
  
    $\Delta; \Phi_a; \cdot \jmintypesamet{0}{e}{ (\tcprod{C} \tbox{\tau}) \to  \tbox{(\tcprod{C} \tau)} }$\\

\end{mainitem}

\end{proof}

\begin{thm} [Types are preserved by embedding for RelRef]\label{relref-min-soundness}
\mbox{} \begin{enumerate}
  % \item If $\Delta; \Phi_a; \Omega \jelabun{}{}{e}{e^*}{\grt}$, then
  %   $\Delta; \Phi_a; \Omega \jtypeM{}{}{e^*}{\grt}$ and $\Delta; \Phi_a; \Omega \jtype{}{}{e}{\grt}$.
  \item If
    $\Delta; \Phi_a; \Gamma \jelabt{t}{e_1}{e_2}{e_1^*}{e_2^*}{\tau}$,
    then $\Delta; \Phi_a; \Gamma \jstypet{e_1^*}{e_2^*}{\tau}$ and
    $\Delta; \Phi_a; \Gamma \jstype{e_1}{e_2}{\tau}$.
\end{enumerate}
\end{thm}
 \begin{proof}
    Proof is by  induction on the embedding derivations. 

\begin{mainitem} 
   \caseL{$\relrefembedsub[(\star)][(\diam)][(\dagg)]$}
  By IH on $(\star)$,  $\Delta; \Phi_a; \Gamma \jtypediffMt{t}{e_1^*}{e_2^*}{\tau}~~(\star\star)$ and  $\Delta; \Phi_a; \Gamma \jstype{e_1}{e_2}{\tau}~~(\star\star\star)$. \\
  By \Cref{lem:relref-elab} using $(\diam)$, we know that $\Delta; \Phi_a; \cdot \jtypediffMt{0}{e'}{e'}{\tau \to \tau'}~~(\diam\diam)$.\\
  By applying \textbf{c-r-app} rule and $(\star\star)$ and $(\diam\diam)$, we get
  $\Delta; \Phi_a; \Gamma \jtypediffMt{t}{e' \eapp e_1^*}{e' \eapp e_2^*}{\tau'}~~(\spadesuit)$. \\
  By reflexivity of binary type equivalence, we know 
  $\Delta; \Phi_a \jeqtype{\tau'}{\tau'}~~(\spadesuit\spadesuit)$.\\
  Then, we conclude as
  follows:
  \begin{mathpar}
       \inferrule{ 
     \ctx \jtypediffMt{t}{e' \eapp e_1^*}{e' \eapp e_2^*}{\tau'}~~(\spadesuit)\\
     \Delta; \Phi_a \jeqtype{\tau'}{\tau'} ~~(\spadesuit\spadesuit)\\
  }
  {\ctx \jtypediffMt{t'}{e' \eapp e_1^*}{e' \eapp e_2^*}{\tau'} }
  ~{\textbf{c-r}-\pmb{\sqsubseteq}}
  \end{mathpar}
  By $(\star\star\star)$ and $(\diam)$ and \textbf{rr-$\sqsubseteq$}, we also conclude 
  $\Delta; \Phi_a; \Gamma \jstype{e_1}{e_2}{\tau'}$. 
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
  \caseL{\relrefembedfix}
  By IH on the premise $ \Delta; \Phi_a;  x: \tau_1, f : \tau_1 \to \tau_2, \Gamma
       \jelabct{t}{e_1}{e_2}{\tau_2} $, $\Delta; \Phi_a;  x: \tau_1, f : \tau_1 \to \tau_2,  \Gamma
       \jtypediffMt{t}{e_1^*}{e_2^*}{\tau_2}~~(\star)$.\\
  By applying \textbf{c-r-fix} rule and $(\star)$, we get
  $\Delta; \Phi_a; \Gamma \jtypediffMt{t}{ \efix f(x). e_1^*}{\efix
    f(x). e_2^*}{\tau_1 \to \tau_2}~~(\spadesuit)$. \\
    Similarly, using \textbf{rr-fix}, we conclude   $\Delta; \Phi_a; \Gamma \jstype{\efix f(x).e_1}{\efix f(x).e_2}{\tau_1 \to \tau_2}$. 
   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
  \caseL{ \relrefembedfixnc}
  By IH on the premise $\Delta; \Phi_a;  x: \tau_1, f : \tbox{(\tau_1
    \to \tau_2)}, \Gamma \jelabct{t}{e}{e}{\tau_2} $, we have :\\
     $\Delta; \Phi_a;  x: \tau_1, f : \tbox{(\tau_1
    \to \tau_2)}, \Gamma \jtypediffMt{t}{e^*}{e^*}{\tau_2}~~(\star)$\\
    and    $\Delta; \Phi_a; \Gamma \jstype{e}{e}{\tau_2}~~(\star\star)$. \\
TS: $\Delta; \Phi_a; \Gamma \jtypediffMt{t}{e^{**}}{e^{**}}{\square (\tau_1
  \to \tau_2)} $\\
  By applying \textbf{c-r-let} rule on $e^{**}$.\\
   \begin{mathpar}
     \inferrule{
  \ctx \jtypediffMt{t_1}{ e_i \eapp x_i}{ e_i \eapp x_i}{\tbox{\Gamma(x_i) } }\\
  \Delta; \Phi_a; \overline{y_i: \tbox{\Gamma(x_i)} }, \Gamma  \jtypediffMt{t_2}{
    \efixNC f(x).e^*[\overline{\eder y_i/x_i}]}{ \efixNC
    f(x).e^*[\overline{\eder y_i/x_i}]}{ \tbox{(\tau_1 \to \tau_2)} }
}
{ \ctx \jtypediffMt{t_1+t_2}{  \elet \overline{ y_i = e_i \eapp x_i}
    \ein \efixNC f(x).e^*[\overline{\eder y_i/x_i}]}{ \elet \overline{ y_i =
      e_i \eapp x_i} \ein \efixNC f(x).e^*[\overline{\eder y_i/x_i}]}{
  \tbox{(\tau_1 \to \tau_2)}  } }~\textbf{c-r-let}
    \end{mathpar}
   
   Set $\Gamma= \overline{x_i:\Gamma(x_i)}$, $\Gamma_1= \overline{y_i:
   \Gamma(x_i)}$.\\
   STS: $ \Delta; \Phi_a; \square \Gamma_1, \Gamma  \jtypediffMt{t_2}{
    \efixNC f(x).e^*[\overline{\eder y_i/x_i}]}{ \efixNC
    f(x).e^*[\overline{\eder y_i/x_i}]}{ \tbox{(\tau_1 \to \tau_2)}
  }$.\\

   By \textbf{c-r-fixNC},\\
  $ \inferrule
  {
    \Delta; \Phi_a;  x: \tau_1, f : \tbox{(\tau_1 \to \tau_2)}, \tbox{\Gamma_1} \jstypet{e^*[\overline{\eder y_i/x_i}]}{e^*[\overline{\eder y_i/x_i}]}{\tau_2}~~(\diam)
  }
  {\Delta; \Phi_a; \square \Gamma_1, \Gamma  \jstypet{\efixNC
      f(x).e^*[\overline{\eder y_i/x_i}]}{ \efixNC f(x).e^*[\overline{\eder y_i/x_i}] }{
              \tbox{(\tau_1 \to \tau_2)}}}~\textbf{c-r-fixNC} $\\
STS: $ \Delta; \Phi_a;  x: \tau_1, f : \tbox{(\tau_1 \to \tau_2)},
\tbox{\Gamma_1} \jstypet{e^*[\overline{\eder
    y_i/x_i}]}{e^*[\overline{\eder y_i/x_i}]}{\tau_2}$.\\
   From $(\star)$, we extend the context and get $\Delta; \Phi_a;  x: \tau_1, f : \tbox{(\tau_1
    \to \tau_2)}, \tbox{\Gamma_1}, \Gamma \jtypediffMt{t}{e^*}{e^*}{\tau_2}~~(\star\star)$.\\
   By \Cref{lem:relref-substitution} on $(\star\star)$ for the number of
  $x_i$ in $\Gamma$ times, we conclude :\\
$  \Delta; \Phi_a;  x: \tau_1, f : \tbox{(\tau_1
    \to \tau_2)}, \tbox{\Gamma_1} \jtypediffMt{t}{e^*[\overline{\eder
    y_i/x_i}] }{e^*[\overline{\eder
    y_i/x_i}]}{\tau_2}$.\\ 
   
   Similarly, using $(\star\star)$ and the third premise and \textbf{rr-fixNC}, we conclude
     $\Delta; \Phi_a; \Gamma \jstype{\efix f(x).e}{\efix f(x).e}{\tbox{\tau_1 \to \tau_2}}$.

   
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
  \caseL{ $\relrefembedconsOne[(\star)][(\diam)]$}
   By IH on the premise $\star $, $\Delta; \Phi_a; \Gamma
   \jtypediffMt{t}{e_1^*}{e_1'^*}{\tau}~~(\star\star)$\\
    By IH on the premise $\diam $, $\Delta; \Phi_a; \Gamma
   \jtypediffMt{t}{e_2^*}{e_2'^*}{ \tlist{n}{\alpha}{\tau}  }~~(\diam\diam)$\\
  By applying \textbf{c-r-con1} rule using $\star\star$ and $\diam\diam$. we get\\
  $\Delta; \Phi_a; \Gamma \jtypediffMt{t}{  \econsC(e_1^*,e_2^*)}{
    \econsC(e_1^*,e_2^*)}{   \tlist{n+1}{\alpha+1}{\tau}  }~~(\spadesuit)$. \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
\caseL{ \relrefembednochange}
 TS:$\ctx,\Gamma' \jtypediffMt{t_1+t_2}{ \elet \overline{ y_i = e_i \eapp x_i}
    \ein \enoch e^* [\overline{\eder y_i/x_i}] }{ \elet \overline{ y_i
      = e_i \eapp x_i} \ein \enoch e^* [\overline{\eder y_i/x_i}] }{
  \tbox{\tau }  }$.\\
 By IH on the first premise $\Delta; \Phi_a; \Gamma
 \jelabt{t}{e}{e}{e^*}{e^*}{\tau}$, \\
 $\Delta; \Phi_a; \Gamma
 \jtypediffMt{t}{e^*}{e^*}{\tau}~~(\star)$\\
 and   $\Delta; \Phi_a; \Gamma \jstype{e}{e}{\tau}~~(\star\star)$.\\
By applying \textbf{c-r-let} rule.\\
   \begin{mathpar}
     \inferrule{
  \ctx,\Gamma' \jtypediffMt{t_1}{ e_i \eapp x_i}{ e_i \eapp x_i}{\tbox{\Gamma(x_i) } }\\
  \Delta; \Phi_a;\square \Gamma_1, \Gamma,\Gamma'  \jtypediffMt{t_2}{
    \enoch e^*[\overline{\eder y_i/x_i}]}{ \enoch e^*[\overline{\eder y_i/x_i}]}{
    \tbox{ \tau} }
}
{ \ctx,\Gamma' \jtypediffMt{t_1+t_2}{ \elet \overline{ y_i = e_i \eapp x_i}
    \ein \enoch e^* [\overline{\eder y_i/x_i}] }{ \elet \overline{ y_i
      = e_i \eapp x_i} \ein \enoch e^* [\overline{\eder y_i/x_i}] }{
  \tbox{\tau }  } }~\textbf{c-r-let}
    \end{mathpar}
   Set $\Gamma= \overline{x_i:\Gamma(x_i)}$, $\Gamma_1= \overline{y_i:
   \Gamma(x_i)}$.\\
   STS:$  \Delta; \Phi_a;\square \Gamma_1, \Gamma,\Gamma'  \jtypediffMt{t_2}{
    \enoch e^*[\overline{\eder y_i/x_i}]}{ \enoch e^*[\overline{\eder y_i/x_i}]}{
    \tbox{ \tau}}$.\\
  By applying \textbf{c-nochange}.\\
   \begin{mathpar}
    \inferrule
{
\Delta; \Phi_a; \tbox{\Gamma_1} \jstypet{e^*[\overline{y_i/x_i}]}{e^*[\overline{y_i/x_i}]}{\tau}
}
{
\Delta; \Phi_a;\square \Gamma_1, \Gamma,\Gamma'  \jtypediffMt{t_2}{
    \enoch e^*[\overline{\eder y_i/x_i}]}{ \enoch e^*[\overline{\eder y_i/x_i}]}{
    \tbox{ \tau} } 
} ~\textbf{c-nochange}
  \end{mathpar}
STS: $\Delta; \Phi_a; \tbox{\Gamma_1}
\jstypet{e^*[\overline{y_i/x_i}]}{e^*[\overline{y_i/x_i}]}{\tau}$.\\
 From $(\star)$, we extend the context and get \\
$\Delta; \Phi_a; \Gamma,\tbox{\Gamma_1}
 \jtypediffMt{t}{e^*}{e^*}{\tau}~~(\star\star)$\\
  By \Cref{lem:relref-substitution} on $(\star\star)$ for the number of
  $x_i$ of $\Gamma$ times, we conclude :\\
$\Delta; \Phi_a; \tbox{\Gamma_1}
\jstypet{e^*[\overline{y_i/x_i}]}{e^*[\overline{y_i/x_i}]}{\tau}$.\\
Similarly, using $(\star\star)$ and the third premise and \textbf{rr-nochange}, we conclude
  $\Delta; \Phi_a; \Gamma \jstype{e}{e}{\tbox{\tau}}$.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


  \end{mainitem}
\end{proof}


\begin{thm} [Completeness of embedding] \label{thm:relref-min-completeness}
  \mbox{}
  \begin{enumerate}
  % \item If $\Delta; \Phi_a; \Omega \jtype{}{}{e}{\grt}$, then there
  %   exists an $ e^*$ such that $\Delta; \Phi; \Omega
  %   \jelabun{}{}{e}{e^*}{\grt}$.
    \item If $\Delta; \Phi_a; \Gamma  \jstype{e_1}{e_2}{\tau}$,
      then there exist $ e_1^*, e_2^*$ such that $\Delta; \Phi_a; \Gamma
      \jelabt{t}{e_1}{e_2}{e_1^*}{e_2^*}{\tau}$.
  \end{enumerate}
\end{thm}
\begin{proof}
By induction on the typing derivations.
\begin{mainitem}
    
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \caseL{\relreftync[(\star)][(\diam)]}
    By IH on $(\star)$, we get $\exists\, e^*$ such that $\Delta; \Phi_a; \Gamma \jelabt{t}{e}{e}{e^*}{e^*}{\tau} ~~(\dagg)$. \\
    By \lemref{lem:relref-elab} on $(\diam)$, we get $\exists e_i= \ecoerce{\Gamma(x_i)}{\tbox{(\Gamma(x_i)}}$ for all $x_i \in dom(\Gamma)~~(\dagg\dagg)$.\\
    By \textbf{e-nochange} embedding rule using $(\dagg)$ and $(\dagg\dagg )$, we can conclude as follows:\\
    $\relrefembednochange[(\dagg)][(\dagg\dagg)]$. 
    
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
   \caseL{\relreftycaseL[(\star)][(\diam)][(\dagg)][(\spadesuit)]}
    By IH on $(\star)$, we get $\exists\, e^*$  and $\exists\, e'^*$ s.t. $\Delta; \Phi_a; \Gamma \jelabt{t}{e}{e'}{e^*}{e'^*}{\tlist{n}{\alpha}{\tau}} ~~(\star\star)$. \\
   By IH on $(\diam)$, we get $\exists\, e_1^*$  and $\exists\, e_1'^*$ s.t. $\Delta; \ceqz{n} \wedge \Phi_a; \Gamma \jelabt{t}{e_1}{e_1'}{e_1^*}{e_1'^*}{\tau'} ~~(\diam\diam)$. \\
   By IH on $(\dagg)$, we get $\exists\, e_2^*$  and $\exists\, e_2'^*$ s.t. \\$\sorted{i}, \Delta; \ceq{n}{i+1} \wedge \Phi_a; h :\tbox{\tau}, tl : \tlist{i}{\alpha}{\tau}, \Gamma \jelabt{t}{e_2}{e_2'}{e_2^*}{e_2'^*}{\tau'} ~(\dagg\dagg)$. \\
   By IH on $(\spadesuit)$, we get $\exists\, e_2^{**}$  and $\exists\, e_2'^{**}$ s.t.\\ $\sorted{i}, \sorted{\beta}, \Delta; \ceq{n}{i+1} \wedge \ceq{\alpha}{\beta+1} \wedge \Phi_a; h :\tau, tl : \tlist{i}{\beta}{\tau}, \Gamma \jelabt{t}{e_2}{e_2'}{e_2^{**}}{e_2'^{**}}{\tau'} ~(\spadesuit\spadesuit)$. \\
    
    By \textbf{e-caseL} embedding rule using $(\star\star)$, $(\diam\diam)$, and $(\spadesuit\spadesuit)$, we can conclude as follows\\
    $\relrefembedcaseL$

     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

    \caseL{\relreftyfixnc[(\star)][(\diam)]}
    By IH on $(\star)$, we get $\exists\, e^*$ such that $\Delta; \Phi_a; x: \tau_1, f: \tbox{(\tau_1 \to \tau_2)}, \Gamma \jelabt{t}{e}{e}{e^*}{e^*}{\tau_2} ~~(\star\star)$. \\
    By \lemref{lem:relref-elab} on $(\diam)$, we get $\exists e_i= \ecoerce{\Gamma(x_i)}{\tbox{(\Gamma(x_i)}}$ for all $x_i \in dom(\Gamma)~~(\diam\diam)$.\\
    
    By \textbf{e-fixNC} embedding rule using $(\star\star)$ and $(\diam\diam )$, we can conclude as follows:\\
    $\relrefembedfixnc$. 


    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
    \caseL{\relreftyilam[(\star)]}
    By IH on $(\star)$, we get $\exists\, e^*$ and $\exists\, e'^*$ such that $\sorted{i}, \Delta; \Phi_a; \Gamma \jelabt{t}{e}{e'}{e^*}{e'^*}{\tau} ~~(\star\star)$. \\
    By \textbf{e-iLam} embedding rule using $(\star\star)$ , we can conclude as follows:\\
    $\relrefembedilam$. 

    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
    \caseL{\relreftyiapp[(\star)][(\diam)]}
    By IH on $(\star)$, we get $\exists\, e^*$ such that $\Delta; \Phi_a; \Gamma \jelabt{t}{e}{e'}{e^*}{e'^*}{\tsforall{i} \tau} ~~(\star\star)$. \\
    By \textbf{e-iApp} embedding rule using $(\star\star)$ and $(\diam)$, we can conclude as follows:\\
    $\relrefembediapp$. 

    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
    \caseL{\relreftypack[(\star)][(\diam)]}
    By IH on $(\star)$, we get $\exists\, e^*$ and $\exists\, e'^*$ such that $\Delta; \Phi_a; \Gamma \jelabt{t}{e}{e'}{e^*}{e'^*}{\tau\{I/i\}} ~~(\star\star)$. \\
    By \textbf{e-pack} embedding rule using $(\star\star)$ and $(\diam)$ , we can conclude as follows:\\
    $\relrefembedpack$. 

    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
    \caseL{\relreftyunpack[(\star)][(\diam)]}
    By IH on $(\star)$, we get $\exists\, e_1^*$ and $\exists\, e_1'^*$ such that $\Delta; \Phi_a; \Gamma \jelabt{t}{e_1}{e_1'}{e_1^*}{e_1'^*}{\texists{i} \tau_1} ~~(\star\star)$. \\
    By IH on $(\diam)$, we get $\exists\, e_2^*$ and $\exists\, e_2'^*$ such that $\sorted{i}, \Delta; \Phi_a; x: \tau_1, \Gamma \jelabt{t}{e_2}{e_2'}{e_2^*}{e_2'^*}{\tau_2} ~~(\diam\diam)$. \\
    By \textbf{e-unpack} embedding rule using $(\star\star)$ and $(\diam\diam)$ , we can conclude as follows:\\
    $\relrefembedunpack$. 

   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
    \caseL{$\relreftysub[(\star)][(\diam)]$}  
    By IH on $(\star)$, we get $\exists\, e_1^*,e_2^*$ such that $\Delta; \Phi_a; \Gamma \jelabct{t}{e_1}{e_2}{\tau} ~~(\star\star)$. \\
    By \Cref{lem:relref-elab} on $(\diam)$, we can show that $\exists e' = \ecoerce{\tau}{\tau'}~~(\diam\diam)$.\\
    By \textbf{e-r-$\sqsubseteq$} rule using $(\star\star)$,
    $(\diam\diam)$ and $(\diam)$, we conclude as follows\\ 
   $\relrefembedsub$

\end{mainitem}
\end{proof}

\begin{thm}[Soundness of algorithmic typechecking]\label{thm:alg-typing-soundness-rr}
\mbox{}
  \begin{enumerate}
 
\item Assume that $\bctx \chdifft{e}{e'}{\tau}{t}{\Phi}$ and
  $\fivars{\Phi_a,\Gamma,\tau} \subseteq dom(\Delta, \psi_a)$ and
  $\theta_a$ is a valid substitution for $\psi_a$ such that
  $\Delta; \suba{\Phi_a} \sat \suba{\Phi}$ holds. Then,
  $\Delta; \suba{\Phi_a}; \suba{\Gamma}
  \jtypediffMt{\suba{t}}{\erty{e}}{\erty{e'}}{\suba{\tau}}$.

\item Assume that $\bctx \infdifft{e}{e'}{\tau}{\psi}{t}{\Phi}$ and
  $\fivars{\Phi_a,\Gamma} \subseteq dom(\Delta, \psi_a) $ and $
  \theta_a$ is a valid substitution for $\psi_a$
  such that $\Delta; \suba{\Phi_a} \sat \suba{\Phi}$ holds. Then,
  $\Delta; \suba{\Phi_a}; \suba{\Gamma}
  \jtypediffMt{\subta{t}}{\erty{e}}{\erty{e'}}{\suba{\tau}}$.
\end{enumerate}  
\end{thm}
%
\begin{proof}
By simultaneous induction on the given algorithmic typing derivations.
\begin{spacing}{1.3}
  \hspace{-1cm} \textbf{Proof of \Cref{thm:alg-typing-soundness-rr}.1:} \\
\begin{mainitem} 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \caseL{\relrefalgtynochange}
  TS: $\Delta; \suba{\Phi_a}; \suba{\Gamma'}, \tbox{\suba{\Gamma}} \jtypedifft{\suba{t}}{\enoch |e|}{\enoch |e|}{\tbox{\suba{\tau}}}$.\\
  By the main assumptions, we have
  $\fivars{\Phi_a,\Gamma', \tbox{\Gamma}, \tau} \subseteq dom(\Delta, \psi_a)~~(\star)$ and \\
  $\Delta; \suba{\Phi_a} \sat \suba{\Phi}~~(\star\star)$ \\
  Using $(\star)$, we can show that
  \begin{enumih}
  \item $\fivars{\Phi_a,\tbox{\Gamma}, \tau} \subseteq  dom(\Delta, \psi_a).$
  \end{enumih}
  % Using $(\star)$,  $(\star\star)$'s derivation must be in a form such that we have
  % \begin{enumih} [resume]
  % \item $\Delta; \suba{\Phi_a} \sat \ceq{0}{\suba{t}}$
  % \item $\Delta \sty{T'}{\scost}$ for some $T'$
  % \item $\Delta; \suba{\Phi_a} \sat \subaex{\Phi}{t' \mapsto T'}$
  % \end{enumih}

By IH1 on the premise using a) and $(\star\star)$, we can show that
  \begin{equation}
    \label{eq:relref-alg-bsound-noch}
    \Delta;\suba{\Phi_a}; \suba{\tbox{\Gamma}}  \jtypedifft{T'}{\erty{e}}{\erty{e}}{\suba{\tau}}
  \end{equation}
  By the \textbf{c-nochange} rule using
  \cref{eq:relref-alg-bsound-noch}, we obtain  $\Delta; \suba{\Phi_a};
  \suba{\Gamma'}, \tbox{\suba{\Gamma}}  \jtypedifft{0}{\enoch \erty{e}
  }{\enoch \erty{e} }{\tbox{\suba{\tau}}}$.\\

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \caseL{\relrefalgtycaseL}
TS:\begin{mathpar}
\Delta; \suba{\Phi_a}; \suba{\Gamma} \jtypedifft{\suba{t}}{\hspace{-1em}
       \begin{minipage}[c]{10em}
         ~ $\ecase e \eof \enil \, \rightarrow \erty{e_1}$ \\
         $~~~~~~~~|~h\,::_{N} tl\, \rightarrow \erty{e_2}$ \\
         $~~~~~~~~|~h::_{C} tl \rightarrow \erty{e_3}$
       \end{minipage}\hspace{-1em}
     }{\hspace{-1em}
       \begin{minipage}[c]{10em}
         ~ $\ecase e' \eof \enil \, \rightarrow \erty{e_1'}$ \\
         $~~~~~~~~|~h\,::_{N} tl\, \rightarrow \erty{e_2'}$ \\
         $~~~~~~~~|~h::_{C} tl \rightarrow \erty{e_3'}$
       \end{minipage}
     }{\suba{\tau'}}
\end{mathpar}\\
  By the main assumptions, we have
  $\fivars{\Phi_a,\Gamma, \tau'} \subseteq dom(\Delta, \psi_a)~~(\star)$ and \\
  $\Delta; \suba{\Phi_a} \sat \suba{(\cand{\Phi_e}{\Phi_{body}})}~~(\star\star)$ \\
% By $(\star)$, we get $ \fivars{\tlist{n}{\alpha}{\tau}, t_1,\Phi_e} \subseteq dom(\Delta, \psi; \psi_a)~(\diam)$.\\
Using $(\star)$, $(\star\star)$'s derivation must be in a form such that we have
\begin{enumih}
\item $\Delta; \suba{\Phi_a} \sat \suba{\Phi_e}$
\item $\Delta; {\ceq{\suba{n}}{0}} \wedge \suba{\Phi_a} \sat \suba{\Phi_1}$
\item $\sorted{i}, \Delta; {\ceq{\suba{n}}{i+1}} \wedge \suba{\Phi_a} \sat \suba{\Phi_2}$
\item $\sorted{i},\sorted{\beta}, \Delta; {\ceq{\suba{n}}{i+1}} \wedge{\ceq{\suba{\alpha}}{\beta+1}} \wedge \suba{\Phi_a} \sat \suba{\Phi_3}$
\end{enumih}
By IH2 on the first premise using a) and $(\star)$, we can show that
  \begin{equation}
    \label{eq:relref-bsound-caseL1}
    \Delta;\suba{\Phi_a}; \suba{\Gamma}  \jtypedifft{\subta{t_1}}{\erty{e}}{\erty{e'}}{\tlist{\suba{n}}{\suba{\alpha}}{\suba{\tau}}}
  \end{equation}

By IH1 on the second premise using b) and $(\star)$, we can show that
  \begin{equation}
    \label{eq:relref-bsound-caseL2}
    \Delta; {\ceq{\suba{n}}{0}} \wedge \suba{\Phi_a}; \suba{\Gamma}  \jtypedifft{T_2}{\erty{e_1}}{\erty{e_1'}}{{\suba{\tau'}}}
  \end{equation}

By IH1 on the third premise using c) and $(\star)$, we can show that
  \begin{equation}
    \label{eq:relref-bsound-caseL3}
    \sorted{i}, \Delta; {\ceq{\suba{n}}{i+1}} \wedge \suba{\Phi_a}; \suba{\Gamma}  \jtypedifft{T_2}{\erty{e_2}}{\erty{e_2'}}{{\suba{\tau'}}}
  \end{equation}

By IH1 on the fourth premise using d) and $(\star)$, we can show that
  \begin{equation}
    \label{eq:relref-bsound-caseL4}
    \sorted{i}, \sorted{\beta}, \Delta; {\ceq{\suba{n}}{i+1}} \wedge{\ceq{\suba{\alpha}}{\beta+1}} \wedge \suba{\Phi_a}; \suba{\Gamma}  \jtypedifft{T_2}{\erty{e_3}}{\erty{e_3'}}{{\suba{\tau'}}}
  \end{equation}
  Then by \textbf{c-r-caseL} rule using
  \cref{eq:relref-bsound-caseL1,eq:relref-bsound-caseL2,eq:relref-bsound-caseL3,eq:relref-bsound-caseL4},
  we can show that 
 \begin{mathpar}
\Delta; \suba{\Phi_a}; \suba{\Gamma} \jtypedifft{\subta{t_1}+T_2}{\hspace{-1em}
       \begin{minipage}[c]{10em}
         ~ $\ecase e \eof \enil \, \rightarrow \erty{e_1}$ \\
         $~~~~~~~~|~h\,::_{N} tl\, \rightarrow \erty{e_2}$ \\
         $~~~~~~~~|~h::_{C} tl \rightarrow \erty{e_3}$
       \end{minipage}\hspace{-1em}
     }{\hspace{-1em}
       \begin{minipage}[c]{10em}
         ~ $\ecase e' \eof \enil \, \rightarrow \erty{e_1'}$ \\
         $~~~~~~~~|~h\,::_{N} tl\, \rightarrow \erty{e_2'}$ \\
         $~~~~~~~~|~h::_{C} tl \rightarrow \erty{e_3'}$
       \end{minipage}
     }{\suba{\tau'}}
\end{mathpar}\\

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \caseL{\relrefalgtyconsnc}
 TS: $\Delta; \suba{\Phi_a}; \suba{\Gamma} \jtypedifft{\suba{t}}{\econsNC(\erty{e_1},\erty{e_2})}{\econsNC(\erty{e_1'},\erty{e_2'})}{\tlist{\suba{n}}{\suba{\alpha}}{\suba{\tau}}}$.\\
 By the main assumptions, we have
  $\fivars{\Phi_a,\Gamma, \tlist{n}{\alpha}{\tau}} \subseteq dom(\Delta, \psi_a)~~(\star)$ and \\
 $\Delta; \suba{\Phi_a} \sat \suba{({\cand{\Phi_1}{\cexists{i}{\ssize}{\Phi_2'}}})}~~(\star\star)$ \\
Using $(\star)$,  $(\star\star)$'s derivation must be in a form such that we have
\begin{enumih}
\item $\Delta; \suba{\Phi_a} \sat \suba{\Phi_1}$
\item  $\Delta \sty{I}{\ssize}$ 
\item $\Delta; \suba{\Phi_a} \sat \subaex{\Phi_2}{ i \mapsto I}$
\item $\Delta; \suba{\Phi_a} \sat \ceq{(I+1)}{\suba{n}}$
\end{enumih}

By IH1 on the second premise using $(\star)$ and a), we can show that
\begin{equation}
  \label{eq:relref-bsound-cons1}
      \Delta; \suba{\Phi_a}; \suba{\Gamma}  \jtypedifft{T_1}{\erty{e_1}}{\erty{e_1'}}{\tbox{\suba{\tau}}}
\end{equation}

By IH1 on the third premise using $(\star)$ and b), we can show that
\begin{equation}
  \label{eq:relref-bsound-cons2}
      \Delta; \suba{\Phi_a}; \suba{\Gamma}  \jtypedifft{T_2}{\erty{e_2}}{\erty{e_2'}}{\tlist{I}{\suba{\alpha}}{\suba{\tau}}}
\end{equation}
By \textbf{c-r-cons2} typing rule using \cref{eq:relref-bsound-cons1,eq:relref-bsound-cons2}, we obtain
\\ $\Delta; \suba{\Phi_a}; \suba{\Gamma} \jtypedifft{T_1+T_2}{\econsNC(\erty{e_1},\erty{e_2})}{\econsNC(\erty{e_1'},\erty{e_2'})}{\tlist{I+1}{\suba{\alpha}}{\suba{\tau}}}$. \\
We conclude by applying \textbf{c-r-}${\pmb{\sqsubseteq}}$ rule to this using d) .

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\end{mainitem}
\end{spacing}



\begin{spacing}{1.3}
  \hspace{-1cm} \textbf{Proof of \Cref{thm:alg-typing-soundness-rr}.2:} \\
\begin{mainitem} 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\caseL{\relrefalgtyanno}
  TS: $\Delta; \suba{\Phi_a}; \suba{\Gamma}  \jtypedifft{\suba{t}}{\erty{\eannobi{e}{\tau}{t}}}{\erty{\eannobi{e'}{\tau}{t}}}{\suba{\tau}}$. \\  
Since by definition,  $\forall e. ~\erty{({e:}{\_})} = \erty{e}$, STS: $\Delta; \suba{\Phi_a}; \suba{\Gamma}  \jtypedifft{\suba{t}}{\erty{e}}{\erty{e'}}{\suba{\tau}}$. \\  
By the main assumptions, we have
$\fivars{\Phi_a,\Gamma} \subseteq dom(\Delta, \psi_a)~~(\star)$ and $\Delta; \suba{\Phi_a} \sat \suba{\Phi}~~(\star\star)$ \\
Using the third premise, we can show that
\begin{enumih}
\item $\fivars{\Phi_a,\Gamma, \tau} \subseteq dom(\Delta, \psi_a).$
\end{enumih}
By IH2 on the first premise using $(\star\star)$ and a), we can conclude that\\
$ \Delta; \suba{\Phi_a}; \suba{\Gamma}
\jtypedifft{\suba{t}}{\erty{e}}{\erty{e'}}{\suba{\tau}}.$

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \caseL{\relrefalgtyder}
  TS: $\Delta; \suba{\Phi_a}; \suba{\Gamma}
  \jtypediffMt{\subta{t}}{\eder \erty{e}}{\eder \erty{e'}}{\subta{\tau}}$. \\
By the main assumptions, we have
$\fivars{\Phi_a,\Gamma} \subseteq dom(\Delta, \psi_a)~~(\star)$ and \\
$\Delta; \suba{\Phi_a} \sat \suba{\Phi}~~(\star\star)$ such that $\subsat{\Delta}{\theta_a}{\psi_a}$ are derivable. \\
By IH2  on the first premise using
$(\star)$ and $\star\star$, we obtain
\begin{equation}
 \Delta; \suba{\Phi_a}; \suba{\Gamma}  \jtypedifft{\suba{t}}{\erty{e}}{\erty{e'}}{\tbox{\suba{\tau}}}\label{eq:alg-bsound-der1}
\end{equation} 
Then, by \textbf{c-der} rule using \cref{eq:alg-bsound-der1}, we can
conclude that\\  $\Delta; \suba{\Phi_a}; \suba{\Gamma}
\jtypedifft{\subta{t}}{\eder \erty{e}}{\eder \erty{e'}}{\subta{\tau}}$.

\end{mainitem}
\end{spacing}
\end{proof}

\begin{thm}[Completeness of algorithmic typechecking]\label{thm:relref-alg-typing-completeness}
\mbox{}
  \begin{enumerate}
  % \item Assume that $\Delta; \Phi_a; \Omega \jtypeM{}{}{e}{\grt}$.
  %   Then, there exists $ e'$ such that $\Delta; \cdot; \Phi_a; \Omega
  %   \chexect{e'}{\grt}{k}{t}{\Phi}$ and $\Delta; \Phi_a \sat \Phi$ and
  %   $\erty{e'} = e$.
  \item Assume that $\Delta; \Phi_a; \Gamma
    \jtypediffMt{t}{e_1}{e_2}{\tau}$.  Then, there exist $e_1',e_2'$
    such that $\Delta; \cdot; \Phi_a; \Gamma
    \chdifft{e_1'}{e_2'}{\tau}{t}{\Phi}$ and $\Delta; \Phi_a \sat \Phi$
    and $\erty{e_1'} = e_1$ and $\erty{e_2'} = e_2$.
  \end{enumerate}  
\end{thm}
%
\begin{proof}
By simultaneous induction on the given Core typing derivations.

\begin{mainitem} 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\caseL{\relrefcoreder}

By IH on the premise, $\exists e_1',e_2'$ such that 
\begin{enumih}
\item $\Delta; \cdot; \Phi_a; \Gamma \chdiff{e_1'}{e_2'}{\tau}{t}{\Phi}$
\item $\Delta; \Phi_a  \sat \Phi$
\item $\erty{e_1'} = e_1$ and $\erty{e_2'} = e_2$
\end{enumih}
Then, we can conclude by using a), b) and c) as follows:\\
 $\chRdert[\cdot][']$ and 

 \begin{enumconc}
 \item \begin{mathpar}
     \inferrule { {\inferrule { \chRdert[\cdot]['] } {\Delta; \cdot;
           \Phi_a; \Gamma \infdifft{(\eder
               e_1':\tau)}{(\eder
             e_2':\tau)}{\tau}{\cdot}{t}{\Phi} }
         ~\textbf{alg-r-anno-$\uparrow$}
       } \\
       \Delta ; \Phi_a \jalgeqtype{\tau}{\tau}{\Phi'}~~\text{by~}\Cref{lem:relref-refl-ty-eq} } { \Delta;
       \cdot; \Phi_a; \Gamma \chdifft{ (\eder
           e_1':\tau)}{(\eder
           e_2':\tau)}{\tau}{t}{\cand{\Phi}{\Phi'}}
     } ~\textbf{alg-r-$\uparrow\downarrow$}
   \end{mathpar}
\item By c), $\erty{(\eder
           e_i':\tau)} = \eder{\erty{e_i'}}$.
\item By b) and \Cref{lem:relref-refl-ty-eq}.
 \end{enumconc}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\caseL{$\relrefcoresub$}
By IH on the first premise, $\exists e_1',e_2'$ such that 
\begin{enumih}
\item $\Delta; \cdot; \Phi_a; \Gamma \chdifft{e_1'}{e_2'}{\tau}{t}{\Phi_1}$
\item $\Delta; \Phi_a  \sat \Phi_1$
\item $\erty{e_1'} = e$ and $\erty{e_2'} = e'$
\end{enumih}
By IH on the second premise, 
\begin{enumih}[resume]
\item $\Delta ; \Phi_a \jalgeqtype{\tau}{\tau'}{\Phi_2}$ 
\item  $\Delta; \Phi_a \sat \Phi_2$.
\end{enumih}
Then, we can conclude as follows
\begin{enumconc}
\item By using a) and d) 
  \begin{mathpar}
    \inferrule
    {
      {\inferrule
        {
          \Delta; \cdot; \Phi_a; \Gamma \chdifft{e_1'}{e_2'}{\tau}{t}{\Phi_1}
        }
        {\Delta; \cdot; \Phi_a; \Gamma  \infdifft{(e_1':\tau)}{(e_2':\tau)}{\tau}{\cdot}{t}{\Phi_1}
        } ~\textbf{alg-r-anno-$\uparrow$} 
      } \\
      \Delta ; \Phi_a \jalgeqtype{\tau}{\tau'}{\Phi_2} 
    }
    { \Delta; \cdot; \Phi_a; \Gamma \chdifft{ (e_1':\tau) }{(e_2':\tau)}{\tau'}{t'}{\cand{\Phi_1}{\Phi_2}}
       } ~\textbf{alg-r-$\uparrow\downarrow$}
  \end{mathpar}
\item By using b), e) ,we can show that $\Delta; \Phi_a \sat {\cand{\Phi_1}{\Phi_2}}$
\item By c), $\erty{(e_1':\tau)} = e_1'$ and $(e_2':\tau) = e_2'$
\end{enumconc}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\caseL{$\relrefcoreapp$}
By IH on the first premise, $\exists \e_1,\e_1'$ such that 
\begin{enumih}
\item $\Delta; \cdot; \Phi_a; \Gamma \chdifft{\e_1}{\e_1'}{\tau_1 \to \tau_2}{t_1}{\Phi_1}$
\item $\Delta; \Phi_a  \sat \Phi_1$
\item $\erty{\e_1} = e_1$ and $\erty{\e_1'} = e_1'$
\end{enumih}

By IH on the second premise, $\exists \e_2,\e_2'$ such that 
\begin{enumih}[resume]
\item $\Delta; \cdot; \Phi_a; \Gamma \chdifft{\e_2}{\e_2'}{\tau_1}{t_2}{\Phi_2}$
\item $\Delta; \Phi_a  \sat \Phi_2$
\item $\erty{\e_2} = e_2$ and $\erty{\e_2'} = e_2'$
\end{enumih}

Then, we can conclude as follows
\begin{enumconc}
\item 
  \begin{mathpar}
    \inferrule
    {\inferrule
      {
        {\inferrule
          {
            \Delta; \cdot; \Phi_a; \Gamma \chdifft{\e_1}{\e_1'}{\tau_1 \to \tau_2}{t_1}{\Phi_1}
          }
          {\Delta; \cdot; \Phi_a; \Gamma \infdifft{(\e_1:{\tau_1 \to \tau_2})}{\e_1':{\tau_1 \to \tau_2})}{\tau_1 \to \tau_2}{\cdot}{t_1}{\Phi_1} }~\textbf{alg-r-anno-$\uparrow$} 
        } \\
        \Delta;  \cdot; \Phi_a; \Gamma \chdifft{\e_2}{\e_2'}{\tau_1}{t_2'}{\Phi_2}
      }
      {
        \Delta; \cdot; \Phi_a; \Gamma \infdifft{E_1}{E_2}{\tau_2}{t_2'}{t_1+t+t_2'}{\cand{\Phi_1}{\Phi_2}}
    }~\textbf{c-r-app}}
  {
    \Delta; \cdot; \Phi_a; \Gamma \chdifft{E_1}{E_2}{\tau_2}{t_1+t+t_2}{\cand{\Phi_1}{\Phi_2}}
  }~\textbf{alg-r-$\uparrow\downarrow$} 
\end{mathpar} \\
where $E_1= (\e_1:\tau_1 \to \tau_2) \eapp \e_2$ and $E_2= (\e_1':\tau_1 \to \tau_2) \eapp \e_2'$.
\item By using b) and e) .
\item Using c) and f),  $\erty{ (\e_1:\tau_1 \to \tau_2)  \eapp \e_2} = e_1 \eapp e_2$ and $\erty{ (\e_1':\tau_1 \to \tau_2)  \eapp \e_2'} = e_1' \eapp e_2'$.
\end{enumconc}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\caseL{$\relrefcoreunpack$}
By IH on the first premise, $\exists \e_1,\e_1'$ such that 
\begin{enumih}
\item $\Delta; \cdot; \Phi_a; \Gamma \chdifft{\e_1}{\e_1'}{\texists{i}\tau_1}{t_1}{\Phi_1}$
\item $\Delta; \Phi_a  \sat \Phi_1$
\item $\erty{\e_1} = e_1$ and $\erty{\e_1'} = e_1'$
\end{enumih}

By IH on the second premise, $\exists \e_2,\e_2'$ such that 
\begin{enumih}[resume]
\item $\sorted{i}, \Delta; \cdot; \Phi_a; x: \tau_1, \Gamma \chdifft{\e_2}{\e_2'}{\tau_2}{t_2}{\Phi_2}$
\item $\sorted{i}, \Delta; \Phi_a  \sat \Phi_2$
\item $\erty{\e_2} = e_2$ and $\erty{\e_2'} = e_2'$
\end{enumih}

Then, we can conclude as follows
\begin{enumconc}
\item \begin{mathpar}
    \inferrule { {\inferrule{ \Delta; \cdot; \Phi_a; \Gamma
          \chdifft{\e_1}{\e_1'}{\texists{i}\tau_1}{t_1}{\Phi_1}~~(a) }
        { \Delta; \cdot; \Phi_a; \Gamma
          \infdifft{E_1}{E_1'}{\texists{i}\tau_1}{\cdot}{t_1}{\Phi_1}
        }~\textbf{alg-r-anno-$\uparrow$} } \\
      \sorted{i}, \Delta;  \Phi_a; x: \tau_1, \Gamma \chdifft{\e_2}{\e_2'}{\tau_2}{t_2'}{\Phi_2} \\
      \Phi'=
      {\cand{\Phi_1}{\Phi_2'}}
    } {\Delta; \cdot; \Phi_a; \Gamma \chdifft{\eunpack E_1 \eas (x, i)
        \ein \e_2}{\eunpack E_1' \eas (x, i) \ein
        \e_2'}{\tau_2}{t_1+t_2}{\Phi'}
    }~\textbf{alg-r-unpack-$\downarrow$}
  \end{mathpar}
  where $E_1= (\e_1:\texists{i}\tau_1)$ and
  $E_2= (\e_1':\texists{i}\tau_1)$
\item By using b) and e).
\item Using c) and f),  $\erty{\eunpack  (\e_1:\texists{i}\tau_1) \eas (x,i) \ein \e_2} = \eunpack e_1 \eas (x,i) \ein e_2$ and  $\erty{\eunpack  (\e_1':\texists{i}\tau_1) \eas (x,i) \ein \e_2'} = \eunpack e_1' \eas (x,i) \ein e_2'$.
\end{enumconc}

\end{mainitem}
\end{proof}



==> RSTLC/relstlc_figures.tex <==
\begin{figure}
  \centering
\[
\begin{array}{llll}
 \label{fig:syntax}
   \mbox{Types} 
  &  \tau & ::= & \trbool ~|~ \tubool ~|~  \tau_1 \to \tau_2  \\

  \mbox{Expressions} & e & ::= & x  ~|~ \etrue ~|~ \efalse ~|~ \eif e
                                 \ethen e_1 \eelse e_2 ~|~ \elam x. e
                                 ~|~ e_1 \eapp e_2  \\
  \mbox{Value} & v& := & \etrue ~|~ \efalse ~|~ \elam x. e  
\end{array}
\] 
 \caption{Syntax of values and expressions in RSTLC} 
  
\end{figure}

\begin{figure}
  \centering
\[
\begin{array}{llll}
 \label{fig:syntax}
   \mbox{Types} 
  &  \tau & ::= & \trbool ~|~ \tubool ~|~  \tau_1 \to \tau_2  \\

  \mbox{Expressions} & e & ::= & x  ~|~ \etrue ~|~ \efalse ~|~ \eif e \ethen e_1 \eelse e_2 ~|~ \elam x. e ~|~ e_1 \eapp e_2 \\
  \mbox{Value} & v& := & \etrue ~|~ \efalse ~|~ \elam x. e  
\end{array}
\] 
 \caption{Syntax of values and expressions in RSTLC-CORE} 
  
\end{figure}

\begin{figure}
  \centering
\[
\begin{array}{llll}
 \label{fig:syntax}
   \mbox{Types} 
  &  \tau & ::= & \trbool ~|~ \tubool ~|~  \tau_1 \to \tau_2  \\

  \mbox{Expressions} & e & ::= & x  ~|~ \etrue ~|~ \efalse ~|~ \eif e
                                 \ethen e_1 \eelse e_2 ~|~ \elam x. e
                                 ~|~ e_1 \eapp e_2  ~|~ (e:\tau)\\
  \mbox{Value} & v& := & \etrue ~|~ \efalse ~|~ \elam x. e  
\end{array}
\] 
 \caption{Syntax of values and expressions in BiRSTLC} 
  
\end{figure}


\begin{figure}
  \centering 
  \begin{mathpar}
    \rstlcvar
    \and
    \rstlcbool
    \and
    \rstlcboolu
    \and
    \rstlcif
    \and
   \rstlcfix
    \and
    \rstlcapp
   \and
   \rstlcsub
  \end{mathpar}
 \caption{Relational STLC typing rules}
\label{fig:rel-stlc-typing}
\end{figure}

\begin{figure}
  \centering 
  \begin{mathpar}
    \inferrule{
    }
    {
      \jsubtype{\trbool}{\tubool}
    }~\textbf{bool}
    \and
     \inferrule{
       \jsubtype{\tau_1'}{\tau_1} \\
       \jsubtype{\tau_2}{\tau_2'}
     }
     {
       \jsubtype{\tau_1 \to \tau_2}{\tau_1' \to \tau_2'}
     }~\textbf{$\to$}
     \and
     \inferrule
     {
     }
     {  \jsubtype{\tau}{\tau}
     }\textbf{refl}
     \and
     \inferrule{
       \jsubtype{\tau_1}{\tau_2} \\
       \jsubtype{\tau_2}{\tau_3}
     }
     {
       \jsubtype{\tau_1}{\tau_3}
     }\textbf{trans}
   \end{mathpar}
   \caption{Subtyping rules for RSTLC}
   \label{fig:rel-stlc-subtyping}
 \end{figure}
  
\begin{figure}
  \centering 
  \begin{mathpar}
    \inferrule
    {\Gamma(x) = \tau } 
    { \Gamma \infsdiff{x}{x}{\tau}}~\textbf{alg-r-var}
    \and
    \rstlcalgboolr
    \and
\boxed{
    \inferrule
    { \kw{b_1, b_2}  \in \{\etrue, \efalse \}  \\
    b_1 \not = b_2 }
    { \Gamma
      \chsdiff{\kw{b_1}}{\kw{b_2}}{\tubool}}~\textbf{alg-r-u-bool} }
    \and
    \inferrule{\Gamma \infsdiff{e}{e'}{\trbool} \\
      \Gamma \chsdiff{ e_1}{e_1'}{\tau} \\
      \Gamma \chsdiff{ e_2}{e_2'}{\tau}
    }
    {\Gamma \chsdiff{\eif e \ethen e_1 \eelse e_2}{\eif e' \ethen e_1' \eelse e_2'}{\tau}}~\textbf{alg-r-if}
    \and
    \rstlcalgfix
    \and
    \rstlcalgapp
    \and
    \inferrule{
      \Gamma \infsdiff{e}{e'}{\tau'}\\
      \jalgssubtype{\tau'}{\tau} \\
    }
    { 
      \Gamma \chsdiff{e}{e'}{\tau}
    }~\textbf{alg-$\uparrow\downarrow$}
    \and
    \rstlcalganno
  \end{mathpar}
 \caption{Algorithmic typing rules for RSTLC}
\label{fig:rel-stlc-alg-typing}
\end{figure}

\begin{figure}
  \centering 
  \begin{mathpar}
    \rstlcsubalgboolr
    \and
   \rstlcsubalgboolu
    \and
   \rstlcsubalgbool
    \and
    \rstlcsubalgto
   \end{mathpar}
   \caption{Algorithmic subtyping rules for Relational STLC}
   \label{fig:rel-stlc-alg-subtyping}
 \end{figure}

\begin{figure*}
  \centering
  \vspace{-1ex}
  \raggedright
  \[\begin{array}{ lc  l} 
      \erty{.} &:& \text{Expression}   \to \text{Expression}   \\\\
     % \erty{\kw{n}} &=& \kw{n} \\
     % \erty{()} &=& () \\
      \erty{x} &=& x \\
    %  \erty{\efix f(x). e} &=& \efix f(x). \erty{e} \\
     % \erty{\efixNC f(x). e} &=& \efixNC f(x). \erty{e} \\
      \erty{e_1 \eapp e_2} &=& \erty{e_1} \eapp \erty{e_2} \\
      \vdots &&\\
      \erty{(e:\tau) } &=& \erty{e} \\
     % \erty{(e:\grt)} &=& \erty{e} \\
    \end{array}\]
  \caption{Annotation erasure}
  \label{fig:ty-annot-erasure}
\end{figure*}


==> RSTLC/relstlc_lemmas.tex <==
\subsection{RelSTLC Lemmas}
\begin{lem}[Reflexivity of algorithmic subtyping] The
  reflexivity property holds for algorithm subtyping for RelSTLC.\\
 $\jalgssubtype{\tau}{\tau}$.
  \label{lem:rstlc-refl}
\end{lem} 


\begin{proof}
   By induction on the binary type.

   \begin{mainitem}
    \caseL{$\trbool$}
     It is proved by \textbf{alg-bool-r}.

     \caseL{$\tubool$}
    It is proved by \textbf{alg-bool-u}.

     \caseL{$\tau_1 \to \tau_2$}
     By \textbf{alg-$\to$}, TS: $\jalgssubtype{\tau_1}{\tau_1}$ and
     $\jalgssubtype{\tau_2}{\tau_2}$, which is obtained by IH on
     $\tau_1$ and $\tau_2$ respectively.
   \end{mainitem}
 \end{proof}

\begin{lem}[ Transitivity of algorithmic subtyping]  The
  transitivity property holds for algorithm subtyping for RelSTLC.\\
 $\jalgssubtype{\tau_1}{\tau_2}$ and $\jalgssubtype{\tau_2}{\tau_3}$,
 then $\jalgssubtype{\tau_1}{\tau_3}$.
\label{lem:rstlc-trans}
\end{lem}
\begin{proof}
By simultaneous induction on the first two subtyping derivation.\\
 \begin{mainitem}
  \caseL{\rstlcsubalgboolr, \rstlcsubalgboolr } 
         
         TS: $\jalgssubtype{\trbool}{\trbool}  $, which is proved by
         \textbf{alg-bool-r}.
%%%%%%%%%%%%%%%%
     \caseL{ \rstlcsubalgboolu, \rstlcsubalgboolu  }
      TS: $\jalgssubtype{\tubool}{\tubool} $,  which is proved by \textbf{alg-bool-u}.  

%%%%%%%%%%%%%%%%%
     \caseL{  \rstlcsubalgbool, \rstlcsubalgboolu  }
      TS: $\jalgssubtype{ \trbool }{ \tubool }$, which is proved by
      \textbf{alg-bool}.  

%%%%%%%%%%%%%%%
    \caseL{\rstlcsubalgboolr , \rstlcsubalgbool}
    TS:  TS: $\jalgssubtype{ \trbool }{ \tubool }$, which is proved by
      \textbf{alg-bool}.  
%%%%%%%%%%%%%%%%%%%%
    \caseL{\rstlcsubalgto, \inferrule{
       \jalgssubtype{\tau_1''}{\tau_1'} \\
       \jalgssubtype{\tau_2'}{\tau_2''}
     }
     {
       \jalgssubtype{\tau_1' \to \tau_2'}{\tau_1'' \to \tau_2''}
     }~\textbf{alg-$\to$} }
     TS: $ \jalgssubtype{\tau_1 \to \tau_2 }{\tau_1'' \to \tau_2''  }
     $.\\
     By IH on $\jalgssubtype{\tau_1''}{\tau_1'}$ and
     $\jalgssubtype{\tau_1'}{\tau_1}$,
     $\jalgssubtype{\tau_1''}{\tau_1}$.\\
    
     By IH on $\jalgssubtype{\tau_2'}{\tau_1''}$ and
     $\jalgssubtype{\tau_2}{\tau_2'}$,
     $\jalgssubtype{\tau_2}{\tau_2''}$.\\

   It is proved by using the two statements and rule \textbf{alg-$\to$}.
     
      \end{mainitem}
\end{proof}

Next, we can show that the algorithmic formulation of subtyping
($\tau_1 \leq \tau_2$) coincides with the declarative formulation of
subtyping ($\tau_1 \sqsubseteq \tau_2$). We do this in two steps.

\begin{lem} [Soundness of algorithmic subtyping]
  If $\jalgssubtype{\tau}{\tau'}$ then  $\jsubtype{\tau}{\tau'}$.\label{lem:alg-sub-stlc-soundness}
\end{lem}
\begin{proof}
  Proof is by straightforward induction on the given algorithmic
  subtyping derivation.\\
  \begin{mainitem}
   \caseL{ \rstlcsubalgto  }
    TS: $\vDash \tau_1 \to \tau_2 \sqsubseteq \tau_1' \to \tau_2'$\\
    By IH on $\jalgssubtype{\tau_1'}{\tau_1}$, $\vDash \tau_1' \sqsubseteq
    \tau_1$.\\
By IH on $\jalgssubtype{\tau_2}{\tau_2'}$, $\vDash \tau_2 \sqsubseteq \tau_2'$.\\
    It is proved using these two statements and subtyping rule \textbf{$\to$}.
   %%%%%
    \caseL{ \rstlcsubalgbool }
    TS: $\vDash \trbool \sqsubseteq \tubool$, which is proved by subtyping
    rule \textbf{bool}.
   %%%%%%
   \caseL{ \rstlcsubalgboolu }
      TS: $\vDash \tubool \sqsubseteq \tubool$, which is proved by subtyping
    rule \textbf{refl}.
  %%%%%%%
   \caseL{\rstlcsubalgboolr}
      TS: $\vDash \trbool \sqsubseteq \trbool$, which is proved by subtyping
    rule \textbf{refl}.
  \end{mainitem}
\end{proof}

\begin{lem} [Completeness of algorithmic subtyping]
  If $\jsubtype{\tau}{\tau'}$ then  $\jalgssubtype{\tau}{\tau'}$.\label{lem:alg-sub-stlc-completeness}
\end{lem}
\begin{proof}
  Proof is by induction on the given subtyping derivation.
   \begin{mainitem}
   \caseL{ \rstlcsubto  }
    TS: $\vDash\tau_1 \to \tau_2  \leq \tau_1' \to \tau_2'$\\
    By IH on $\jsubtype{\tau_1'}{\tau_1}$, $\vDash\tau_1'  \leq
    \tau_1$.\\
    By IH on $\jsubtype{\tau_2}{\tau_2'}$, $\vDash\tau_2  \leq \tau_2'$.\\
    It is proved using these two statements and algorithmic subtyping rule \textbf{alg-$\to$}.
   %%%%%
    \caseL{ \rstlcsubbool }
    TS: $\vDash\trbool  \leq \tubool$, which is proved by algorithmic subtyping
    rule \textbf{alg-bool}.
   %%%%%%
   \caseL{ \rstlcsubrefl }
      TS: $\vDash \tau  \leq \tau$, which is proved by \Cref{lem:rstlc-refl}.
  %%%%%%%
   \caseL{\rstlcsubtrans}
      TS: $\vDash \tau_1  \leq \tau_3 $.\\
     By IH on $\jsubtype{\tau_1}{\tau_2}$,
     $\jalgssubtype{\tau_1}{\tau_2}$.\\
     By IH on $\jsubtype{\tau_2}{\tau_3}$,
     $\jalgssubtype{\tau_2}{\tau_3}$.\\
     It is proved using these two statements and \Cref{lem:rstlc-trans}.
  \end{mainitem}
\end{proof}


\begin{lem} [Soundness of algorithmic typing]
  The following holds, $|.|$ is the annotation erasure function.
  \begin{enumerate}
  \item If $ \Gamma \chsdiff{e_1}{e_2}{\tau}$ then
    $ \Gamma \jstype{|e_1|}{|e_2|}{\tau}$.
  \item If $ \Gamma \infsdiff{e_1}{e_2}{\tau}$ then
    $  \Gamma \jstype{|e_1|}{|e_2|}{\tau}$.\label{lem:alg-stlc-soundness}
\end{enumerate}

\end{lem}
\begin{proof}
  Proof is by simultaneous induction on the given algorithmic checking
  and inference derivations and \Cref{lem:alg-sub-stlc-soundness}.\\
  \begin{mainitem}
   \caseL{ \rstlcalgvar}
    TS: $  \Gamma \jstype{|x|}{|x|}{\tau}$ \\
    It is proved by using the premise $\Gamma(x)=\tau$ and typing rule \textbf{r-var}.
   %%%%%%%%%%%
  \caseL{ \rstlcalgif  }
   TS:    $  \Gamma \jstype{| \eif e \ethen e_1 \eelse e_2  |}{|\eif
     e' \ethen e_1' \eelse e_2' |}{\tau}$ \\
   By IH2 on $\Gamma \infsdiff{e}{e'}{\trbool}$,$\Gamma
   \jstype{|e|}{|e'|}{\trbool}$. \\
   By IH on $ \Gamma \chsdiff{ e_1}{e_1'}{\tau} $, $\Gamma
   \jstype{|e_1|}{|e_1'|}{\tau}$. \\
   By IH on $ \Gamma \chsdiff{ e_2}{e_2'}{\tau} $, $\Gamma
   \jstype{|e_2|}{|e_2'|}{\tau}$. \\
    Because $|  \eif e \ethen e_1 \eelse e_2   | =  \eif |e| \ethen |e_1|
    \eelse | e_2  |$.
   By using these three statements and typing rule \textbf{r-if}, we
   get the conclusion.
  %%%%%%%%%%%%%%
  \caseL{ \rstlcalgfix }
   TS: $ \Gamma \jstype{ \elam x.|e_1| }{ \elam x.|e_1| }{ \tau_1 \to
     \tau_2 }  $.\\
   By IH on $\Gamma, x: \tau_1  \chsdiff{e_1}{e_2}{\tau_2}$,  $\Gamma,
   x: \tau_1  \jstype{|e_1|}{|e_2|}{ \tau_2} $.\\
    It is proved by the above statment and tying rule \textbf{ r-fix}.
  
   %%%%%%%%%%%%%5
    \caseL{\rstlcalgsub}
   TS: $ \Gamma \jstype{ |e| }{ |e'| }{ \tau  }  $.\\
   By \Cref{lem:alg-sub-stlc-soundness} on $\jalgssubtype{\tau}{\tau'} $, $\jsubtype{\tau}{\tau'}$.\\
   By IH2 on $\Gamma \infsdiff{e}{e'}{\tau}$,  $\Gamma,  \jstype{|e|}{|e'|}{\tau} $.\\
    It is proved by the above statment and tying rule \textbf{r-}\pmb{$\sqsubseteq$}.


    %%%%%%%%%%%
    \caseL{\rstlcalganno} 
     TS: $ \Gamma \jstype{ |(e:\tau)| }{ |(e':\tau)| }{ \tau  } $,
     which is simplified as $ \Gamma \jstype{ e }{ e' }{ \tau  } $.\\
     By IH on $\Gamma \chsdiff{e}{e'}{\tau} $, $ \Gamma \jstype{ e
     }{e'}{\tau}$.\\
     It is proved by the above statement.
  \end{mainitem}
\end{proof}

\begin{lem} [Completeness of algorithmic typing]
  If $ \Gamma \jstype{e_1}{e_2}{\tau}$ then there exists $e_1'$ and $e_2'$ such that $ \Gamma \chsdiff{e_1'}{e_2'}{\tau}$ and $|e_i'| = e_i$ for $i \in \{1,2\}$.\label{lem:alg-stlc-completeness}
\end{lem}
\begin{proof}
  Proof is by induction on the given typing derivation and
  \Cref{lem:alg-sub-stlc-completeness}.
  \begin{mainitem}
   \caseL{ \rstlcfix }
   By IH on $ \Gamma,  x: \tau_1 \jstype{e_1}{e_2}{\tau_2}$, $\exists
   e_1',e_2'. \Gamma, x: \tau_1 \chsdiff{e_1'}{e_2'}{\tau_2} $ and $|e_i'|=e_i$.\\
   Then, using the above statement and algorithmic typing rule
   \textbf{alg-r-fix}, we can construct the derivation where $e_1''=
   \elam x.e_1'$ and $e_2''= \elam x.e_2'$ .\\
   $$\Gamma\chsdiff{e_1''}{e_2''}{\tau_1 \to \tau_2}  $$\\
   And we show that $|e_i''|=|\elam x.e_i'|=\elam x.|e_i'|= \elam x.e_i'$.
   %%%%%%%%%%
    \caseL{ \rstlcif }
     By IH on $\Gamma \jstype{e}{e'}{\trbool}$,  $\exists
   e'',e'''. \Gamma, \chsdiff{e''}{e'''}{\trbool}$ and $|e''|=e,
   |e'''|=e'$. \\
   By using algorithmic typing rule \textbf{alg-r-anno-$\uparrow$}, $
   \Gamma \infsdiff{(e'':\trbool)}{(e''':\trbool)}{\trbool}$. \\
    By IH on  $\Gamma \jstype{ e_1}{e_1'}{\tau}$,  $\exists
   e_1'',e_1'''. \Gamma, \chsdiff{e_1''}{e_1'''}{\tau}$ and
   $|e_1''|=e_1, |e_1'''|=e_1'$. \\
    By IH on  $\Gamma \jstype{ e_2}{e_2'}{\tau}$,  $\exists
   e_2'',e_2'''. \Gamma, \chsdiff{e_2''}{e_2'''}{\tau}$ and
   $|e_2''|=e_2, |e_2'''|=e_2'$. \\
    Then, using the above statement and algorithmic typing rule
   \textbf{alg-r-if}, we can construct the derivation where $e_3=
   \eif (e'':\trbool) \ethen e_1'' \eelse e_2''$ and $e_4= \eif (e''':\trbool) \ethen e_1''' \eelse e_2'''$ .\\
   $$\Gamma\chsdiff{e_3}{e_4}{\tau}  $$\\
   And we show that $|e_3|=|\eif (e'':\trbool) \ethen e_1'' \eelse
   e_2''|=\eif |(e'':\trbool)| \ethen |e_1''| \eelse |e_2''|= \eif e
   \ethen e_1 \eelse e_2$, similarly for $e_4$.

   %%%%%%%%
   \caseL{\rstlcapp}
    By IH on $\Gamma \jstype{e_1}{e_1'}{\tau_1 \to \tau_2}$,  $\exists
   e_1'',e_1'''. \Gamma, \chsdiff{e_1''}{e_1'''}{\tau_1 \to \tau_2}$ and $|e_1''|=e_1,
   |e_1'''|=e_1'$. \\
   By using algorithmic typing rule \textbf{alg-r-anno-$\uparrow$}, $
   \Gamma \infsdiff{(e_1'':\tau_1 \to \tau_2 )}{(e_1''':\tau_1 \to
     \tau_2)}{\tau_1 \to \tau_2}$. \\
     By IH on  $\Gamma \jstype{ e_2}{e_2'}{\tau_1}$,  $\exists
   e_2'',e_2'''. \Gamma, \chsdiff{e_2''}{e_2'''}{\tau_1}$ and
   $|e_2''|=e_2, |e_2'''|=e_2'$. \\
   Then, using the above statement and algorithmic typing rule
   \textbf{alg-r-app}, we can construct the derivation where $e_3=
   e_1'' \eapp e_2''$ and $e_4=  e_1''' \eapp e_2'''$ .\\
   $$\Gamma\chsdiff{e_3}{e_4}{\tau_2}  $$\\
   And we show that $|e_3|=| e_1'' \eapp e_2''|= |e_1''| \eapp |e_2''|=  e_1 \eapp e_2$, , similarly for $e_4$.

     %%%%%%%
   \caseL{\rstlcsub}
    By IH on $\Gamma \jstype{e_1}{e_2}{\tau}$,  $\exists
   e_1',e_2'. \Gamma, \chsdiff{e_1'}{e_2'}{\tau}$ and $|e_1'|=e_1,
   |e_2'|=e_2$. \\
   By using algorithmic typing rule \textbf{alg-r-anno-$\uparrow$}, $
   \Gamma \infsdiff{(e_1':\tau )}{(e_2':\tau)}{\tau}$. \\
   By using \Cref{lem:alg-sub-stlc-soundness} on premise $
   \jsubtype{\tau}{\tau'}$, $ \jalgssubtype{\tau}{\tau'}$.   \\
   Then, using the above statement and algorithmic typing rule
   \textbf{alg-r-$\uparrow\downarrow$}, we can construct the derivation where $e_3=
   (e_1':\tau) $ and $e_4=(e_2':\tau) $ .\\
   $$\Gamma\chsdiff{e_3}{e_4}{\tau}  $$\\
   And we show that $|e_3|=| (e_1':\tau) |= |e_1'|=e_1$, similarly for $e_4$.
  \end{mainitem}
\end{proof}

==> alg-type-system.tex <==
\subsection{Algorithmic (Bidirectional) Type System}
\label{sec:alg-type-system}

Next, we describe an algorithmic type system for {\tnamemin}. We still
rely
on bidirectionality, which allows us to type check with very few type
annotations. We call our bidirectional system {\bitname}.
%
%% Even though the type system of {\tnamemin} is significantly less
%% nondeterministic than that of {\tname}, it still cannot be
%% implemented directly. This is because, in some of the typing rules,
%% the expression itself does not prescribe the type. For instance,
%% the term $\lambda x.x$ can be typed at $\tau \tarrd{k} \tau$ for
%% any $k$ and $\tau$. To eliminate this kind of nondeterminism with
%% minimal annotation, we develop a bidirectional type system for
%% {\tnamemin}. We call this bidirectional type system {\bitname}.
%


Like all other bidirectional
systems~\cite{Pierce:2000,xi99:dependent,XiThesis}, the goal of
{\bitname} is to eliminate the nondeterminism inherent in typing
Curry-style unannotated terms (e.g., the term $\lambda x.x$ can be
given the type $\tau \tarrd{k} \tau$ for any $\tau$ and $k$) using
minimal type annotations. This is done by typing every expression
construct in one of the two modes: \textit{synthesis/inference} mode,
where the type is inferred or \textit{checking} mode, where a provided
type is checked. The additional aspect in {\bitname} is that not only
a type, but also a cost (effect) must be inferred or checked. In
general, the cost follows the same mode as the type: If for an
expression, the type is inferred (checked), then so is the cost.

%% We believe that this observation will generalize to bidirectional
%% versions of all type and effect systems.

% Another complicating aspect is the use of type refinements in
% {\tnamemin} and {\tname}. To handle these, our type system generates
% arithmetic constraints that stipulate relations between, e.g., sizes
% of various lists and the costs of various subexpressions. This is
% similar to the treatment of refinements in
% DML~\cite{xi99:dependent,XiThesis}, but we additionally handle
% relational refinements and both unary and relational costs.

%% When we write a typechecker, the type system developed in
%% {\tnamemin} does not fully specify whether the type declarations
%% should be treated as an input or output. Bidirectional type
%% systems~\cite{xi99:dependent,Pierce:2000} make this distinction
%% explicit by operating in two modes: \textit{synthesis/inference}
%% mode, where typing information is obtained as an output by
%% propagating upward from subexpressions, and \textit{checking} mode,
%% where information is provided as input by the enclosing
%% expressions, which is propagated downwards afterwards. In
%% {\bitname}, we observe that execution and relational cost
%% information can also be treated as type information, i.e. whenever
%% the type can be checked (inferred), the execution costs and the
%% relational cost can also be checked (inferred) as well.
% Below, we
% describe {\bitname}'s bidirectional typechecking judgments in which
% the outputs are represented in {\color{red} red} and the inputs are
% represented in {\color{black} black}.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Algorithmic typechecking as constraint satisfaction} 
% To develop the bidirectional type system, we add some syntactic
% classes and extend the existing ones.

% \[ \begin{array}{@{}l@{~~}l@{~}l@{~}l@{}l}
%     \text{meta~variables} & M & \bnfdef & i,n,m, \cdots \\
%     \text{index~terms} & I,k,t & \bnfdef & \cdots~|~ M \\
%     \text{meta~contexts} & \psi &  \bnfdef & \emptyset~ |~ \psi, M : \sort\\
%     \text{meta~substitutions} & \theta &  \bnfdef & []~ |~ \theta[M \mapsto I]\\
%     \text{constraints} & C &  \bnfdef & \cdots ~ |~ \cforallS{i}{S}{C} ~|~ \cexistsK{i}{S}{C} \\
%     \text{expressions} & e &  \bnfdef & \cdots ~ |~ \eanno{e}{\grt}{k}{t} ~|~ \eannobi{e}{\tau}{t} \\
%     \end{array}\]
% One class of note is the meta variables $i, n, m$, etc. Also known as
% existential variables, meta variables represent unknown index terms
% that appear in types and costs. These meta variables are resolved by
% constraint solving.
In the expression syntax of {\bitname}, we modify the type-annoated
expressions with cost: $\eanno{e}{\grt}{k}{t} $ and
$\eannobi{e}{\tau}{t}$. % Since {\tnamemin} has two typing judgments---a unary judgment and a
% relational judgment---{\bitname} has four mutually recursive
% algorithmic typing judgments: one each to synthesize and check a unary
% type, and one each to synthesize and check a relational type.
The
relational checking judgment
$\Delta; \psi_a; \Phi_a; \Gamma \chdiff{e_1}{e_2}{\tau}{t}{\Phi}$
% means that, \emph{assuming that the constraint \textcolor{red}{$\Phi$}
%   holds}, $e_1$ and $e_2$ check against the relational input type
% $\tau$ and 
takes as input the relative cost $t$. % under the assumption $\Phi_a$.
% All
% index and meta variables must occur in $\Delta$ and $\psi_a$. When the
% judgment is read operationally or is implemented, the constraint
% \textcolor{red}{$\Phi$} is an output; all other components are
% inputs. (As a convention, we write all outputs in \textcolor{red}{red}
% and all inputs in black.) 
The relational inference judgment
$\Delta; \psi_a; \Phi_a; \Gamma
\infdiff{e_1}{e_2}{\tau}{\psi}{t}{\Phi}$ % means that, if
% \textcolor{red}{$\Phi$} holds, then it can be inferred that the
% relational type of $e_1$ and $e_2$ is \textcolor{red}{$\tau$} and 
outputs the relative cost \textcolor{red}{$t$}%  under the assumption
% $\exists {\color{red} \psi}. {\color{red} \Phi_a}$. Here,
% \textcolor{red}{$\Phi$}, \textcolor{red}{$\tau$},
% \textcolor{red}{$\psi$} and \textcolor{red}{$t$} are all outputs. 
The
meta variable context \textcolor{red}{$\psi$} tracks newly generated
cost variables that may appear in the inferred type or cost. Its
significance will be explained below.

% Intuitively, the checking mode is used when the surrounding
% outer context determines the type and the cost of the expression. This
% happens at all introduction forms and in case-like elimination
% forms. The inference mode is used when there is no outer restriction
% on the type or the cost of an expression. This happens for the
% principal term in all elimination forms.

The unary checking and inference judgments, $\Delta; \psi_a; \Phi_a;
\Omega \chexec{e}{\grt}{k}{t}{\Phi}$ and $\Delta; \psi_a; \Phi_a;
\Omega \infexec{e}{\grt}{\psi}{k}{t}{\Phi}$, are to be understood
similarly.

  % The checking judgment of form
  % $\Delta; \psi_a; \Phi_a; \Gamma \chdiff{e_1}{e_2}{\tau}{t}{\Phi}$
  % means that $e$ checks against input type $\tau$ and cost $t$ under
  % the assumption $\Phi_a$ in which all the index and meta variables
  % are declared in $\Delta$ and $\psi_a$, respectively and it generates
  % the constraint $\Phi$. Similarly, inference judgment of form
  % $\Delta; \psi_a; \Phi_a; \Gamma
  % \infdiff{e_1}{e_2}{\tau}{\psi}{t}{\Phi}$ means that $e_1$ and $e_2$
  % synthesizes an output type $\tau$ and cost $t$ under the assumption
  % $\Phi_a$ in which all the index and meta variables are declared in
  % $\Delta$ and $\psi_a$, respectively and it also generates the
  % constraint $\Phi$ and a context $\psi$ containing all the newly
  % declared meta variables. The meta context $\psi_a$ (denoted on the
  % left side of the $\vdash$) contains all the existential meta
  % variables that occur in the checked type and cost which is
  % determined by the surrounding outer context and $\psi_a$ is always
  % given to both the inference and the checking judgments. On the other
  % hand, the meta context $\psi$ (denoted on the right side of the
  % $\vdash$) contains all the existential meta variables that occur in
  % the synthesized type and cost, therefore it is generated only for
  % the inference judgment. Their interaction is described below in
  % detail in the algorithmic rule \textbf{alg-r-app$\uparrow$}.
 

  % \ezgi{fix here: $\psi_a$ is not universally quantified. Need
  %   to explain the purpose of $\psi$ and $\psi_a$.}  The variables in
  % the meta context $\psi_a$ (given on the left side of the $\vdash$),
  % can be thought as being universally quantified, whereas the
  % variables in the meta context $\psi$ (defined only in the inference
  % judgment) can be thought as being existentially quantified. The
  % distinction will be explained in detail below.

\begin{figure}[t]
% \fbox{$\Delta; \psi_a; \Phi_a   \subtype{\grt_1}{\grt_2}{\Phi}$}~~~checks whether $\grt_1$ is a subtype of $\grt_2$ and generates constraints in $\Phi$\\
  \fbox{$\Delta; \psi_a; \Phi_a \jalgeqtype{\tau_1}{\tau_2}{\Phi}$}~~~checks whether $\tau_1$ is equivalent to $\tau_2$ and generates constraints in $\Phi$\\
\begin{mathpar}
  \astfunPLDI
  \and
  \astlistPLDI 
\end{mathpar}
% \nocaptionrule

% Definitions at appendix/alg-type-eq-rules-defs.tex
\caption{Selected algorithmic type equivalence rules}
\label{fig:alg-type-eq-rules}  
\end{figure} 


\paragraph{Algorithmic typing rules} 
Figures~\ref{fig:selected-alg-typing-rules}
and~\ref{fig:selected-alg-typing-rules2} list a few selected
algorithmic relational typing rules; algorithmic unary typing rules
follow similar guidelines (except that they track two costs) and,
hence, we omit them here. Since we already explain the main principles
in {\birelref}, we will focus on the principles related to cost and
discuss some selected rules.  
 % We first explain the main principles behind
% the bidirectional typing rules and then discuss selected rules. While
% some of these principles are standard, those related to cost are
% new.
We also highlight other {\bitname}-specific principles.
\begin{itemize} 
% \item Types and costs of variables and elimination forms are inferred
%   (e.g., rules \textbf{alg-r-var}$\uparrow$,
%   \textbf{alg-r-app}$\uparrow$) whereas types and costs of
%   introduction forms are checked (e.g., rules
%   \textbf{alg-r-fix}$\downarrow$, \textbf{alg-r-consC}$\downarrow$).
%   There are a few exceptions to this principle: the type of the
%   branches in case analyses or the continuation in let-bindings is
%   checked.
\item (Specific to {\bitname}) If an expression consists of a
  subexpression that must be checked against a type, we generate a
  fresh meta variable for the subexpression's cost. This is necessary
  since at the point we reach the subexpression, we don't know what
  cost to check against. When we check the subexpression, constraints
  that determine this meta variable are generated.  If the whole
  expression is in checking mode, we existentially quantify over the
  freshly generated variable in the constraint (e.g., rule
  \textbf{alg-r-consC$\downarrow$}). If the whole expression is in
  inference mode, we simply add the meta variable to the inferred cost
  and append it to $\psi$ (e.g. rule \textbf{alg-r-app$\uparrow$}).
% \item In checking mode, if no other checking rule matches the given
%   expression, then the rule \textbf{alg-r-$\uparrow\downarrow$} allows
%   switching to inference mode in the premise. The requirement is that
%   the inferred type must be equivalent to the checked type and the
%   inferred cost must be no greater than the checked cost. In the
%   algorithmic system, we have an algorithmic type equivalence relation
%   $\jalgeqtype{\tau}{\tau'}{\Phi}$ whose selected rules are shown in
%   Figure~\ref{fig:alg-type-eq-rules}. The meaning of the judgment is
%   that if \textcolor{red}{$\Phi$} holds, then $\tau \pmb{\equiv}
%   \tau'$. Like other bidirectional systems, this is the only place
%   where type equivalence ({\tnamemin}'s reduct of subtyping) is used.
% \item In inference mode, it is permissible to switch to checking mode
%   when an expression's type and cost have been explicitly annotated by
%   the programmer (rule \textbf{alg-r-anno-$\uparrow$}). It can be shown that it suffices to annotate only at
%   explicit $\beta$-redexes (although there is no prohibition on
%   annotating at other places).
\item (Specific to {\bitname}) The algorithmic version of the rule
  \textbf{c-nochange}, called \textbf{alg-r-nochange}, applies in
  checking mode since it introduces the type $\tbox{\tau}$. The
  algorithmic version of the rule \textbf{c-der}, called
  \textbf{alg-r-der}, applies in inference mode since it eliminates
  the type $\tbox{\tau}$.
\end{itemize}

% Switching to unary mode in {\bitname} is possible both in checking
% (rule \textbf{alg-r-switch-$\downarrow$}) and inference (rule
% \textbf{alg-r-switch-$\uparrow$}) modes. This is because often we
% switch to the unary mode for elimination forms where the eliminated
% type is of form $\tcho{\grt}$. Hence, since elimination forms can be
% typed both in inference mode (e.g.\ rule \textbf{alg-r-app-$\uparrow$})
% as well as checking mode (e.g.\ rule
% \textbf{alg-r-caseL-$\downarrow$}), to eliminate unnecessary
% annotations, {\bitname} supports two modes for typing $\eswitch$
% expressions.

Functions are typed in checking mode (rule
\textbf{alg-r-fix-$\downarrow$}) by checking the related function
bodies in the checking mode against the relative cost of the function
bodies. Since functions are values, we add the additional constraint
that the total cost of the functions, $t$, is equal to zero.  Dually,
function applications are typed in inference mode (rule
\textbf{alg-r-app-}$\uparrow$). We first infer the type and the cost
of the related functions and then use the (inferred) argument type to
switch to the checking mode for the related argument
expressions. Since we do not know the cost with which to check the
arguments, we also generate a fresh cost variable $t_2$ to check the
arguments. Finally, the result type is the return type of the inferred
function type, and the total cost is sum of the inferred cost for the
function, the relative cost of the bodies of the related functions and
$t_2$, the as-yet unknown cost of the arguments. Note that since all
the newly generated variables, i.e.\ $\psi$ and $t_2$, may occur in
the resulting type and the cost, inference mode passes them to the
surrounding context.

% \wq{consC explained in relref, without cost} The list constructors are typed in the checking mode. We explain only
% the rule \textbf{alg-r-consC-}$\downarrow$ for typing two non-empty
% lists with type $\tlist{n}{\alpha}{\tau}$ where the heads of the two
% lists may differ. The two related tails are checked with type
% $\tlist{i}{\beta}{\tau}$, where $i$ and $\beta$ are newly generated
% meta variables with the constraint that $\alpha=\beta+1$ and
% $n=i+1$. Since we do not know how the total cost $t$ is distributed
% between the heads and the tails, we generate two new cost variables
% $t_1$ and $t_2$ to check the heads and the tails, respectively and
% generate the constraint $t = t_1 + t_2$.


A particularly interesting aspect of bidirectional typing in
{\bitname} is that the effects (costs), both unary and relational, are
constraint-dependent. For example, the relative cost of a function's
body might depend on the sizes of its inputs. In this case, a
constraint will relate the cost and the inputs' sizes. In existing
bidirectional systems with refinement types, similar interactions show
up among the sizes of data structures like
lists~\cite{xi99:dependent,XiThesis}.


%% What makes bidirectional typing in {\bitname} interesting is that
%% unary and relational effects are constraint-dependent: e.g. the
%% relational cost of a function might depend on the size of its inputs
%% on which constraints get accumulated as the derivation is
%% constructed. Just like in bidirectional systems for refinement
%% types~\cite{xi99:dependent}, things like list sizes are resolved using
%% constrains, here the costs are resolved in the same way.

%% The treatment of the comonadic type $\tbox{\tau}$ in {\bitname} is
%% worth mentioning: since $\enoch e$ is an introduction form, it is
%% typechecked in checking mode (rule
%% \textbf{alg-r-nochange$\downarrow$}) whereas $\eder e$ is an
%% elimination form, hence it is typechecked in the inference mode (rule
%% \textbf{alg-r-der$\uparrow$}).
  
  % In
  % addition to two standard judgments, we also have an additional
  % judgment of form
  % $\Delta; \psi_a; \Phi_a; \Gamma
  % \chdiffNC{e_1}{e_2}{\tbox{\tau}}{t}{\Phi}$ which checks against the
  % type $\tbox{\tau}$ and requires the cost to be $0$. This judgment
  % corresponds to the non-deterministic \textbf{nochange} rule in
  % {\tname} and has only a single algorithmic typing rule in
  % {\bitname}: rule NC-$\downarrow$ checks that all free variables of
  % $e$ are non-changing (by invoking algorithmic subtyping) and makes
  % sure that the cost is 0. It is only invoked at specific points in
  % {\bitname}: \textbf{caseL1}-$\downarrow$ and
  % \textbf{cons}-$\downarrow$ rules.

  % Variables are typed in the inference mode with 0 cost and an empty
  % meta variable context since there is no generated meta variable
  % (rule \textbf{alg-r-var}$\uparrow$). The rule \textbf{alg-r-consC$\downarrow$}


  % In {\tname}, the expression
  % $\econs(e_1,e_2)$ has two corresponding rules: \textbf{cons1} for
  % stable head and \textbf{cons2} for possibly changing head. These two
  % cases are handled simultaneously in the algorithmic rule
  % \textbf{consCP}-$\downarrow$ by combining the resulting constraints
  % with a disjunction. If $e_1$ can not change, then we check $e_1$
  % with the nochange judgment and $e_2$ is allowed $\alpha$ changes. If
  % $e_1$ can change, then $e_2$ is allowed $\beta$ changes, in which
  % $\beta$ is a newly generated meta variable with a constraint
  % $\beta+1 = \alpha$. In both cases, we generate a new meta variable
  % $m$ for $e_2$'s size and add the constraint $m+1 = n$. For the cost
  % of typechecking $e_1$, because we do not know how the total cost $t$
  % is divided between two premises, we generate a new meta variable
  % $t'$. Then, $e_2$ is checked with $t-t'$ cost. In all the premises,
  % corresponding newly generated constraints are appended to the meta
  % variable context $\psi_a$ for checking the premises. The final
  % constraint quantifies over the generated meta variables
  % existentially. % Typechecking $\cons{e_1}{e_2}$ in the $\vfr$ typing
  % % mode is simpler since we do not have to care 

  % Rule $\textbf{caseL-}\downarrow$ typechecks the case analysis on
  % lists. This rule looks complicated (/ is technically involved) since
  % it incorporates a case analysis on the index domain, in particular
  % on $\alpha$, the number of changes of the pattern-matched list of
  % type $\tlist{n}{\alpha}{\tau}$. In {\tname}, such case analysis
  % on the index domain is non-deterministic and is always used in
  % combination with \textbf{nochange} rule. In {\bitname}, we make this
  % reasoning deterministic by incorporating it into the
  % $\textbf{caseL-}\downarrow$ rule by considering two cases : $\alpha
  % = 0$ and $1 \leq \alpha$. For typechecking the body of the case when
  % $\alpha=0$, we invoke the nochange checking judgment as well as the
  % usual checking judgment; their constraints are combined with
  % disjunction. Newly generated existential variables from the
  % inference of the pattern-matched list are passed to the assumed meta
  % context of body of the case and are quantified existentially in the
  % final constraint.

  % \ezgi{explain app rule}

  % A technical subtlety worth mentioning is the treatment of
  % existential variables in {\bitname}. In DML~\cite{xi99:dependent},
  % existential variables are collected in a single context that is
  % provided as an input for the checking mode and obtained as an output
  % for the inference mode. However, whenever there is a switch from
  % checking mode (which is given as an existential context $\psi$) to
  % inference mode (which infers some existential context $\psi'$), the
  % existential context $\psi$ must be adjusted to $\psi'$ by a
  % weakening rule. Similarly, whenever inference mode invokes multiple
  % inference modes, a similar adjustment is necessary to make sure that
  % all free variables of the typing context are defined in the
  % existential context. Instead, we employ two existential contexts for
  % the inference mode: $\psi_a$ (a for assumed) that is given as an
  % input containing all the existential variables from the outer
  % context, and generated $\psi$ which is obtained as an output
  % containing all the newly generated existential variables. The
  % advantage of this approach is that we do not need to do such
  % adjustments and our algorithmic typing rules directly correspond to
  % the implementation.
  

  % \paragraph{Algorithmic subtyping}
  % Figure~% \ref{fig:alg-subtyping-rules}
  % lists selected algorithmic
  % subtyping rules. Similar to the algorithmic typing, algorithmic
  % subtyping also generates a constraint. The algorithmic subtyping
  % judgment $\Delta; \psi_a; \Phi_a \jalgeqtype{\tau}{\tau'}{\Phi}$
  % means that under the context $\Delta$ and assumption $\Phi_a$ where
  % the meta variables are defined in $\psi_a$, type $\tau$ is a subtype
  % of $\tau'$ with respect to the subtyping mode $\epsilon$ if the
  % constraint $\Phi$ is satisfied. Most of the rules are the same as
  % {\tname}'s subtyping rules with additional constraint tracking. For
  % list types in change-propagation mode, {\bitname} has a single rule
  % \textbf{listCP} that combines \textbf{l1*} and \textbf{l2} rules of
  % {\tname} with a disjunction.

 


\begin{figure*}
  \raggedright
  \fbox{$\Delta; \psi_a; \Phi_a; \Gamma
    \chdiff{e_1}{e_2}{\tau}{t}{\Phi}$} ~$e_1$ and $e_2$ check against
  the input type $\tau$
  and the cost $t$ under the assumption $\Phi_a$ in which all the meta vars are declared in $\psi_a$ while generating the constraint $\Phi$.\\
  \fbox{$\Delta; \psi_a ; \Phi_a; \Gamma
    \infdiff{e_1}{e_2}{\tau}{\psi}{t}{\Phi}$} ~ $e_1$ and $e_2$
  synthesize the output type $\tau$ and the cost $t$ under the
  assumption $\Phi_a$ while generating the constraint $\Phi$ in which
  all the newly generated meta vars are declared in $\psi$.

\begin{mathpar}
  \infRswitch
  \and
  \chRswitch
  \and
  \chRnochange
  \and
  \infRder
  \and
 \chRupdown
\and
    \chRsplit
  % \chRder
  % \and
  % \infRvar
  % \and
  % \chRfix
  % \and
  % \infRapp
  % \and
  % \chRcons
  % \and
  % \chRconsbox
  % \and
  % \chRcaseL
  % \and
  % \chRsplit
\end{mathpar}

% \nocaptionrule
% Definitions at alg-typing-rules-defs.tex
\caption{Selected algorithmic typing rules (Part 1).}
\label{fig:selected-alg-typing-rules} 
\end{figure*} 

 
% \begin{figure*}
%   \begin{mathpar}
%     \chRiLam
%     \and
%     \infRiApp
%     \and
%     \chRcandElim
%     \and
%     \chRupdown
%     \and
%     \infRanno
%     \and
%     \chRsplit
%   \end{mathpar}
% \caption{Selected algorithmic typing rules (Part 2).}
% \label{fig:selected-alg-typing-rules2} 
% \end{figure*} 





\paragraph{Soundness and completeness}
We prove that the algorithmic type system is sound and complete
w.r.t.\ the type system of {\tnamemin}. Specifically, soundness says
that any inference or checking judgment provable in the algorithmic
type system can be simulated in {\tnamemin} if the output constraints
\textcolor{red}{$\Phi$} are satisfiable. Dually, completeness says
that any typeable {\tnamemin} program can be sufficiently annotated
(with types) to make its type checkable in {\bitname}, with
satisfiable output constraints. We define $\erty{e}$ to be the
function that erases typing annotations from a {\bitname} expression
$e$ to yield a {\tnamemin} expression. Important cases of its
definition are shown in the appendix.

% \begin{thm}[Soundness of algorithmic typechecking]\label{thm:alg-typing-soundness}
% \mbox{}
%   \begin{enumerate}
%   \item Assume $\uctx \chexec{e}{\grt}{k}{t}{\Phi}$ ,
%   \\ and $\fivars{\Phi_a,\Omega,\grt,k, t} \subseteq dom(\Delta,
%   \psi_a) $, \\
%     $\theta_a$ is a valid substitution for $\psi_a$ s.t.
%     $\Delta; \suba{\Phi_a} \sat \suba{\Phi}$ holds. Then,
%     $\Delta; \suba{\Phi_a}; \suba{\Omega}
%     \jtypeM{\suba{k}}{\suba{t}}{\erty{e}}{\suba{\grt}}$.

%   \item Assume that $\uctx \infexec{e}{\grt}{\psi}{k}{t}{\Phi}$ and
%     $\fivars{\Phi_a,\Omega} \subseteq dom(\Delta, \psi_a)$ and
%     $\theta$ and $ \theta_a$ are valid substitutions for $\psi$ and
%     $\psi_a$ such that $\Delta; \suba{\Phi_a} \sat \subta{\Phi}$
%     holds. Then,
%     $\Delta; \suba{\Phi_a}; \suba{\Omega}
%     \jtypeM{\subta{k}}{\subta{t}}{\erty{e}}{\subta{\grt}}$.
%     % and $\Delta; \psi_a; \Phi_a \awfty{\grt} $

% \item Assume that $\bctx \chdiff{e}{e'}{\tau}{t}{\Phi}$ and
%   $\fivars{\Phi_a,\Gamma,\tau,t} \subseteq dom(\Delta, \psi_a)$ and
%   $\theta_a$ is a valid substitution for $\psi_a$ such that
%   $\Delta; \suba{\Phi_a} \sat \suba{\Phi}$ holds. Then,
%   $\Delta; \suba{\Phi_a}; \suba{\Gamma}
%   \jtypediffM{\suba{t}}{\erty{e}}{\erty{e'}}{\suba{\tau}}$.

% \item Assume that $\bctx \infdiff{e}{e'}{\tau}{\psi}{t}{\Phi}$ and
%   $\fivars{\Phi_a,\Gamma} \subseteq dom(\Delta, \psi_a) $ and $\theta$
%   and $ \theta_a$ are valid substitutions for $\psi$ and $\psi_a$
%   such that $\Delta; \suba{\Phi_a} \sat \subta{\Phi}$ holds. Then,
%   $\Delta; \suba{\Phi_a}; \suba{\Gamma}
%   \jtypediffM{\subta{t}}{\erty{e}}{\erty{e'}}{\subta{\tau}}$.
% \end{enumerate}  
% \end{thm}
% %
% \begin{proof}
% By simultaneous induction on the given algorithmic typing derivations.
% \end{proof}

% \begin{thm}[Completeness of algorithmic typechecking]\label{thm:alg-typing-completeness}
% \mbox{}
%   \begin{enumerate}
%   \item Assume that $\Delta; \Phi_a; \Omega \jtypeM{k}{t}{e}{\grt}$.
%     Then, there exists $ e'$ such that $\Delta; \cdot; \Phi_a; \Omega
%     \chexec{e'}{\grt}{k}{t}{\Phi}$ and $\Delta; \Phi_a \sat \Phi$ and
%     $\erty{e'} = e$.
%   \item Assume that $\Delta; \Phi_a; \Gamma
%     \jtypediffM{t}{e_1}{e_2}{\tau}$.  Then, there exist $e_1',e_2'$
%     such that $\Delta; \cdot; \Phi_a; \Gamma
%     \chdiff{e_1'}{e_2'}{\tau}{t}{\Phi}$ and $\Delta; \Phi_a \sat \Phi$
%     and $\erty{e_1'} = e_1$ and $\erty{e_2'} = e_2$.
%   \end{enumerate}  
% \end{thm}
% %
% \begin{proof}
% By simultaneous induction on the given {\tnamemin} typing derivations.
% \end{proof}
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 
 


==> elaboration.tex <==
\subsection{Embedding into {\tnamemin}}
\label{sec:elab}

Several aspects of {\tname}'s type system make it hard to
algorithmize. considering the experience we algorithmize previous
systems, we highlight some of these aspects below.

%% We have so far presented the declarative specification language
%% {\tname}. Although {\tname} is compact and easy to reason about for
%% programmers, it has serious drawbacks in terms of algorithmic
%% typechecking:
% there is an inherent nondeterminism and constraint-dependence in
% the typing and subtyping rules of {\tname}:
\begin{description}
\item \emph{Non-syntax-directed rules}: The typing rules
  \textbf{switch}, \textbf{r-split}, \textbf{r-contra} and
  \textbf{nochange} are not syntax-directed.%  Hence, these rules
  % introduce nondeterminism in an implementation.
\item \emph{Two ways to type ``{\econs}'' construct}: There are two
  typing rules for constructing non-empty lists in {\tname}: the rule
  \textbf{r-cons1} applies when the heads of the two related lists may
  differ and the rule \textbf{r-cons2} applies when the heads may not
  differ. Hence, the typing of the {\econs} construct is
  context-specific.
\item \emph{List-case branch is typed twice}: In the list case
  analysis rule, \textbf{r-caseL}, the {\econs} case branch is typed
  twice in the premises, to account for the aforementioned two
  introduction rules. Hence, the branch must be typed in a
  non-syntax-directed manner. A consequence of this double-typing of
  the same branch is that, in {\tname}, index terms cannot appear in
  expressions (since the two typings of a cons-branch may instantiate
  universally quantified index variables differently). This makes
  typechecking harder.
\item \emph{Subtyping with $\tbox{\tau}$ and $(\tcho{\grt})$}: It is
  unclear how to implement the \textbf{trans} rule of the relational
  subtyping rules of {\tname} (Figure~\ref{fig:subtyping-rules}). The
  usual solution would be to prove that transitivity is admissible
  among the remaining rules. However, it is unclear how to prove the
  admissibility of transitivity in the presence of the comonadic type
  $\tbox{\tau}$ and the modality $\tcho{\grt}$, whose subtyping rules
  interact with the other connectives in nontrivial ways.
%
%% It is also not unclear whether the rule is admissible. Relational
%% subtyping rules of {\tname} turn out to be particularly challenging
%% for algorithmization. In particular, it is not clear how the rule of
%% transitivity of subtyping can be shown admissible in the algorithmic
%% system due to the nontrivial interactions with the comonadic type
%% $\tbox{\tau}$ and constraints.

% Moreover, admissibility of transitivity of the subtyping rules for
% the comonadic type $\tbox{\tau}$ is extremely difficult considering
% the potential interaction with the constraints in rule \textbf{l2}
% of Figure \ref{fig:subtyping-rules}.
%
\end{description}

% All these difficulties, with the exception of those due to the rules
% \textbf{split} and \textbf{r-contra}, are a consequence of the
% presence of either relational refinements or relational
% effects. Consequently, they do not arise in other type and effect
% systems. In particular, the difficulty with transitivity is specific
% to the relational subtyping; in unary subtyping, transitivity is
% admissible and poses no difficulty.

% The goal of this
% embedding is purely to make a theoretical point---that there is a
% language ({\tnamemin}) that is as expressive as {\tname} and that is
% also amenable to a complete bidirectional typing
% procedure. {\tnamemin} has explicit syntactic markers to indicate
% which typing rules to apply where, thus resolving the nondeterminism
% in the first two points above. Additionally, {\tnamemin}'s list case
% construct has two separate branches for the two typings of the cons
% case, thus allowing {\tnamemin} to include instantiations of
% universally quantified parameters explicitly in expressions. This
% resolves the difficulty mentioned in the third point above. Finally,
% we address the fourth point by replacing all occurrences of relational
% subtyping with explicit coercion functions (that we show to exist) in
% the embedding. 
% Elimination of subtyping is a common technique for
% simplifying
% typechecking~\cite{Breazu-Tannen:1991,Crary:2000}. However, as
% explained below, {\tname}'s subtyping is constraint-dependent, so
% extra care is needed when dealing with index terms appearing in the
% types.

%% To remedy the
%% problems that arise from the lack of syntax-directedness (first two
%% points above), we give an \emph{embedding} of {\tname} programs into
%% an intermediate language called {\tnamemin}. This embedding is type-derivation-directed. Hence, by
%% examining the type derivation, our embedding adds syntactic markers
%% into the program expressions and duplicates the \kw{cons} case
%% branches on lists, thus eliminating the nondeterminism.


%% To remedy the problem of subtyping (third point above), we eliminate
%% relational subtyping during this embedding phase by replacing
%% occurrences of relational subtyping with explicit coercions in
%% {\tnamemin}. This idea is not new: 

To address these difficulties, we give an \emph{embedding} of {\tname}
into an intermediate language we call {\tnamemin} that has only
type-directed rules and no relational subtyping. We prove that our
embedding is complete and sound. (Theorem~\ref{thm:relcost-min-completeness}).
% Although the embedding of {\tname} into {\tnamemin} is specific to
% {\tname},   
Consider the previous systems, we believe 
the methodology of using such an embedding to prove
completeness modulo nondeterminism is more general and could be useful
for other systems as well. In particular, relational systems that have
nondeterministic rules to switch to unary mode or implicit coercions
could benefit from this method.


%% Below, we first present the syntax and typing rules of the
%% intermediate language {\tnamemin} and then we explain these two points
%% in detail.

% \paragraph{Syntax of {\tnamemin}} The expression syntax of {\tnamemin}
% is an extension of {\tname}'s syntax with additional syntactic
% constructs. Each syntactic construct is a specific marker getting rid
% of the nondeterminism in {\tname}'s typing rules.

% The construct ``$\eswitch e$'' marks the use of \textbf{switch} rule
% that switches to the unary reasoning whereas the construct ``$\enoch e$'' marks the use of the \textbf{nochange} rule.  The construct
% ``$\esplit(e_1,e_2) \ewith C$'' records the constraint $C$ that is used
% to case analyze the index domain (rule \textbf{r-split}). The
% construct ``$\econtra e$'' is used to make contradiction in the
% constraint domain explicit (rule \textbf{contra}). In addition, we add
% index terms to expressions. For instance, the elimination form for
% universally quantified types in {\tnamemin} is ``$e [I]$'' as opposed
% to {\tname}'s ``$e \eApp$''. The list constructor ``$\econs$'' in
% {\tname} is duplicated in {\tnamemin} as ``$\econsC$'' and
% ``$\econsNC$'' corresponding to the two rule \textbf{r-cons1} and
% \textbf{r-cons2}. The list case construct has two separate branches
% for these two {\econs} cases.
% %
% \[ \begin{array}{@{}l@{~}l@{~}l@{~}l@{}l}
%      \text{Expr.~} & e & \bnfdef & \cdots ~|~ \eswitch e ~|~ \enoch e ~|~ \esplit(e_1,e_2) \ewith C ~|~ \econtra e ~|~\eder e  ~|~ \eLam i. e ~|~ e [I] ~|~ \epack e \ewith I ~|~ \\
%                    &&& \eunpack e_1 \eas (x,i) \ein e_2 
%                        ~|~ \econsNC(e_1,e_2) ~|~ \econsC(e_1,e_2) ~|~
%                        \left(\begin{minipage}[c]{13em}
%                            $\ecase e \eof \enil \, \rightarrow e_1$ \\
%                            $|~h\,::_{NC} tl\, \rightarrow e_2
%                            ~|~h::_{C} tl~ \rightarrow e_3$
%        \end{minipage}\right)
%    \end{array}\]


% \paragraph{{\tnamemin} typing rules}
% Like {\tname}, there are two typing judgments in {\tnamemin}: $\Delta;
% \Phi_a; \Omega \jtypeM{k}{t}{e}{\grt}$ for unary typing and $\Delta;
% \Phi_a; \Gamma \jtypediffM{t}{e_1}{e_2}{\tau}$ for relational
% typing. These two judgments are distinguished from their {\tname}
% counterparts by the superscript $c$ in $:^c$. Selected rules are shown
% in \Cref{fig:relcore-typing-rules}. Most of {\tnamemin}'s unary and
% relational typing rules mimic {\tname}'s. However, there are key
% differences. First, the rules \textbf{nochange}, \textbf{switch},
% \textbf{r-contra}, \textbf{r-split}, \textbf{r-cons1} and
% \textbf{r-cons2} are now syntax-directed. Second, there is no
% relational subtyping in {\tnamemin} ({\tname}'s unary subtyping is
% retained in {\tnamemin}, since it poses no difficulty for
% algorithmization). Instead, there is equivalence checking for
% relational types, written $\pmb{\equiv}$ (rule
% \textbf{c-r-$\equiv$}). Equivalence is a very simple relation. It only
% lifts equality modulo constraints to types (e.g.,
% $\tlist{1+2}{\alpha}{\tau} \pmb{\equiv} \tlist{3}{\alpha}{\tau}$) and
% it can be easily implemented algorithmically (modulo constraint
% solving). Some of its rules are shown in \Cref{fig:type-eq-rules}. In
% particular, equivalence at $\tbox{}$-ed and $U$-annotated types is
% very straightforward (rules \textbf{eq-B-$\tbox{}$} and \textbf{eq-U}
% for $\tbox{}$- and $U$-annotated types, respectively in
% \Cref{fig:type-eq-rules}).

%% except that {\tnamemin}'s expressions are explicitly
%% annotated with syntactic markers. The interesting rules are the ones
%% that deal with the comonadic type $\tbox{\tau}$, shown in
%% Figure~\ref{fig:core-typing-rules}. The rule \textbf{c-der} is the
%% $\square$ elimination rule, corresponding to the subtyping coercion
%% for $\tbox{\tau} \sqsubseteq \tau$ (rule \textbf{T} in
%% Figure~\ref{fig:subtyping-rules}). The introduction form for the
%% comonadic construct $\square$ is the \textbf{c-nochange} rule in which
%% the expressions are explicitly annotated with $\enoch$marker. In
%% comparison to the declarative \textbf{nochange} rule where we insist
%% that $\Gamma(x) \sqsubseteq \tbox{\Gamma(x)}$ for all the variables $x
%% \in dom(\Gamma)$, in \textbf{c-nochange} rule, all the types in the
%% context $\Gamma$ must have $\tbox{}$ at the top-level. The subsumption
%% rule \textbf{r-}$\pmb{\sqsubseteq}$ is also simplified, in {\tname} is
%% simulated by the rule \textbf{c-r-}$\pmb{\equiv}$ in {\tnamemin}.

\paragraph{Simulating relational subtyping with coercions}
Just like what we see in {\relref},
in the course of embedding {\tname} into {\tnamemin}, we replace all occurrences
of relational subtyping with explicit coercion functions in
{\tnamemin}. To do this, we have to show that if $\tau \sqsubseteq
\tau'$ in {\tname}, then there is a coercion function of type $\tau
\rightarrow \tau'$ in {\tnamemin}. % To handle cases with $\tbox{}$, we
% add one additional syntactic construct, $\eder e$, and a corresponding
% typing rule, \textbf{c-der}, to {\tnamemin}
% (\Cref{fig:relcore-typing-rules}). This typing rule corresponds to the
% coercion $\tbox{\tau} \rightarrow \tau$. Using this rule and the
% simple type equivalence $\pmb{\equiv}$, we show that all subtyping
% rules of {\tname} can be realized as coercion functions in
% {\tnamemin}. 
Importantly, the coercion functions have zero relative
cost, so applying the coercions (in place of the subtyping) does not
change the relative costs of the expressions.This time, we will show
some cases in the proof of \Cref{lem:sub-ela}.

%% In the
%% \textbf{c-r-}$\pmb{\equiv}$ rule, instead of the relational subtyping
%% judgment $\tau \sqsubseteq \tau'$, we have the type equivalence
%% judgment $\tau \equiv \tau'$. Since our typing is constraint-based,
%% mere syntactic coercions do not suffice: e.g. syntactic equality would
%% fail to show that $\tlist{1}{0}{\tau}$ is equivalent to
%% $\tlist{1+2}{0}{\tau}$. Instead, we have a constraint-based relational
%% type equality judgment $\Delta; \Phi_a \jeqtype{\tau}{\tau'}$ which is
%% homomorphic equality of relational types, modulo the constraints that
%% require the corresponding index terms to be equal (selected rules
%% shown in in Figure~\ref{fig:type-eq-rules}).

%% Apart from the constraint-based type equivalence, which is trivial to
%% algorithmize, we show that all the relational subtyping rules of
%% {\tname} can be converted to explicit syntactic coercions in
%% {\tnamemin}.
% \begin{figure*}
%   \raggedright
%   \fbox{$\Delta; \Phi_a \jeqtype{\tau_1}{\tau_2}$}~~~checks
%   whether $\tau_1$ is equivalent to $\tau_2$.
%   \begin{mathpar}
%   \etfun
%   \and
%   \etlist
%   \and 
%   \etboxB
%   \and 
%   \etun
% \end{mathpar}
%   \caption{Selected relational type equivalence rules}
%   \label{fig:type-eq-rules}
% \end{figure*}


\begin{lem} [Existence of coercions for relational subtyping] \label{lem:sub-elab}
  If $\Delta; \Phi_a \jsubtype{\tau}{\tau'}$ then there exists
  $\ecoerce{\tau}{\tau'}\!\!\in \mbox{\tnamemin}$ s.t.\ $\Delta; \Phi;
  \cdot
  \jtypediffM{0}{\ecoerce{\tau}{\tau'}}{\ecoerce{\tau}{\tau'}}{\tau
    \tarrd{0} \tau'}$.
\end{lem}

\noindent
We show the coercions for some of the subtyping rules of
Figure~\ref{fig:subtyping-rules} below.
\begin{itemize}
% \item (Rule \textbf{$\to \square \wdiff$}) For
%   $\tau = \tbox{(\tau_1 \tarrd{t} \tau_2)}$ and
%   $\tau' = \tbox{\tau_1} \tarrd{0} \tbox{\tau_2}$,
%   $\ecoerce{\tau}{\tau'} = \elam x. \elam y. \enoch ((\eder x) \eapp
%   (\eder y))$.
%   %% $ \jmintypesame{0}{e}{\tbox{(\tau_1 \tarrd{t} \tau_2)} \to \tbox{\tau_1} \tarrd{0} \tbox{\tau_2}}$ where $e= \elam x. \elam y. \enoch (\eder x) \eapp (\eder y))$ % (for rule $\to\square \wdiff$).
% \item (Rule \textbf{T}) For $\tau = \tbox{\tau'}$,
%   $\ecoerce{\tau}{\tau'} =\elam x. \eder x$.
% \item (Rule \textbf{D}) For $\tau = \tbox{\tau_1}$ and $\tau' = \tbox{\tbox{\tau_1}}$,
%   $\ecoerce{\tau}{\tau'}=\elam x. \enoch x$.
\item (Rule \textbf{l$\square$}) For $\tau = \tlist{n}{\alpha}{\tbox{\tau}}$ and $\tau' =
  \tbox{(\tlist{n}{\alpha}{\tau})}$, $\ecoerce{\tau}{\tau'} = \elam
  x. \mbox{fList} \eapp () \eapp [n] [\alpha] \eapp x$ where
  \mbox{fList} is % equal to
  \begin{nstabbing}
      $\efix \mbox{fList}(\_). \eLam n. \eLam \alpha. \elam x.$ \\
      $\ecase e \eof $\=$\enil \rightarrow \enoch (\mbox{nil})  $\\
      \>$|~h\,::_{N} tl\, \rightarrow \elet r = \mbox{fList} \eapp ()
      \,[n-1] \, [\alpha] \eapp tl$ \\ \>$\ein \enoch (\econsNC(\eder h, \eder r))$ \\
      \>$|~h::_{C} tl\, \rightarrow ~\elet r = \mbox{fList} \eapp () \,
      [n-1] \,[\alpha-1] \eapp tl $ \\ \>$\ein \enoch(\econsC(\eder h, \eder r)).  $ 
    \end{nstabbing}
\item (Rule \textbf{$\to \wexec\wdiff$}) For $\tau = \tcho{(\grt_1 \uarr{k}{t} \grt_2)}$ and $\tau'=
  \tcho{\grt_1} \tarrd{t-k} \tcho{\grt_2}$, $\ecoerce{\tau}{\tau'}=
  \elam x. \elam y. \eswitch (x \eapp y)$.
\item (Rule \textbf{trans}) Transitivity of subtyping corresponds to
  the composition of coercion functions.
\end{itemize}

%The remaining coercions are shown in the appendix.


%% We show respective coercions for several relational subtyping rules in
%% Figure~\ref{fig:subtyping-rules}:
%% \footnote{For readability, we use
%%   ``$\to$'' to stand for ``$\xrightarrow{\wdiff(0)}$''.}

 % The rule \textbf{c-switch} is the
% counterpart of {\tname} rule \textbf{switch} where the additional
% syntactic marker $\eswitch$specifies the switch from the relational to
% the unary typing explicitly.


\begin{figure*}
  \centering
  \begin{mathpar}
    % \mtyswitch 
    % \and
    % \mtyrcons
    % \and
    % \mtyrconsbox
    % \and
    % \mtyrcaseL
    % \and
    \mtyder 
    \and 
    \mtynochange
    % \and
    % \mtyrsubsum
    % \and
    % \mtysubsum
    \and
    \mtyswitch
  \end{mathpar}
  % Definitions at typing-rules-min-defs.tex
  \caption{Selected {\tnamemin} typing rules}
  \label{fig:relcore-typing-rules}
\end{figure*}

 

\begin{figure*}
  \raggedright
  \fbox{$\Delta; \Phi_a; \Gamma
    \jelab{t}{e_1}{e_2}{e_1^*}{e_2^*}{\tau}$} ~ $e_1$ and $e_2$ 
  translate to $e_1^* $ and $ e_1^*$, respectively with relational type
  $\tau$
  and relative cost $t$.\\
  \fbox{$\Delta; \Phi_a; \Omega \jelabun{k}{t}{e}{e^*}{\grt}$} ~ $e$
  translates to $e^*$ with unary type $\grt$ and min.\ and
  max.\ costs $k$ and $t$, respectively.

  \begin{mathpar}
    \elswitch
    \and
    \elnochange
    \and
    \elrsplit
    % \and
    % \elrcaseL
    % \and
    % \elriLam
    % \and
    % \elriApp
    % \and
    % \elrsubsum
  \end{mathpar}
  % Definitions at appendix/elaboration-rules-defs.tex
  \caption{Selected embedding rules}
  \label{fig:elab-rules}
\end{figure*} 

\paragraph{Embedding}
Similar in spirit to {\relinfrefcore}, the embedding of {\tnamemin} transforms a well-typed {\tname} program to a well-typed
{\tnamemin} program and it is defined by induction on {\tname} typing
derivations.The only point to notice is that right now the embedding
also considers the minimum and maximum cost in the unary embedding and
relative cost in the relational embedding.
% The unary embedding judgment of the form  $\Delta; \Phi_a; \Omega
% \jelabun{k}{t}{e}{e^*}{\grt}$ means that the {\tname} expression $e$
% of type $\grt$ with minimum and maximum costs $k$ and $t$,
% respectively, translates to the {\tnamemin} expressions $e^*$ of the
% same type and with the same minimum and maximum costs. In essence, the
% unary embedding is trivial since most of the nondeterminism lies in
% the relational typing. Nonetheless, to have a uniform syntax for
% {\tnamemin}, a unary embedding is necessary to deal with the syntactic
% markers introduced by the surrounding relational expressions
% (e.g.\ the two cons branches in list case analysis). We omit the rules
% of the unary embedding.


% The relational embedding judgment $\Delta; \Phi_a; \Gamma
% \jelab{t}{e_1}{e_2}{e_1^*}{e_2^*}{\tau}$ transforms a pair of
% (related) programs.
% A few selected rules defining the relational
% embedding are shown in \Cref{fig:elab-rules}.
% The rule
% \textbf{e-switch} adds the {\tnamemin} expression construct $\eswitch$to the transformed left and right expressions. The rule
% \textbf{e-nochange} coerces all the free variables in the context
% $\Gamma$ to their $\tbox{}$-ed forms and then adds the expression
% construct $\enoch$\hspace{-0.2em}. The rule \textbf{e-r-split} adds the {\tnamemin}
% expression construct $\esplit$to the transformed left and right
% expressions with the case-analyzed constraint $C$. The rule
% \textbf{e-r-caseL} duplicates the cons case branch in the list-case
% construct (with possibly different instantiations of universally
% quantified variables). 
% The rules \textbf{e-r-iLam} and
% \textbf{e-r-iApp} add the index variable and the index term,
% respectively to the corresponding introduction and elimination forms
% of the universally quantified types. The rule
% \textbf{e-r-$\sqsubseteq$} transforms uses of relational subtyping to
% the application of coercion functions.

%% Elaboration is determined by typing
%% derivations (not by the expressions themselves), therefore it is
%% defined as a type-directed translation. Since we have two typing
%% judgments, elaboration has two corresponding judgments. The unary
%% elaboration judgment
%% $\Delta; \Phi_a; \Omega \jelabun{k}{t}{e}{e^*}{\grt}$ means that $e$
%% translates to $e^*$ with type $\grt$ and minimum and maximum costs $k$
%% and $t$, respectively, whereas the relational elaboration judgment
%% $\Delta; \Phi_a; \Gamma \jelab{t}{e_1}{e_2}{e_1^*}{e_2^*}{\tau}$ means
%% that $e_1$ and $e_2$ translate to $e_1^*$ and $e_2^*$ with type $\tau$
%% and relational cost $t$. 

The embedding also preserves well-typedness and is complete, the
formalized theorems can be found in the appendix.% , as formalized
% in the following theorems.

% \begin{thm} [Types are preserved by embedding]
% \mbox{} \begin{enumerate}
%   \item If $\Delta; \Phi_a; \Omega \jelabun{k}{t}{e}{e^*}{\grt}$, then
%     $\Delta; \Phi_a; \Omega \jtypeM{k}{t}{e^*}{\grt}$ and $\Delta; \Phi_a; \Omega \jtype{k}{t}{e}{\grt}$.
%   \item If
%     $\Delta; \Phi_a; \Gamma \jelab{t}{e_1}{e_2}{e_1^*}{e_2^*}{\tau}$,
%    \\  then $\Delta; \Phi_a; \Gamma \jtypediffM{t}{e_1^*}{e_2^*}{\tau}$ and
%     $\Delta; \Phi_a; \Gamma \jtypediff{t}{e_1}{e_2}{\tau}$.
% \end{enumerate}
% \end{thm}
% %
% \begin{proof}
% By simultaneous induction on the given derivations.
% \end{proof}

% \begin{thm} [Completeness of embedding] \label{thm:relcost-min-completeness}
%   \mbox{}
%   \begin{enumerate}
%   \item If $\Delta; \Phi_a; \Omega \jtype{k}{t}{e}{\grt}$, then there
%     exists an $ e^*$ such that $\Delta; \Phi; \Omega
%     \jelabun{k}{t}{e}{e^*}{\grt}$.
%     \item If $\Delta; \Phi_a; \Gamma \jtypediff{t}{e_1}{e_2}{\tau}$,
%       then there exist $ e_1^*, e_2^*$ such that $\Delta; \Phi_a; \Gamma
%       \jelab{t}{e_1}{e_2}{e_1^*}{e_2^*}{\tau}$.
%   \end{enumerate}
% \end{thm}
% \begin{proof}
% By simultaneous induction on the given {\tname} derivations.
% \end{proof}



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> rel-inf-alg-typing-rules.tex <==


\begin{figure}
  \centering 
  \begin{mathpar}
  %   \relinfalgusub
% \and
%    \relinfalguanno
%  \and
%  \relinfalguif
%  \and
 \inferrule
  {
     \trm{\Gamma}{1}  \infexect{e_1}{\grt_1}{}{}{}{}\\
     \trm{\Gamma}{2}  \infexect{e_2}{\grt_2}{}{}{}{}
  }
  {
    \Gamma  \infdiffT{\eswitch e_1}{\eswitch e_2}{\tch{\grt_1}{\grt_2}}{}{}{}}~\textbf{alg-r-switch$\uparrow$}
   \and
    \inferrule
  {
   \trm{\Gamma}{1}  \chexect{e_1}{\grt_1}{}{}{}\\
   \trm{\Gamma}{2}  \chexect{e_2}{\grt_2}{}{}{}
  }
  {
    \Gamma  \chdiffT{\eswitch e_1}{\eswitch e_2}{\tch{\grt_1}{\grt_2}}{}{}
   }~\textbf{alg-r-switch$\downarrow$}
   %  \and
 % \inferrule{
 %      \Gamma \infdiffT{e}{e'}{\tau'}{}{}{}\\
 %      \jeqtype{\tau'}{\tau} \\
 %    }
 %    { 
 %      \Gamma \chdiffT{e}{e'}{\tau}{}{}
 %    }~\textbf{alg-$\uparrow\downarrow$}
 %    \and
 % \inferrule
 %    {
 %      \Gamma \chdiffT{e}{e'}{\tau}{}{}    
 %    }
 %    {
 %      \Gamma  \infdiffT{(e:\tau)}{(e:\tau)}{\tau}{}{}{}
 %    } ~\textbf{alg-r-anno-$\uparrow$} 
   \end{mathpar}
   \caption{\relinfref algorithmic typing rules}
   \label{fig:rel-inf-alg-typing}
 \end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> rel-inf-binary-subtyping-rules.tex <==


\begin{figure}
  \centering 
  \begin{mathpar}
    \inferrule
{
\strut
}
{
 \jsubtype{\tch{\grt_1 \to \grt_2}{ \grt_1' \to \grt_2'  }  }{ \tch{\grt_1}{\grt_1'}
    \to \tch{\grt_2}{\grt_2'}  }
}~\textbf{$\to \wexec \wdiff$}
    \and
   \inferrule
{
  \jasubtype{\grt_1}{\grt_1'} \\
  \jasubtype{\grt_2}{\grt_2'} 
}
{
 \jsubtype{\tch{\grt_1}{\grt_2}}{\tch{\grt_1'}{
\grt_2'}}
}~\textbf{U}
    \and
    \inferrule{ }
{
 \jsubtype{\tau}{\tch{\trm{\tau}{1}}{\trm{\tau}{2}  }}
}~\textbf{W}
   \end{mathpar}
   \caption{Relational subtyping rules for Relational Information Flow}
   \label{fig:rel-inf-binary-subtyping}
 \end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> rel-inf-ref-alg-unary-typing-rules.tex <==


\begin{figure}
  \centering 
  \begin{mathpar}
   \rrfinfvar
\and
\rrfchfix
\and
\rrfinfapp
\and
\rrfchiLam
\and 
\rrfchcons
\and
\rrfchnil
\and
\rrfchcaseL
\and
\rrfinfanno
\and
\rrfchupdown
% \and
% \rrfchsplit
   \end{mathpar}
   \caption{Unary algorithmic typing rules for RelInfRef}
   \label{fig:rel-inf-ref-alg-unary-typing}
 \end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> rel-inf-ref-binary-subtyping-rules.tex <==


\begin{figure}
  \centering 
  \begin{mathpar}
\inferrule
{
\strut
}
{
 \jsubtype{\tch{\grt_1 \to \grt_2}{ \grt_1' \to \grt_2'  }  }{ \tch{\grt_1}{\grt_1'}
    \to \tch{\grt_2}{\grt_2'}  }
}~\textbf{$\to \wexec \wdiff$}
    \and
   \inferrule
{
  \jasubtype{\grt_1}{\grt_1'} \\
  \jasubtype{\grt_2}{\grt_2'} 
}
{
 \jsubtype{\tch{\grt_1}{\grt_2}}{\tch{\grt_1'}{
\grt_2'}}
}~\textbf{U}
    \and
    \inferrule{ }
{
 \jsubtype{\tau}{\tch{\trm{\tau}{1}}{\trm{\tau}{2}  }}
}~\textbf{W}
% \and
%     \stintU
%     \and
%     \inferrule{   }
%      {
%        \Delta; \Phi_a\jsubtype{\tch{\tsforall{i} \grt}{\tsforall{i}
%            \grt' } }{    
%          \tsforall{i}  \tch{\grt}{\grt'}  }
%      }\textbf{$\forall $ U}
   \end{mathpar}
   \caption{Relational subtyping rules for Relational Information Flow
   Refinement}
   \label{fig:rel-inf-ref-binary-subtyping}
 \end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> rel-inf-unary-subtyping-rules.tex <==


\begin{figure}
  \centering 
  \begin{mathpar}
     \inferrule{
 \jasubtype{\grt_1'}{\grt_1} \\
 \jasubtype{\grt_2}{\grt_2'} \\
}
{
 \jasubtype{\grt_1 \to \grt_2}{\grt_1' \to \grt_2'}
}~\textbf{$\to \wexec$}
\and
   \inferrule
{
}
{ \jasubtype{\grt}{\grt}
}\textbf{u-refl}
\and
\inferrule{
 \jasubtype{\grt_1}{\grt_2} \\
 \jasubtype{\grt_2}{\grt_3}
}
{
 \jasubtype{\grt_1}{\grt_3}
}\textbf{u-tran}
   \end{mathpar}
   \caption{Unary subtyping rules for Relational Information Flow}
   \label{fig:rel-inf-unary-subtyping}
 \end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> rel-inf-unary-typing-rules.tex <==


\begin{figure}
  \centering 
  \begin{mathpar}
\inferrule{\Omega(x) = \grt }{\Omega \jtype{}{}{x}{\grt}}~\textbf{var}
  \and
\inferrule{
    {\ifextra
    \awfty{\grt_1 \to \grt_2}
    \fi} \\
     x: \grt_1, f : \grt_1 \to
    \grt_2, \Omega  \jtype{}{}{e}{\grt_2}}
  {
    \Omega
    \jtype{}{}{ \efix f(x).e}{\grt_1 \to
    \grt_2}
   }~\textbf{fix}
  \and
\inferrule{
  \Omega \jtype{}{}{e_1}{\grt_1\to \grt_2} \\
  \Omega \jtype{}{}{e_2}{\grt_1}}
 {
  \Omega \jtype{}{}{ e_1 \eapp e_2}{
  \grt_2}}~\textbf{app}
\and
    \inferrule{
    \Omega \jtype{}{}{e}{\grt} \\
    \jasubtype{\grt}{\grt'} \\
}{
  \Omega \jtype{}{}{e}{\grt'}
}~{\pmb{\sqsubseteq}\wexec}
   \end{mathpar}
   \caption{Unary typing rules for RelInfU}
   \label{fig:rel-infU-unary-typing}
 \end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> rel-ref-alg-eq-rules.tex <==


\begin{figure}
  \centering 
  \begin{mathpar}
     \relrefalgeqfun
  \and
  \relrefalgeqlista
  \and
\relrefalgeqcprod
\and
 \relrefalgeqforall
   \end{mathpar}
   \caption{Algorithmic equivalence rules for Relational Refinement}
   \label{fig:rel-ref-alg-eq}
 \end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> rel-ref-alg-typing-rules.tex <==

\begin{figure}
  \centering 
  \begin{mathpar}
    \inferrule
  {
    \Delta; { \psi_a}; \Phi_a; \tbox{\Gamma}  \chdifft{e}{e}{\tau}{t'}{\Phi}
  }
  {
    \Delta; \psi_a; \Phi_a; \Gamma', \tbox{\Gamma} \chdifft{\enoch e}{\enoch e}{\tbox{\tau}}{t}{\Phi}
  } ~\textbf{alg-r-nochange-$\downarrow$}
  \and
 %  \inferrule
% {
%   \bctx \infdifft{e_1}{e_2}{\tbox{\tau}}{\psi}{t}{\Phi}
% }
% {
%   \bctx \infdifft{\eder e_1}{\eder e_2}{\tau}{\psi}{t}{\Phi}
% }~\textbf{alg-r-der-$\uparrow$}
% \and
% \inferrule
% {
% \Gamma(x) = \tau
% }
% {
% \bctx \infdifft{x}{x}{\tau}{\emptypsi}{0}{\ctrue}
% } ~\textbf{alg-r-var-$\uparrow$}
%  \and
  \inferrule
{
 \Delta; {\psi_a};  \Phi_a; f : \tau_1 \to \tau_2, x:\tau_1, \Gamma \chdifft{e}{e'}{\tau_2}{t'}{\Phi}
}
{
\bctx \chdifft{\efix f(x).e}{\efix f(x).e'}{\tau_1 \to \tau_2}{t}{\Phi}
} ~\textbf{alg-r-fix-$\downarrow$}
  \and
   \inferrule
{
    % \forall x_i \in \fvars{\efixNC f(x).e}.~ \exists \tau_i. ~\Gamma(x_i) = \tbox{\tau_i}\\
    \Delta; {\psi_a};  \Phi_a; f : \tbox{(\tau_1 \to \tau_2)}, x:\tau_1, \tbox{\Gamma} \chdifft{e}{e'}{\tau_2}{t'}{\Phi}
}
{
\Delta; \psi_a; \Phi_a; \Gamma', \tbox{\Gamma} \chdifft{\efixNC f(x).e}{\efixNC f(x).e}{\tbox{(\tau_1 \to \tau_2)}}{t}{\Phi}
}\\ ~\textbf{alg-r-fix-$\downarrow\square$}
\and
  \inferrule
{
\bctx  \infdifft{e_1}{e_1'}{\tau_1 \to \tau_2}{\psi}{t_1}{\Phi_1} \\
\Delta; {\psi_a}; \Phi_a; \Gamma \chdifft{e_2}{e_2'}{\tau_1}{t_2}{\Phi_2}
}
{
\bctx  \infdifft{e_1 \eapp e_2}{e_1' \eapp e_2'}{\tau_2}{\psi}{t_1+t_2+t_e}{\cand{\Phi_1}{\Phi_2}}
}~\textbf{alg-r-app-$\uparrow$}
%   \and
% \inferrule
% {
% \Delta, \psi_a; \Phi \wfty{\tau}
% }
% {
% \bctx  \chdifft{\enil}{\enil}{\tlist{n}{\alpha}{\tau}}{t}{\ceq{n}{0}}
% }~\textbf{alg-r-nil-$\downarrow$}
%   \and
%    \inferrule
% {
% \freshSize{i,\beta} \\
% \Delta; {\psi_a}; \Phi_a; \Gamma  \chdifft{e_1}{e_1'}{\tau}{t_1}{\Phi_1} \\
% \Delta; {i,\beta,\psi_a}; \Phi_a; \Gamma
% \chdifft{e_2}{e_2'}{\tlist{i}{\beta}{\tau}}{t_2}{\Phi_2}\\
% \Phi_2' = \cand{\ceq{n}{(i+1)}}{\cexists{\beta}{\ssize}{\cand{\Phi_2}{\ceq{\alpha}{\beta+1}}}}
% }
% {
%   \bctx \chdifft{\econsC(e_1,e_2)}{\econsC(e_1',e_2')}{\tlist{n}{\alpha}{\tau}}{t}{\cand{\Phi_1}{\cexists{i}{\ssize}{\Phi_2'}}}
% }~\textbf{alg-r-consC-$\downarrow$}
%   \and
%   \inferrule
% {
% \freshSize{i} \\
% \Delta; {\psi_a}; \Phi_a; \Gamma  \chdifft{e_1}{e_1'}{\tbox{\tau}}{t_1}{\Phi_1} \\
% \Delta; {i,\psi_a}; \Phi_a; \Gamma
% \chdifft{e_2}{e_2'}{\tlist{i}{\alpha}{\tau}}{t_2}{\Phi_2}\\
% \Phi_2' = \cand{\Phi_2}{\ceq{n}{(i+1)}}
% }
% {
% \bctx \chdifft{\econsNC(e_1,e_2)}{\econsNC(e_1',e_2')}{\tlist{n}{\alpha}{\tau}}{t}{\cand{\Phi_1}{\cexists{i}{\ssize}{\Phi_2'}}}
% }~\textbf{alg-r-consNC-$\downarrow$}
  \end{mathpar}
 \caption{Algorithmic typing rules for Relational Refinement}
\label{fig:rel-ref-alg-typing}
\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> rel-ref-core-rules.tex <==

\begin{figure}
  \centering 
  \begin{mathpar}
    \inferrule{
       {\ifextra
       \Delta; \Phi_a \wfty{\tau_1 \to \tau_2}
       \fi} \\
       \Delta; \Phi_a;  x: \tau_1, f : \tau_1 \to \tau_2, \Gamma  \jstypet{e_1}{e_2}{\tau_2}}
            {\ctx \jstypet{ \efix f(x).e_1}{\efix f(x).e_2}{
              \tau_1 \to \tau_2}}~\textbf{c-r-fix}
   \and
\inferrule
  {
    {\ifextra \Delta; \Phi_a \wfty{\tau_1 \to \tau_2}
      \fi} \\
    \Delta; \Phi_a;  x: \tau_1, f : \tbox{(\tau_1 \to \tau_2)}, \tbox{\Gamma} \jstypet{e}{e}{\tau_2}
  }
  {\nctx,\Gamma' \jstypet{\efixNC f(x).e}{\efixNC f(x).e}{
              \tbox{(\tau_1 \to \tau_2)}}}\\~\textbf{c-r-fixNC}
  \and
     \inferrule
  { \ctx \jstypet{e_1}{e_1'}{\tau} \\
    \ctx \jstypet{e_2}{e_2'}{\tlist{n}{\alpha}{\tau}}
  }
  { \ctx \jstypet{ \econsC(e_1,e_2) }{ \econsC(e_1',e_2')}{\tlist{n+1}{\alpha+1}{\tau}}}\\~\textbf{c-r-cons1}
    \and
   \inferrule
  { \ctx \jstypet{e_1}{e_1'}{\tbox{\tau}} \\
    \ctx \jstypet{e_2}{e_2'}{\tlist{n}{\alpha}{\tau}}}
  { \ctx \jstypet{ \econsNC(e_1,e_2) }{
      \econsNC(e_1',e_2')}{\tlist{n+1}{\alpha}{\tau}}}\\~\textbf{c-r-cons2}
\and
    \inferrule
{
\Delta; \Phi_a; \Gamma  \jstypet{e_1}{e_2}{\tbox{\tau}}
}
{
\Delta; \Phi_a; \Gamma  \jstypet{\eder e_1}{\eder e_2}{\tau}
} ~\textbf{c-der}
    \and 
    \inferrule
{
\Delta; \Phi_a; \tbox{\Gamma} \jstypet{e}{e}{\tau}
}
{
\Delta; \Phi_a; \tbox{\Gamma}, \Gamma' \jstypet{\enoch e}{\enoch e}{\tbox{\tau}}
} ~\textbf{c-nochange}
\and
    \inferrule{
     \ctx \jstypet{e}{e'}{\tau}\\
     \Delta; \Phi_a \jeqtype{\tau}{\tau'} 
  }
  {\ctx \jstypet{e}{e'}{\tau'} }
  ~{\textbf{c-r-$\equiv$}}
    \and
    \inferrule
  {
    \Delta; \Phi_a \wedge C; \Gamma \jstypet{e_1}{e_2}{\tau}\\
    \Delta; \Phi_a \wedge \neg C; \Gamma \jstypet{e_1'}{e_2'}{\tau}\\
  }
  {
    \ctx \jstypet{\esplit (e_1,e_1') \ewith C}{\esplit
      (e_2,e_2') \ewith C}{\tau} }\\ ~\textbf{c-r-split}
  \end{mathpar}
 \caption{Typing rules for Relational Refinement Core}
\label{fig:rel-ref-core-typing}
\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> rel-ref-embed-rules.tex <==

\begin{figure}
  \centering 
  \begin{mathpar}
\relrefembedfix
    \and
\relrefembedfixnc
       \and
\relrefembedconsOne
  \and
\relrefembedconsTwo
\and
\relrefembedsplit
  \end{mathpar}
 \caption{Embedding rules for Relational Refinement}
\label{fig:rel-ref-embed-typing}
\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> rel-ref-eq-rules.tex <==

\begin{figure}
  \centering 
  \begin{mathpar}
   \relrefeqfun
  \and
  \relrefeqlist
\and
\relrefeqcimpl
\and
\relrefeqforall
  \end{mathpar}
 \caption{Equivalence rules for Relational Refinement Core}
\label{fig:rel-ref-eq-typing}
\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> rel-ref-subtyping-rules.tex <==


\begin{figure}
  \centering 
  \begin{mathpar}
     \inferrule{
     }
     {
       \jsubtype{\square (\tau_1 \to \tau_2)}{ \square \tau_1 \to
         \square \tau_2}
     }\textbf{$\to\square$diff}
     \and
  \stlist
  %
\and
%
\stlistzero
\and
%
\stlistbox
\and
\stbox
%
\and
%\stboxD
%\and
%
\stboxB

\stcprod

   \end{mathpar}
   \caption{Subtyping rules for Relational Refinement}
   \label{fig:rel-ref-subtyping}
 \end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> rel-ref-typing-rules.tex <==

\begin{figure}
  \centering 
  \begin{mathpar}
    
      \inferrule
{
\Delta; \Phi_a; \Gamma \jstype{e}{e}{\tau}~~\\\\
\forall x \in dom(\Gamma).~~
\Delta; \Phi_a  \jsubtype{\Gamma(x)}{\tbox{\Gamma(x)}} ~~
}
{
\Delta; \Phi_a; \Gamma,\Gamma' \jstype{e}{e}{\tbox{\tau}}
} ~\textbf{rr-nochange}

\and
\inferrule{
    \ctx \jstype{e_1}{e_2}{\tau}~~\\
    \Delta; \Phi_a \jsubtype{\tau}{\tau'}~~ 
  }
  {\ctx \jstype{e_1}{e_2}{\tau'}
  }~{\textbf{rr-}\pmb{\sqsubseteq}}

  % \and
  %   \inferrule{
  %      \Delta; \Phi_a;  x: \tau_1, f : \tau_1 \to \tau_2, \Gamma   \jstype{e_1}{e_2}{\tau_2}
  %    }
  %    {\ctx \jstype{ \efix f(x).e_1}{\efix f(x).e_2}{
  %               \tau_1 \to \tau_2}}~\textbf{rr-fix}
\and
     \inferrule
  {
    {\ifextra \Delta; \Phi_a \wfty{\tau_1 \to \tau_2}
      \fi} \\
    \Delta; \Phi_a;  x: \tau_1, f : \tbox{(\tau_1 \to \tau_2)}, \Gamma \jstype{e}{e}{\tau_2}~~\\
    \forall x \in dom(\Gamma).~~
    \Delta; \Phi_a  \jsubtype{\Gamma(x)}{\tbox{\Gamma(x)}}
  }
  {\ctx \jstype{ \efix f(x).e}{\efix f(x).e}{
              \tbox{(\tau_1 \to \tau_2)}}}~\textbf{rr-fixNC}
    \and
\inferrule
  { \ctx \jstype{e_1}{e_1'}{\tau} \\
    \ctx \jstype{e_2}{e_2'}{\tlist{n}{\alpha}{\tau}}
  }
  { \ctx \jstype{ \econs(e_1,e_2) }{ \econs(e_1',e_2')}{\tlist{n+1}{\alpha+1}{\tau}}}~\textbf{rr-cons1}
\and
 \inferrule
  { \ctx \jstype{e_1}{e_1'}{\tbox{\tau}} \\
    \ctx \jstype{e_2}{e_2'}{\tlist{n}{\alpha}{\tau}}}
  { \ctx \jstype{ \econs(e_1,e_2) }{
      \econs(e_1',e_2')}{\tlist{n+1}{\alpha}{\tau}}}~\textbf{rr-cons2}
\and
\inferrule
  {
    \Delta; \Phi_a \wedge C; \Gamma  \jstype{e_1}{e_2}{\tau}\\
    \Delta; \Phi_a \wedge \neg C; \Gamma  \jstype{e_1}{e_2}{\tau}\\
    \Delta \wfcs{C}
  }
  {
    \ctx  \jstype{e_1}{e_2}{\tau} } ~\textbf{rr-split}
\and
\inferrule
{
\Delta; \Phi_a \sat \bot \\
  \Delta; \Phi_a \wfty{\Gamma}
}
{
  \ctx \jstype{e_1}{e_2}{\tau}
} ~\textbf{rr-contra}
%               \and
% \inferrule{
%     i::S, \ctx \jstype{e}{e'}{\tau}~~ \\\\
%     i \not \in \fiv{\Phi_a; \Gamma}
%   }
%   { \ctx \jstype{\eLam e}{\eLam e'}{\tsforall{i} \tau }}~\textbf{rr-iLam}

% \and
%  \inferrule{
%     \ctx \jstype{e}{e'}{\tsforall{i} \tau } ~~\\\\
%     \Delta \vdash I : S ~~
%   }
%   {\ctx \jstype{e \eApp}{e' \eApp}{\tau\{ I/
%       i\}}}~\textbf{rr-iApp}
% \and
%       \inferrule
% {
%   \Delta; \Phi_a \wedge C; \Gamma \jstype{e}{e'}{\tau}
% }
% {
%   \ctx  \jstype{e}{e'}{\tcimpl{C}{\tau}}
% } ~\textbf{rr-c-impII}
% \and
% \inferrule
% {
%   \ctx \jstype{e_1}{e_1 '}{\tcimpl{C}{\tau}}\\
%   \Delta; \Phi_a \vDash C
% }
% {
%   \ctx  \jstype{\ecelim e }{\ecelim e' }{\tau}
% } ~\textbf{rr-c-implE}
  \end{mathpar}
 \caption{Relational Refinement typing rules}
\label{fig:rel-ref-typing}
\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> rel-stlc-alg-subtyping-rules.tex <==


\begin{figure}
  \centering 
  \begin{mathpar}
    \inferrule{
    }
    {
      \jalgssubtype{\trbool}{\trbool}
    }~\textbf{alg-bl-r}
    \and
    \inferrule{
    }
    {
      \jalgssubtype{\tubool}{\tubool}
    }~\textbf{alg-bl-u}
    \and
    \inferrule{~\textbf{alg-bl}
    }
    {
      \jalgssubtype{\trbool}{\tubool}
    }
    \and
     \inferrule{
       \jalgssubtype{\tau_1'}{\tau_1} \\
       \jalgssubtype{\tau_2}{\tau_2'}
     }
     {
       \jalgssubtype{\tau_1 \to \tau_2}{\tau_1' \to \tau_2'}
     }~\textbf{alg-$\to$}
   \end{mathpar}
   \caption{Algorithmic subtyping rules for Relational STLC}
   \label{fig:rel-stlc-alg-subtyping}
 \end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> rel-stlc-alg-typing-rules.tex <==

\begin{figure}
  \centering 
  \begin{mathpar}
    \inferrule
    {\Gamma(x) = \tau } 
    { \Gamma \infsdiff{x}{x}{\tau}}~\textbf{alg-r-var}
    \and
    \inferrule
    { \kw{b}  \in \{\etrue, \efalse \}}  
    { \Gamma \infsdiff{\kw{b}}{\kw{b}}{\trbool}}~\textbf{alg-r-bool}
    \and
    \inferrule
    { \kw{b_1, b_2}  \in \{\etrue, \efalse \}  \\
    b_1 \not = b_2 }
    { \Gamma \chsdiff{\kw{b_1}}{\kw{b_2}}{\tubool}}~\textbf{alg-r-u-bool}
    \and
    \inferrule{\Gamma \infsdiff{e}{e'}{\trbool} \\
      \Gamma \chsdiff{ e_1}{e_1'}{\tau} \\
      \Gamma \chsdiff{ e_2}{e_2'}{\tau}
    }
    {\Gamma \chsdiff{\eif e \ethen e_1 \eelse e_2}{\eif e' \ethen e_1' \eelse e_2'}{\tau}}~\textbf{alg-r-if}
    \and
    \inferrule{
       \Gamma, x: \tau_1  \chsdiff{e_1}{e_2}{\tau_2}
     }
     {\Gamma \chsdiff{ \elam x.e_1}{\elam x.e_2}{
                \tau_1 \to \tau_2}}~\textbf{alg-r-fix}
    \and
    \inferrule{
      \Gamma \infsdiff{e_1}{e_1'}{\tau_1
        \to \tau_2} \\
      \Gamma \chsdiff{ e_2}{e_2'}{\tau_1}}
    {\Gamma \infsdiff{e_1 \eapp e_2}{e_1' \eapp e_2'}{\tau_2}}~\textbf{alg-r-app}
    \and
    \inferrule{
      \Gamma \infsdiff{e}{e'}{\tau'}\\
      \jalgssubtype{\tau'}{\tau} \\
    }
    { 
      \Gamma \chsdiff{e}{e'}{\tau}
    }~\textbf{alg-$\uparrow\downarrow$}
    \and
    \inferrule
    {
      \Gamma \chsdiff{e}{e'}{\tau}    
    }
    {
      \Gamma  \infsdiff{(e:\tau)}{(e:\tau)}{\tau}
    } ~\textbf{alg-r-anno-$\uparrow$} 
  \end{mathpar}
 \caption{Algorithmic typing rules for Relational STLC}
\label{fig:rel-stlc-alg-typing}
\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> rel-stlc-subtyping-rules.tex <==


\begin{figure}
  \centering 
  \begin{mathpar}
    \inferrule{
    }
    {
      \jsubtype{\trbool}{\tubool}
    }~\textbf{bool}
    \and
     \inferrule{
       \jsubtype{\tau_1'}{\tau_1} \\
       \jsubtype{\tau_2}{\tau_2'}
     }
     {
       \jsubtype{\tau_1 \to \tau_2}{\tau_1' \to \tau_2'}
     }~\textbf{$\to$}
     \and
     \inferrule
     {
     }
     {  \jsubtype{\tau}{\tau}
     }\textbf{refl}
     \and
     \inferrule{
       \jsubtype{\tau_1}{\tau_2} \\
       \jsubtype{\tau_2}{\tau_3}
     }
     {
       \jsubtype{\tau_1}{\tau_3}
     }\textbf{trans}
   \end{mathpar}
   \caption{Subtyping rules for Relational STLC}
   \label{fig:rel-stlc-subtyping}
 \end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> rel-stlc-typing-rules.tex <==

\begin{figure}
  \centering 
  \begin{mathpar}
    \inferrule
    {\Gamma(x) = \tau } 
    { \Gamma \jstype{x}{x}{\tau}}~\textbf{r-var}
    \and
    \inferrule
    { \kw{b}  \in \{\etrue, \efalse \}}  
    { \Gamma \jstype{\kw{b}}{\kw{b}}{\trbool}}~\textbf{r-bool}
    \and
    \inferrule
    { \kw{b_1, b_2}  \in \{\etrue, \efalse \}}  
    { \Gamma \jstype{\kw{b_1}}{\kw{b_2}}{\tubool}}~\textbf{r-u-bool}
    \and
    \inferrule{\Gamma \jstype{e}{e'}{\trbool} \\
      \Gamma \jstype{ e_1}{e_1'}{\tau} \\
      \Gamma \jstype{ e_2}{e_2'}{\tau}
    }
    {\Gamma \jstype{\eif e \ethen e_1 \eelse e_2}{\eif e' \ethen e_1' \eelse e_2'}{\tau}}~\textbf{r-if}
    \and
    \inferrule{
       \Gamma,  x: \tau_1 \jstype{e_1}{e_2}{\tau_2}
     }
     {\Gamma \jstype{ \elam x.e_1}{\elam x.e_2}{
                \tau_1 \to \tau_2}}~\textbf{r-fix}
    \and
    \inferrule{\Gamma \jstype{e_1}{e_1'}{\tau_1}
      \to \tau_2 \\
      \Gamma \jstype{ e_2}{e_2'}{\tau_1}}
    {\Gamma \jstype{e_1 \eapp e_2}{e_1' \eapp
        e_2'}{\tau_2}}~\textbf{r-app}
\and 
\rstlcsub
  \end{mathpar}
 \caption{Relational STLC typing rules}
\label{fig:rel-stlc-typing}
\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> relcost-overview.tex <==
\section{RelCost}
\label{sec:relcost}


% \paragraph{Relational cost analysis}
% As mentioned before, the goal of relational cost analysis is to derive an upper bound on
% the \emph{difference} in the execution costs of two programs, say
% $e_1$ and $e_2$. This difference, i.e.\ $cost(e_1) - cost(e_2)$, is
% also called the \emph{relative cost} of $e_1$ with respect to
% $e_2$.
% When $e_1$ and $e_2$ have the forms $f \eapp e_1'$ and
% $f \eapp e_2'$, the same analysis can be used to determine how the
% cost of a function $f$ varies with the argument. Relational cost
% analysis is relevant in many settings: to show that a compiler
% optimization reduces the execution cost; in preventing timing
% side-channel attacks, by showing that two runs of a function with
% different secret inputs have zero relative cost; in approximate
% computing, to show that the approximate version of the program is
% faster than the more accurate one, etc. 


% A naive way to statically establish this relative cost is to do
% separate non-relational (unary) cost analyses to obtain $e_1$'s
% worst-case cost and $e_2$'s best-case cost. The relative cost of $e_1$
% w.r.t.\ $e_2$ is then upper-bounded by the difference of these two.
% However, as described in ~\cite{Cicek:2017}, this is often imprecise,
% tedious or even impossible since it does not exploit the similarities
% between $e_1$ and $e_2$ or their inputs.

%% when the two programs (or
%% their inputs) are closely related, it is often imprecise, tedious or
%% even impossible to do such a naive cost analysis. Yet, a direct
%% relational cost analysis, that exploits the similarities in the
%% structures of $e_1$ and $e_2$ may be more feasible and precise.


By adding effects to the refinement type system {\relinfref}, we can
easily get {\tname}. Intuitively, the
algorithmization of {\tname} is not far. We first look at {\tname}'s syntax and type system.


\subsection{Types and Syntax}
Precise relational cost analysis requires understanding which
expressions and values may be related. %  {\tname}'s types (shown in
% Figure~\ref{fig:type-syntax}) make this explicit by syntactically (as
% well as semantically) separating the relational types $\tau$ from the
% non-relational ones $\grt$: the former represent a pair of
% \textit{related} values (expressions), capturing the similarities
% between them, whereas the latter represent individual values
% (expressions). Both types include standard base types (like $\tint$
% and $\tunit$, and their relational counterparts $\trint$ and
% $\trunit$) and
We get the syntax of {\tname} by extension of standard type constructors $\ttimes$ and $\tsum$ for
products and sums as well as embedding cost into type syntax. % Any non-relational type $\grt$ can be trivially
% made relational by encapsulating it within the weakest relation using
% the $\tcho{\cdot}$ modality. For instance, the type $(\tcho{\tint})$
% represents a pair of unrelated integers whereas the type $\trint$
% represents a pair of identical integers.
One thing to pay attention is that relative cost is often a function of the length of an input list or
the number of elements that differ between two lists. % Therefore, unary
% list types in {\tname} are \emph{refined} to $\ulist{n}{\grt}$, where
% $n$ specifies the exact length of the list. Relational list types are
% refined to $\tlist{n}{\alpha}{\tau}$, where $n$ specifies the lengths
% of the two related list and $\alpha$ specifies the maximum number of
% elements that are allowed to differ between the two related
% lists.
\footnote{Note that $n$ in $\ulist{n}{\grt}$ is a unary
  refinement whereas the $n$ and $\alpha$ in $\tlist{n}{\alpha}{\tau}$
  are relational refinements, relating a pair of list values.} % To
% statically deal with the remaining $n-\alpha$ elements that are not
% allowed to differ between the two lists, {\tname} introduces the
% comonadic type $\tbox{\tau}$, representing the (strongest) diagonal
% relation that relates only syntactically equal values
% (expressions). The type $\tlist{n}{\alpha}{\tau}$ is interpreted such
% that at most $\alpha$ elements of the two lists are of type $\tau$ and
% at least $n-\alpha$ elements are of type $\tbox{\tau}$,
% i.e.\ identical. 
% Additionally, the type constructor $\tbox{}$ interacts with other
% type constructors in nontrivial ways. For example, $(\trint \tsum
% \tcho{\tint})$ contains pairs of tagged values with the same tag but
% whose content can differ if the tag is $\mbox{inr}$. The stronger type
% $\tbox{(\trint \tsum \tcho{\tint})}$ forces both values to be
% syntactically equal and is, in fact, semantically equal to $(\trint
% \tsum \trint)$. Technically, $\tbox{}$ is a constructive S4
% necessitation modality, but with a relational interpretation.


\paragraph{{\tname} syntax} Let us look at how {\relinfref}
is extended to {\tname}. First, worst-/best-case execution costs and relative costs are treated as
unary and relational \emph{effects}, respectively. Then, function types are
annotated with the costs of their bodies. The relational type $\tau_1
\tarrd{t} \tau_2$ ascribes a pair of related functions, whose bodies'
relative cost is upper-bounded by $t$, while the unary type $\grt_1
\uarr{k}{t} \grt_2$ ascribes a single function whose body's cost is
lower- and upper-bounded by $k$ and $t$ respectively. Similar cost
annotations are written on universally quantified types. 

% Finally, to represent arithmetic relations between parameters like $n,
% \alpha, t$ and $k$, {\tname} includes \emph{constraints}, denoted
% $C$. The constrained type $\tcprod{C}{\grt}$ means that $C$ holds and
% the type is $\grt$. $\tcprod{C}{\tau}$ is defined similarly. For
% instance, $(\tcprod{(\cleq{1}{n})}{\ulist{n}{\grt}})$ specifies
% non-empty lists. Constraints are drawn from a rich language of
% predicates.


% The syntax of {\tname}'s expressions is
% similar as the ones except \wq{To DO} .
% shown in Figure~\ref{fig:terms}. The language is standard
% call-by-value and includes the usual introduction and elimination
% forms for {\tname}'s types.
% The construct ``$\zeta e$'' corresponds to the
% application of a primitive function $\zeta$. 
% The construct
% ``$\clet e_1 \eas x \ein e_2$'' is the elimination form for the
% constrained type $\tcprod{C}{\tau}$ and the constructs ``$\epack e$''
% and ``$\eunpack e_1 \eas x \ein e_2$'' are the introduction and
% elimination forms for existentially quantified types. The constructs
% ``$\eLam. e$'' and ``$e \eApp$'' are the introduction and elimination
% forms for universally quantified types. By design, index terms do not
% appear in {\tname} expressions. 

Let us look at the example map again and this time, we consider cost.
\begin{nstabbing}
 $\efix \kw{map}(f).\elam l. \ecase l $\=$\eof \enil \rightarrow \enil$ \\
\>$ |~ h :: tl \rightarrow \econs(f \eapp h, \eapp \kw{map} \eapp f \eapp tl) $
\end{nstabbing}
Assume that $f$ has the relational type $\tbox{(\tau_1 \tarrd{t}
  \tau_2)}$, meaning that in any two runs of $\kw{map}$, $f$ will be
the same (outer $\tbox{}$) and that $f$'s body has relative cost
$t$. % What can we say about the \textit{relative cost} of two runs of
% $\kw{map}$ given two input lists related at type
% $\tlist{n}{\alpha}{\tau_1}$ (i.e., two lists that differ in at most
% $\alpha$ positions)?
Since we know that $f$ itself does not change
across the two executions, at most $\alpha$ applications of $f$ may
differ in the two executions, while at least $n-\alpha$ applications
must be identical. Hence, the relative cost of the two runs of
$\kw{map}$ will be bounded by $\alpha \cdot t$. Moreover, we can show
that the output lists will differ in at most $\alpha$
positions. Therefore, $\kw{map}$ can be given the following relational
type:\footnote{When a cost annotation is missing from an $\to$ or a $\forall$, it is
  implicitly assumed to be $0$.}
\begin{equation*}
\forall t.(\tbox{(\tau_1 \tarrd{t} \tau_2)}) \to \forall
  n,\alpha. \tlist{n}{\alpha}{\tau_1} \tarrd{t \cdot \alpha}
  \tlist{n}{\alpha}{\tau_2}\label{eq:1}
\end{equation*}
% Next, we briefly explain how this type is derived in {\tname} as this
% highlights several key rules of the type system. The typing proceeds
% by induction on $l$. The interesting part is establishing the relative
% cost for the cons branch in the definition of $\kw{map}$. We have to
% establish an upper bound of $\alpha \cdot t$ for the branch. From the
% type of $l$, we know that at most $\alpha$ elements in $h::tl$ may
% differ in the two runs. However, we do not know statically whether $h$
% (the current head) is among those elements. Therefore, {\tname}'s
% \textbf{r-caseL} types the $\kw{cons}$ branch twice: once assuming
% that $h$ will not differ in the two runs and then assuming that $h$
% may differ. We explain the analysis of these two cases.

% We start from the second case where $h$ may differ, i.e. $h: \tau_1$
% and $tl:\tlist{n-1}{\alpha-1}{\tau_1}$ (note the $\alpha-1$ in the
% tail's type). The expression $f\eapp h$ can be shown to have relative
% cost $\alpha$ by first supertyping $f$ from $\tbox{(\tau_1 \tarrd{t}
%   \tau_2)}$ to $\tau_1 \tarrd{t} \tau_2$ (using the subtyping rule
% \textbf{T} of Figure~\ref{fig:subtyping-rules}) and then applying the
% rule \textbf{r-app}. The recursive call $(\kw{map}\eapp f \eapp tl)$
% has cost $(\alpha-1)\cdot t$, inductively. When added, these two yield
% exactly $\alpha \cdot t$, as required.

%% (Technically, we use rule
%% \textbf{r-cons1} of Figure~\ref{fig:synch-rel-typing-rules}.)

% The analysis of the first case, where $h$ may not differ, is more
% interesting. Here, \textbf{r-caseL} provides us that $h:
% \tbox{\tau_1}$ (the $\tbox{}$ indicates that the head is the same in
% the two runs) and $tl:\tlist{n-1}{\alpha}{\tau_1}$ (note the $\alpha$
% in the tail's type). In this case, the inductive cost of
% $(\kw{map}\eapp f \eapp tl)$ is already $\alpha \cdot t$. Hence, we
% must show that $f\eapp h$ has a relative cost of $0$. This can be
% established in two ways: a) By using the subtyping rule $\to \square
% \wdiff$ of Figure~\ref{fig:subtyping-rules}, we can supertype $f$ to
% $\tbox{\tau_1} \tarrd{0} \tbox{\tau_2}$, and then apply it to get a
% relative cost of $0$ or, b) We can use a special reasoning principle:
% If all free variables of an expression have $\tbox{}$-annotated types,
% then the cost of the expression relative to itself is $0$. The
% assumption that all free variables be $\tbox{}$-annotated is
% important; without it, the substituted expression that is actually
% executed may differ in the two runs and the relative cost may not be
% zero. Here, since both free variables, $f, h$ in $f \eapp h$ are
% $\tbox{}$-annotated, we can derive a relative cost of $0$ for $f
% \eapp h$. Technically, the typing rule that embodies this special
% reasoning principle is called \textbf{nochange}.

%% In either case, the analysis is officially completed using
%% the rule \textbf{r-cons2}.


Note that if we were to do a naive analysis by computing the
difference of the worst- and best-case execution costs of $\kw{map}$,
we could only obtain a bound linear in $n$, not in $\alpha$. Thus,
relational analysis in {\tname} improves the precision of reasoning
about relative cost.




% The two modes of the type system are reflected at the type
% level: {\tname} has unary types and relational types. The type
% grammar is shown in Figure~\ref{fig:type-syntax}. Unary types include
% standard basic types as $\tunit$ and $\tint$, standard type
% constructors $\ttimes, \tsum$ for products and sums, and sized lists
% $\tlist{I}{}{\tau}$. Unary types also contains cost annotated functions types of the form
% $\grt_1 \uarr{k}{t} \grt_2$ where $k$ and $t$ are index terms
% expressing worst and best cost bounds. Similar annotation appear on
% universally quantified types such as $\tforall{i}{k}{t} \grt$ where
% $i$ is an index term variable and $S$ is it's sort. Finally, unary types contain existentially
% quantified types of the form $\texists{i} \grt$, and types with constraints of the form
% $\tcprod{C}{\grt}$.

% Relational types are defined by a grammar similar to the one for unary types
% but they are used to type two expressions rather than one like in the
% case of unary types. So, the meaning of relational types is
% different. Relational types include relational basic types as
% $\trunit$ and $\trint$, which can be used to type two expressions that will
% evaluate to the same value of type $\tunit$ or $\tint$, and relational
% type constructors for sum and product. Lists
% $\tlist{I}{\alpha}{\tau}$ are additionally indexed by an index
% term $\alpha$ expressing the number of elements that can differ in the
% two lists.
% Function types and universally quantified types are annotated with a
% cost expressing the differential cost between two expressions while
% existential types and types with constraints have the same syntax as
% their unary counterpart. Additionally, relational types include a
% modality $\tcho{}$ representing the weakest relation that relates
% every two expressions of the underlying unary type. Moreover, they include a
% modality $\tbox{}$ representing the diagonal relation that relates
% expressions evaluating to the same value of the underlying 
% type. 





% \begin{figure}
%   \centering
% \[
% \begin{array}{ll}
%  \label{fig:syntax}
%   \mbox{U types} \
%   \grt  ::= & \tunit ~|~ \tint ~|~ \grt_1 \ttimes \grt_2 ~|~  \grt_1 \tsum \grt_2
%   ~|~ \ulist{I}{\grt} \\ & ~|~ \grt_1 \uarr{k}{t} \grt_2
%   ~|~ \tforall{i}{k}{t} \grt \\ &
%   ~|~  \texists{i} \grt ~|~\tcprod{C}{\grt}  % ~|~ \tcimpl{C}{\grt} 
%   \\[2mm]
%   \mbox{R types} 
% \   \tau  ::= & \trunit ~|~ \trint ~|~ \tau_1 \ttimes \tau_2 ~|~  \tau_1 \tsum \tau_2
%   ~|~ \tlist{I}{\alpha}{\tau} \\ & ~|~ \tau_1 \tarrd{t} \tau_2 
%   ~|~ \tforalld{i}{t} \tau
%  ~|~ \texists{i} \tau \\ &  ~|~ \tcprod{C}{\tau}  % \tcimpl{C}{\tau} ~|~ 
%          % \tch{\grt_1}{\grt_2}
%         \tcho{\grt} ~|~ \tbox{\tau} 
% %
%  \\[2mm]

% \mbox{Sorts}
%  \  \sort  \bnfdef &
% \ssize \bnfalt
% \scost 
% \\[2mm]

% \mbox{Idx terms} 
%  \ I, k,  \bnfdef & 
% i \bnfalt
% \szero \bnfalt 
% \sinf \bnfalt
% \splusone{I} \bnfalt
% \splus{I_1}{I_2} \bnfalt
% \sminus{I_1}{I_2} \bnfalt
% \sdiv{I_1}{I_2} \bnfalt \\ &
% \smult{I_1}{I_2} \bnfalt
% \sceil{I} \bnfalt
% \sfloor{I} \bnfalt
%  \\ 
%  \hspace{.8cm}   t, \alpha   \bnfdef  &
% \slog{I} \bnfalt
% \spower{I_1}{I_2} \bnfalt
% \ssum{i}{I_1}{I_n}{I} \bnfalt
% \smin{I_1}{I_2} \bnfalt
% \smax{I_1}{I_2} 

% \\[2mm]


% \mbox{Constr}
% \  C  \bnfdef &
% \ceq{I_1}{I_2} \bnfalt
% \clt{I_1}{I_2} \bnfalt
% \cneg{C} 
% \\[2mm]

% \mbox{Constr env.}
%  \ \Phi  \bnfdef &
% \ctrue \bnfalt
% \cand{C}{\Phi}
% \\
% \\[2mm]

% \mbox{Sort env.}
%  \ \Delta  \bnfdef &
% \emptyset \bnfalt
% \Delta, i :: S 

% \\[2mm]
% \mbox{U type env.}
%  \ \Omega  \bnfdef &
% \emptyset \bnfalt
% \Omega, x : {\grt} 
% \\[2mm]

% \mbox{R type env.}
%  \ \Gamma  \bnfdef &
% \emptyset \bnfalt
% \Gamma, x : {\tau} 
% %% \\[2mm]

% %% \mbox{Primitive env.}
% %% & \primctx & \bnfdef &
% %% \emptyset \bnfalt
% %% \primctx, \zeta: \tau_1 \tarrd{t} \tau_2 \bnfalt \\
% %% & & &
% %% \primctx, \zeta: \grt_1 \uarr{k}{t} \grt_2

% \end{array}
% \]
%   \caption{Syntax of {\tname} types}
% \label{fig:type-syntax}
% \end{figure}
 


% \begin{figure}
%   \centering
% \[
% \begin{array}{llll}
%   \mbox{Expr.} & e & ::= & x  ~|~ \econst ~|~ \efix f(x). e ~|~ e_1 \eapp e_2 ~|~ \zeta \eapp e ~|~ \la e_1, e_2 \ra 
%  ~|~  \eleft(e) ~|~ \eright(e)  \\ &&&
%            ~|~    \einl e ~|~ \einr e ~|~ \ecase (e, x.e_1, y.e_2) 
%     |~ \enil ~|~ \econs(e_1,e_2) \\ &&& ~|~ (\hspace{-0.3em}{\ecase e \eof \enil \rightarrow e_1 ~|~ h ::tl \rightarrow e_2})
%            ~|~ \eLam e ~|~ e \eApp 
%   \\ & & & |~ \epack e ~|~ \eunpack e_1 \eas x \ein e_2  ~|~ \clet e_1 \eas x \ein e_2 

% % \\
% %   \mbox{Values} & v & ::= & \econst ~|~ \efix f(x).v ~|~ \la  v_1, v_2 \ra ~|~ \einl v ~|~ \einr
% %   ~|~ \enil
% %   \\ & & & |~ \econs(v_1,v_2) ~|~  \eLam e~|~ \epack v ~|~ \eunit 
% \end{array}
% \]
% \caption{Syntax of {\tname} expressions}
%   \label{fig:terms}
% \end{figure}




\begin{figure}
  \centering
  \begin{mathpar}
    % \tyvar
    % \and
    % \tyconst
    % \and
    % \tynil 
    % \and
    % \tycons
    % \and
    \tyfix
    \and
    \tyapp
    \and
    % \tyinl
    % \and
    % \tycase
    \and
    \tysubsum
  \end{mathpar}
  \caption{{Selected {\tname} unary typing rules}}
  \label{fig:typing-rules}
\end{figure}



 \begin{figure*}
    \centering
    \begin{mathpar}
      % \tyrvar
      % \and
      % \tyrconst
      % \and
      % \tyrnil 
      % \and
      % \tyrcons
      % \and
      % \tyrconsbox
      % \and
      % \tyrcaseL
      % \and
      \tyrfix
      \and
      \tyrappD
      % \and
      % \tyriLam
      % \and
      % \tyriApp
      \and
     % \tyrinl
      % \and
      % \tyrcase
      % \and
      % \tynochange
      % \and
      % \tyrsubsum 
      % \and
      % \tyrsplit
      % \and 
      % \tyrfixNC
      \tyswitch
      \and
     \tyrletMax
     % \and
     % \tyrcontra
    \end{mathpar} 
    % Definitions at typing-rules-defs.tex
    \caption{Selected {\tname} relational typing rules}
    \label{fig:synch-rel-typing-rules}
  \end{figure*}
 


\begin{figure}
  \raggedright
  \fbox{$\Delta; \Phi_a \jsubtype{\tau_1}{\tau_2}$}~~~ $\tau_1$ is a subtype of  $\tau_2$ \text{~~~~~~~~~~~~}
  \fbox{$\Delta; \Phi_a \jasubtype{\grt_1}{\grt_2}$}~~~ $\grt_1$ is a subtype of $\grt_2$\\

\raggedright
\begin{mathpar}
% \stgrt
% %
% \and
% %
% \stincl
% %
% \and
%
\starrE
%
\and
%
\starrD
%
\and
%
\starrW
%
\and
%
\starrboxD
%
% \and
% %
% \stlist
% %
% \and
% %
% \stlistzero
%
% \and
% %
% \stlistbox
% %
% \and
% %
% \stint
% %
% \and
% %
% \stbox
% %
% \and
% %
% \stboxD
% %
% \and
% %
% \stboxB
% %
% \and
% \sttrans
\end{mathpar} 
%\nocaptionrule
% Definitions at subtyping-rules-defs.tex
\caption{Selected  {\tname} relational subtyping rules}
\label{fig:subtyping-rules}  
\end{figure} 

\subsection{{\tname} Typing} {\tname} has two kinds of typing
judgments: a unary (non-relational) one for typing single expressions
in isolation and a binary (relational) one for typing a pair of
related expressions. The unary judgment $\Delta; \Phi_a; \Omega
\jtype{k}{t}{e}{\grt}$ means that the execution cost of $e$ is lower
bounded by $k$ and upper bounded by $t$ and $e$ has type $\grt$.  The
binary judgment $\Delta; \Phi_a; \Gamma \jtypediff{t}{e_1}{e_2}{\tau}$
means that the cost of $e_1$ relative to $e_2$ is upper bounded by $t$
and the expressions have the relational type $\tau$. The contexts
$\Omega$ and $\Gamma$ contain the unary and binary types of variables,
respectively. % The context $\Delta$ lists universally quantified index
% (refinement) variables. In addition, both judgments include a set of
% constraints $\Phi_a$ on the index variables under which the typing
% holds.

\paragraph{Unary typing} Selected unary typing rules are shown in
Figure~\ref{fig:typing-rules}. Unary typing establishes lower and
upper bounds on the cost of a single program. By design, only
elimination forms add cost (e.g., the cost $\kapp$ in the rule
\textbf{app}). The remaining cost of an expression is simply the sum
total of the costs of its subexpressions. The rule $\sqsubseteq\wexec$
allows subtyping. It also allows decreasing the cost lower bound $k$
and increasing the cost upper bound $t$. The definition of the unary
subtyping $\sat^{\mathsf{\grt}}$ is unsurprising; we omit its rules.

\paragraph{Relational typing}
Selected relational typing rules are shown in
Figure~\ref{fig:synch-rel-typing-rules}. The general principle behind
relational typing is that no cost is added for the top-level syntactic
construct when it is the same on the two sides (e.g. rule
\textbf{r-app}). Structurally dissimilar expressions can either be
typed 1) non-relationally by switching to unary typing as in the rule
\textbf{switch} and taking a difference of the best- and worst-case
costs, or 2) by using local similarities as in the rule
\textbf{let-r-e}. % For the former, in the premise of the
% \textbf{switch} rule, the two expressions are typed independently in
% an erased environment $\trmo{\Gamma}$ where the relational refinements
% in $\Gamma$ are forgotten via the refinement erasure function
% $\trmo{.}$. For instance, $\trmo{\tlist{n}{\alpha}{\tau}} =
% \ulist{n}{\trmo{\tau}}$, $\trmo{\tcho{\grt}} = \grt$ and $\trmo{\tau_1
%   \tarrd{t} \tau_2}= \trmo{\tau_1} \uarr{0}{\sinf}
% \trmo{\tau_2}$.

% Somewhat unusually, there are two typing rules for the cons
% constructor for lists. The rule \textbf{r-cons1} applies when the head
% elements of the two cons-ed lists may differ, whereas the rule
% \textbf{r-cons2} applies only when the head elements may not
% differ. Correspondingly the list-case elimination rule,
% \textbf{r-caseL}, requires typing the cons branch of the list-case
% twice, once under the assumption that head elements may not differ and
% once without this assumption. These design decisions are a consequence
% of having the relational refinement $\alpha$ in the list type
% $\tlist{n}{\alpha}{\tau}$. They make it simpler to write programs
% without annotations, but make it much harder to algorithmize the type
% system (see Section~\ref{sec:elab} for details).

% Additionally, there are several generic rules. As explained in the
% earlier example, the rule \textbf{nochange} establishes that the
% relative cost of an expression relative to itself is $0$, if all its
% free variables can be supertyped to $\tbox{}$-annotated counterparts.
% The rule \textbf{r-split} allows case analysis on the index
% domain. For example, when typing a divide-and-conquer algorithm that
% operates on a pair of lists in {\tname}, one often needs to analyze
% the cases $\alpha=0$ (where the two lists may not differ) and $\alpha
% > 0$ (where the two lists may differ) separately. This rule allows
% doing that. The rule \textbf{r-contra} gives a pair of expression any
% type (or cost) when the constraints are invalid.
%
% By design, the rules \textbf{nochange}, \textbf{switch},
% \textbf{r-contra} and \textbf{r-split} are not syntax-directed and the
% latter three can be applied anywhere. This complicates
% algorithmization of the type system.
 
\paragraph{Relational subtyping}
% Relational subtyping $\tau \sqsubseteq \tau'$ in {\tname} is
% complex. Some of its rules are shown in
% Figure~\ref{fig:subtyping-rules}.  First, subtyping is
% constraint-dependent, because it must, for instance, be able to show
% that $\tlist{n}{\alpha}{\tau} \sqsubseteq \tlist{m}{\alpha}{\tau}$
% when $n = m$. Second, in {\tname}, $\tbox{}$'s comonadic properties
% manifest themselves via subtyping. This results in interactions
% between $\tbox{}$ and other connectives as, for instance, in the rules
% \textbf{$\to \square \wdiff$}, \textbf{l2} and
% \textbf{l$\tbox{}$}.
%Similar interactions exist between the modality
%$\tcho{\grt}$ and other connectives.

We explain some of the subtyping rules.%  The rule \textbf{U} allows
% lifting subtyping from unary types to relational types at the weakest
% relation $\achange$. The rule \textbf{W} allows weakening the type
% $\tau$ to its weakest form $\tcho{\trmo{\tau}}$.
The rule
\textbf{${\to \wdiff}$} is the usual subtyping rule for relational
function types where upper bounds on costs are covariant (in unary
subtyping, lower bounds are contavariant). We have two additional
subtyping rules for function types. The rule \textbf{$\to
  \wexec\wdiff$} allows converting two unrelated functions---with
minimum and maximum execution costs $k$ and $t$, respectively---to
related functions with relative cost $t-k$, but with unrelated
arguments and results. The rule \textbf{$\to \square \wdiff$} allows
converting syntactically equal functions to related functions that
when applied to equal arguments, produce equal results and have
relative cost $0$.

% The rule \textbf{l1} allows the number of elements that differ in a
% list to be weakened covariantly. The rule \textbf{l2} allows two
% related lists with zero differences to be retyped as two related lists
% whose elements are in the diagonal relation. The rule \textbf{l$\square$}
% % $\tlist{n}{\alpha}{\tbox{\tau}} \sqsubseteq
% % \tbox{(\tlist{n}{\alpha}{\tau})}$,
% allows two related lists whose elements are equal % pointwise
% to be
% retyped as two equal lists, represented by the outer $\square$.
% The rule \textbf{T} allows ignoring the $\square$ annotation of the
% subtype whereas the rule \textbf{B-$\square$} allows ignoring the
% outer $\square$ annotations of both the sub and the super
% type.

% Finally, the transitivity rule, \textbf{trans}, makes subtyping
% transitive. The \textbf{trans} rule cannot be algorithmized directly
% since the middle type in its premise ($\tau_2$) must be guessed in an
% implementation. The usual method of algorithmizing subtyping
% eliminates the \textbf{trans} rule by showing it admissible. However,
% in {\tname}, proving transitivity admissible seems very
% difficult. This is because of the interaction of \textbf{trans} with
% specific rules for $\tbox{}$, such as \textbf{$\to \square \wdiff$}
% and \textbf{l$\tbox{}$}.


%% This issue, coupled with the nondeterminism in the typing rules
%% mentioned above, is what motivated us to define an embedding from
%% {\tname} to {\tnamemin}. We turn to this next.


%
% We note that the type $\tbox{\tau}$ follows the standard co-monadic
% rules: $\tbox{\tau} \sqsubseteq \tau$, $\tbox{(\tau_1 \tarrd{t}
%   \tau_2)} \sqsubseteq \tbox{\tau_1} \tarrd{0} \tbox{\tau_2}$ and
% $\tbox{(\tau_1 \ttimes \tau_2)} \sqsubseteq \tbox{\tau_1 \ttimes
%   \tbox{\tau_2}}$ (the rule for the last subtyping is not shown here).
  
%% Corresponding to two modes of typing, {\tname} has two kinds of
%% subtyping judgments: $\Delta; \Phi_a \jasubtype{\grt}{\grt'}$ for
%% unary types (whose rules are omitted) and $\Delta; \Phi_a
%% \jsubtype{\tau}{\tau'}$ for relational types (whose rules are shown in
%% Figure~\ref{fig:subtyping-rules}). In the relational typing, $\square$
%% and $U$ interact non-trivially with other constructs. In {\tname},
%% $\tbox{}$ corresponds to the S4 modality while $U$ is neither a monad
%% nor a standard comonad.


%% Next, we illustrate typing and subtyping rules of {\tname} via an
%% example.

% \paragraph{Example (map)} Consider the standard $\kw{map}$ function
% that maps over a list using a function $f$.  \vspace{2mm}
% \begin{nstabbing}
%  $\efix \kw{map}(f).\elam l. \ecase l $\=$\eof \enil \rightarrow \enil$ \\
% \>$ |~ h :: tl \rightarrow \econs(f \eapp h, \eapp \kw{map} \eapp f \eapp tl) $
% \end{nstabbing}
% Assume that $f$ has the relational type $\tbox{(\tau_1 \tarrd{t}
%   \tau_2)}$ with relative cost $t$. What can we say about the
% \textit{relative cost} of two runs of $\kw{map}$ given two input lists
% related at type $\tlist{n}{\alpha}{\tau_1}$ (i.e., two lists that
% differ in at most $\alpha$ positions)? Since we know that $f$ itself
% does not change across the two executions (represented by the outer
% $\tbox{}$ in its type), at most $\alpha$ applications of $f$ may
% differ in the two executions, while at least $n-\alpha$ applications
% must be identical. Hence, the relative cost of the two runs of
% $\kw{map}$ will be bounded by $\alpha \cdot t$. Moreover, we can show
% that the output lists will differ in at most $\alpha$
% positions. Therefore, $\kw{map}$ can be given the following relational
% type:
% \begin{equation*}
% (\tbox{(\tau_1 \tarrd{t} \tau_2)}) \to \forall
%   n,\alpha. \tlist{n}{\alpha}{\tau_1} \tarrd{t \cdot \alpha}
%   \tlist{n}{\alpha}{\tau_2}\label{eq:1}
% \end{equation*}
% Next, we briefly explain how this type is derived in {\tname} as this
% highlights several key rules of the type system. The typing proceeds
% by induction on $l$. The interesting part is establishing the relative
% cost for the cons branch in the definition of $\kw{map}$. We have to
% establish an upper bound of $\alpha \cdot t$ for the branch. From the
% type of $l$, we know that at most $\alpha$ elements in $h::tl$ may
% differ in the two runs. However, we do not know statically whether $h$
% (the current head) is among those elements. Therefore, {\tname}'s
% \textbf{r-caseL} types the $\kw{cons}$ branch twice: once assuming
% that $h$ will not differ in the two runs and then assuming that $h$
% may differ. We explain the analysis of these two cases.

% We start from the second case where $h$ may differ, i.e. $h: \tau_1$
% and $tl:\tlist{n-1}{\alpha-1}{\tau_1}$ (note the $\alpha-1$ in the
% tail's type). The expression $f\eapp h$ can be shown to have relative
% cost $\alpha$ by first supertyping $f$ from $\tbox{(\tau_1 \tarrd{t}
%   \tau_2)}$ to $\tau_1 \tarrd{t} \tau_2$ (using the subtyping rule
% \textbf{T} of Figure~\ref{fig:subtyping-rules}) and then applying the
% rule \textbf{r-app}. The recursive call $(\kw{map}\eapp f \eapp tl)$
% has cost $(\alpha-1)\cdot t$, inductively. When added, these two yield
% exactly $\alpha \cdot t$, as required. (Technically, we use rule
% \textbf{r-cons1} of Figure~\ref{fig:synch-rel-typing-rules}.)

% The analysis of the first case, where $h$ may not differ, is more
% interesting. Here, \textbf{r-caseL} provides us that $h:
% \tbox{\tau_1}$ (the $\tbox{}$ indicates that the head is the same in
% the two runs) and $tl:\tlist{n-1}{\alpha}{\tau_1}$ (note the $\alpha$
% in the tail's type). In this case, the inductive cost of
% $(\kw{map}\eapp f \eapp tl)$ is already $\alpha \cdot t$. Hence, we
% must show that $f\eapp h$ has a relative cost of $0$. This can be
% established in two ways: a) By using the subtyping rule $\to \square
% \wdiff$ of Figure~\ref{fig:subtyping-rules}, we can supertype $f$ to
% $\tbox{\tau_1} \tarrd{0} \tbox{\tau_2}$, and then apply it to get a
% relative cost of $0$ or, b) We can use the \textbf{nochange} rule
% since both free variables, $f, h$ in $f \eapp h$ are
% $\tbox{}$-annotated. In either case, the analysis is officially
% completed using the rule \textbf{r-cons2}.


%  the minimum and maximum execution costs of
% $f$ are $t$ and $k$, respectively, i.e. it has type
% $\grt_1 \uarr{k}{t} \grt_2$. What can we say about the
% \textit{relative cost} of two runs of $\kw{map}$?

% \ezgi{Just show the relational part. To be cont. after dinner break!}

% Then, using the unary typing, $\kw{map}$
% can be given the non-relational type
% $(\grt_1 \uarr{k}{t} \grt_2) \to \forall n. \ulist{n}{\grt_1}
% \uarr{k\cdot n}{t \cdot n} \ulist{n}{\grt_2}$.\footnote{For
%   simplicity, we only account for the cost of applications only.} What
% about the \textit{relative execution cost} of the two runs of
% $\kw{map}$ given two input lists, of type
% $\tlist{n}{\alpha}{\tcho{\grt_1}}$, that differ by at most $\alpha$
% elements? If we know that $f$ will not differ in the two executions,
% i.e. it can be given the relational type
% $\tbox{(\tcho(\grt_1 \uarr{k}{t} \grt_2))}$, then since only $\alpha$
% applications of $f$ will differ in the two executions, the relative
% cost of $\kw{map}$ will be bounded by $(t-k) \cdot \alpha$. Moreover,
% we can show that at most $\alpha$ elements will differ in the
% resulting lists. Hence, $\kw{map}$ can be given the relational type:
% $\tbox{(\tcho{(\grt_1 \uarr{k}{t} \grt_2)})} \to \forall
% n,\alpha. \tlist{n}{\alpha}{\tcho{\grt_1}} \tarrd{(t-k) \cdot \alpha}
% \tlist{n}{\alpha}{\tcho{\grt_2}}$.

% Note that by doing a naive analysis that compares the difference of
% the worst- and best-case execution costs of $\kw{map}$, we could only
% obtain a linear bound.


% Next, let's see how this typed is derived in {\tname}.

%Instead,
% thanks to a powerful relational type and effect system, {\tname}'s
% \textit{relational cost analysis} is able to cultivate the similarity
% of the inputs lists, as well as the structural behavior of $\kw{map}$,
% to obtain a more precise bound $O(\alpha \cdot k)$.



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

